Generating Families of Practical Fast Matrix Multiplication Algorithms

Matrix multiplication (GEMM) is a core operation to numerous scientific applications. Traditional implementations of Strassen-like fast matrix multiplication (FMM) algorithms often do not perform well except for very large matrix sizes, due to the increased cost of memory movement, which is particularly noticeable for non-square matrices. Such implementations also require considerable workspace and modifications to the standard BLAS interface. We propose a code generator framework to automatically implement a large family of FMM algorithms suitable for multiplications of arbitrary matrix sizes and shapes. By representing FMM with a triple of matrices [U,V,W] that capture the linear combinations of submatrices that are formed, we can use the Kronecker product to define a multi-level representation of Strassen-like algorithms. Incorporating the matrix additions that must be performed for Strassen-like algorithms into the inherent packing and micro-kernel operations inside GEMM avoids extra workspace and reduces the cost of memory movement. Adopting the same loop structures as high-performance GEMM implementations allows parallelization of all FMM algorithms with simple but efficient data parallelism without the overhead of task parallelism. We present a simple performance model for general FMM algorithms and compare actual performance of 20+ FMM algorithms to modeled predictions. Our implementations demonstrate a performance benefit over conventional GEMM on single core and multi-core systems. This study shows that Strassen-like fast matrix multiplication can be incorporated into libraries for practical use.

==> X.tex <==
\def \tikzexternallastkey {8DF08D1D6855EED3870D6912B63C07FB}%


==> contribution.tex <==
- we extend our SC work to more variations of Strassen
- we define the new Kronecker product method to generalize more levels of Strassen

a framework for generating any level Strassen-like algorithm

performance analysis

- extend to Wingrad variable

index -> is changing...

any combination of Strassen-like algorithm:
e.g.
first level -> (2,2,2)
second level -> (3,2,3)

Extend to more levels of Strassen

Bandwidth?
Over heat -> multi-core perf, 




==> fig_actual_vs_model/fig_actual_model_side_by_side.tex <==
\definecolor{colorbrewer1}{RGB}{228,26,28}
\definecolor{colorbrewer2}{RGB}{55,126,184}
\definecolor{colorbrewer3}{RGB}{77,175,74}
\definecolor{colorbrewer4}{RGB}{152,78,163}
\definecolor{colorbrewer5}{RGB}{255,127,0}
%\definecolor{colorbrewer6}{RGB}{255,255,51}
\definecolor{colorbrewer7}{RGB}{166,86,40}
\definecolor{colorbrewer8}{RGB}{247,129,191}
\definecolor{colorbrewer9}{RGB}{153,153,153}

\definecolor{darkgreen}{rgb}{0,0.5,0}

\definecolor{darkred}{rgb}{0.44,0,0}
\definecolor{darkgreen}{rgb}{0,0.44,0}
\definecolor{darkblue}{rgb}{0,0,0.44}
\definecolor{enrique}{rgb}{0,0,0}


\pgfplotscreateplotcyclelist{jianyu0color}{%
ultra thick,colorbrewer1,every mark/.append style={fill=colorbrewer1},mark=triangle*\\%
orange,every mark/.append style={fill=orange},mark=square*\\%
cyan,every mark/.append style={fill=cyan},mark=otimes*\\%
red!70!white,mark=star\\%
lime!80!black,every mark/.append style={fill=lime},mark=diamond*\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
thick,yellow!60!black,every mark/.append style={solid,fill=yellow!80!black},mark=square*\\%
purple,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=star,every mark/.append style=solid\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*\\%
thick,colorbrewer4,mark=x\\%
blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=diamond*\\%
thick,darkgreen,mark=star\\%
blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
brown!60!black,densely dashed,every mark/.append style={
solid,fill=brown!80!black},mark=square*\\%
darkred,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=oplus,every mark/.append style=solid\\%
colorbrewer5,densely dashed,every mark/.append style={solid,fill=colorbrewer5},mark=diamond*\\%
darkgreen,densely dashed,mark=+,every mark/.append style=solid\\%
%red,blue,black,yellow,brown,teal,orange,violet\\%
thick,colorbrewer7,mark=triangle*\\%
thick,black\\%
}

\pgfplotscreateplotcyclelist{jianyucolor}{%
ultra thick,colorbrewer1,every mark/.append style={fill=colorbrewer1},mark=triangle*\\%
orange,every mark/.append style={fill=orange},mark=square*\\%
cyan,every mark/.append style={fill=cyan},mark=otimes*\\%
red!70!white,mark=star\\%
lime!80!black,every mark/.append style={fill=lime},mark=diamond*\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
thick,yellow!60!black,every mark/.append style={solid,fill=yellow!80!black},mark=square*\\%
purple,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=star,every mark/.append style=solid\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*\\%
thick,colorbrewer4,mark=x\\%
blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=diamond*\\%
thick,darkgreen,mark=star\\%
blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
brown!60!black,densely dashed,every mark/.append style={
solid,fill=brown!80!black},mark=square*\\%
darkred,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=oplus,every mark/.append style=solid\\%
colorbrewer5,densely dashed,every mark/.append style={solid,fill=colorbrewer5},mark=diamond*\\%
darkgreen,densely dashed,mark=+,every mark/.append style=solid\\%
%red,blue,black,yellow,brown,teal,orange,violet\\%
thick,colorbrewer7,mark=triangle*\\%
thick,black,densely dashed\\%
thick,black\\%
}

\newcommand{\MYRANKK}{$ m \!\!=\!\! n \!\!=\!\! 14400 $, $ k $ varies}

\begin{figure*}[htp!]
\input fig_actual_vs_model/my_rankk_2level_abc_1core_large
\input fig_actual_vs_model/model_rankk_2level_abc_1core_large
\caption{Performance of generated two-level ABC FMM implementations on single core when \MYRANKK{}.
Left: actual performance; Right: modeled performance.
}
\label{fig:actual_vs_model}
\end{figure*}



==> fig_actual_vs_model/model_rankk_2level_abc_1core_large.tex <==
\begin{tikzpicture}[scale=1.0]
\begin{axis}[
    title={$m = n = 14400$, 2 level, ABC, 1 core, \emph{modeled}},
    xlabel={ $k$ },
    ylabel={\emph{Effective} GFLOPS ($ 2 \cdot  m \cdot  n \cdot k / time $)},
    xmin=0,
    xmax=12000,
    ymin=20,
    ymax=34,
    xtick={1000,2000,3000,4000,5000,6000,7000,8000,9000,10000,11000,12000},
    ytick={5, 10, 15, 20, 25, 28.36, 30, 34},
    scaled x ticks=false,
    scaled x ticks=base 10:-3,
    grid=major,
    axis background/.style={fill=lightgray!20},
    mark size=0.8pt,
    cycle list name=jianyu0color,
    legend style={
        at={(0.99,0.01)},
        anchor=south east,
        legend columns=4,
        font=\tiny,
        rounded corners=1pt,
        nodes={scale=0.8, transform shape},
        %cells={anchor=west},
    },
    %legend entries = {
    %    $ \langle 2, 2, 2 \rangle $\\
    %    $ \langle 2, 3, 2 \rangle $\\ 
    %    $ \langle 2, 3, 4 \rangle $\\ 
    %    $ \langle 2, 4, 3 \rangle $\\ 
    %    $ \langle 2, 5, 2 \rangle $\\ 
    %    $ \langle 3, 2, 2 \rangle $\\ 
    %    $ \langle 3, 2, 3 \rangle $\\ 
    %    $ \langle 3, 2, 4 \rangle $\\ 
    %    $ \langle 3, 3, 2 \rangle $\\ 
    %    $ \langle 3, 3, 3 \rangle $\\ 
    %    $ \langle 3, 3, 6 \rangle $\\ 
    %    $ \langle 3, 4, 2 \rangle $\\ 
    %    $ \langle 3, 4, 3 \rangle $\\ 
    %    $ \langle 3, 5, 3 \rangle $\\ 
    %    $ \langle 3, 6, 3 \rangle $\\ 
    %    $ \langle 4, 2, 2 \rangle $\\ 
    %    $ \langle 4, 2, 3 \rangle $\\ 
    %    $ \langle 4, 2, 4 \rangle $\\ 
    %    $ \langle 4, 3, 2 \rangle $\\ 
    %    $ \langle 4, 3, 3 \rangle $\\ 
    %    $ \langle 4, 4, 2 \rangle $\\ 
    %    $ \langle 5, 2, 2 \rangle $\\ 
    %    $ \langle 6, 3, 3 \rangle $\\
    %    $ GEMM $\\
    %},
    ]
\addplot table[x=dim,y=222,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=232,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=234,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=243,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=252,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=322,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=323,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=324,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=332,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=333,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=336,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=342,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=343,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=353,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=363,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=422,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=423,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=424,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=432,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=433,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=442,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=522,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=633,col sep=comma] {fig_actual_vs_model/model_rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=gemm,col sep=comma] {fig_actual_vs_model/model_rankk_gemm_1core.csv};
\end{axis}
\end{tikzpicture}


==> fig_actual_vs_model/my_rankk_2level_abc_1core_large.tex <==
\begin{tikzpicture}[scale=1.0]
\begin{axis}[
    title={$m = n = 14400$, 2 level, ABC, 1 core, \emph{actual}},
    xlabel={ $k$ },
    ylabel={\emph{Effective} GFLOPS ($ 2 \cdot  m \cdot  n \cdot k / time $)},
    xmin=0,
    xmax=12000,
    ymin=20,
    ymax=34,
    xtick={1000,2000,3000,4000,5000,6000,7000,8000,9000,10000,11000,12000},
    ytick={5, 10, 15, 20, 25, 28.36, 30, 34},
    scaled x ticks=false,
    scaled x ticks=base 10:-3,
    grid=major,
    axis background/.style={fill=lightgray!20},
    mark size=0.8pt,
    cycle list name=jianyucolor,
    restrict y to domain=1:inf,
    legend style={
        at={(0.99,0.01)},
        anchor=south east,
        legend columns=4,
        font=\tiny,
        rounded corners=1pt,
        nodes={scale=0.8, transform shape},
        %cells={anchor=west},
    },
    legend entries = {
        $ \langle 2, 2, 2 \rangle $\\
        $ \langle 2, 3, 2 \rangle $\\ 
        $ \langle 2, 3, 4 \rangle $\\ 
        $ \langle 2, 4, 3 \rangle $\\ 
        $ \langle 2, 5, 2 \rangle $\\ 
        $ \langle 3, 2, 2 \rangle $\\ 
        $ \langle 3, 2, 3 \rangle $\\ 
        $ \langle 3, 2, 4 \rangle $\\ 
        $ \langle 3, 3, 2 \rangle $\\ 
        $ \langle 3, 3, 3 \rangle $\\ 
        $ \langle 3, 3, 6 \rangle $\\ 
        $ \langle 3, 4, 2 \rangle $\\ 
        $ \langle 3, 4, 3 \rangle $\\ 
        $ \langle 3, 5, 3 \rangle $\\ 
        $ \langle 3, 6, 3 \rangle $\\ 
        $ \langle 4, 2, 2 \rangle $\\ 
        $ \langle 4, 2, 3 \rangle $\\ 
        $ \langle 4, 2, 4 \rangle $\\ 
        $ \langle 4, 3, 2 \rangle $\\ 
        $ \langle 4, 3, 3 \rangle $\\ 
        $ \langle 4, 4, 2 \rangle $\\ 
        $ \langle 5, 2, 2 \rangle $\\ 
        $ \langle 6, 3, 3 \rangle $\\
        $ BLIS $\\
        $ MKL $\\
    },
    ]
\addplot table[x=dim,y=222,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=232,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=234,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=243,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=252,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=322,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=323,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=324,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=332,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=333,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=336,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=342,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=343,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=353,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=363,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=422,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=423,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=424,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=432,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=433,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=442,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=522,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=633,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=blis,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\addplot table[x=dim,y=mkl,col sep=comma] {fig_actual_vs_model/rankk_2level_abc_1core.csv};
\end{axis}
\end{tikzpicture}


==> figures/hybrid_script/hybrid_fixk1440_abc_10core.tex <==
\begin{tikzpicture}[scale=.7]
\begin{axis}[
    title={$k = 1440$, ABC, 10 core},
    xlabel={ $m = n$ },
    ylabel={\emph{Effective} GFLOPS ($ 2 \cdot  m \cdot  n \cdot k / time $)},
    xmin=0,
    xmax=16000,
    ymin=50,
    ymax=255,
    xtick={1000,2000,3000,4000,5000,6000,7000,8000,9000,10000,11000,12000,13000,14000,15000,16000},
    ytick={50, 100, 150, 200, 248},
    scaled x ticks=false,
    scaled x ticks=base 10:-3,
    grid=major,
    axis background/.style={fill=lightgray!20},
    mark size=0.8pt,
    cycle list name=jianyu3color,
    legend style={
        at={(0.99,0.01)},
        anchor=south east,
        legend columns=1,
        font=\tiny,
        rounded corners=1pt,
        nodes={scale=0.8, transform shape},
    },
    legend entries = {
        $ BLIS    $\\
        $ MKL     $\\
        $ \langle 2, 2, 2 \rangle, 1~level$\\
        $ \langle 2, 2, 2 \rangle, 1~level$\\
        $ \langle 2, 3, 2 \rangle, 2~level$\\ 
        $ \langle 2, 3, 2 \rangle, 2~level$\\ 
        $ \langle 2, 2, 2 \rangle \!+\! \langle 2, 3, 2 \rangle $\\ 
    },
    ]
\addplot table[x=dim,y=blis,col sep=comma] {plotdata/fixk1440_10core.csv};
\addplot table[x=dim,y=mkl,col sep=comma] {plotdata/fixk1440_10core.csv};
\addplot table[x=dim,y=222_1,col sep=comma] {plotdata/fixk1440_10core.csv};
\addplot table[x=dim,y=232_1,col sep=comma] {plotdata/fixk1440_10core.csv};
\addplot table[x=dim,y=222_2,col sep=comma] {plotdata/fixk1440_10core.csv};
\addplot table[x=dim,y=232_2,col sep=comma] {plotdata/fixk1440_10core.csv};
\addplot table[x=dim,y=hybrid,col sep=comma] {plotdata/fixk1440_10core.csv};
\end{axis}
\end{tikzpicture}


==> figures/hybrid_script/hybrid_fixk1440_abc_1core.tex <==
\begin{tikzpicture}[scale=.7]
\begin{axis}[
    title={$k = 1440$, ABC, 1 core},
    xlabel={ $m = n$ },
    ylabel={\emph{Effective} GFLOPS ($ 2 \cdot  m \cdot  n \cdot k / time $)},
    xmin=0,
    xmax=12000,
    ymin=20,
    ymax=34,
    xtick={1000,2000,3000,4000,5000,6000,7000,8000,9000,10000,11000,12000},
    ytick={5, 10, 15, 20, 25, 28.36, 30, 34},
    scaled x ticks=false,
    scaled x ticks=base 10:-3,
    grid=major,
    axis background/.style={fill=lightgray!20},
    mark size=0.8pt,
    cycle list name=jianyu3color,
    legend style={
        at={(0.99,0.01)},
        anchor=south east,
        legend columns=1,
        font=\tiny,
        rounded corners=1pt,
        nodes={scale=0.8, transform shape},
    },
    legend entries = {
        $ BLIS    $\\
        $ MKL     $\\
        $ \langle 2, 2, 2 \rangle, 1~level$\\
        $ \langle 2, 2, 2 \rangle, 1~level$\\
        $ \langle 2, 3, 2 \rangle, 2~level$\\ 
        $ \langle 2, 3, 2 \rangle, 2~level$\\ 
        $ \langle 2, 2, 2 \rangle \!+\! \langle 2, 3, 2 \rangle $\\ 
    },
    ]
\addplot table[x=dim,y=blis,col sep=comma] {plotdata/fixk1440_1core.csv};
\addplot table[x=dim,y=mkl,col sep=comma] {plotdata/fixk1440_1core.csv};
\addplot table[x=dim,y=222_1,col sep=comma] {plotdata/fixk1440_1core.csv};
\addplot table[x=dim,y=232_1,col sep=comma] {plotdata/fixk1440_1core.csv};
\addplot table[x=dim,y=222_2,col sep=comma] {plotdata/fixk1440_1core.csv};
\addplot table[x=dim,y=232_2,col sep=comma] {plotdata/fixk1440_1core.csv};
\addplot table[x=dim,y=hybrid,col sep=comma] {plotdata/fixk1440_1core.csv};
\end{axis}
\end{tikzpicture}


==> ignore/pgflibrarypgfplots.colorbrewer.code.tex <==
\usetikzlibrary{colorbrewer}
\pgfplotscreateplotcyclelist{YlGn-3}{%
  YlGn-3-1\\%
  YlGn-3-2\\%
  YlGn-3-3\\%
}
\pgfplotscreateplotcyclelist{YlGn-4}{%
  YlGn-4-1\\%
  YlGn-4-2\\%
  YlGn-4-3\\%
  YlGn-4-4\\%
}
\pgfplotscreateplotcyclelist{YlGn-5}{%
  YlGn-5-1\\%
  YlGn-5-2\\%
  YlGn-5-3\\%
  YlGn-5-4\\%
  YlGn-5-5\\%
}
\pgfplotscreateplotcyclelist{YlGn-6}{%
  YlGn-6-1\\%
  YlGn-6-2\\%
  YlGn-6-3\\%
  YlGn-6-4\\%
  YlGn-6-5\\%
  YlGn-6-6\\%
}
\pgfplotscreateplotcyclelist{YlGn-7}{%
  YlGn-7-1\\%
  YlGn-7-2\\%
  YlGn-7-3\\%
  YlGn-7-4\\%
  YlGn-7-5\\%
  YlGn-7-6\\%
  YlGn-7-7\\%
}
\pgfplotscreateplotcyclelist{YlGn-8}{%
  YlGn-8-1\\%
  YlGn-8-2\\%
  YlGn-8-3\\%
  YlGn-8-4\\%
  YlGn-8-5\\%
  YlGn-8-6\\%
  YlGn-8-7\\%
  YlGn-8-8\\%
}
\pgfplotscreateplotcyclelist{YlGn-9}{%
  YlGn-9-1\\%
  YlGn-9-2\\%
  YlGn-9-3\\%
  YlGn-9-4\\%
  YlGn-9-5\\%
  YlGn-9-6\\%
  YlGn-9-7\\%
  YlGn-9-8\\%
  YlGn-9-9\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-3}{%
  YlGnBu-3-1\\%
  YlGnBu-3-2\\%
  YlGnBu-3-3\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-4}{%
  YlGnBu-4-1\\%
  YlGnBu-4-2\\%
  YlGnBu-4-3\\%
  YlGnBu-4-4\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-5}{%
  YlGnBu-5-1\\%
  YlGnBu-5-2\\%
  YlGnBu-5-3\\%
  YlGnBu-5-4\\%
  YlGnBu-5-5\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-6}{%
  YlGnBu-6-1\\%
  YlGnBu-6-2\\%
  YlGnBu-6-3\\%
  YlGnBu-6-4\\%
  YlGnBu-6-5\\%
  YlGnBu-6-6\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-7}{%
  YlGnBu-7-1\\%
  YlGnBu-7-2\\%
  YlGnBu-7-3\\%
  YlGnBu-7-4\\%
  YlGnBu-7-5\\%
  YlGnBu-7-6\\%
  YlGnBu-7-7\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-8}{%
  YlGnBu-8-1\\%
  YlGnBu-8-2\\%
  YlGnBu-8-3\\%
  YlGnBu-8-4\\%
  YlGnBu-8-5\\%
  YlGnBu-8-6\\%
  YlGnBu-8-7\\%
  YlGnBu-8-8\\%
}
\pgfplotscreateplotcyclelist{YlGnBu-9}{%
  YlGnBu-9-1\\%
  YlGnBu-9-2\\%
  YlGnBu-9-3\\%
  YlGnBu-9-4\\%
  YlGnBu-9-5\\%
  YlGnBu-9-6\\%
  YlGnBu-9-7\\%
  YlGnBu-9-8\\%
  YlGnBu-9-9\\%
}
\pgfplotscreateplotcyclelist{GnBu-3}{%
  GnBu-3-1\\%
  GnBu-3-2\\%
  GnBu-3-3\\%
}
\pgfplotscreateplotcyclelist{GnBu-4}{%
  GnBu-4-1\\%
  GnBu-4-2\\%
  GnBu-4-3\\%
  GnBu-4-4\\%
}
\pgfplotscreateplotcyclelist{GnBu-5}{%
  GnBu-5-1\\%
  GnBu-5-2\\%
  GnBu-5-3\\%
  GnBu-5-4\\%
  GnBu-5-5\\%
}
\pgfplotscreateplotcyclelist{GnBu-6}{%
  GnBu-6-1\\%
  GnBu-6-2\\%
  GnBu-6-3\\%
  GnBu-6-4\\%
  GnBu-6-5\\%
  GnBu-6-6\\%
}
\pgfplotscreateplotcyclelist{GnBu-7}{%
  GnBu-7-1\\%
  GnBu-7-2\\%
  GnBu-7-3\\%
  GnBu-7-4\\%
  GnBu-7-5\\%
  GnBu-7-6\\%
  GnBu-7-7\\%
}
\pgfplotscreateplotcyclelist{GnBu-8}{%
  GnBu-8-1\\%
  GnBu-8-2\\%
  GnBu-8-3\\%
  GnBu-8-4\\%
  GnBu-8-5\\%
  GnBu-8-6\\%
  GnBu-8-7\\%
  GnBu-8-8\\%
}
\pgfplotscreateplotcyclelist{GnBu-9}{%
  GnBu-9-1\\%
  GnBu-9-2\\%
  GnBu-9-3\\%
  GnBu-9-4\\%
  GnBu-9-5\\%
  GnBu-9-6\\%
  GnBu-9-7\\%
  GnBu-9-8\\%
  GnBu-9-9\\%
}
\pgfplotscreateplotcyclelist{BuGn-3}{%
  BuGn-3-1\\%
  BuGn-3-2\\%
  BuGn-3-3\\%
}
\pgfplotscreateplotcyclelist{BuGn-4}{%
  BuGn-4-1\\%
  BuGn-4-2\\%
  BuGn-4-3\\%
  BuGn-4-4\\%
}
\pgfplotscreateplotcyclelist{BuGn-5}{%
  BuGn-5-1\\%
  BuGn-5-2\\%
  BuGn-5-3\\%
  BuGn-5-4\\%
  BuGn-5-5\\%
}
\pgfplotscreateplotcyclelist{BuGn-6}{%
  BuGn-6-1\\%
  BuGn-6-2\\%
  BuGn-6-3\\%
  BuGn-6-4\\%
  BuGn-6-5\\%
  BuGn-6-6\\%
}
\pgfplotscreateplotcyclelist{BuGn-7}{%
  BuGn-7-1\\%
  BuGn-7-2\\%
  BuGn-7-3\\%
  BuGn-7-4\\%
  BuGn-7-5\\%
  BuGn-7-6\\%
  BuGn-7-7\\%
}
\pgfplotscreateplotcyclelist{BuGn-8}{%
  BuGn-8-1\\%
  BuGn-8-2\\%
  BuGn-8-3\\%
  BuGn-8-4\\%
  BuGn-8-5\\%
  BuGn-8-6\\%
  BuGn-8-7\\%
  BuGn-8-8\\%
}
\pgfplotscreateplotcyclelist{BuGn-9}{%
  BuGn-9-1\\%
  BuGn-9-2\\%
  BuGn-9-3\\%
  BuGn-9-4\\%
  BuGn-9-5\\%
  BuGn-9-6\\%
  BuGn-9-7\\%
  BuGn-9-8\\%
  BuGn-9-9\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-3}{%
  PuBuGn-3-1\\%
  PuBuGn-3-2\\%
  PuBuGn-3-3\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-4}{%
  PuBuGn-4-1\\%
  PuBuGn-4-2\\%
  PuBuGn-4-3\\%
  PuBuGn-4-4\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-5}{%
  PuBuGn-5-1\\%
  PuBuGn-5-2\\%
  PuBuGn-5-3\\%
  PuBuGn-5-4\\%
  PuBuGn-5-5\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-6}{%
  PuBuGn-6-1\\%
  PuBuGn-6-2\\%
  PuBuGn-6-3\\%
  PuBuGn-6-4\\%
  PuBuGn-6-5\\%
  PuBuGn-6-6\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-7}{%
  PuBuGn-7-1\\%
  PuBuGn-7-2\\%
  PuBuGn-7-3\\%
  PuBuGn-7-4\\%
  PuBuGn-7-5\\%
  PuBuGn-7-6\\%
  PuBuGn-7-7\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-8}{%
  PuBuGn-8-1\\%
  PuBuGn-8-2\\%
  PuBuGn-8-3\\%
  PuBuGn-8-4\\%
  PuBuGn-8-5\\%
  PuBuGn-8-6\\%
  PuBuGn-8-7\\%
  PuBuGn-8-8\\%
}
\pgfplotscreateplotcyclelist{PuBuGn-9}{%
  PuBuGn-9-1\\%
  PuBuGn-9-2\\%
  PuBuGn-9-3\\%
  PuBuGn-9-4\\%
  PuBuGn-9-5\\%
  PuBuGn-9-6\\%
  PuBuGn-9-7\\%
  PuBuGn-9-8\\%
  PuBuGn-9-9\\%
}
\pgfplotscreateplotcyclelist{PuBu-3}{%
  PuBu-3-1\\%
  PuBu-3-2\\%
  PuBu-3-3\\%
}
\pgfplotscreateplotcyclelist{PuBu-4}{%
  PuBu-4-1\\%
  PuBu-4-2\\%
  PuBu-4-3\\%
  PuBu-4-4\\%
}
\pgfplotscreateplotcyclelist{PuBu-5}{%
  PuBu-5-1\\%
  PuBu-5-2\\%
  PuBu-5-3\\%
  PuBu-5-4\\%
  PuBu-5-5\\%
}
\pgfplotscreateplotcyclelist{PuBu-6}{%
  PuBu-6-1\\%
  PuBu-6-2\\%
  PuBu-6-3\\%
  PuBu-6-4\\%
  PuBu-6-5\\%
  PuBu-6-6\\%
}
\pgfplotscreateplotcyclelist{PuBu-7}{%
  PuBu-7-1\\%
  PuBu-7-2\\%
  PuBu-7-3\\%
  PuBu-7-4\\%
  PuBu-7-5\\%
  PuBu-7-6\\%
  PuBu-7-7\\%
}
\pgfplotscreateplotcyclelist{PuBu-8}{%
  PuBu-8-1\\%
  PuBu-8-2\\%
  PuBu-8-3\\%
  PuBu-8-4\\%
  PuBu-8-5\\%
  PuBu-8-6\\%
  PuBu-8-7\\%
  PuBu-8-8\\%
}
\pgfplotscreateplotcyclelist{PuBu-9}{%
  PuBu-9-1\\%
  PuBu-9-2\\%
  PuBu-9-3\\%
  PuBu-9-4\\%
  PuBu-9-5\\%
  PuBu-9-6\\%
  PuBu-9-7\\%
  PuBu-9-8\\%
  PuBu-9-9\\%
}
\pgfplotscreateplotcyclelist{BuPu-3}{%
  BuPu-3-1\\%
  BuPu-3-2\\%
  BuPu-3-3\\%
}
\pgfplotscreateplotcyclelist{BuPu-4}{%
  BuPu-4-1\\%
  BuPu-4-2\\%
  BuPu-4-3\\%
  BuPu-4-4\\%
}
\pgfplotscreateplotcyclelist{BuPu-5}{%
  BuPu-5-1\\%
  BuPu-5-2\\%
  BuPu-5-3\\%
  BuPu-5-4\\%
  BuPu-5-5\\%
}
\pgfplotscreateplotcyclelist{BuPu-6}{%
  BuPu-6-1\\%
  BuPu-6-2\\%
  BuPu-6-3\\%
  BuPu-6-4\\%
  BuPu-6-5\\%
  BuPu-6-6\\%
}
\pgfplotscreateplotcyclelist{BuPu-7}{%
  BuPu-7-1\\%
  BuPu-7-2\\%
  BuPu-7-3\\%
  BuPu-7-4\\%
  BuPu-7-5\\%
  BuPu-7-6\\%
  BuPu-7-7\\%
}
\pgfplotscreateplotcyclelist{BuPu-8}{%
  BuPu-8-1\\%
  BuPu-8-2\\%
  BuPu-8-3\\%
  BuPu-8-4\\%
  BuPu-8-5\\%
  BuPu-8-6\\%
  BuPu-8-7\\%
  BuPu-8-8\\%
}
\pgfplotscreateplotcyclelist{BuPu-9}{%
  BuPu-9-1\\%
  BuPu-9-2\\%
  BuPu-9-3\\%
  BuPu-9-4\\%
  BuPu-9-5\\%
  BuPu-9-6\\%
  BuPu-9-7\\%
  BuPu-9-8\\%
  BuPu-9-9\\%
}
\pgfplotscreateplotcyclelist{RdPu-3}{%
  RdPu-3-1\\%
  RdPu-3-2\\%
  RdPu-3-3\\%
}
\pgfplotscreateplotcyclelist{RdPu-4}{%
  RdPu-4-1\\%
  RdPu-4-2\\%
  RdPu-4-3\\%
  RdPu-4-4\\%
}
\pgfplotscreateplotcyclelist{RdPu-5}{%
  RdPu-5-1\\%
  RdPu-5-2\\%
  RdPu-5-3\\%
  RdPu-5-4\\%
  RdPu-5-5\\%
}
\pgfplotscreateplotcyclelist{RdPu-6}{%
  RdPu-6-1\\%
  RdPu-6-2\\%
  RdPu-6-3\\%
  RdPu-6-4\\%
  RdPu-6-5\\%
  RdPu-6-6\\%
}
\pgfplotscreateplotcyclelist{RdPu-7}{%
  RdPu-7-1\\%
  RdPu-7-2\\%
  RdPu-7-3\\%
  RdPu-7-4\\%
  RdPu-7-5\\%
  RdPu-7-6\\%
  RdPu-7-7\\%
}
\pgfplotscreateplotcyclelist{RdPu-8}{%
  RdPu-8-1\\%
  RdPu-8-2\\%
  RdPu-8-3\\%
  RdPu-8-4\\%
  RdPu-8-5\\%
  RdPu-8-6\\%
  RdPu-8-7\\%
  RdPu-8-8\\%
}
\pgfplotscreateplotcyclelist{RdPu-9}{%
  RdPu-9-1\\%
  RdPu-9-2\\%
  RdPu-9-3\\%
  RdPu-9-4\\%
  RdPu-9-5\\%
  RdPu-9-6\\%
  RdPu-9-7\\%
  RdPu-9-8\\%
  RdPu-9-9\\%
}
\pgfplotscreateplotcyclelist{PuRd-3}{%
  PuRd-3-1\\%
  PuRd-3-2\\%
  PuRd-3-3\\%
}
\pgfplotscreateplotcyclelist{PuRd-4}{%
  PuRd-4-1\\%
  PuRd-4-2\\%
  PuRd-4-3\\%
  PuRd-4-4\\%
}
\pgfplotscreateplotcyclelist{PuRd-5}{%
  PuRd-5-1\\%
  PuRd-5-2\\%
  PuRd-5-3\\%
  PuRd-5-4\\%
  PuRd-5-5\\%
}
\pgfplotscreateplotcyclelist{PuRd-6}{%
  PuRd-6-1\\%
  PuRd-6-2\\%
  PuRd-6-3\\%
  PuRd-6-4\\%
  PuRd-6-5\\%
  PuRd-6-6\\%
}
\pgfplotscreateplotcyclelist{PuRd-7}{%
  PuRd-7-1\\%
  PuRd-7-2\\%
  PuRd-7-3\\%
  PuRd-7-4\\%
  PuRd-7-5\\%
  PuRd-7-6\\%
  PuRd-7-7\\%
}
\pgfplotscreateplotcyclelist{PuRd-8}{%
  PuRd-8-1\\%
  PuRd-8-2\\%
  PuRd-8-3\\%
  PuRd-8-4\\%
  PuRd-8-5\\%
  PuRd-8-6\\%
  PuRd-8-7\\%
  PuRd-8-8\\%
}
\pgfplotscreateplotcyclelist{PuRd-9}{%
  PuRd-9-1\\%
  PuRd-9-2\\%
  PuRd-9-3\\%
  PuRd-9-4\\%
  PuRd-9-5\\%
  PuRd-9-6\\%
  PuRd-9-7\\%
  PuRd-9-8\\%
  PuRd-9-9\\%
}
\pgfplotscreateplotcyclelist{OrRd-3}{%
  OrRd-3-1\\%
  OrRd-3-2\\%
  OrRd-3-3\\%
}
\pgfplotscreateplotcyclelist{OrRd-4}{%
  OrRd-4-1\\%
  OrRd-4-2\\%
  OrRd-4-3\\%
  OrRd-4-4\\%
}
\pgfplotscreateplotcyclelist{OrRd-5}{%
  OrRd-5-1\\%
  OrRd-5-2\\%
  OrRd-5-3\\%
  OrRd-5-4\\%
  OrRd-5-5\\%
}
\pgfplotscreateplotcyclelist{OrRd-6}{%
  OrRd-6-1\\%
  OrRd-6-2\\%
  OrRd-6-3\\%
  OrRd-6-4\\%
  OrRd-6-5\\%
  OrRd-6-6\\%
}
\pgfplotscreateplotcyclelist{OrRd-7}{%
  OrRd-7-1\\%
  OrRd-7-2\\%
  OrRd-7-3\\%
  OrRd-7-4\\%
  OrRd-7-5\\%
  OrRd-7-6\\%
  OrRd-7-7\\%
}
\pgfplotscreateplotcyclelist{OrRd-8}{%
  OrRd-8-1\\%
  OrRd-8-2\\%
  OrRd-8-3\\%
  OrRd-8-4\\%
  OrRd-8-5\\%
  OrRd-8-6\\%
  OrRd-8-7\\%
  OrRd-8-8\\%
}
\pgfplotscreateplotcyclelist{OrRd-9}{%
  OrRd-9-1\\%
  OrRd-9-2\\%
  OrRd-9-3\\%
  OrRd-9-4\\%
  OrRd-9-5\\%
  OrRd-9-6\\%
  OrRd-9-7\\%
  OrRd-9-8\\%
  OrRd-9-9\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-3}{%
  YlOrRd-3-1\\%
  YlOrRd-3-2\\%
  YlOrRd-3-3\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-4}{%
  YlOrRd-4-1\\%
  YlOrRd-4-2\\%
  YlOrRd-4-3\\%
  YlOrRd-4-4\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-5}{%
  YlOrRd-5-1\\%
  YlOrRd-5-2\\%
  YlOrRd-5-3\\%
  YlOrRd-5-4\\%
  YlOrRd-5-5\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-6}{%
  YlOrRd-6-1\\%
  YlOrRd-6-2\\%
  YlOrRd-6-3\\%
  YlOrRd-6-4\\%
  YlOrRd-6-5\\%
  YlOrRd-6-6\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-7}{%
  YlOrRd-7-1\\%
  YlOrRd-7-2\\%
  YlOrRd-7-3\\%
  YlOrRd-7-4\\%
  YlOrRd-7-5\\%
  YlOrRd-7-6\\%
  YlOrRd-7-7\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-8}{%
  YlOrRd-8-1\\%
  YlOrRd-8-2\\%
  YlOrRd-8-3\\%
  YlOrRd-8-4\\%
  YlOrRd-8-5\\%
  YlOrRd-8-6\\%
  YlOrRd-8-7\\%
  YlOrRd-8-8\\%
}
\pgfplotscreateplotcyclelist{YlOrRd-9}{%
  YlOrRd-9-1\\%
  YlOrRd-9-2\\%
  YlOrRd-9-3\\%
  YlOrRd-9-4\\%
  YlOrRd-9-5\\%
  YlOrRd-9-6\\%
  YlOrRd-9-7\\%
  YlOrRd-9-8\\%
  YlOrRd-9-9\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-3}{%
  YlOrBr-3-1\\%
  YlOrBr-3-2\\%
  YlOrBr-3-3\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-4}{%
  YlOrBr-4-1\\%
  YlOrBr-4-2\\%
  YlOrBr-4-3\\%
  YlOrBr-4-4\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-5}{%
  YlOrBr-5-1\\%
  YlOrBr-5-2\\%
  YlOrBr-5-3\\%
  YlOrBr-5-4\\%
  YlOrBr-5-5\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-6}{%
  YlOrBr-6-1\\%
  YlOrBr-6-2\\%
  YlOrBr-6-3\\%
  YlOrBr-6-4\\%
  YlOrBr-6-5\\%
  YlOrBr-6-6\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-7}{%
  YlOrBr-7-1\\%
  YlOrBr-7-2\\%
  YlOrBr-7-3\\%
  YlOrBr-7-4\\%
  YlOrBr-7-5\\%
  YlOrBr-7-6\\%
  YlOrBr-7-7\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-8}{%
  YlOrBr-8-1\\%
  YlOrBr-8-2\\%
  YlOrBr-8-3\\%
  YlOrBr-8-4\\%
  YlOrBr-8-5\\%
  YlOrBr-8-6\\%
  YlOrBr-8-7\\%
  YlOrBr-8-8\\%
}
\pgfplotscreateplotcyclelist{YlOrBr-9}{%
  YlOrBr-9-1\\%
  YlOrBr-9-2\\%
  YlOrBr-9-3\\%
  YlOrBr-9-4\\%
  YlOrBr-9-5\\%
  YlOrBr-9-6\\%
  YlOrBr-9-7\\%
  YlOrBr-9-8\\%
  YlOrBr-9-9\\%
}
\pgfplotscreateplotcyclelist{Purples-3}{%
  Purples-3-1\\%
  Purples-3-2\\%
  Purples-3-3\\%
}
\pgfplotscreateplotcyclelist{Purples-4}{%
  Purples-4-1\\%
  Purples-4-2\\%
  Purples-4-3\\%
  Purples-4-4\\%
}
\pgfplotscreateplotcyclelist{Purples-5}{%
  Purples-5-1\\%
  Purples-5-2\\%
  Purples-5-3\\%
  Purples-5-4\\%
  Purples-5-5\\%
}
\pgfplotscreateplotcyclelist{Purples-6}{%
  Purples-6-1\\%
  Purples-6-2\\%
  Purples-6-3\\%
  Purples-6-4\\%
  Purples-6-5\\%
  Purples-6-6\\%
}
\pgfplotscreateplotcyclelist{Purples-7}{%
  Purples-7-1\\%
  Purples-7-2\\%
  Purples-7-3\\%
  Purples-7-4\\%
  Purples-7-5\\%
  Purples-7-6\\%
  Purples-7-7\\%
}
\pgfplotscreateplotcyclelist{Purples-8}{%
  Purples-8-1\\%
  Purples-8-2\\%
  Purples-8-3\\%
  Purples-8-4\\%
  Purples-8-5\\%
  Purples-8-6\\%
  Purples-8-7\\%
  Purples-8-8\\%
}
\pgfplotscreateplotcyclelist{Purples-9}{%
  Purples-9-1\\%
  Purples-9-2\\%
  Purples-9-3\\%
  Purples-9-4\\%
  Purples-9-5\\%
  Purples-9-6\\%
  Purples-9-7\\%
  Purples-9-8\\%
  Purples-9-9\\%
}
\pgfplotscreateplotcyclelist{Blues-3}{%
  Blues-3-1\\%
  Blues-3-2\\%
  Blues-3-3\\%
}
\pgfplotscreateplotcyclelist{Blues-4}{%
  Blues-4-1\\%
  Blues-4-2\\%
  Blues-4-3\\%
  Blues-4-4\\%
}
\pgfplotscreateplotcyclelist{Blues-5}{%
  Blues-5-1\\%
  Blues-5-2\\%
  Blues-5-3\\%
  Blues-5-4\\%
  Blues-5-5\\%
}
\pgfplotscreateplotcyclelist{Blues-6}{%
  Blues-6-1\\%
  Blues-6-2\\%
  Blues-6-3\\%
  Blues-6-4\\%
  Blues-6-5\\%
  Blues-6-6\\%
}
\pgfplotscreateplotcyclelist{Blues-7}{%
  Blues-7-1\\%
  Blues-7-2\\%
  Blues-7-3\\%
  Blues-7-4\\%
  Blues-7-5\\%
  Blues-7-6\\%
  Blues-7-7\\%
}
\pgfplotscreateplotcyclelist{Blues-8}{%
  Blues-8-1\\%
  Blues-8-2\\%
  Blues-8-3\\%
  Blues-8-4\\%
  Blues-8-5\\%
  Blues-8-6\\%
  Blues-8-7\\%
  Blues-8-8\\%
}
\pgfplotscreateplotcyclelist{Blues-9}{%
  Blues-9-1\\%
  Blues-9-2\\%
  Blues-9-3\\%
  Blues-9-4\\%
  Blues-9-5\\%
  Blues-9-6\\%
  Blues-9-7\\%
  Blues-9-8\\%
  Blues-9-9\\%
}
\pgfplotscreateplotcyclelist{Greens-3}{%
  Greens-3-1\\%
  Greens-3-2\\%
  Greens-3-3\\%
}
\pgfplotscreateplotcyclelist{Greens-4}{%
  Greens-4-1\\%
  Greens-4-2\\%
  Greens-4-3\\%
  Greens-4-4\\%
}
\pgfplotscreateplotcyclelist{Greens-5}{%
  Greens-5-1\\%
  Greens-5-2\\%
  Greens-5-3\\%
  Greens-5-4\\%
  Greens-5-5\\%
}
\pgfplotscreateplotcyclelist{Greens-6}{%
  Greens-6-1\\%
  Greens-6-2\\%
  Greens-6-3\\%
  Greens-6-4\\%
  Greens-6-5\\%
  Greens-6-6\\%
}
\pgfplotscreateplotcyclelist{Greens-7}{%
  Greens-7-1\\%
  Greens-7-2\\%
  Greens-7-3\\%
  Greens-7-4\\%
  Greens-7-5\\%
  Greens-7-6\\%
  Greens-7-7\\%
}
\pgfplotscreateplotcyclelist{Greens-8}{%
  Greens-8-1\\%
  Greens-8-2\\%
  Greens-8-3\\%
  Greens-8-4\\%
  Greens-8-5\\%
  Greens-8-6\\%
  Greens-8-7\\%
  Greens-8-8\\%
}
\pgfplotscreateplotcyclelist{Greens-9}{%
  Greens-9-1\\%
  Greens-9-2\\%
  Greens-9-3\\%
  Greens-9-4\\%
  Greens-9-5\\%
  Greens-9-6\\%
  Greens-9-7\\%
  Greens-9-8\\%
  Greens-9-9\\%
}
\pgfplotscreateplotcyclelist{Oranges-3}{%
  Oranges-3-1\\%
  Oranges-3-2\\%
  Oranges-3-3\\%
}
\pgfplotscreateplotcyclelist{Oranges-4}{%
  Oranges-4-1\\%
  Oranges-4-2\\%
  Oranges-4-3\\%
  Oranges-4-4\\%
}
\pgfplotscreateplotcyclelist{Oranges-5}{%
  Oranges-5-1\\%
  Oranges-5-2\\%
  Oranges-5-3\\%
  Oranges-5-4\\%
  Oranges-5-5\\%
}
\pgfplotscreateplotcyclelist{Oranges-6}{%
  Oranges-6-1\\%
  Oranges-6-2\\%
  Oranges-6-3\\%
  Oranges-6-4\\%
  Oranges-6-5\\%
  Oranges-6-6\\%
}
\pgfplotscreateplotcyclelist{Oranges-7}{%
  Oranges-7-1\\%
  Oranges-7-2\\%
  Oranges-7-3\\%
  Oranges-7-4\\%
  Oranges-7-5\\%
  Oranges-7-6\\%
  Oranges-7-7\\%
}
\pgfplotscreateplotcyclelist{Oranges-8}{%
  Oranges-8-1\\%
  Oranges-8-2\\%
  Oranges-8-3\\%
  Oranges-8-4\\%
  Oranges-8-5\\%
  Oranges-8-6\\%
  Oranges-8-7\\%
  Oranges-8-8\\%
}
\pgfplotscreateplotcyclelist{Oranges-9}{%
  Oranges-9-1\\%
  Oranges-9-2\\%
  Oranges-9-3\\%
  Oranges-9-4\\%
  Oranges-9-5\\%
  Oranges-9-6\\%
  Oranges-9-7\\%
  Oranges-9-8\\%
  Oranges-9-9\\%
}
\pgfplotscreateplotcyclelist{Reds-3}{%
  Reds-3-1\\%
  Reds-3-2\\%
  Reds-3-3\\%
}
\pgfplotscreateplotcyclelist{Reds-4}{%
  Reds-4-1\\%
  Reds-4-2\\%
  Reds-4-3\\%
  Reds-4-4\\%
}
\pgfplotscreateplotcyclelist{Reds-5}{%
  Reds-5-1\\%
  Reds-5-2\\%
  Reds-5-3\\%
  Reds-5-4\\%
  Reds-5-5\\%
}
\pgfplotscreateplotcyclelist{Reds-6}{%
  Reds-6-1\\%
  Reds-6-2\\%
  Reds-6-3\\%
  Reds-6-4\\%
  Reds-6-5\\%
  Reds-6-6\\%
}
\pgfplotscreateplotcyclelist{Reds-7}{%
  Reds-7-1\\%
  Reds-7-2\\%
  Reds-7-3\\%
  Reds-7-4\\%
  Reds-7-5\\%
  Reds-7-6\\%
  Reds-7-7\\%
}
\pgfplotscreateplotcyclelist{Reds-8}{%
  Reds-8-1\\%
  Reds-8-2\\%
  Reds-8-3\\%
  Reds-8-4\\%
  Reds-8-5\\%
  Reds-8-6\\%
  Reds-8-7\\%
  Reds-8-8\\%
}
\pgfplotscreateplotcyclelist{Reds-9}{%
  Reds-9-1\\%
  Reds-9-2\\%
  Reds-9-3\\%
  Reds-9-4\\%
  Reds-9-5\\%
  Reds-9-6\\%
  Reds-9-7\\%
  Reds-9-8\\%
  Reds-9-9\\%
}
\pgfplotscreateplotcyclelist{Greys-3}{%
  Greys-3-1\\%
  Greys-3-2\\%
  Greys-3-3\\%
}
\pgfplotscreateplotcyclelist{Greys-4}{%
  Greys-4-1\\%
  Greys-4-2\\%
  Greys-4-3\\%
  Greys-4-4\\%
}
\pgfplotscreateplotcyclelist{Greys-5}{%
  Greys-5-1\\%
  Greys-5-2\\%
  Greys-5-3\\%
  Greys-5-4\\%
  Greys-5-5\\%
}
\pgfplotscreateplotcyclelist{Greys-6}{%
  Greys-6-1\\%
  Greys-6-2\\%
  Greys-6-3\\%
  Greys-6-4\\%
  Greys-6-5\\%
  Greys-6-6\\%
}
\pgfplotscreateplotcyclelist{Greys-7}{%
  Greys-7-1\\%
  Greys-7-2\\%
  Greys-7-3\\%
  Greys-7-4\\%
  Greys-7-5\\%
  Greys-7-6\\%
  Greys-7-7\\%
}
\pgfplotscreateplotcyclelist{Greys-8}{%
  Greys-8-1\\%
  Greys-8-2\\%
  Greys-8-3\\%
  Greys-8-4\\%
  Greys-8-5\\%
  Greys-8-6\\%
  Greys-8-7\\%
  Greys-8-8\\%
}
\pgfplotscreateplotcyclelist{Greys-9}{%
  Greys-9-1\\%
  Greys-9-2\\%
  Greys-9-3\\%
  Greys-9-4\\%
  Greys-9-5\\%
  Greys-9-6\\%
  Greys-9-7\\%
  Greys-9-8\\%
  Greys-9-9\\%
}
\pgfplotscreateplotcyclelist{PuOr-3}{%
  PuOr-3-1\\%
  PuOr-3-2\\%
  PuOr-3-3\\%
}
\pgfplotscreateplotcyclelist{PuOr-4}{%
  PuOr-4-1\\%
  PuOr-4-2\\%
  PuOr-4-3\\%
  PuOr-4-4\\%
}
\pgfplotscreateplotcyclelist{PuOr-5}{%
  PuOr-5-1\\%
  PuOr-5-2\\%
  PuOr-5-3\\%
  PuOr-5-4\\%
  PuOr-5-5\\%
}
\pgfplotscreateplotcyclelist{PuOr-6}{%
  PuOr-6-1\\%
  PuOr-6-2\\%
  PuOr-6-3\\%
  PuOr-6-4\\%
  PuOr-6-5\\%
  PuOr-6-6\\%
}
\pgfplotscreateplotcyclelist{PuOr-7}{%
  PuOr-7-1\\%
  PuOr-7-2\\%
  PuOr-7-3\\%
  PuOr-7-4\\%
  PuOr-7-5\\%
  PuOr-7-6\\%
  PuOr-7-7\\%
}
\pgfplotscreateplotcyclelist{PuOr-8}{%
  PuOr-8-1\\%
  PuOr-8-2\\%
  PuOr-8-3\\%
  PuOr-8-4\\%
  PuOr-8-5\\%
  PuOr-8-6\\%
  PuOr-8-7\\%
  PuOr-8-8\\%
}
\pgfplotscreateplotcyclelist{PuOr-9}{%
  PuOr-9-1\\%
  PuOr-9-2\\%
  PuOr-9-3\\%
  PuOr-9-4\\%
  PuOr-9-5\\%
  PuOr-9-6\\%
  PuOr-9-7\\%
  PuOr-9-8\\%
  PuOr-9-9\\%
}
\pgfplotscreateplotcyclelist{PuOr-10}{%
  PuOr-10-1\\%
  PuOr-10-2\\%
  PuOr-10-3\\%
  PuOr-10-4\\%
  PuOr-10-5\\%
  PuOr-10-6\\%
  PuOr-10-7\\%
  PuOr-10-8\\%
  PuOr-10-9\\%
  PuOr-10-10\\%
}
\pgfplotscreateplotcyclelist{PuOr-11}{%
  PuOr-11-1\\%
  PuOr-11-2\\%
  PuOr-11-3\\%
  PuOr-11-4\\%
  PuOr-11-5\\%
  PuOr-11-6\\%
  PuOr-11-7\\%
  PuOr-11-8\\%
  PuOr-11-9\\%
  PuOr-11-10\\%
  PuOr-11-11\\%
}
\pgfplotscreateplotcyclelist{BrBG-3}{%
  BrBG-3-1\\%
  BrBG-3-2\\%
  BrBG-3-3\\%
}
\pgfplotscreateplotcyclelist{BrBG-4}{%
  BrBG-4-1\\%
  BrBG-4-2\\%
  BrBG-4-3\\%
  BrBG-4-4\\%
}
\pgfplotscreateplotcyclelist{BrBG-5}{%
  BrBG-5-1\\%
  BrBG-5-2\\%
  BrBG-5-3\\%
  BrBG-5-4\\%
  BrBG-5-5\\%
}
\pgfplotscreateplotcyclelist{BrBG-6}{%
  BrBG-6-1\\%
  BrBG-6-2\\%
  BrBG-6-3\\%
  BrBG-6-4\\%
  BrBG-6-5\\%
  BrBG-6-6\\%
}
\pgfplotscreateplotcyclelist{BrBG-7}{%
  BrBG-7-1\\%
  BrBG-7-2\\%
  BrBG-7-3\\%
  BrBG-7-4\\%
  BrBG-7-5\\%
  BrBG-7-6\\%
  BrBG-7-7\\%
}
\pgfplotscreateplotcyclelist{BrBG-8}{%
  BrBG-8-1\\%
  BrBG-8-2\\%
  BrBG-8-3\\%
  BrBG-8-4\\%
  BrBG-8-5\\%
  BrBG-8-6\\%
  BrBG-8-7\\%
  BrBG-8-8\\%
}
\pgfplotscreateplotcyclelist{BrBG-9}{%
  BrBG-9-1\\%
  BrBG-9-2\\%
  BrBG-9-3\\%
  BrBG-9-4\\%
  BrBG-9-5\\%
  BrBG-9-6\\%
  BrBG-9-7\\%
  BrBG-9-8\\%
  BrBG-9-9\\%
}
\pgfplotscreateplotcyclelist{BrBG-10}{%
  BrBG-10-1\\%
  BrBG-10-2\\%
  BrBG-10-3\\%
  BrBG-10-4\\%
  BrBG-10-5\\%
  BrBG-10-6\\%
  BrBG-10-7\\%
  BrBG-10-8\\%
  BrBG-10-9\\%
  BrBG-10-10\\%
}
\pgfplotscreateplotcyclelist{BrBG-11}{%
  BrBG-11-1\\%
  BrBG-11-2\\%
  BrBG-11-3\\%
  BrBG-11-4\\%
  BrBG-11-5\\%
  BrBG-11-6\\%
  BrBG-11-7\\%
  BrBG-11-8\\%
  BrBG-11-9\\%
  BrBG-11-10\\%
  BrBG-11-11\\%
}
\pgfplotscreateplotcyclelist{PRGn-3}{%
  PRGn-3-1\\%
  PRGn-3-2\\%
  PRGn-3-3\\%
}
\pgfplotscreateplotcyclelist{PRGn-4}{%
  PRGn-4-1\\%
  PRGn-4-2\\%
  PRGn-4-3\\%
  PRGn-4-4\\%
}
\pgfplotscreateplotcyclelist{PRGn-5}{%
  PRGn-5-1\\%
  PRGn-5-2\\%
  PRGn-5-3\\%
  PRGn-5-4\\%
  PRGn-5-5\\%
}
\pgfplotscreateplotcyclelist{PRGn-6}{%
  PRGn-6-1\\%
  PRGn-6-2\\%
  PRGn-6-3\\%
  PRGn-6-4\\%
  PRGn-6-5\\%
  PRGn-6-6\\%
}
\pgfplotscreateplotcyclelist{PRGn-7}{%
  PRGn-7-1\\%
  PRGn-7-2\\%
  PRGn-7-3\\%
  PRGn-7-4\\%
  PRGn-7-5\\%
  PRGn-7-6\\%
  PRGn-7-7\\%
}
\pgfplotscreateplotcyclelist{PRGn-8}{%
  PRGn-8-1\\%
  PRGn-8-2\\%
  PRGn-8-3\\%
  PRGn-8-4\\%
  PRGn-8-5\\%
  PRGn-8-6\\%
  PRGn-8-7\\%
  PRGn-8-8\\%
}
\pgfplotscreateplotcyclelist{PRGn-9}{%
  PRGn-9-1\\%
  PRGn-9-2\\%
  PRGn-9-3\\%
  PRGn-9-4\\%
  PRGn-9-5\\%
  PRGn-9-6\\%
  PRGn-9-7\\%
  PRGn-9-8\\%
  PRGn-9-9\\%
}
\pgfplotscreateplotcyclelist{PRGn-10}{%
  PRGn-10-1\\%
  PRGn-10-2\\%
  PRGn-10-3\\%
  PRGn-10-4\\%
  PRGn-10-5\\%
  PRGn-10-6\\%
  PRGn-10-7\\%
  PRGn-10-8\\%
  PRGn-10-9\\%
  PRGn-10-10\\%
}
\pgfplotscreateplotcyclelist{PRGn-11}{%
  PRGn-11-1\\%
  PRGn-11-2\\%
  PRGn-11-3\\%
  PRGn-11-4\\%
  PRGn-11-5\\%
  PRGn-11-6\\%
  PRGn-11-7\\%
  PRGn-11-8\\%
  PRGn-11-9\\%
  PRGn-11-10\\%
  PRGn-11-11\\%
}
\pgfplotscreateplotcyclelist{PiYG-3}{%
  PiYG-3-1\\%
  PiYG-3-2\\%
  PiYG-3-3\\%
}
\pgfplotscreateplotcyclelist{PiYG-4}{%
  PiYG-4-1\\%
  PiYG-4-2\\%
  PiYG-4-3\\%
  PiYG-4-4\\%
}
\pgfplotscreateplotcyclelist{PiYG-5}{%
  PiYG-5-1\\%
  PiYG-5-2\\%
  PiYG-5-3\\%
  PiYG-5-4\\%
  PiYG-5-5\\%
}
\pgfplotscreateplotcyclelist{PiYG-6}{%
  PiYG-6-1\\%
  PiYG-6-2\\%
  PiYG-6-3\\%
  PiYG-6-4\\%
  PiYG-6-5\\%
  PiYG-6-6\\%
}
\pgfplotscreateplotcyclelist{PiYG-7}{%
  PiYG-7-1\\%
  PiYG-7-2\\%
  PiYG-7-3\\%
  PiYG-7-4\\%
  PiYG-7-5\\%
  PiYG-7-6\\%
  PiYG-7-7\\%
}
\pgfplotscreateplotcyclelist{PiYG-8}{%
  PiYG-8-1\\%
  PiYG-8-2\\%
  PiYG-8-3\\%
  PiYG-8-4\\%
  PiYG-8-5\\%
  PiYG-8-6\\%
  PiYG-8-7\\%
  PiYG-8-8\\%
}
\pgfplotscreateplotcyclelist{PiYG-9}{%
  PiYG-9-1\\%
  PiYG-9-2\\%
  PiYG-9-3\\%
  PiYG-9-4\\%
  PiYG-9-5\\%
  PiYG-9-6\\%
  PiYG-9-7\\%
  PiYG-9-8\\%
  PiYG-9-9\\%
}
\pgfplotscreateplotcyclelist{PiYG-10}{%
  PiYG-10-1\\%
  PiYG-10-2\\%
  PiYG-10-3\\%
  PiYG-10-4\\%
  PiYG-10-5\\%
  PiYG-10-6\\%
  PiYG-10-7\\%
  PiYG-10-8\\%
  PiYG-10-9\\%
  PiYG-10-10\\%
}
\pgfplotscreateplotcyclelist{PiYG-11}{%
  PiYG-11-1\\%
  PiYG-11-2\\%
  PiYG-11-3\\%
  PiYG-11-4\\%
  PiYG-11-5\\%
  PiYG-11-6\\%
  PiYG-11-7\\%
  PiYG-11-8\\%
  PiYG-11-9\\%
  PiYG-11-10\\%
  PiYG-11-11\\%
}
\pgfplotscreateplotcyclelist{RdBu-3}{%
  RdBu-3-1\\%
  RdBu-3-2\\%
  RdBu-3-3\\%
}
\pgfplotscreateplotcyclelist{RdBu-4}{%
  RdBu-4-1\\%
  RdBu-4-2\\%
  RdBu-4-3\\%
  RdBu-4-4\\%
}
\pgfplotscreateplotcyclelist{RdBu-5}{%
  RdBu-5-1\\%
  RdBu-5-2\\%
  RdBu-5-3\\%
  RdBu-5-4\\%
  RdBu-5-5\\%
}
\pgfplotscreateplotcyclelist{RdBu-6}{%
  RdBu-6-1\\%
  RdBu-6-2\\%
  RdBu-6-3\\%
  RdBu-6-4\\%
  RdBu-6-5\\%
  RdBu-6-6\\%
}
\pgfplotscreateplotcyclelist{RdBu-7}{%
  RdBu-7-1\\%
  RdBu-7-2\\%
  RdBu-7-3\\%
  RdBu-7-4\\%
  RdBu-7-5\\%
  RdBu-7-6\\%
  RdBu-7-7\\%
}
\pgfplotscreateplotcyclelist{RdBu-8}{%
  RdBu-8-1\\%
  RdBu-8-2\\%
  RdBu-8-3\\%
  RdBu-8-4\\%
  RdBu-8-5\\%
  RdBu-8-6\\%
  RdBu-8-7\\%
  RdBu-8-8\\%
}
\pgfplotscreateplotcyclelist{RdBu-9}{%
  RdBu-9-1\\%
  RdBu-9-2\\%
  RdBu-9-3\\%
  RdBu-9-4\\%
  RdBu-9-5\\%
  RdBu-9-6\\%
  RdBu-9-7\\%
  RdBu-9-8\\%
  RdBu-9-9\\%
}
\pgfplotscreateplotcyclelist{RdBu-10}{%
  RdBu-10-1\\%
  RdBu-10-2\\%
  RdBu-10-3\\%
  RdBu-10-4\\%
  RdBu-10-5\\%
  RdBu-10-6\\%
  RdBu-10-7\\%
  RdBu-10-8\\%
  RdBu-10-9\\%
  RdBu-10-10\\%
}
\pgfplotscreateplotcyclelist{RdBu-11}{%
  RdBu-11-1\\%
  RdBu-11-2\\%
  RdBu-11-3\\%
  RdBu-11-4\\%
  RdBu-11-5\\%
  RdBu-11-6\\%
  RdBu-11-7\\%
  RdBu-11-8\\%
  RdBu-11-9\\%
  RdBu-11-10\\%
  RdBu-11-11\\%
}
\pgfplotscreateplotcyclelist{RdGy-3}{%
  RdGy-3-1\\%
  RdGy-3-2\\%
  RdGy-3-3\\%
}
\pgfplotscreateplotcyclelist{RdGy-4}{%
  RdGy-4-1\\%
  RdGy-4-2\\%
  RdGy-4-3\\%
  RdGy-4-4\\%
}
\pgfplotscreateplotcyclelist{RdGy-5}{%
  RdGy-5-1\\%
  RdGy-5-2\\%
  RdGy-5-3\\%
  RdGy-5-4\\%
  RdGy-5-5\\%
}
\pgfplotscreateplotcyclelist{RdGy-6}{%
  RdGy-6-1\\%
  RdGy-6-2\\%
  RdGy-6-3\\%
  RdGy-6-4\\%
  RdGy-6-5\\%
  RdGy-6-6\\%
}
\pgfplotscreateplotcyclelist{RdGy-7}{%
  RdGy-7-1\\%
  RdGy-7-2\\%
  RdGy-7-3\\%
  RdGy-7-4\\%
  RdGy-7-5\\%
  RdGy-7-6\\%
  RdGy-7-7\\%
}
\pgfplotscreateplotcyclelist{RdGy-8}{%
  RdGy-8-1\\%
  RdGy-8-2\\%
  RdGy-8-3\\%
  RdGy-8-4\\%
  RdGy-8-5\\%
  RdGy-8-6\\%
  RdGy-8-7\\%
  RdGy-8-8\\%
}
\pgfplotscreateplotcyclelist{RdGy-9}{%
  RdGy-9-1\\%
  RdGy-9-2\\%
  RdGy-9-3\\%
  RdGy-9-4\\%
  RdGy-9-5\\%
  RdGy-9-6\\%
  RdGy-9-7\\%
  RdGy-9-8\\%
  RdGy-9-9\\%
}
\pgfplotscreateplotcyclelist{RdGy-10}{%
  RdGy-10-1\\%
  RdGy-10-2\\%
  RdGy-10-3\\%
  RdGy-10-4\\%
  RdGy-10-5\\%
  RdGy-10-6\\%
  RdGy-10-7\\%
  RdGy-10-8\\%
  RdGy-10-9\\%
  RdGy-10-10\\%
}
\pgfplotscreateplotcyclelist{RdGy-11}{%
  RdGy-11-1\\%
  RdGy-11-2\\%
  RdGy-11-3\\%
  RdGy-11-4\\%
  RdGy-11-5\\%
  RdGy-11-6\\%
  RdGy-11-7\\%
  RdGy-11-8\\%
  RdGy-11-9\\%
  RdGy-11-10\\%
  RdGy-11-11\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-3}{%
  RdYlBu-3-1\\%
  RdYlBu-3-2\\%
  RdYlBu-3-3\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-4}{%
  RdYlBu-4-1\\%
  RdYlBu-4-2\\%
  RdYlBu-4-3\\%
  RdYlBu-4-4\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-5}{%
  RdYlBu-5-1\\%
  RdYlBu-5-2\\%
  RdYlBu-5-3\\%
  RdYlBu-5-4\\%
  RdYlBu-5-5\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-6}{%
  RdYlBu-6-1\\%
  RdYlBu-6-2\\%
  RdYlBu-6-3\\%
  RdYlBu-6-4\\%
  RdYlBu-6-5\\%
  RdYlBu-6-6\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-7}{%
  RdYlBu-7-1\\%
  RdYlBu-7-2\\%
  RdYlBu-7-3\\%
  RdYlBu-7-4\\%
  RdYlBu-7-5\\%
  RdYlBu-7-6\\%
  RdYlBu-7-7\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-8}{%
  RdYlBu-8-1\\%
  RdYlBu-8-2\\%
  RdYlBu-8-3\\%
  RdYlBu-8-4\\%
  RdYlBu-8-5\\%
  RdYlBu-8-6\\%
  RdYlBu-8-7\\%
  RdYlBu-8-8\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-9}{%
  RdYlBu-9-1\\%
  RdYlBu-9-2\\%
  RdYlBu-9-3\\%
  RdYlBu-9-4\\%
  RdYlBu-9-5\\%
  RdYlBu-9-6\\%
  RdYlBu-9-7\\%
  RdYlBu-9-8\\%
  RdYlBu-9-9\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-10}{%
  RdYlBu-10-1\\%
  RdYlBu-10-2\\%
  RdYlBu-10-3\\%
  RdYlBu-10-4\\%
  RdYlBu-10-5\\%
  RdYlBu-10-6\\%
  RdYlBu-10-7\\%
  RdYlBu-10-8\\%
  RdYlBu-10-9\\%
  RdYlBu-10-10\\%
}
\pgfplotscreateplotcyclelist{RdYlBu-11}{%
  RdYlBu-11-1\\%
  RdYlBu-11-2\\%
  RdYlBu-11-3\\%
  RdYlBu-11-4\\%
  RdYlBu-11-5\\%
  RdYlBu-11-6\\%
  RdYlBu-11-7\\%
  RdYlBu-11-8\\%
  RdYlBu-11-9\\%
  RdYlBu-11-10\\%
  RdYlBu-11-11\\%
}
\pgfplotscreateplotcyclelist{Spectral-3}{%
  Spectral-3-1\\%
  Spectral-3-2\\%
  Spectral-3-3\\%
}
\pgfplotscreateplotcyclelist{Spectral-4}{%
  Spectral-4-1\\%
  Spectral-4-2\\%
  Spectral-4-3\\%
  Spectral-4-4\\%
}
\pgfplotscreateplotcyclelist{Spectral-5}{%
  Spectral-5-1\\%
  Spectral-5-2\\%
  Spectral-5-3\\%
  Spectral-5-4\\%
  Spectral-5-5\\%
}
\pgfplotscreateplotcyclelist{Spectral-6}{%
  Spectral-6-1\\%
  Spectral-6-2\\%
  Spectral-6-3\\%
  Spectral-6-4\\%
  Spectral-6-5\\%
  Spectral-6-6\\%
}
\pgfplotscreateplotcyclelist{Spectral-7}{%
  Spectral-7-1\\%
  Spectral-7-2\\%
  Spectral-7-3\\%
  Spectral-7-4\\%
  Spectral-7-5\\%
  Spectral-7-6\\%
  Spectral-7-7\\%
}
\pgfplotscreateplotcyclelist{Spectral-8}{%
  Spectral-8-1\\%
  Spectral-8-2\\%
  Spectral-8-3\\%
  Spectral-8-4\\%
  Spectral-8-5\\%
  Spectral-8-6\\%
  Spectral-8-7\\%
  Spectral-8-8\\%
}
\pgfplotscreateplotcyclelist{Spectral-9}{%
  Spectral-9-1\\%
  Spectral-9-2\\%
  Spectral-9-3\\%
  Spectral-9-4\\%
  Spectral-9-5\\%
  Spectral-9-6\\%
  Spectral-9-7\\%
  Spectral-9-8\\%
  Spectral-9-9\\%
}
\pgfplotscreateplotcyclelist{Spectral-10}{%
  Spectral-10-1\\%
  Spectral-10-2\\%
  Spectral-10-3\\%
  Spectral-10-4\\%
  Spectral-10-5\\%
  Spectral-10-6\\%
  Spectral-10-7\\%
  Spectral-10-8\\%
  Spectral-10-9\\%
  Spectral-10-10\\%
}
\pgfplotscreateplotcyclelist{Spectral-11}{%
  Spectral-11-1\\%
  Spectral-11-2\\%
  Spectral-11-3\\%
  Spectral-11-4\\%
  Spectral-11-5\\%
  Spectral-11-6\\%
  Spectral-11-7\\%
  Spectral-11-8\\%
  Spectral-11-9\\%
  Spectral-11-10\\%
  Spectral-11-11\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-3}{%
  RdYlGn-3-1\\%
  RdYlGn-3-2\\%
  RdYlGn-3-3\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-4}{%
  RdYlGn-4-1\\%
  RdYlGn-4-2\\%
  RdYlGn-4-3\\%
  RdYlGn-4-4\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-5}{%
  RdYlGn-5-1\\%
  RdYlGn-5-2\\%
  RdYlGn-5-3\\%
  RdYlGn-5-4\\%
  RdYlGn-5-5\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-6}{%
  RdYlGn-6-1\\%
  RdYlGn-6-2\\%
  RdYlGn-6-3\\%
  RdYlGn-6-4\\%
  RdYlGn-6-5\\%
  RdYlGn-6-6\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-7}{%
  RdYlGn-7-1\\%
  RdYlGn-7-2\\%
  RdYlGn-7-3\\%
  RdYlGn-7-4\\%
  RdYlGn-7-5\\%
  RdYlGn-7-6\\%
  RdYlGn-7-7\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-8}{%
  RdYlGn-8-1\\%
  RdYlGn-8-2\\%
  RdYlGn-8-3\\%
  RdYlGn-8-4\\%
  RdYlGn-8-5\\%
  RdYlGn-8-6\\%
  RdYlGn-8-7\\%
  RdYlGn-8-8\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-9}{%
  RdYlGn-9-1\\%
  RdYlGn-9-2\\%
  RdYlGn-9-3\\%
  RdYlGn-9-4\\%
  RdYlGn-9-5\\%
  RdYlGn-9-6\\%
  RdYlGn-9-7\\%
  RdYlGn-9-8\\%
  RdYlGn-9-9\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-10}{%
  RdYlGn-10-1\\%
  RdYlGn-10-2\\%
  RdYlGn-10-3\\%
  RdYlGn-10-4\\%
  RdYlGn-10-5\\%
  RdYlGn-10-6\\%
  RdYlGn-10-7\\%
  RdYlGn-10-8\\%
  RdYlGn-10-9\\%
  RdYlGn-10-10\\%
}
\pgfplotscreateplotcyclelist{RdYlGn-11}{%
  RdYlGn-11-1\\%
  RdYlGn-11-2\\%
  RdYlGn-11-3\\%
  RdYlGn-11-4\\%
  RdYlGn-11-5\\%
  RdYlGn-11-6\\%
  RdYlGn-11-7\\%
  RdYlGn-11-8\\%
  RdYlGn-11-9\\%
  RdYlGn-11-10\\%
  RdYlGn-11-11\\%
}
\pgfplotscreateplotcyclelist{Set3-3}{%
  Set3-3-1\\%
  Set3-3-2\\%
  Set3-3-3\\%
}
\pgfplotscreateplotcyclelist{Set3-4}{%
  Set3-4-1\\%
  Set3-4-2\\%
  Set3-4-3\\%
  Set3-4-4\\%
}
\pgfplotscreateplotcyclelist{Set3-5}{%
  Set3-5-1\\%
  Set3-5-2\\%
  Set3-5-3\\%
  Set3-5-4\\%
  Set3-5-5\\%
}
\pgfplotscreateplotcyclelist{Set3-6}{%
  Set3-6-1\\%
  Set3-6-2\\%
  Set3-6-3\\%
  Set3-6-4\\%
  Set3-6-5\\%
  Set3-6-6\\%
}
\pgfplotscreateplotcyclelist{Set3-7}{%
  Set3-7-1\\%
  Set3-7-2\\%
  Set3-7-3\\%
  Set3-7-4\\%
  Set3-7-5\\%
  Set3-7-6\\%
  Set3-7-7\\%
}
\pgfplotscreateplotcyclelist{Set3-8}{%
  Set3-8-1\\%
  Set3-8-2\\%
  Set3-8-3\\%
  Set3-8-4\\%
  Set3-8-5\\%
  Set3-8-6\\%
  Set3-8-7\\%
  Set3-8-8\\%
}
\pgfplotscreateplotcyclelist{Set3-9}{%
  Set3-9-1\\%
  Set3-9-2\\%
  Set3-9-3\\%
  Set3-9-4\\%
  Set3-9-5\\%
  Set3-9-6\\%
  Set3-9-7\\%
  Set3-9-8\\%
  Set3-9-9\\%
}
\pgfplotscreateplotcyclelist{Set3-10}{%
  Set3-10-1\\%
  Set3-10-2\\%
  Set3-10-3\\%
  Set3-10-4\\%
  Set3-10-5\\%
  Set3-10-6\\%
  Set3-10-7\\%
  Set3-10-8\\%
  Set3-10-9\\%
  Set3-10-10\\%
}
\pgfplotscreateplotcyclelist{Set3-11}{%
  Set3-11-1\\%
  Set3-11-2\\%
  Set3-11-3\\%
  Set3-11-4\\%
  Set3-11-5\\%
  Set3-11-6\\%
  Set3-11-7\\%
  Set3-11-8\\%
  Set3-11-9\\%
  Set3-11-10\\%
  Set3-11-11\\%
}
\pgfplotscreateplotcyclelist{Set3-12}{%
  Set3-12-1\\%
  Set3-12-2\\%
  Set3-12-3\\%
  Set3-12-4\\%
  Set3-12-5\\%
  Set3-12-6\\%
  Set3-12-7\\%
  Set3-12-8\\%
  Set3-12-9\\%
  Set3-12-10\\%
  Set3-12-11\\%
  Set3-12-12\\%
}
\pgfplotscreateplotcyclelist{Pastel1-3}{%
  Pastel1-3-1\\%
  Pastel1-3-2\\%
  Pastel1-3-3\\%
}
\pgfplotscreateplotcyclelist{Pastel1-4}{%
  Pastel1-4-1\\%
  Pastel1-4-2\\%
  Pastel1-4-3\\%
  Pastel1-4-4\\%
}
\pgfplotscreateplotcyclelist{Pastel1-5}{%
  Pastel1-5-1\\%
  Pastel1-5-2\\%
  Pastel1-5-3\\%
  Pastel1-5-4\\%
  Pastel1-5-5\\%
}
\pgfplotscreateplotcyclelist{Pastel1-6}{%
  Pastel1-6-1\\%
  Pastel1-6-2\\%
  Pastel1-6-3\\%
  Pastel1-6-4\\%
  Pastel1-6-5\\%
  Pastel1-6-6\\%
}
\pgfplotscreateplotcyclelist{Pastel1-7}{%
  Pastel1-7-1\\%
  Pastel1-7-2\\%
  Pastel1-7-3\\%
  Pastel1-7-4\\%
  Pastel1-7-5\\%
  Pastel1-7-6\\%
  Pastel1-7-7\\%
}
\pgfplotscreateplotcyclelist{Pastel1-8}{%
  Pastel1-8-1\\%
  Pastel1-8-2\\%
  Pastel1-8-3\\%
  Pastel1-8-4\\%
  Pastel1-8-5\\%
  Pastel1-8-6\\%
  Pastel1-8-7\\%
  Pastel1-8-8\\%
}
\pgfplotscreateplotcyclelist{Pastel1-9}{%
  Pastel1-9-1\\%
  Pastel1-9-2\\%
  Pastel1-9-3\\%
  Pastel1-9-4\\%
  Pastel1-9-5\\%
  Pastel1-9-6\\%
  Pastel1-9-7\\%
  Pastel1-9-8\\%
  Pastel1-9-9\\%
}
\pgfplotscreateplotcyclelist{Set1-3}{%
  Set1-3-1\\%
  Set1-3-2\\%
  Set1-3-3\\%
}
\pgfplotscreateplotcyclelist{Set1-4}{%
  Set1-4-1\\%
  Set1-4-2\\%
  Set1-4-3\\%
  Set1-4-4\\%
}
\pgfplotscreateplotcyclelist{Set1-5}{%
  Set1-5-1\\%
  Set1-5-2\\%
  Set1-5-3\\%
  Set1-5-4\\%
  Set1-5-5\\%
}
\pgfplotscreateplotcyclelist{Set1-6}{%
  Set1-6-1\\%
  Set1-6-2\\%
  Set1-6-3\\%
  Set1-6-4\\%
  Set1-6-5\\%
  Set1-6-6\\%
}
\pgfplotscreateplotcyclelist{Set1-7}{%
  Set1-7-1\\%
  Set1-7-2\\%
  Set1-7-3\\%
  Set1-7-4\\%
  Set1-7-5\\%
  Set1-7-6\\%
  Set1-7-7\\%
}
\pgfplotscreateplotcyclelist{Set1-8}{%
  Set1-8-1\\%
  Set1-8-2\\%
  Set1-8-3\\%
  Set1-8-4\\%
  Set1-8-5\\%
  Set1-8-6\\%
  Set1-8-7\\%
  Set1-8-8\\%
}
\pgfplotscreateplotcyclelist{Set1-9}{%
  Set1-9-1\\%
  Set1-9-2\\%
  Set1-9-3\\%
  Set1-9-4\\%
  Set1-9-5\\%
  Set1-9-6\\%
  Set1-9-7\\%
  Set1-9-8\\%
  Set1-9-9\\%
}
\pgfplotscreateplotcyclelist{Pastel2-3}{%
  Pastel2-3-1\\%
  Pastel2-3-2\\%
  Pastel2-3-3\\%
}
\pgfplotscreateplotcyclelist{Pastel2-4}{%
  Pastel2-4-1\\%
  Pastel2-4-2\\%
  Pastel2-4-3\\%
  Pastel2-4-4\\%
}
\pgfplotscreateplotcyclelist{Pastel2-5}{%
  Pastel2-5-1\\%
  Pastel2-5-2\\%
  Pastel2-5-3\\%
  Pastel2-5-4\\%
  Pastel2-5-5\\%
}
\pgfplotscreateplotcyclelist{Pastel2-6}{%
  Pastel2-6-1\\%
  Pastel2-6-2\\%
  Pastel2-6-3\\%
  Pastel2-6-4\\%
  Pastel2-6-5\\%
  Pastel2-6-6\\%
}
\pgfplotscreateplotcyclelist{Pastel2-7}{%
  Pastel2-7-1\\%
  Pastel2-7-2\\%
  Pastel2-7-3\\%
  Pastel2-7-4\\%
  Pastel2-7-5\\%
  Pastel2-7-6\\%
  Pastel2-7-7\\%
}
\pgfplotscreateplotcyclelist{Pastel2-8}{%
  Pastel2-8-1\\%
  Pastel2-8-2\\%
  Pastel2-8-3\\%
  Pastel2-8-4\\%
  Pastel2-8-5\\%
  Pastel2-8-6\\%
  Pastel2-8-7\\%
  Pastel2-8-8\\%
}
\pgfplotscreateplotcyclelist{Set2-3}{%
  Set2-3-1\\%
  Set2-3-2\\%
  Set2-3-3\\%
}
\pgfplotscreateplotcyclelist{Set2-4}{%
  Set2-4-1\\%
  Set2-4-2\\%
  Set2-4-3\\%
  Set2-4-4\\%
}
\pgfplotscreateplotcyclelist{Set2-5}{%
  Set2-5-1\\%
  Set2-5-2\\%
  Set2-5-3\\%
  Set2-5-4\\%
  Set2-5-5\\%
}
\pgfplotscreateplotcyclelist{Set2-6}{%
  Set2-6-1\\%
  Set2-6-2\\%
  Set2-6-3\\%
  Set2-6-4\\%
  Set2-6-5\\%
  Set2-6-6\\%
}
\pgfplotscreateplotcyclelist{Set2-7}{%
  Set2-7-1\\%
  Set2-7-2\\%
  Set2-7-3\\%
  Set2-7-4\\%
  Set2-7-5\\%
  Set2-7-6\\%
  Set2-7-7\\%
}
\pgfplotscreateplotcyclelist{Set2-8}{%
  Set2-8-1\\%
  Set2-8-2\\%
  Set2-8-3\\%
  Set2-8-4\\%
  Set2-8-5\\%
  Set2-8-6\\%
  Set2-8-7\\%
  Set2-8-8\\%
}
\pgfplotscreateplotcyclelist{Dark2-3}{%
  Dark2-3-1\\%
  Dark2-3-2\\%
  Dark2-3-3\\%
}
\pgfplotscreateplotcyclelist{Dark2-4}{%
  Dark2-4-1\\%
  Dark2-4-2\\%
  Dark2-4-3\\%
  Dark2-4-4\\%
}
\pgfplotscreateplotcyclelist{Dark2-5}{%
  Dark2-5-1\\%
  Dark2-5-2\\%
  Dark2-5-3\\%
  Dark2-5-4\\%
  Dark2-5-5\\%
}
\pgfplotscreateplotcyclelist{Dark2-6}{%
  Dark2-6-1\\%
  Dark2-6-2\\%
  Dark2-6-3\\%
  Dark2-6-4\\%
  Dark2-6-5\\%
  Dark2-6-6\\%
}
\pgfplotscreateplotcyclelist{Dark2-7}{%
  Dark2-7-1\\%
  Dark2-7-2\\%
  Dark2-7-3\\%
  Dark2-7-4\\%
  Dark2-7-5\\%
  Dark2-7-6\\%
  Dark2-7-7\\%
}
\pgfplotscreateplotcyclelist{Dark2-8}{%
  Dark2-8-1\\%
  Dark2-8-2\\%
  Dark2-8-3\\%
  Dark2-8-4\\%
  Dark2-8-5\\%
  Dark2-8-6\\%
  Dark2-8-7\\%
  Dark2-8-8\\%
}
\pgfplotscreateplotcyclelist{Paired-3}{%
  Paired-3-1\\%
  Paired-3-2\\%
  Paired-3-3\\%
}
\pgfplotscreateplotcyclelist{Paired-4}{%
  Paired-4-1\\%
  Paired-4-2\\%
  Paired-4-3\\%
  Paired-4-4\\%
}
\pgfplotscreateplotcyclelist{Paired-5}{%
  Paired-5-1\\%
  Paired-5-2\\%
  Paired-5-3\\%
  Paired-5-4\\%
  Paired-5-5\\%
}
\pgfplotscreateplotcyclelist{Paired-6}{%
  Paired-6-1\\%
  Paired-6-2\\%
  Paired-6-3\\%
  Paired-6-4\\%
  Paired-6-5\\%
  Paired-6-6\\%
}
\pgfplotscreateplotcyclelist{Paired-7}{%
  Paired-7-1\\%
  Paired-7-2\\%
  Paired-7-3\\%
  Paired-7-4\\%
  Paired-7-5\\%
  Paired-7-6\\%
  Paired-7-7\\%
}
\pgfplotscreateplotcyclelist{Paired-8}{%
  Paired-8-1\\%
  Paired-8-2\\%
  Paired-8-3\\%
  Paired-8-4\\%
  Paired-8-5\\%
  Paired-8-6\\%
  Paired-8-7\\%
  Paired-8-8\\%
}
\pgfplotscreateplotcyclelist{Paired-9}{%
  Paired-9-1\\%
  Paired-9-2\\%
  Paired-9-3\\%
  Paired-9-4\\%
  Paired-9-5\\%
  Paired-9-6\\%
  Paired-9-7\\%
  Paired-9-8\\%
  Paired-9-9\\%
}
\pgfplotscreateplotcyclelist{Paired-10}{%
  Paired-10-1\\%
  Paired-10-2\\%
  Paired-10-3\\%
  Paired-10-4\\%
  Paired-10-5\\%
  Paired-10-6\\%
  Paired-10-7\\%
  Paired-10-8\\%
  Paired-10-9\\%
  Paired-10-10\\%
}
\pgfplotscreateplotcyclelist{Paired-11}{%
  Paired-11-1\\%
  Paired-11-2\\%
  Paired-11-3\\%
  Paired-11-4\\%
  Paired-11-5\\%
  Paired-11-6\\%
  Paired-11-7\\%
  Paired-11-8\\%
  Paired-11-9\\%
  Paired-11-10\\%
  Paired-11-11\\%
}
\pgfplotscreateplotcyclelist{Paired-12}{%
  Paired-12-1\\%
  Paired-12-2\\%
  Paired-12-3\\%
  Paired-12-4\\%
  Paired-12-5\\%
  Paired-12-6\\%
  Paired-12-7\\%
  Paired-12-8\\%
  Paired-12-9\\%
  Paired-12-10\\%
  Paired-12-11\\%
  Paired-12-12\\%
}
\pgfplotscreateplotcyclelist{Accent-3}{%
  Accent-3-1\\%
  Accent-3-2\\%
  Accent-3-3\\%
}
\pgfplotscreateplotcyclelist{Accent-4}{%
  Accent-4-1\\%
  Accent-4-2\\%
  Accent-4-3\\%
  Accent-4-4\\%
}
\pgfplotscreateplotcyclelist{Accent-5}{%
  Accent-5-1\\%
  Accent-5-2\\%
  Accent-5-3\\%
  Accent-5-4\\%
  Accent-5-5\\%
}
\pgfplotscreateplotcyclelist{Accent-6}{%
  Accent-6-1\\%
  Accent-6-2\\%
  Accent-6-3\\%
  Accent-6-4\\%
  Accent-6-5\\%
  Accent-6-6\\%
}
\pgfplotscreateplotcyclelist{Accent-7}{%
  Accent-7-1\\%
  Accent-7-2\\%
  Accent-7-3\\%
  Accent-7-4\\%
  Accent-7-5\\%
  Accent-7-6\\%
  Accent-7-7\\%
}
\pgfplotscreateplotcyclelist{Accent-8}{%
  Accent-8-1\\%
  Accent-8-2\\%
  Accent-8-3\\%
  Accent-8-4\\%
  Accent-8-5\\%
  Accent-8-6\\%
  Accent-8-7\\%
  Accent-8-8\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-3}{%
 YlGn-3-1!70!black, every mark/.append style={solid,fill=YlGn-3-1},mark=*\\%
 YlGn-3-2!70!black, every mark/.append style={solid,fill=YlGn-3-2},mark=square*\\%
 YlGn-3-3!70!black, every mark/.append style={solid,fill=YlGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-4}{%
 YlGn-4-1!70!black, every mark/.append style={solid,fill=YlGn-4-1},mark=*\\%
 YlGn-4-2!70!black, every mark/.append style={solid,fill=YlGn-4-2},mark=square*\\%
 YlGn-4-3!70!black, every mark/.append style={solid,fill=YlGn-4-3},mark=triangle*\\%
 YlGn-4-4!70!black, every mark/.append style={solid,fill=YlGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-5}{%
 YlGn-5-1!70!black, every mark/.append style={solid,fill=YlGn-5-1},mark=*\\%
 YlGn-5-2!70!black, every mark/.append style={solid,fill=YlGn-5-2},mark=square*\\%
 YlGn-5-3!70!black, every mark/.append style={solid,fill=YlGn-5-3},mark=triangle*\\%
 YlGn-5-4!70!black, every mark/.append style={solid,fill=YlGn-5-4},mark=diamond*\\%
 YlGn-5-5!70!black, every mark/.append style={solid,fill=YlGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-6}{%
 YlGn-6-1!70!black, every mark/.append style={solid,fill=YlGn-6-1},mark=*\\%
 YlGn-6-2!70!black, every mark/.append style={solid,fill=YlGn-6-2},mark=square*\\%
 YlGn-6-3!70!black, every mark/.append style={solid,fill=YlGn-6-3},mark=triangle*\\%
 YlGn-6-4!70!black, every mark/.append style={solid,fill=YlGn-6-4},mark=diamond*\\%
 YlGn-6-5!70!black, every mark/.append style={solid,fill=YlGn-6-5},mark=pentagon*\\%
 YlGn-6-6!70!black, every mark/.append style={solid,fill=YlGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-7}{%
 YlGn-7-1!70!black, every mark/.append style={solid,fill=YlGn-7-1},mark=*\\%
 YlGn-7-2!70!black, every mark/.append style={solid,fill=YlGn-7-2},mark=square*\\%
 YlGn-7-3!70!black, every mark/.append style={solid,fill=YlGn-7-3},mark=triangle*\\%
 YlGn-7-4!70!black, every mark/.append style={solid,fill=YlGn-7-4},mark=diamond*\\%
 YlGn-7-5!70!black, every mark/.append style={solid,fill=YlGn-7-5},mark=pentagon*\\%
 YlGn-7-6!70!black, every mark/.append style={solid,fill=YlGn-7-6},mark=x\\%
 YlGn-7-7!70!black, every mark/.append style={solid,fill=YlGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-8}{%
 YlGn-8-1!70!black, every mark/.append style={solid,fill=YlGn-8-1},mark=*\\%
 YlGn-8-2!70!black, every mark/.append style={solid,fill=YlGn-8-2},mark=square*\\%
 YlGn-8-3!70!black, every mark/.append style={solid,fill=YlGn-8-3},mark=triangle*\\%
 YlGn-8-4!70!black, every mark/.append style={solid,fill=YlGn-8-4},mark=diamond*\\%
 YlGn-8-5!70!black, every mark/.append style={solid,fill=YlGn-8-5},mark=pentagon*\\%
 YlGn-8-6!70!black, every mark/.append style={solid,fill=YlGn-8-6},mark=x\\%
 YlGn-8-7!70!black, every mark/.append style={solid,fill=YlGn-8-7},mark=+\\%
 YlGn-8-8!70!black, every mark/.append style={solid,fill=YlGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGn-9}{%
 YlGn-9-1!70!black, every mark/.append style={solid,fill=YlGn-9-1},mark=*\\%
 YlGn-9-2!70!black, every mark/.append style={solid,fill=YlGn-9-2},mark=square*\\%
 YlGn-9-3!70!black, every mark/.append style={solid,fill=YlGn-9-3},mark=triangle*\\%
 YlGn-9-4!70!black, every mark/.append style={solid,fill=YlGn-9-4},mark=diamond*\\%
 YlGn-9-5!70!black, every mark/.append style={solid,fill=YlGn-9-5},mark=pentagon*\\%
 YlGn-9-6!70!black, every mark/.append style={solid,fill=YlGn-9-6},mark=x\\%
 YlGn-9-7!70!black, every mark/.append style={solid,fill=YlGn-9-7},mark=+\\%
 YlGn-9-8!70!black, every mark/.append style={solid,fill=YlGn-9-8},mark=star\\%
 YlGn-9-9!70!black, every mark/.append style={solid,fill=YlGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-3}{%
 YlGnBu-3-1!70!black, every mark/.append style={solid,fill=YlGnBu-3-1},mark=*\\%
 YlGnBu-3-2!70!black, every mark/.append style={solid,fill=YlGnBu-3-2},mark=square*\\%
 YlGnBu-3-3!70!black, every mark/.append style={solid,fill=YlGnBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-4}{%
 YlGnBu-4-1!70!black, every mark/.append style={solid,fill=YlGnBu-4-1},mark=*\\%
 YlGnBu-4-2!70!black, every mark/.append style={solid,fill=YlGnBu-4-2},mark=square*\\%
 YlGnBu-4-3!70!black, every mark/.append style={solid,fill=YlGnBu-4-3},mark=triangle*\\%
 YlGnBu-4-4!70!black, every mark/.append style={solid,fill=YlGnBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-5}{%
 YlGnBu-5-1!70!black, every mark/.append style={solid,fill=YlGnBu-5-1},mark=*\\%
 YlGnBu-5-2!70!black, every mark/.append style={solid,fill=YlGnBu-5-2},mark=square*\\%
 YlGnBu-5-3!70!black, every mark/.append style={solid,fill=YlGnBu-5-3},mark=triangle*\\%
 YlGnBu-5-4!70!black, every mark/.append style={solid,fill=YlGnBu-5-4},mark=diamond*\\%
 YlGnBu-5-5!70!black, every mark/.append style={solid,fill=YlGnBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-6}{%
 YlGnBu-6-1!70!black, every mark/.append style={solid,fill=YlGnBu-6-1},mark=*\\%
 YlGnBu-6-2!70!black, every mark/.append style={solid,fill=YlGnBu-6-2},mark=square*\\%
 YlGnBu-6-3!70!black, every mark/.append style={solid,fill=YlGnBu-6-3},mark=triangle*\\%
 YlGnBu-6-4!70!black, every mark/.append style={solid,fill=YlGnBu-6-4},mark=diamond*\\%
 YlGnBu-6-5!70!black, every mark/.append style={solid,fill=YlGnBu-6-5},mark=pentagon*\\%
 YlGnBu-6-6!70!black, every mark/.append style={solid,fill=YlGnBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-7}{%
 YlGnBu-7-1!70!black, every mark/.append style={solid,fill=YlGnBu-7-1},mark=*\\%
 YlGnBu-7-2!70!black, every mark/.append style={solid,fill=YlGnBu-7-2},mark=square*\\%
 YlGnBu-7-3!70!black, every mark/.append style={solid,fill=YlGnBu-7-3},mark=triangle*\\%
 YlGnBu-7-4!70!black, every mark/.append style={solid,fill=YlGnBu-7-4},mark=diamond*\\%
 YlGnBu-7-5!70!black, every mark/.append style={solid,fill=YlGnBu-7-5},mark=pentagon*\\%
 YlGnBu-7-6!70!black, every mark/.append style={solid,fill=YlGnBu-7-6},mark=x\\%
 YlGnBu-7-7!70!black, every mark/.append style={solid,fill=YlGnBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-8}{%
 YlGnBu-8-1!70!black, every mark/.append style={solid,fill=YlGnBu-8-1},mark=*\\%
 YlGnBu-8-2!70!black, every mark/.append style={solid,fill=YlGnBu-8-2},mark=square*\\%
 YlGnBu-8-3!70!black, every mark/.append style={solid,fill=YlGnBu-8-3},mark=triangle*\\%
 YlGnBu-8-4!70!black, every mark/.append style={solid,fill=YlGnBu-8-4},mark=diamond*\\%
 YlGnBu-8-5!70!black, every mark/.append style={solid,fill=YlGnBu-8-5},mark=pentagon*\\%
 YlGnBu-8-6!70!black, every mark/.append style={solid,fill=YlGnBu-8-6},mark=x\\%
 YlGnBu-8-7!70!black, every mark/.append style={solid,fill=YlGnBu-8-7},mark=+\\%
 YlGnBu-8-8!70!black, every mark/.append style={solid,fill=YlGnBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-YlGnBu-9}{%
 YlGnBu-9-1!70!black, every mark/.append style={solid,fill=YlGnBu-9-1},mark=*\\%
 YlGnBu-9-2!70!black, every mark/.append style={solid,fill=YlGnBu-9-2},mark=square*\\%
 YlGnBu-9-3!70!black, every mark/.append style={solid,fill=YlGnBu-9-3},mark=triangle*\\%
 YlGnBu-9-4!70!black, every mark/.append style={solid,fill=YlGnBu-9-4},mark=diamond*\\%
 YlGnBu-9-5!70!black, every mark/.append style={solid,fill=YlGnBu-9-5},mark=pentagon*\\%
 YlGnBu-9-6!70!black, every mark/.append style={solid,fill=YlGnBu-9-6},mark=x\\%
 YlGnBu-9-7!70!black, every mark/.append style={solid,fill=YlGnBu-9-7},mark=+\\%
 YlGnBu-9-8!70!black, every mark/.append style={solid,fill=YlGnBu-9-8},mark=star\\%
 YlGnBu-9-9!70!black, every mark/.append style={solid,fill=YlGnBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-3}{%
 GnBu-3-1!70!black, every mark/.append style={solid,fill=GnBu-3-1},mark=*\\%
 GnBu-3-2!70!black, every mark/.append style={solid,fill=GnBu-3-2},mark=square*\\%
 GnBu-3-3!70!black, every mark/.append style={solid,fill=GnBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-4}{%
 GnBu-4-1!70!black, every mark/.append style={solid,fill=GnBu-4-1},mark=*\\%
 GnBu-4-2!70!black, every mark/.append style={solid,fill=GnBu-4-2},mark=square*\\%
 GnBu-4-3!70!black, every mark/.append style={solid,fill=GnBu-4-3},mark=triangle*\\%
 GnBu-4-4!70!black, every mark/.append style={solid,fill=GnBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-5}{%
 GnBu-5-1!70!black, every mark/.append style={solid,fill=GnBu-5-1},mark=*\\%
 GnBu-5-2!70!black, every mark/.append style={solid,fill=GnBu-5-2},mark=square*\\%
 GnBu-5-3!70!black, every mark/.append style={solid,fill=GnBu-5-3},mark=triangle*\\%
 GnBu-5-4!70!black, every mark/.append style={solid,fill=GnBu-5-4},mark=diamond*\\%
 GnBu-5-5!70!black, every mark/.append style={solid,fill=GnBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-6}{%
 GnBu-6-1!70!black, every mark/.append style={solid,fill=GnBu-6-1},mark=*\\%
 GnBu-6-2!70!black, every mark/.append style={solid,fill=GnBu-6-2},mark=square*\\%
 GnBu-6-3!70!black, every mark/.append style={solid,fill=GnBu-6-3},mark=triangle*\\%
 GnBu-6-4!70!black, every mark/.append style={solid,fill=GnBu-6-4},mark=diamond*\\%
 GnBu-6-5!70!black, every mark/.append style={solid,fill=GnBu-6-5},mark=pentagon*\\%
 GnBu-6-6!70!black, every mark/.append style={solid,fill=GnBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-7}{%
 GnBu-7-1!70!black, every mark/.append style={solid,fill=GnBu-7-1},mark=*\\%
 GnBu-7-2!70!black, every mark/.append style={solid,fill=GnBu-7-2},mark=square*\\%
 GnBu-7-3!70!black, every mark/.append style={solid,fill=GnBu-7-3},mark=triangle*\\%
 GnBu-7-4!70!black, every mark/.append style={solid,fill=GnBu-7-4},mark=diamond*\\%
 GnBu-7-5!70!black, every mark/.append style={solid,fill=GnBu-7-5},mark=pentagon*\\%
 GnBu-7-6!70!black, every mark/.append style={solid,fill=GnBu-7-6},mark=x\\%
 GnBu-7-7!70!black, every mark/.append style={solid,fill=GnBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-8}{%
 GnBu-8-1!70!black, every mark/.append style={solid,fill=GnBu-8-1},mark=*\\%
 GnBu-8-2!70!black, every mark/.append style={solid,fill=GnBu-8-2},mark=square*\\%
 GnBu-8-3!70!black, every mark/.append style={solid,fill=GnBu-8-3},mark=triangle*\\%
 GnBu-8-4!70!black, every mark/.append style={solid,fill=GnBu-8-4},mark=diamond*\\%
 GnBu-8-5!70!black, every mark/.append style={solid,fill=GnBu-8-5},mark=pentagon*\\%
 GnBu-8-6!70!black, every mark/.append style={solid,fill=GnBu-8-6},mark=x\\%
 GnBu-8-7!70!black, every mark/.append style={solid,fill=GnBu-8-7},mark=+\\%
 GnBu-8-8!70!black, every mark/.append style={solid,fill=GnBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-GnBu-9}{%
 GnBu-9-1!70!black, every mark/.append style={solid,fill=GnBu-9-1},mark=*\\%
 GnBu-9-2!70!black, every mark/.append style={solid,fill=GnBu-9-2},mark=square*\\%
 GnBu-9-3!70!black, every mark/.append style={solid,fill=GnBu-9-3},mark=triangle*\\%
 GnBu-9-4!70!black, every mark/.append style={solid,fill=GnBu-9-4},mark=diamond*\\%
 GnBu-9-5!70!black, every mark/.append style={solid,fill=GnBu-9-5},mark=pentagon*\\%
 GnBu-9-6!70!black, every mark/.append style={solid,fill=GnBu-9-6},mark=x\\%
 GnBu-9-7!70!black, every mark/.append style={solid,fill=GnBu-9-7},mark=+\\%
 GnBu-9-8!70!black, every mark/.append style={solid,fill=GnBu-9-8},mark=star\\%
 GnBu-9-9!70!black, every mark/.append style={solid,fill=GnBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-3}{%
 BuGn-3-1!70!black, every mark/.append style={solid,fill=BuGn-3-1},mark=*\\%
 BuGn-3-2!70!black, every mark/.append style={solid,fill=BuGn-3-2},mark=square*\\%
 BuGn-3-3!70!black, every mark/.append style={solid,fill=BuGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-4}{%
 BuGn-4-1!70!black, every mark/.append style={solid,fill=BuGn-4-1},mark=*\\%
 BuGn-4-2!70!black, every mark/.append style={solid,fill=BuGn-4-2},mark=square*\\%
 BuGn-4-3!70!black, every mark/.append style={solid,fill=BuGn-4-3},mark=triangle*\\%
 BuGn-4-4!70!black, every mark/.append style={solid,fill=BuGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-5}{%
 BuGn-5-1!70!black, every mark/.append style={solid,fill=BuGn-5-1},mark=*\\%
 BuGn-5-2!70!black, every mark/.append style={solid,fill=BuGn-5-2},mark=square*\\%
 BuGn-5-3!70!black, every mark/.append style={solid,fill=BuGn-5-3},mark=triangle*\\%
 BuGn-5-4!70!black, every mark/.append style={solid,fill=BuGn-5-4},mark=diamond*\\%
 BuGn-5-5!70!black, every mark/.append style={solid,fill=BuGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-6}{%
 BuGn-6-1!70!black, every mark/.append style={solid,fill=BuGn-6-1},mark=*\\%
 BuGn-6-2!70!black, every mark/.append style={solid,fill=BuGn-6-2},mark=square*\\%
 BuGn-6-3!70!black, every mark/.append style={solid,fill=BuGn-6-3},mark=triangle*\\%
 BuGn-6-4!70!black, every mark/.append style={solid,fill=BuGn-6-4},mark=diamond*\\%
 BuGn-6-5!70!black, every mark/.append style={solid,fill=BuGn-6-5},mark=pentagon*\\%
 BuGn-6-6!70!black, every mark/.append style={solid,fill=BuGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-7}{%
 BuGn-7-1!70!black, every mark/.append style={solid,fill=BuGn-7-1},mark=*\\%
 BuGn-7-2!70!black, every mark/.append style={solid,fill=BuGn-7-2},mark=square*\\%
 BuGn-7-3!70!black, every mark/.append style={solid,fill=BuGn-7-3},mark=triangle*\\%
 BuGn-7-4!70!black, every mark/.append style={solid,fill=BuGn-7-4},mark=diamond*\\%
 BuGn-7-5!70!black, every mark/.append style={solid,fill=BuGn-7-5},mark=pentagon*\\%
 BuGn-7-6!70!black, every mark/.append style={solid,fill=BuGn-7-6},mark=x\\%
 BuGn-7-7!70!black, every mark/.append style={solid,fill=BuGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-8}{%
 BuGn-8-1!70!black, every mark/.append style={solid,fill=BuGn-8-1},mark=*\\%
 BuGn-8-2!70!black, every mark/.append style={solid,fill=BuGn-8-2},mark=square*\\%
 BuGn-8-3!70!black, every mark/.append style={solid,fill=BuGn-8-3},mark=triangle*\\%
 BuGn-8-4!70!black, every mark/.append style={solid,fill=BuGn-8-4},mark=diamond*\\%
 BuGn-8-5!70!black, every mark/.append style={solid,fill=BuGn-8-5},mark=pentagon*\\%
 BuGn-8-6!70!black, every mark/.append style={solid,fill=BuGn-8-6},mark=x\\%
 BuGn-8-7!70!black, every mark/.append style={solid,fill=BuGn-8-7},mark=+\\%
 BuGn-8-8!70!black, every mark/.append style={solid,fill=BuGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-BuGn-9}{%
 BuGn-9-1!70!black, every mark/.append style={solid,fill=BuGn-9-1},mark=*\\%
 BuGn-9-2!70!black, every mark/.append style={solid,fill=BuGn-9-2},mark=square*\\%
 BuGn-9-3!70!black, every mark/.append style={solid,fill=BuGn-9-3},mark=triangle*\\%
 BuGn-9-4!70!black, every mark/.append style={solid,fill=BuGn-9-4},mark=diamond*\\%
 BuGn-9-5!70!black, every mark/.append style={solid,fill=BuGn-9-5},mark=pentagon*\\%
 BuGn-9-6!70!black, every mark/.append style={solid,fill=BuGn-9-6},mark=x\\%
 BuGn-9-7!70!black, every mark/.append style={solid,fill=BuGn-9-7},mark=+\\%
 BuGn-9-8!70!black, every mark/.append style={solid,fill=BuGn-9-8},mark=star\\%
 BuGn-9-9!70!black, every mark/.append style={solid,fill=BuGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-3}{%
 PuBuGn-3-1!70!black, every mark/.append style={solid,fill=PuBuGn-3-1},mark=*\\%
 PuBuGn-3-2!70!black, every mark/.append style={solid,fill=PuBuGn-3-2},mark=square*\\%
 PuBuGn-3-3!70!black, every mark/.append style={solid,fill=PuBuGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-4}{%
 PuBuGn-4-1!70!black, every mark/.append style={solid,fill=PuBuGn-4-1},mark=*\\%
 PuBuGn-4-2!70!black, every mark/.append style={solid,fill=PuBuGn-4-2},mark=square*\\%
 PuBuGn-4-3!70!black, every mark/.append style={solid,fill=PuBuGn-4-3},mark=triangle*\\%
 PuBuGn-4-4!70!black, every mark/.append style={solid,fill=PuBuGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-5}{%
 PuBuGn-5-1!70!black, every mark/.append style={solid,fill=PuBuGn-5-1},mark=*\\%
 PuBuGn-5-2!70!black, every mark/.append style={solid,fill=PuBuGn-5-2},mark=square*\\%
 PuBuGn-5-3!70!black, every mark/.append style={solid,fill=PuBuGn-5-3},mark=triangle*\\%
 PuBuGn-5-4!70!black, every mark/.append style={solid,fill=PuBuGn-5-4},mark=diamond*\\%
 PuBuGn-5-5!70!black, every mark/.append style={solid,fill=PuBuGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-6}{%
 PuBuGn-6-1!70!black, every mark/.append style={solid,fill=PuBuGn-6-1},mark=*\\%
 PuBuGn-6-2!70!black, every mark/.append style={solid,fill=PuBuGn-6-2},mark=square*\\%
 PuBuGn-6-3!70!black, every mark/.append style={solid,fill=PuBuGn-6-3},mark=triangle*\\%
 PuBuGn-6-4!70!black, every mark/.append style={solid,fill=PuBuGn-6-4},mark=diamond*\\%
 PuBuGn-6-5!70!black, every mark/.append style={solid,fill=PuBuGn-6-5},mark=pentagon*\\%
 PuBuGn-6-6!70!black, every mark/.append style={solid,fill=PuBuGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-7}{%
 PuBuGn-7-1!70!black, every mark/.append style={solid,fill=PuBuGn-7-1},mark=*\\%
 PuBuGn-7-2!70!black, every mark/.append style={solid,fill=PuBuGn-7-2},mark=square*\\%
 PuBuGn-7-3!70!black, every mark/.append style={solid,fill=PuBuGn-7-3},mark=triangle*\\%
 PuBuGn-7-4!70!black, every mark/.append style={solid,fill=PuBuGn-7-4},mark=diamond*\\%
 PuBuGn-7-5!70!black, every mark/.append style={solid,fill=PuBuGn-7-5},mark=pentagon*\\%
 PuBuGn-7-6!70!black, every mark/.append style={solid,fill=PuBuGn-7-6},mark=x\\%
 PuBuGn-7-7!70!black, every mark/.append style={solid,fill=PuBuGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-8}{%
 PuBuGn-8-1!70!black, every mark/.append style={solid,fill=PuBuGn-8-1},mark=*\\%
 PuBuGn-8-2!70!black, every mark/.append style={solid,fill=PuBuGn-8-2},mark=square*\\%
 PuBuGn-8-3!70!black, every mark/.append style={solid,fill=PuBuGn-8-3},mark=triangle*\\%
 PuBuGn-8-4!70!black, every mark/.append style={solid,fill=PuBuGn-8-4},mark=diamond*\\%
 PuBuGn-8-5!70!black, every mark/.append style={solid,fill=PuBuGn-8-5},mark=pentagon*\\%
 PuBuGn-8-6!70!black, every mark/.append style={solid,fill=PuBuGn-8-6},mark=x\\%
 PuBuGn-8-7!70!black, every mark/.append style={solid,fill=PuBuGn-8-7},mark=+\\%
 PuBuGn-8-8!70!black, every mark/.append style={solid,fill=PuBuGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBuGn-9}{%
 PuBuGn-9-1!70!black, every mark/.append style={solid,fill=PuBuGn-9-1},mark=*\\%
 PuBuGn-9-2!70!black, every mark/.append style={solid,fill=PuBuGn-9-2},mark=square*\\%
 PuBuGn-9-3!70!black, every mark/.append style={solid,fill=PuBuGn-9-3},mark=triangle*\\%
 PuBuGn-9-4!70!black, every mark/.append style={solid,fill=PuBuGn-9-4},mark=diamond*\\%
 PuBuGn-9-5!70!black, every mark/.append style={solid,fill=PuBuGn-9-5},mark=pentagon*\\%
 PuBuGn-9-6!70!black, every mark/.append style={solid,fill=PuBuGn-9-6},mark=x\\%
 PuBuGn-9-7!70!black, every mark/.append style={solid,fill=PuBuGn-9-7},mark=+\\%
 PuBuGn-9-8!70!black, every mark/.append style={solid,fill=PuBuGn-9-8},mark=star\\%
 PuBuGn-9-9!70!black, every mark/.append style={solid,fill=PuBuGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-3}{%
 PuBu-3-1!70!black, every mark/.append style={solid,fill=PuBu-3-1},mark=*\\%
 PuBu-3-2!70!black, every mark/.append style={solid,fill=PuBu-3-2},mark=square*\\%
 PuBu-3-3!70!black, every mark/.append style={solid,fill=PuBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-4}{%
 PuBu-4-1!70!black, every mark/.append style={solid,fill=PuBu-4-1},mark=*\\%
 PuBu-4-2!70!black, every mark/.append style={solid,fill=PuBu-4-2},mark=square*\\%
 PuBu-4-3!70!black, every mark/.append style={solid,fill=PuBu-4-3},mark=triangle*\\%
 PuBu-4-4!70!black, every mark/.append style={solid,fill=PuBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-5}{%
 PuBu-5-1!70!black, every mark/.append style={solid,fill=PuBu-5-1},mark=*\\%
 PuBu-5-2!70!black, every mark/.append style={solid,fill=PuBu-5-2},mark=square*\\%
 PuBu-5-3!70!black, every mark/.append style={solid,fill=PuBu-5-3},mark=triangle*\\%
 PuBu-5-4!70!black, every mark/.append style={solid,fill=PuBu-5-4},mark=diamond*\\%
 PuBu-5-5!70!black, every mark/.append style={solid,fill=PuBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-6}{%
 PuBu-6-1!70!black, every mark/.append style={solid,fill=PuBu-6-1},mark=*\\%
 PuBu-6-2!70!black, every mark/.append style={solid,fill=PuBu-6-2},mark=square*\\%
 PuBu-6-3!70!black, every mark/.append style={solid,fill=PuBu-6-3},mark=triangle*\\%
 PuBu-6-4!70!black, every mark/.append style={solid,fill=PuBu-6-4},mark=diamond*\\%
 PuBu-6-5!70!black, every mark/.append style={solid,fill=PuBu-6-5},mark=pentagon*\\%
 PuBu-6-6!70!black, every mark/.append style={solid,fill=PuBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-7}{%
 PuBu-7-1!70!black, every mark/.append style={solid,fill=PuBu-7-1},mark=*\\%
 PuBu-7-2!70!black, every mark/.append style={solid,fill=PuBu-7-2},mark=square*\\%
 PuBu-7-3!70!black, every mark/.append style={solid,fill=PuBu-7-3},mark=triangle*\\%
 PuBu-7-4!70!black, every mark/.append style={solid,fill=PuBu-7-4},mark=diamond*\\%
 PuBu-7-5!70!black, every mark/.append style={solid,fill=PuBu-7-5},mark=pentagon*\\%
 PuBu-7-6!70!black, every mark/.append style={solid,fill=PuBu-7-6},mark=x\\%
 PuBu-7-7!70!black, every mark/.append style={solid,fill=PuBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-8}{%
 PuBu-8-1!70!black, every mark/.append style={solid,fill=PuBu-8-1},mark=*\\%
 PuBu-8-2!70!black, every mark/.append style={solid,fill=PuBu-8-2},mark=square*\\%
 PuBu-8-3!70!black, every mark/.append style={solid,fill=PuBu-8-3},mark=triangle*\\%
 PuBu-8-4!70!black, every mark/.append style={solid,fill=PuBu-8-4},mark=diamond*\\%
 PuBu-8-5!70!black, every mark/.append style={solid,fill=PuBu-8-5},mark=pentagon*\\%
 PuBu-8-6!70!black, every mark/.append style={solid,fill=PuBu-8-6},mark=x\\%
 PuBu-8-7!70!black, every mark/.append style={solid,fill=PuBu-8-7},mark=+\\%
 PuBu-8-8!70!black, every mark/.append style={solid,fill=PuBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PuBu-9}{%
 PuBu-9-1!70!black, every mark/.append style={solid,fill=PuBu-9-1},mark=*\\%
 PuBu-9-2!70!black, every mark/.append style={solid,fill=PuBu-9-2},mark=square*\\%
 PuBu-9-3!70!black, every mark/.append style={solid,fill=PuBu-9-3},mark=triangle*\\%
 PuBu-9-4!70!black, every mark/.append style={solid,fill=PuBu-9-4},mark=diamond*\\%
 PuBu-9-5!70!black, every mark/.append style={solid,fill=PuBu-9-5},mark=pentagon*\\%
 PuBu-9-6!70!black, every mark/.append style={solid,fill=PuBu-9-6},mark=x\\%
 PuBu-9-7!70!black, every mark/.append style={solid,fill=PuBu-9-7},mark=+\\%
 PuBu-9-8!70!black, every mark/.append style={solid,fill=PuBu-9-8},mark=star\\%
 PuBu-9-9!70!black, every mark/.append style={solid,fill=PuBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-3}{%
 BuPu-3-1!70!black, every mark/.append style={solid,fill=BuPu-3-1},mark=*\\%
 BuPu-3-2!70!black, every mark/.append style={solid,fill=BuPu-3-2},mark=square*\\%
 BuPu-3-3!70!black, every mark/.append style={solid,fill=BuPu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-4}{%
 BuPu-4-1!70!black, every mark/.append style={solid,fill=BuPu-4-1},mark=*\\%
 BuPu-4-2!70!black, every mark/.append style={solid,fill=BuPu-4-2},mark=square*\\%
 BuPu-4-3!70!black, every mark/.append style={solid,fill=BuPu-4-3},mark=triangle*\\%
 BuPu-4-4!70!black, every mark/.append style={solid,fill=BuPu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-5}{%
 BuPu-5-1!70!black, every mark/.append style={solid,fill=BuPu-5-1},mark=*\\%
 BuPu-5-2!70!black, every mark/.append style={solid,fill=BuPu-5-2},mark=square*\\%
 BuPu-5-3!70!black, every mark/.append style={solid,fill=BuPu-5-3},mark=triangle*\\%
 BuPu-5-4!70!black, every mark/.append style={solid,fill=BuPu-5-4},mark=diamond*\\%
 BuPu-5-5!70!black, every mark/.append style={solid,fill=BuPu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-6}{%
 BuPu-6-1!70!black, every mark/.append style={solid,fill=BuPu-6-1},mark=*\\%
 BuPu-6-2!70!black, every mark/.append style={solid,fill=BuPu-6-2},mark=square*\\%
 BuPu-6-3!70!black, every mark/.append style={solid,fill=BuPu-6-3},mark=triangle*\\%
 BuPu-6-4!70!black, every mark/.append style={solid,fill=BuPu-6-4},mark=diamond*\\%
 BuPu-6-5!70!black, every mark/.append style={solid,fill=BuPu-6-5},mark=pentagon*\\%
 BuPu-6-6!70!black, every mark/.append style={solid,fill=BuPu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-7}{%
 BuPu-7-1!70!black, every mark/.append style={solid,fill=BuPu-7-1},mark=*\\%
 BuPu-7-2!70!black, every mark/.append style={solid,fill=BuPu-7-2},mark=square*\\%
 BuPu-7-3!70!black, every mark/.append style={solid,fill=BuPu-7-3},mark=triangle*\\%
 BuPu-7-4!70!black, every mark/.append style={solid,fill=BuPu-7-4},mark=diamond*\\%
 BuPu-7-5!70!black, every mark/.append style={solid,fill=BuPu-7-5},mark=pentagon*\\%
 BuPu-7-6!70!black, every mark/.append style={solid,fill=BuPu-7-6},mark=x\\%
 BuPu-7-7!70!black, every mark/.append style={solid,fill=BuPu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-8}{%
 BuPu-8-1!70!black, every mark/.append style={solid,fill=BuPu-8-1},mark=*\\%
 BuPu-8-2!70!black, every mark/.append style={solid,fill=BuPu-8-2},mark=square*\\%
 BuPu-8-3!70!black, every mark/.append style={solid,fill=BuPu-8-3},mark=triangle*\\%
 BuPu-8-4!70!black, every mark/.append style={solid,fill=BuPu-8-4},mark=diamond*\\%
 BuPu-8-5!70!black, every mark/.append style={solid,fill=BuPu-8-5},mark=pentagon*\\%
 BuPu-8-6!70!black, every mark/.append style={solid,fill=BuPu-8-6},mark=x\\%
 BuPu-8-7!70!black, every mark/.append style={solid,fill=BuPu-8-7},mark=+\\%
 BuPu-8-8!70!black, every mark/.append style={solid,fill=BuPu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-BuPu-9}{%
 BuPu-9-1!70!black, every mark/.append style={solid,fill=BuPu-9-1},mark=*\\%
 BuPu-9-2!70!black, every mark/.append style={solid,fill=BuPu-9-2},mark=square*\\%
 BuPu-9-3!70!black, every mark/.append style={solid,fill=BuPu-9-3},mark=triangle*\\%
 BuPu-9-4!70!black, every mark/.append style={solid,fill=BuPu-9-4},mark=diamond*\\%
 BuPu-9-5!70!black, every mark/.append style={solid,fill=BuPu-9-5},mark=pentagon*\\%
 BuPu-9-6!70!black, every mark/.append style={solid,fill=BuPu-9-6},mark=x\\%
 BuPu-9-7!70!black, every mark/.append style={solid,fill=BuPu-9-7},mark=+\\%
 BuPu-9-8!70!black, every mark/.append style={solid,fill=BuPu-9-8},mark=star\\%
 BuPu-9-9!70!black, every mark/.append style={solid,fill=BuPu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-3}{%
 RdPu-3-1!70!black, every mark/.append style={solid,fill=RdPu-3-1},mark=*\\%
 RdPu-3-2!70!black, every mark/.append style={solid,fill=RdPu-3-2},mark=square*\\%
 RdPu-3-3!70!black, every mark/.append style={solid,fill=RdPu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-4}{%
 RdPu-4-1!70!black, every mark/.append style={solid,fill=RdPu-4-1},mark=*\\%
 RdPu-4-2!70!black, every mark/.append style={solid,fill=RdPu-4-2},mark=square*\\%
 RdPu-4-3!70!black, every mark/.append style={solid,fill=RdPu-4-3},mark=triangle*\\%
 RdPu-4-4!70!black, every mark/.append style={solid,fill=RdPu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-5}{%
 RdPu-5-1!70!black, every mark/.append style={solid,fill=RdPu-5-1},mark=*\\%
 RdPu-5-2!70!black, every mark/.append style={solid,fill=RdPu-5-2},mark=square*\\%
 RdPu-5-3!70!black, every mark/.append style={solid,fill=RdPu-5-3},mark=triangle*\\%
 RdPu-5-4!70!black, every mark/.append style={solid,fill=RdPu-5-4},mark=diamond*\\%
 RdPu-5-5!70!black, every mark/.append style={solid,fill=RdPu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-6}{%
 RdPu-6-1!70!black, every mark/.append style={solid,fill=RdPu-6-1},mark=*\\%
 RdPu-6-2!70!black, every mark/.append style={solid,fill=RdPu-6-2},mark=square*\\%
 RdPu-6-3!70!black, every mark/.append style={solid,fill=RdPu-6-3},mark=triangle*\\%
 RdPu-6-4!70!black, every mark/.append style={solid,fill=RdPu-6-4},mark=diamond*\\%
 RdPu-6-5!70!black, every mark/.append style={solid,fill=RdPu-6-5},mark=pentagon*\\%
 RdPu-6-6!70!black, every mark/.append style={solid,fill=RdPu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-7}{%
 RdPu-7-1!70!black, every mark/.append style={solid,fill=RdPu-7-1},mark=*\\%
 RdPu-7-2!70!black, every mark/.append style={solid,fill=RdPu-7-2},mark=square*\\%
 RdPu-7-3!70!black, every mark/.append style={solid,fill=RdPu-7-3},mark=triangle*\\%
 RdPu-7-4!70!black, every mark/.append style={solid,fill=RdPu-7-4},mark=diamond*\\%
 RdPu-7-5!70!black, every mark/.append style={solid,fill=RdPu-7-5},mark=pentagon*\\%
 RdPu-7-6!70!black, every mark/.append style={solid,fill=RdPu-7-6},mark=x\\%
 RdPu-7-7!70!black, every mark/.append style={solid,fill=RdPu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-8}{%
 RdPu-8-1!70!black, every mark/.append style={solid,fill=RdPu-8-1},mark=*\\%
 RdPu-8-2!70!black, every mark/.append style={solid,fill=RdPu-8-2},mark=square*\\%
 RdPu-8-3!70!black, every mark/.append style={solid,fill=RdPu-8-3},mark=triangle*\\%
 RdPu-8-4!70!black, every mark/.append style={solid,fill=RdPu-8-4},mark=diamond*\\%
 RdPu-8-5!70!black, every mark/.append style={solid,fill=RdPu-8-5},mark=pentagon*\\%
 RdPu-8-6!70!black, every mark/.append style={solid,fill=RdPu-8-6},mark=x\\%
 RdPu-8-7!70!black, every mark/.append style={solid,fill=RdPu-8-7},mark=+\\%
 RdPu-8-8!70!black, every mark/.append style={solid,fill=RdPu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-RdPu-9}{%
 RdPu-9-1!70!black, every mark/.append style={solid,fill=RdPu-9-1},mark=*\\%
 RdPu-9-2!70!black, every mark/.append style={solid,fill=RdPu-9-2},mark=square*\\%
 RdPu-9-3!70!black, every mark/.append style={solid,fill=RdPu-9-3},mark=triangle*\\%
 RdPu-9-4!70!black, every mark/.append style={solid,fill=RdPu-9-4},mark=diamond*\\%
 RdPu-9-5!70!black, every mark/.append style={solid,fill=RdPu-9-5},mark=pentagon*\\%
 RdPu-9-6!70!black, every mark/.append style={solid,fill=RdPu-9-6},mark=x\\%
 RdPu-9-7!70!black, every mark/.append style={solid,fill=RdPu-9-7},mark=+\\%
 RdPu-9-8!70!black, every mark/.append style={solid,fill=RdPu-9-8},mark=star\\%
 RdPu-9-9!70!black, every mark/.append style={solid,fill=RdPu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-3}{%
 PuRd-3-1!70!black, every mark/.append style={solid,fill=PuRd-3-1},mark=*\\%
 PuRd-3-2!70!black, every mark/.append style={solid,fill=PuRd-3-2},mark=square*\\%
 PuRd-3-3!70!black, every mark/.append style={solid,fill=PuRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-4}{%
 PuRd-4-1!70!black, every mark/.append style={solid,fill=PuRd-4-1},mark=*\\%
 PuRd-4-2!70!black, every mark/.append style={solid,fill=PuRd-4-2},mark=square*\\%
 PuRd-4-3!70!black, every mark/.append style={solid,fill=PuRd-4-3},mark=triangle*\\%
 PuRd-4-4!70!black, every mark/.append style={solid,fill=PuRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-5}{%
 PuRd-5-1!70!black, every mark/.append style={solid,fill=PuRd-5-1},mark=*\\%
 PuRd-5-2!70!black, every mark/.append style={solid,fill=PuRd-5-2},mark=square*\\%
 PuRd-5-3!70!black, every mark/.append style={solid,fill=PuRd-5-3},mark=triangle*\\%
 PuRd-5-4!70!black, every mark/.append style={solid,fill=PuRd-5-4},mark=diamond*\\%
 PuRd-5-5!70!black, every mark/.append style={solid,fill=PuRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-6}{%
 PuRd-6-1!70!black, every mark/.append style={solid,fill=PuRd-6-1},mark=*\\%
 PuRd-6-2!70!black, every mark/.append style={solid,fill=PuRd-6-2},mark=square*\\%
 PuRd-6-3!70!black, every mark/.append style={solid,fill=PuRd-6-3},mark=triangle*\\%
 PuRd-6-4!70!black, every mark/.append style={solid,fill=PuRd-6-4},mark=diamond*\\%
 PuRd-6-5!70!black, every mark/.append style={solid,fill=PuRd-6-5},mark=pentagon*\\%
 PuRd-6-6!70!black, every mark/.append style={solid,fill=PuRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-7}{%
 PuRd-7-1!70!black, every mark/.append style={solid,fill=PuRd-7-1},mark=*\\%
 PuRd-7-2!70!black, every mark/.append style={solid,fill=PuRd-7-2},mark=square*\\%
 PuRd-7-3!70!black, every mark/.append style={solid,fill=PuRd-7-3},mark=triangle*\\%
 PuRd-7-4!70!black, every mark/.append style={solid,fill=PuRd-7-4},mark=diamond*\\%
 PuRd-7-5!70!black, every mark/.append style={solid,fill=PuRd-7-5},mark=pentagon*\\%
 PuRd-7-6!70!black, every mark/.append style={solid,fill=PuRd-7-6},mark=x\\%
 PuRd-7-7!70!black, every mark/.append style={solid,fill=PuRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-8}{%
 PuRd-8-1!70!black, every mark/.append style={solid,fill=PuRd-8-1},mark=*\\%
 PuRd-8-2!70!black, every mark/.append style={solid,fill=PuRd-8-2},mark=square*\\%
 PuRd-8-3!70!black, every mark/.append style={solid,fill=PuRd-8-3},mark=triangle*\\%
 PuRd-8-4!70!black, every mark/.append style={solid,fill=PuRd-8-4},mark=diamond*\\%
 PuRd-8-5!70!black, every mark/.append style={solid,fill=PuRd-8-5},mark=pentagon*\\%
 PuRd-8-6!70!black, every mark/.append style={solid,fill=PuRd-8-6},mark=x\\%
 PuRd-8-7!70!black, every mark/.append style={solid,fill=PuRd-8-7},mark=+\\%
 PuRd-8-8!70!black, every mark/.append style={solid,fill=PuRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PuRd-9}{%
 PuRd-9-1!70!black, every mark/.append style={solid,fill=PuRd-9-1},mark=*\\%
 PuRd-9-2!70!black, every mark/.append style={solid,fill=PuRd-9-2},mark=square*\\%
 PuRd-9-3!70!black, every mark/.append style={solid,fill=PuRd-9-3},mark=triangle*\\%
 PuRd-9-4!70!black, every mark/.append style={solid,fill=PuRd-9-4},mark=diamond*\\%
 PuRd-9-5!70!black, every mark/.append style={solid,fill=PuRd-9-5},mark=pentagon*\\%
 PuRd-9-6!70!black, every mark/.append style={solid,fill=PuRd-9-6},mark=x\\%
 PuRd-9-7!70!black, every mark/.append style={solid,fill=PuRd-9-7},mark=+\\%
 PuRd-9-8!70!black, every mark/.append style={solid,fill=PuRd-9-8},mark=star\\%
 PuRd-9-9!70!black, every mark/.append style={solid,fill=PuRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-3}{%
 OrRd-3-1!70!black, every mark/.append style={solid,fill=OrRd-3-1},mark=*\\%
 OrRd-3-2!70!black, every mark/.append style={solid,fill=OrRd-3-2},mark=square*\\%
 OrRd-3-3!70!black, every mark/.append style={solid,fill=OrRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-4}{%
 OrRd-4-1!70!black, every mark/.append style={solid,fill=OrRd-4-1},mark=*\\%
 OrRd-4-2!70!black, every mark/.append style={solid,fill=OrRd-4-2},mark=square*\\%
 OrRd-4-3!70!black, every mark/.append style={solid,fill=OrRd-4-3},mark=triangle*\\%
 OrRd-4-4!70!black, every mark/.append style={solid,fill=OrRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-5}{%
 OrRd-5-1!70!black, every mark/.append style={solid,fill=OrRd-5-1},mark=*\\%
 OrRd-5-2!70!black, every mark/.append style={solid,fill=OrRd-5-2},mark=square*\\%
 OrRd-5-3!70!black, every mark/.append style={solid,fill=OrRd-5-3},mark=triangle*\\%
 OrRd-5-4!70!black, every mark/.append style={solid,fill=OrRd-5-4},mark=diamond*\\%
 OrRd-5-5!70!black, every mark/.append style={solid,fill=OrRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-6}{%
 OrRd-6-1!70!black, every mark/.append style={solid,fill=OrRd-6-1},mark=*\\%
 OrRd-6-2!70!black, every mark/.append style={solid,fill=OrRd-6-2},mark=square*\\%
 OrRd-6-3!70!black, every mark/.append style={solid,fill=OrRd-6-3},mark=triangle*\\%
 OrRd-6-4!70!black, every mark/.append style={solid,fill=OrRd-6-4},mark=diamond*\\%
 OrRd-6-5!70!black, every mark/.append style={solid,fill=OrRd-6-5},mark=pentagon*\\%
 OrRd-6-6!70!black, every mark/.append style={solid,fill=OrRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-7}{%
 OrRd-7-1!70!black, every mark/.append style={solid,fill=OrRd-7-1},mark=*\\%
 OrRd-7-2!70!black, every mark/.append style={solid,fill=OrRd-7-2},mark=square*\\%
 OrRd-7-3!70!black, every mark/.append style={solid,fill=OrRd-7-3},mark=triangle*\\%
 OrRd-7-4!70!black, every mark/.append style={solid,fill=OrRd-7-4},mark=diamond*\\%
 OrRd-7-5!70!black, every mark/.append style={solid,fill=OrRd-7-5},mark=pentagon*\\%
 OrRd-7-6!70!black, every mark/.append style={solid,fill=OrRd-7-6},mark=x\\%
 OrRd-7-7!70!black, every mark/.append style={solid,fill=OrRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-8}{%
 OrRd-8-1!70!black, every mark/.append style={solid,fill=OrRd-8-1},mark=*\\%
 OrRd-8-2!70!black, every mark/.append style={solid,fill=OrRd-8-2},mark=square*\\%
 OrRd-8-3!70!black, every mark/.append style={solid,fill=OrRd-8-3},mark=triangle*\\%
 OrRd-8-4!70!black, every mark/.append style={solid,fill=OrRd-8-4},mark=diamond*\\%
 OrRd-8-5!70!black, every mark/.append style={solid,fill=OrRd-8-5},mark=pentagon*\\%
 OrRd-8-6!70!black, every mark/.append style={solid,fill=OrRd-8-6},mark=x\\%
 OrRd-8-7!70!black, every mark/.append style={solid,fill=OrRd-8-7},mark=+\\%
 OrRd-8-8!70!black, every mark/.append style={solid,fill=OrRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-OrRd-9}{%
 OrRd-9-1!70!black, every mark/.append style={solid,fill=OrRd-9-1},mark=*\\%
 OrRd-9-2!70!black, every mark/.append style={solid,fill=OrRd-9-2},mark=square*\\%
 OrRd-9-3!70!black, every mark/.append style={solid,fill=OrRd-9-3},mark=triangle*\\%
 OrRd-9-4!70!black, every mark/.append style={solid,fill=OrRd-9-4},mark=diamond*\\%
 OrRd-9-5!70!black, every mark/.append style={solid,fill=OrRd-9-5},mark=pentagon*\\%
 OrRd-9-6!70!black, every mark/.append style={solid,fill=OrRd-9-6},mark=x\\%
 OrRd-9-7!70!black, every mark/.append style={solid,fill=OrRd-9-7},mark=+\\%
 OrRd-9-8!70!black, every mark/.append style={solid,fill=OrRd-9-8},mark=star\\%
 OrRd-9-9!70!black, every mark/.append style={solid,fill=OrRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-3}{%
 YlOrRd-3-1!70!black, every mark/.append style={solid,fill=YlOrRd-3-1},mark=*\\%
 YlOrRd-3-2!70!black, every mark/.append style={solid,fill=YlOrRd-3-2},mark=square*\\%
 YlOrRd-3-3!70!black, every mark/.append style={solid,fill=YlOrRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-4}{%
 YlOrRd-4-1!70!black, every mark/.append style={solid,fill=YlOrRd-4-1},mark=*\\%
 YlOrRd-4-2!70!black, every mark/.append style={solid,fill=YlOrRd-4-2},mark=square*\\%
 YlOrRd-4-3!70!black, every mark/.append style={solid,fill=YlOrRd-4-3},mark=triangle*\\%
 YlOrRd-4-4!70!black, every mark/.append style={solid,fill=YlOrRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-5}{%
 YlOrRd-5-1!70!black, every mark/.append style={solid,fill=YlOrRd-5-1},mark=*\\%
 YlOrRd-5-2!70!black, every mark/.append style={solid,fill=YlOrRd-5-2},mark=square*\\%
 YlOrRd-5-3!70!black, every mark/.append style={solid,fill=YlOrRd-5-3},mark=triangle*\\%
 YlOrRd-5-4!70!black, every mark/.append style={solid,fill=YlOrRd-5-4},mark=diamond*\\%
 YlOrRd-5-5!70!black, every mark/.append style={solid,fill=YlOrRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-6}{%
 YlOrRd-6-1!70!black, every mark/.append style={solid,fill=YlOrRd-6-1},mark=*\\%
 YlOrRd-6-2!70!black, every mark/.append style={solid,fill=YlOrRd-6-2},mark=square*\\%
 YlOrRd-6-3!70!black, every mark/.append style={solid,fill=YlOrRd-6-3},mark=triangle*\\%
 YlOrRd-6-4!70!black, every mark/.append style={solid,fill=YlOrRd-6-4},mark=diamond*\\%
 YlOrRd-6-5!70!black, every mark/.append style={solid,fill=YlOrRd-6-5},mark=pentagon*\\%
 YlOrRd-6-6!70!black, every mark/.append style={solid,fill=YlOrRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-7}{%
 YlOrRd-7-1!70!black, every mark/.append style={solid,fill=YlOrRd-7-1},mark=*\\%
 YlOrRd-7-2!70!black, every mark/.append style={solid,fill=YlOrRd-7-2},mark=square*\\%
 YlOrRd-7-3!70!black, every mark/.append style={solid,fill=YlOrRd-7-3},mark=triangle*\\%
 YlOrRd-7-4!70!black, every mark/.append style={solid,fill=YlOrRd-7-4},mark=diamond*\\%
 YlOrRd-7-5!70!black, every mark/.append style={solid,fill=YlOrRd-7-5},mark=pentagon*\\%
 YlOrRd-7-6!70!black, every mark/.append style={solid,fill=YlOrRd-7-6},mark=x\\%
 YlOrRd-7-7!70!black, every mark/.append style={solid,fill=YlOrRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-8}{%
 YlOrRd-8-1!70!black, every mark/.append style={solid,fill=YlOrRd-8-1},mark=*\\%
 YlOrRd-8-2!70!black, every mark/.append style={solid,fill=YlOrRd-8-2},mark=square*\\%
 YlOrRd-8-3!70!black, every mark/.append style={solid,fill=YlOrRd-8-3},mark=triangle*\\%
 YlOrRd-8-4!70!black, every mark/.append style={solid,fill=YlOrRd-8-4},mark=diamond*\\%
 YlOrRd-8-5!70!black, every mark/.append style={solid,fill=YlOrRd-8-5},mark=pentagon*\\%
 YlOrRd-8-6!70!black, every mark/.append style={solid,fill=YlOrRd-8-6},mark=x\\%
 YlOrRd-8-7!70!black, every mark/.append style={solid,fill=YlOrRd-8-7},mark=+\\%
 YlOrRd-8-8!70!black, every mark/.append style={solid,fill=YlOrRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrRd-9}{%
 YlOrRd-9-1!70!black, every mark/.append style={solid,fill=YlOrRd-9-1},mark=*\\%
 YlOrRd-9-2!70!black, every mark/.append style={solid,fill=YlOrRd-9-2},mark=square*\\%
 YlOrRd-9-3!70!black, every mark/.append style={solid,fill=YlOrRd-9-3},mark=triangle*\\%
 YlOrRd-9-4!70!black, every mark/.append style={solid,fill=YlOrRd-9-4},mark=diamond*\\%
 YlOrRd-9-5!70!black, every mark/.append style={solid,fill=YlOrRd-9-5},mark=pentagon*\\%
 YlOrRd-9-6!70!black, every mark/.append style={solid,fill=YlOrRd-9-6},mark=x\\%
 YlOrRd-9-7!70!black, every mark/.append style={solid,fill=YlOrRd-9-7},mark=+\\%
 YlOrRd-9-8!70!black, every mark/.append style={solid,fill=YlOrRd-9-8},mark=star\\%
 YlOrRd-9-9!70!black, every mark/.append style={solid,fill=YlOrRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-3}{%
 YlOrBr-3-1!70!black, every mark/.append style={solid,fill=YlOrBr-3-1},mark=*\\%
 YlOrBr-3-2!70!black, every mark/.append style={solid,fill=YlOrBr-3-2},mark=square*\\%
 YlOrBr-3-3!70!black, every mark/.append style={solid,fill=YlOrBr-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-4}{%
 YlOrBr-4-1!70!black, every mark/.append style={solid,fill=YlOrBr-4-1},mark=*\\%
 YlOrBr-4-2!70!black, every mark/.append style={solid,fill=YlOrBr-4-2},mark=square*\\%
 YlOrBr-4-3!70!black, every mark/.append style={solid,fill=YlOrBr-4-3},mark=triangle*\\%
 YlOrBr-4-4!70!black, every mark/.append style={solid,fill=YlOrBr-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-5}{%
 YlOrBr-5-1!70!black, every mark/.append style={solid,fill=YlOrBr-5-1},mark=*\\%
 YlOrBr-5-2!70!black, every mark/.append style={solid,fill=YlOrBr-5-2},mark=square*\\%
 YlOrBr-5-3!70!black, every mark/.append style={solid,fill=YlOrBr-5-3},mark=triangle*\\%
 YlOrBr-5-4!70!black, every mark/.append style={solid,fill=YlOrBr-5-4},mark=diamond*\\%
 YlOrBr-5-5!70!black, every mark/.append style={solid,fill=YlOrBr-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-6}{%
 YlOrBr-6-1!70!black, every mark/.append style={solid,fill=YlOrBr-6-1},mark=*\\%
 YlOrBr-6-2!70!black, every mark/.append style={solid,fill=YlOrBr-6-2},mark=square*\\%
 YlOrBr-6-3!70!black, every mark/.append style={solid,fill=YlOrBr-6-3},mark=triangle*\\%
 YlOrBr-6-4!70!black, every mark/.append style={solid,fill=YlOrBr-6-4},mark=diamond*\\%
 YlOrBr-6-5!70!black, every mark/.append style={solid,fill=YlOrBr-6-5},mark=pentagon*\\%
 YlOrBr-6-6!70!black, every mark/.append style={solid,fill=YlOrBr-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-7}{%
 YlOrBr-7-1!70!black, every mark/.append style={solid,fill=YlOrBr-7-1},mark=*\\%
 YlOrBr-7-2!70!black, every mark/.append style={solid,fill=YlOrBr-7-2},mark=square*\\%
 YlOrBr-7-3!70!black, every mark/.append style={solid,fill=YlOrBr-7-3},mark=triangle*\\%
 YlOrBr-7-4!70!black, every mark/.append style={solid,fill=YlOrBr-7-4},mark=diamond*\\%
 YlOrBr-7-5!70!black, every mark/.append style={solid,fill=YlOrBr-7-5},mark=pentagon*\\%
 YlOrBr-7-6!70!black, every mark/.append style={solid,fill=YlOrBr-7-6},mark=x\\%
 YlOrBr-7-7!70!black, every mark/.append style={solid,fill=YlOrBr-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-8}{%
 YlOrBr-8-1!70!black, every mark/.append style={solid,fill=YlOrBr-8-1},mark=*\\%
 YlOrBr-8-2!70!black, every mark/.append style={solid,fill=YlOrBr-8-2},mark=square*\\%
 YlOrBr-8-3!70!black, every mark/.append style={solid,fill=YlOrBr-8-3},mark=triangle*\\%
 YlOrBr-8-4!70!black, every mark/.append style={solid,fill=YlOrBr-8-4},mark=diamond*\\%
 YlOrBr-8-5!70!black, every mark/.append style={solid,fill=YlOrBr-8-5},mark=pentagon*\\%
 YlOrBr-8-6!70!black, every mark/.append style={solid,fill=YlOrBr-8-6},mark=x\\%
 YlOrBr-8-7!70!black, every mark/.append style={solid,fill=YlOrBr-8-7},mark=+\\%
 YlOrBr-8-8!70!black, every mark/.append style={solid,fill=YlOrBr-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-YlOrBr-9}{%
 YlOrBr-9-1!70!black, every mark/.append style={solid,fill=YlOrBr-9-1},mark=*\\%
 YlOrBr-9-2!70!black, every mark/.append style={solid,fill=YlOrBr-9-2},mark=square*\\%
 YlOrBr-9-3!70!black, every mark/.append style={solid,fill=YlOrBr-9-3},mark=triangle*\\%
 YlOrBr-9-4!70!black, every mark/.append style={solid,fill=YlOrBr-9-4},mark=diamond*\\%
 YlOrBr-9-5!70!black, every mark/.append style={solid,fill=YlOrBr-9-5},mark=pentagon*\\%
 YlOrBr-9-6!70!black, every mark/.append style={solid,fill=YlOrBr-9-6},mark=x\\%
 YlOrBr-9-7!70!black, every mark/.append style={solid,fill=YlOrBr-9-7},mark=+\\%
 YlOrBr-9-8!70!black, every mark/.append style={solid,fill=YlOrBr-9-8},mark=star\\%
 YlOrBr-9-9!70!black, every mark/.append style={solid,fill=YlOrBr-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-3}{%
 Purples-3-1!70!black, every mark/.append style={solid,fill=Purples-3-1},mark=*\\%
 Purples-3-2!70!black, every mark/.append style={solid,fill=Purples-3-2},mark=square*\\%
 Purples-3-3!70!black, every mark/.append style={solid,fill=Purples-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-4}{%
 Purples-4-1!70!black, every mark/.append style={solid,fill=Purples-4-1},mark=*\\%
 Purples-4-2!70!black, every mark/.append style={solid,fill=Purples-4-2},mark=square*\\%
 Purples-4-3!70!black, every mark/.append style={solid,fill=Purples-4-3},mark=triangle*\\%
 Purples-4-4!70!black, every mark/.append style={solid,fill=Purples-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-5}{%
 Purples-5-1!70!black, every mark/.append style={solid,fill=Purples-5-1},mark=*\\%
 Purples-5-2!70!black, every mark/.append style={solid,fill=Purples-5-2},mark=square*\\%
 Purples-5-3!70!black, every mark/.append style={solid,fill=Purples-5-3},mark=triangle*\\%
 Purples-5-4!70!black, every mark/.append style={solid,fill=Purples-5-4},mark=diamond*\\%
 Purples-5-5!70!black, every mark/.append style={solid,fill=Purples-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-6}{%
 Purples-6-1!70!black, every mark/.append style={solid,fill=Purples-6-1},mark=*\\%
 Purples-6-2!70!black, every mark/.append style={solid,fill=Purples-6-2},mark=square*\\%
 Purples-6-3!70!black, every mark/.append style={solid,fill=Purples-6-3},mark=triangle*\\%
 Purples-6-4!70!black, every mark/.append style={solid,fill=Purples-6-4},mark=diamond*\\%
 Purples-6-5!70!black, every mark/.append style={solid,fill=Purples-6-5},mark=pentagon*\\%
 Purples-6-6!70!black, every mark/.append style={solid,fill=Purples-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-7}{%
 Purples-7-1!70!black, every mark/.append style={solid,fill=Purples-7-1},mark=*\\%
 Purples-7-2!70!black, every mark/.append style={solid,fill=Purples-7-2},mark=square*\\%
 Purples-7-3!70!black, every mark/.append style={solid,fill=Purples-7-3},mark=triangle*\\%
 Purples-7-4!70!black, every mark/.append style={solid,fill=Purples-7-4},mark=diamond*\\%
 Purples-7-5!70!black, every mark/.append style={solid,fill=Purples-7-5},mark=pentagon*\\%
 Purples-7-6!70!black, every mark/.append style={solid,fill=Purples-7-6},mark=x\\%
 Purples-7-7!70!black, every mark/.append style={solid,fill=Purples-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-8}{%
 Purples-8-1!70!black, every mark/.append style={solid,fill=Purples-8-1},mark=*\\%
 Purples-8-2!70!black, every mark/.append style={solid,fill=Purples-8-2},mark=square*\\%
 Purples-8-3!70!black, every mark/.append style={solid,fill=Purples-8-3},mark=triangle*\\%
 Purples-8-4!70!black, every mark/.append style={solid,fill=Purples-8-4},mark=diamond*\\%
 Purples-8-5!70!black, every mark/.append style={solid,fill=Purples-8-5},mark=pentagon*\\%
 Purples-8-6!70!black, every mark/.append style={solid,fill=Purples-8-6},mark=x\\%
 Purples-8-7!70!black, every mark/.append style={solid,fill=Purples-8-7},mark=+\\%
 Purples-8-8!70!black, every mark/.append style={solid,fill=Purples-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Purples-9}{%
 Purples-9-1!70!black, every mark/.append style={solid,fill=Purples-9-1},mark=*\\%
 Purples-9-2!70!black, every mark/.append style={solid,fill=Purples-9-2},mark=square*\\%
 Purples-9-3!70!black, every mark/.append style={solid,fill=Purples-9-3},mark=triangle*\\%
 Purples-9-4!70!black, every mark/.append style={solid,fill=Purples-9-4},mark=diamond*\\%
 Purples-9-5!70!black, every mark/.append style={solid,fill=Purples-9-5},mark=pentagon*\\%
 Purples-9-6!70!black, every mark/.append style={solid,fill=Purples-9-6},mark=x\\%
 Purples-9-7!70!black, every mark/.append style={solid,fill=Purples-9-7},mark=+\\%
 Purples-9-8!70!black, every mark/.append style={solid,fill=Purples-9-8},mark=star\\%
 Purples-9-9!70!black, every mark/.append style={solid,fill=Purples-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-3}{%
 Blues-3-1!70!black, every mark/.append style={solid,fill=Blues-3-1},mark=*\\%
 Blues-3-2!70!black, every mark/.append style={solid,fill=Blues-3-2},mark=square*\\%
 Blues-3-3!70!black, every mark/.append style={solid,fill=Blues-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-4}{%
 Blues-4-1!70!black, every mark/.append style={solid,fill=Blues-4-1},mark=*\\%
 Blues-4-2!70!black, every mark/.append style={solid,fill=Blues-4-2},mark=square*\\%
 Blues-4-3!70!black, every mark/.append style={solid,fill=Blues-4-3},mark=triangle*\\%
 Blues-4-4!70!black, every mark/.append style={solid,fill=Blues-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-5}{%
 Blues-5-1!70!black, every mark/.append style={solid,fill=Blues-5-1},mark=*\\%
 Blues-5-2!70!black, every mark/.append style={solid,fill=Blues-5-2},mark=square*\\%
 Blues-5-3!70!black, every mark/.append style={solid,fill=Blues-5-3},mark=triangle*\\%
 Blues-5-4!70!black, every mark/.append style={solid,fill=Blues-5-4},mark=diamond*\\%
 Blues-5-5!70!black, every mark/.append style={solid,fill=Blues-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-6}{%
 Blues-6-1!70!black, every mark/.append style={solid,fill=Blues-6-1},mark=*\\%
 Blues-6-2!70!black, every mark/.append style={solid,fill=Blues-6-2},mark=square*\\%
 Blues-6-3!70!black, every mark/.append style={solid,fill=Blues-6-3},mark=triangle*\\%
 Blues-6-4!70!black, every mark/.append style={solid,fill=Blues-6-4},mark=diamond*\\%
 Blues-6-5!70!black, every mark/.append style={solid,fill=Blues-6-5},mark=pentagon*\\%
 Blues-6-6!70!black, every mark/.append style={solid,fill=Blues-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-7}{%
 Blues-7-1!70!black, every mark/.append style={solid,fill=Blues-7-1},mark=*\\%
 Blues-7-2!70!black, every mark/.append style={solid,fill=Blues-7-2},mark=square*\\%
 Blues-7-3!70!black, every mark/.append style={solid,fill=Blues-7-3},mark=triangle*\\%
 Blues-7-4!70!black, every mark/.append style={solid,fill=Blues-7-4},mark=diamond*\\%
 Blues-7-5!70!black, every mark/.append style={solid,fill=Blues-7-5},mark=pentagon*\\%
 Blues-7-6!70!black, every mark/.append style={solid,fill=Blues-7-6},mark=x\\%
 Blues-7-7!70!black, every mark/.append style={solid,fill=Blues-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-8}{%
 Blues-8-1!70!black, every mark/.append style={solid,fill=Blues-8-1},mark=*\\%
 Blues-8-2!70!black, every mark/.append style={solid,fill=Blues-8-2},mark=square*\\%
 Blues-8-3!70!black, every mark/.append style={solid,fill=Blues-8-3},mark=triangle*\\%
 Blues-8-4!70!black, every mark/.append style={solid,fill=Blues-8-4},mark=diamond*\\%
 Blues-8-5!70!black, every mark/.append style={solid,fill=Blues-8-5},mark=pentagon*\\%
 Blues-8-6!70!black, every mark/.append style={solid,fill=Blues-8-6},mark=x\\%
 Blues-8-7!70!black, every mark/.append style={solid,fill=Blues-8-7},mark=+\\%
 Blues-8-8!70!black, every mark/.append style={solid,fill=Blues-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Blues-9}{%
 Blues-9-1!70!black, every mark/.append style={solid,fill=Blues-9-1},mark=*\\%
 Blues-9-2!70!black, every mark/.append style={solid,fill=Blues-9-2},mark=square*\\%
 Blues-9-3!70!black, every mark/.append style={solid,fill=Blues-9-3},mark=triangle*\\%
 Blues-9-4!70!black, every mark/.append style={solid,fill=Blues-9-4},mark=diamond*\\%
 Blues-9-5!70!black, every mark/.append style={solid,fill=Blues-9-5},mark=pentagon*\\%
 Blues-9-6!70!black, every mark/.append style={solid,fill=Blues-9-6},mark=x\\%
 Blues-9-7!70!black, every mark/.append style={solid,fill=Blues-9-7},mark=+\\%
 Blues-9-8!70!black, every mark/.append style={solid,fill=Blues-9-8},mark=star\\%
 Blues-9-9!70!black, every mark/.append style={solid,fill=Blues-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-3}{%
 Greens-3-1!70!black, every mark/.append style={solid,fill=Greens-3-1},mark=*\\%
 Greens-3-2!70!black, every mark/.append style={solid,fill=Greens-3-2},mark=square*\\%
 Greens-3-3!70!black, every mark/.append style={solid,fill=Greens-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-4}{%
 Greens-4-1!70!black, every mark/.append style={solid,fill=Greens-4-1},mark=*\\%
 Greens-4-2!70!black, every mark/.append style={solid,fill=Greens-4-2},mark=square*\\%
 Greens-4-3!70!black, every mark/.append style={solid,fill=Greens-4-3},mark=triangle*\\%
 Greens-4-4!70!black, every mark/.append style={solid,fill=Greens-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-5}{%
 Greens-5-1!70!black, every mark/.append style={solid,fill=Greens-5-1},mark=*\\%
 Greens-5-2!70!black, every mark/.append style={solid,fill=Greens-5-2},mark=square*\\%
 Greens-5-3!70!black, every mark/.append style={solid,fill=Greens-5-3},mark=triangle*\\%
 Greens-5-4!70!black, every mark/.append style={solid,fill=Greens-5-4},mark=diamond*\\%
 Greens-5-5!70!black, every mark/.append style={solid,fill=Greens-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-6}{%
 Greens-6-1!70!black, every mark/.append style={solid,fill=Greens-6-1},mark=*\\%
 Greens-6-2!70!black, every mark/.append style={solid,fill=Greens-6-2},mark=square*\\%
 Greens-6-3!70!black, every mark/.append style={solid,fill=Greens-6-3},mark=triangle*\\%
 Greens-6-4!70!black, every mark/.append style={solid,fill=Greens-6-4},mark=diamond*\\%
 Greens-6-5!70!black, every mark/.append style={solid,fill=Greens-6-5},mark=pentagon*\\%
 Greens-6-6!70!black, every mark/.append style={solid,fill=Greens-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-7}{%
 Greens-7-1!70!black, every mark/.append style={solid,fill=Greens-7-1},mark=*\\%
 Greens-7-2!70!black, every mark/.append style={solid,fill=Greens-7-2},mark=square*\\%
 Greens-7-3!70!black, every mark/.append style={solid,fill=Greens-7-3},mark=triangle*\\%
 Greens-7-4!70!black, every mark/.append style={solid,fill=Greens-7-4},mark=diamond*\\%
 Greens-7-5!70!black, every mark/.append style={solid,fill=Greens-7-5},mark=pentagon*\\%
 Greens-7-6!70!black, every mark/.append style={solid,fill=Greens-7-6},mark=x\\%
 Greens-7-7!70!black, every mark/.append style={solid,fill=Greens-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-8}{%
 Greens-8-1!70!black, every mark/.append style={solid,fill=Greens-8-1},mark=*\\%
 Greens-8-2!70!black, every mark/.append style={solid,fill=Greens-8-2},mark=square*\\%
 Greens-8-3!70!black, every mark/.append style={solid,fill=Greens-8-3},mark=triangle*\\%
 Greens-8-4!70!black, every mark/.append style={solid,fill=Greens-8-4},mark=diamond*\\%
 Greens-8-5!70!black, every mark/.append style={solid,fill=Greens-8-5},mark=pentagon*\\%
 Greens-8-6!70!black, every mark/.append style={solid,fill=Greens-8-6},mark=x\\%
 Greens-8-7!70!black, every mark/.append style={solid,fill=Greens-8-7},mark=+\\%
 Greens-8-8!70!black, every mark/.append style={solid,fill=Greens-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Greens-9}{%
 Greens-9-1!70!black, every mark/.append style={solid,fill=Greens-9-1},mark=*\\%
 Greens-9-2!70!black, every mark/.append style={solid,fill=Greens-9-2},mark=square*\\%
 Greens-9-3!70!black, every mark/.append style={solid,fill=Greens-9-3},mark=triangle*\\%
 Greens-9-4!70!black, every mark/.append style={solid,fill=Greens-9-4},mark=diamond*\\%
 Greens-9-5!70!black, every mark/.append style={solid,fill=Greens-9-5},mark=pentagon*\\%
 Greens-9-6!70!black, every mark/.append style={solid,fill=Greens-9-6},mark=x\\%
 Greens-9-7!70!black, every mark/.append style={solid,fill=Greens-9-7},mark=+\\%
 Greens-9-8!70!black, every mark/.append style={solid,fill=Greens-9-8},mark=star\\%
 Greens-9-9!70!black, every mark/.append style={solid,fill=Greens-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-3}{%
 Oranges-3-1!70!black, every mark/.append style={solid,fill=Oranges-3-1},mark=*\\%
 Oranges-3-2!70!black, every mark/.append style={solid,fill=Oranges-3-2},mark=square*\\%
 Oranges-3-3!70!black, every mark/.append style={solid,fill=Oranges-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-4}{%
 Oranges-4-1!70!black, every mark/.append style={solid,fill=Oranges-4-1},mark=*\\%
 Oranges-4-2!70!black, every mark/.append style={solid,fill=Oranges-4-2},mark=square*\\%
 Oranges-4-3!70!black, every mark/.append style={solid,fill=Oranges-4-3},mark=triangle*\\%
 Oranges-4-4!70!black, every mark/.append style={solid,fill=Oranges-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-5}{%
 Oranges-5-1!70!black, every mark/.append style={solid,fill=Oranges-5-1},mark=*\\%
 Oranges-5-2!70!black, every mark/.append style={solid,fill=Oranges-5-2},mark=square*\\%
 Oranges-5-3!70!black, every mark/.append style={solid,fill=Oranges-5-3},mark=triangle*\\%
 Oranges-5-4!70!black, every mark/.append style={solid,fill=Oranges-5-4},mark=diamond*\\%
 Oranges-5-5!70!black, every mark/.append style={solid,fill=Oranges-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-6}{%
 Oranges-6-1!70!black, every mark/.append style={solid,fill=Oranges-6-1},mark=*\\%
 Oranges-6-2!70!black, every mark/.append style={solid,fill=Oranges-6-2},mark=square*\\%
 Oranges-6-3!70!black, every mark/.append style={solid,fill=Oranges-6-3},mark=triangle*\\%
 Oranges-6-4!70!black, every mark/.append style={solid,fill=Oranges-6-4},mark=diamond*\\%
 Oranges-6-5!70!black, every mark/.append style={solid,fill=Oranges-6-5},mark=pentagon*\\%
 Oranges-6-6!70!black, every mark/.append style={solid,fill=Oranges-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-7}{%
 Oranges-7-1!70!black, every mark/.append style={solid,fill=Oranges-7-1},mark=*\\%
 Oranges-7-2!70!black, every mark/.append style={solid,fill=Oranges-7-2},mark=square*\\%
 Oranges-7-3!70!black, every mark/.append style={solid,fill=Oranges-7-3},mark=triangle*\\%
 Oranges-7-4!70!black, every mark/.append style={solid,fill=Oranges-7-4},mark=diamond*\\%
 Oranges-7-5!70!black, every mark/.append style={solid,fill=Oranges-7-5},mark=pentagon*\\%
 Oranges-7-6!70!black, every mark/.append style={solid,fill=Oranges-7-6},mark=x\\%
 Oranges-7-7!70!black, every mark/.append style={solid,fill=Oranges-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-8}{%
 Oranges-8-1!70!black, every mark/.append style={solid,fill=Oranges-8-1},mark=*\\%
 Oranges-8-2!70!black, every mark/.append style={solid,fill=Oranges-8-2},mark=square*\\%
 Oranges-8-3!70!black, every mark/.append style={solid,fill=Oranges-8-3},mark=triangle*\\%
 Oranges-8-4!70!black, every mark/.append style={solid,fill=Oranges-8-4},mark=diamond*\\%
 Oranges-8-5!70!black, every mark/.append style={solid,fill=Oranges-8-5},mark=pentagon*\\%
 Oranges-8-6!70!black, every mark/.append style={solid,fill=Oranges-8-6},mark=x\\%
 Oranges-8-7!70!black, every mark/.append style={solid,fill=Oranges-8-7},mark=+\\%
 Oranges-8-8!70!black, every mark/.append style={solid,fill=Oranges-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Oranges-9}{%
 Oranges-9-1!70!black, every mark/.append style={solid,fill=Oranges-9-1},mark=*\\%
 Oranges-9-2!70!black, every mark/.append style={solid,fill=Oranges-9-2},mark=square*\\%
 Oranges-9-3!70!black, every mark/.append style={solid,fill=Oranges-9-3},mark=triangle*\\%
 Oranges-9-4!70!black, every mark/.append style={solid,fill=Oranges-9-4},mark=diamond*\\%
 Oranges-9-5!70!black, every mark/.append style={solid,fill=Oranges-9-5},mark=pentagon*\\%
 Oranges-9-6!70!black, every mark/.append style={solid,fill=Oranges-9-6},mark=x\\%
 Oranges-9-7!70!black, every mark/.append style={solid,fill=Oranges-9-7},mark=+\\%
 Oranges-9-8!70!black, every mark/.append style={solid,fill=Oranges-9-8},mark=star\\%
 Oranges-9-9!70!black, every mark/.append style={solid,fill=Oranges-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-3}{%
 Reds-3-1!70!black, every mark/.append style={solid,fill=Reds-3-1},mark=*\\%
 Reds-3-2!70!black, every mark/.append style={solid,fill=Reds-3-2},mark=square*\\%
 Reds-3-3!70!black, every mark/.append style={solid,fill=Reds-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-4}{%
 Reds-4-1!70!black, every mark/.append style={solid,fill=Reds-4-1},mark=*\\%
 Reds-4-2!70!black, every mark/.append style={solid,fill=Reds-4-2},mark=square*\\%
 Reds-4-3!70!black, every mark/.append style={solid,fill=Reds-4-3},mark=triangle*\\%
 Reds-4-4!70!black, every mark/.append style={solid,fill=Reds-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-5}{%
 Reds-5-1!70!black, every mark/.append style={solid,fill=Reds-5-1},mark=*\\%
 Reds-5-2!70!black, every mark/.append style={solid,fill=Reds-5-2},mark=square*\\%
 Reds-5-3!70!black, every mark/.append style={solid,fill=Reds-5-3},mark=triangle*\\%
 Reds-5-4!70!black, every mark/.append style={solid,fill=Reds-5-4},mark=diamond*\\%
 Reds-5-5!70!black, every mark/.append style={solid,fill=Reds-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-6}{%
 Reds-6-1!70!black, every mark/.append style={solid,fill=Reds-6-1},mark=*\\%
 Reds-6-2!70!black, every mark/.append style={solid,fill=Reds-6-2},mark=square*\\%
 Reds-6-3!70!black, every mark/.append style={solid,fill=Reds-6-3},mark=triangle*\\%
 Reds-6-4!70!black, every mark/.append style={solid,fill=Reds-6-4},mark=diamond*\\%
 Reds-6-5!70!black, every mark/.append style={solid,fill=Reds-6-5},mark=pentagon*\\%
 Reds-6-6!70!black, every mark/.append style={solid,fill=Reds-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-7}{%
 Reds-7-1!70!black, every mark/.append style={solid,fill=Reds-7-1},mark=*\\%
 Reds-7-2!70!black, every mark/.append style={solid,fill=Reds-7-2},mark=square*\\%
 Reds-7-3!70!black, every mark/.append style={solid,fill=Reds-7-3},mark=triangle*\\%
 Reds-7-4!70!black, every mark/.append style={solid,fill=Reds-7-4},mark=diamond*\\%
 Reds-7-5!70!black, every mark/.append style={solid,fill=Reds-7-5},mark=pentagon*\\%
 Reds-7-6!70!black, every mark/.append style={solid,fill=Reds-7-6},mark=x\\%
 Reds-7-7!70!black, every mark/.append style={solid,fill=Reds-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-8}{%
 Reds-8-1!70!black, every mark/.append style={solid,fill=Reds-8-1},mark=*\\%
 Reds-8-2!70!black, every mark/.append style={solid,fill=Reds-8-2},mark=square*\\%
 Reds-8-3!70!black, every mark/.append style={solid,fill=Reds-8-3},mark=triangle*\\%
 Reds-8-4!70!black, every mark/.append style={solid,fill=Reds-8-4},mark=diamond*\\%
 Reds-8-5!70!black, every mark/.append style={solid,fill=Reds-8-5},mark=pentagon*\\%
 Reds-8-6!70!black, every mark/.append style={solid,fill=Reds-8-6},mark=x\\%
 Reds-8-7!70!black, every mark/.append style={solid,fill=Reds-8-7},mark=+\\%
 Reds-8-8!70!black, every mark/.append style={solid,fill=Reds-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Reds-9}{%
 Reds-9-1!70!black, every mark/.append style={solid,fill=Reds-9-1},mark=*\\%
 Reds-9-2!70!black, every mark/.append style={solid,fill=Reds-9-2},mark=square*\\%
 Reds-9-3!70!black, every mark/.append style={solid,fill=Reds-9-3},mark=triangle*\\%
 Reds-9-4!70!black, every mark/.append style={solid,fill=Reds-9-4},mark=diamond*\\%
 Reds-9-5!70!black, every mark/.append style={solid,fill=Reds-9-5},mark=pentagon*\\%
 Reds-9-6!70!black, every mark/.append style={solid,fill=Reds-9-6},mark=x\\%
 Reds-9-7!70!black, every mark/.append style={solid,fill=Reds-9-7},mark=+\\%
 Reds-9-8!70!black, every mark/.append style={solid,fill=Reds-9-8},mark=star\\%
 Reds-9-9!70!black, every mark/.append style={solid,fill=Reds-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-3}{%
 Greys-3-1!70!black, every mark/.append style={solid,fill=Greys-3-1},mark=*\\%
 Greys-3-2!70!black, every mark/.append style={solid,fill=Greys-3-2},mark=square*\\%
 Greys-3-3!70!black, every mark/.append style={solid,fill=Greys-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-4}{%
 Greys-4-1!70!black, every mark/.append style={solid,fill=Greys-4-1},mark=*\\%
 Greys-4-2!70!black, every mark/.append style={solid,fill=Greys-4-2},mark=square*\\%
 Greys-4-3!70!black, every mark/.append style={solid,fill=Greys-4-3},mark=triangle*\\%
 Greys-4-4!70!black, every mark/.append style={solid,fill=Greys-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-5}{%
 Greys-5-1!70!black, every mark/.append style={solid,fill=Greys-5-1},mark=*\\%
 Greys-5-2!70!black, every mark/.append style={solid,fill=Greys-5-2},mark=square*\\%
 Greys-5-3!70!black, every mark/.append style={solid,fill=Greys-5-3},mark=triangle*\\%
 Greys-5-4!70!black, every mark/.append style={solid,fill=Greys-5-4},mark=diamond*\\%
 Greys-5-5!70!black, every mark/.append style={solid,fill=Greys-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-6}{%
 Greys-6-1!70!black, every mark/.append style={solid,fill=Greys-6-1},mark=*\\%
 Greys-6-2!70!black, every mark/.append style={solid,fill=Greys-6-2},mark=square*\\%
 Greys-6-3!70!black, every mark/.append style={solid,fill=Greys-6-3},mark=triangle*\\%
 Greys-6-4!70!black, every mark/.append style={solid,fill=Greys-6-4},mark=diamond*\\%
 Greys-6-5!70!black, every mark/.append style={solid,fill=Greys-6-5},mark=pentagon*\\%
 Greys-6-6!70!black, every mark/.append style={solid,fill=Greys-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-7}{%
 Greys-7-1!70!black, every mark/.append style={solid,fill=Greys-7-1},mark=*\\%
 Greys-7-2!70!black, every mark/.append style={solid,fill=Greys-7-2},mark=square*\\%
 Greys-7-3!70!black, every mark/.append style={solid,fill=Greys-7-3},mark=triangle*\\%
 Greys-7-4!70!black, every mark/.append style={solid,fill=Greys-7-4},mark=diamond*\\%
 Greys-7-5!70!black, every mark/.append style={solid,fill=Greys-7-5},mark=pentagon*\\%
 Greys-7-6!70!black, every mark/.append style={solid,fill=Greys-7-6},mark=x\\%
 Greys-7-7!70!black, every mark/.append style={solid,fill=Greys-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-8}{%
 Greys-8-1!70!black, every mark/.append style={solid,fill=Greys-8-1},mark=*\\%
 Greys-8-2!70!black, every mark/.append style={solid,fill=Greys-8-2},mark=square*\\%
 Greys-8-3!70!black, every mark/.append style={solid,fill=Greys-8-3},mark=triangle*\\%
 Greys-8-4!70!black, every mark/.append style={solid,fill=Greys-8-4},mark=diamond*\\%
 Greys-8-5!70!black, every mark/.append style={solid,fill=Greys-8-5},mark=pentagon*\\%
 Greys-8-6!70!black, every mark/.append style={solid,fill=Greys-8-6},mark=x\\%
 Greys-8-7!70!black, every mark/.append style={solid,fill=Greys-8-7},mark=+\\%
 Greys-8-8!70!black, every mark/.append style={solid,fill=Greys-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Greys-9}{%
 Greys-9-1!70!black, every mark/.append style={solid,fill=Greys-9-1},mark=*\\%
 Greys-9-2!70!black, every mark/.append style={solid,fill=Greys-9-2},mark=square*\\%
 Greys-9-3!70!black, every mark/.append style={solid,fill=Greys-9-3},mark=triangle*\\%
 Greys-9-4!70!black, every mark/.append style={solid,fill=Greys-9-4},mark=diamond*\\%
 Greys-9-5!70!black, every mark/.append style={solid,fill=Greys-9-5},mark=pentagon*\\%
 Greys-9-6!70!black, every mark/.append style={solid,fill=Greys-9-6},mark=x\\%
 Greys-9-7!70!black, every mark/.append style={solid,fill=Greys-9-7},mark=+\\%
 Greys-9-8!70!black, every mark/.append style={solid,fill=Greys-9-8},mark=star\\%
 Greys-9-9!70!black, every mark/.append style={solid,fill=Greys-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-3}{%
 PuOr-3-1!70!black, every mark/.append style={solid,fill=PuOr-3-1},mark=*\\%
 PuOr-3-2!70!black, every mark/.append style={solid,fill=PuOr-3-2},mark=square*\\%
 PuOr-3-3!70!black, every mark/.append style={solid,fill=PuOr-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-4}{%
 PuOr-4-1!70!black, every mark/.append style={solid,fill=PuOr-4-1},mark=*\\%
 PuOr-4-2!70!black, every mark/.append style={solid,fill=PuOr-4-2},mark=square*\\%
 PuOr-4-3!70!black, every mark/.append style={solid,fill=PuOr-4-3},mark=triangle*\\%
 PuOr-4-4!70!black, every mark/.append style={solid,fill=PuOr-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-5}{%
 PuOr-5-1!70!black, every mark/.append style={solid,fill=PuOr-5-1},mark=*\\%
 PuOr-5-2!70!black, every mark/.append style={solid,fill=PuOr-5-2},mark=square*\\%
 PuOr-5-3!70!black, every mark/.append style={solid,fill=PuOr-5-3},mark=triangle*\\%
 PuOr-5-4!70!black, every mark/.append style={solid,fill=PuOr-5-4},mark=diamond*\\%
 PuOr-5-5!70!black, every mark/.append style={solid,fill=PuOr-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-6}{%
 PuOr-6-1!70!black, every mark/.append style={solid,fill=PuOr-6-1},mark=*\\%
 PuOr-6-2!70!black, every mark/.append style={solid,fill=PuOr-6-2},mark=square*\\%
 PuOr-6-3!70!black, every mark/.append style={solid,fill=PuOr-6-3},mark=triangle*\\%
 PuOr-6-4!70!black, every mark/.append style={solid,fill=PuOr-6-4},mark=diamond*\\%
 PuOr-6-5!70!black, every mark/.append style={solid,fill=PuOr-6-5},mark=pentagon*\\%
 PuOr-6-6!70!black, every mark/.append style={solid,fill=PuOr-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-7}{%
 PuOr-7-1!70!black, every mark/.append style={solid,fill=PuOr-7-1},mark=*\\%
 PuOr-7-2!70!black, every mark/.append style={solid,fill=PuOr-7-2},mark=square*\\%
 PuOr-7-3!70!black, every mark/.append style={solid,fill=PuOr-7-3},mark=triangle*\\%
 PuOr-7-4!70!black, every mark/.append style={solid,fill=PuOr-7-4},mark=diamond*\\%
 PuOr-7-5!70!black, every mark/.append style={solid,fill=PuOr-7-5},mark=pentagon*\\%
 PuOr-7-6!70!black, every mark/.append style={solid,fill=PuOr-7-6},mark=x\\%
 PuOr-7-7!70!black, every mark/.append style={solid,fill=PuOr-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-8}{%
 PuOr-8-1!70!black, every mark/.append style={solid,fill=PuOr-8-1},mark=*\\%
 PuOr-8-2!70!black, every mark/.append style={solid,fill=PuOr-8-2},mark=square*\\%
 PuOr-8-3!70!black, every mark/.append style={solid,fill=PuOr-8-3},mark=triangle*\\%
 PuOr-8-4!70!black, every mark/.append style={solid,fill=PuOr-8-4},mark=diamond*\\%
 PuOr-8-5!70!black, every mark/.append style={solid,fill=PuOr-8-5},mark=pentagon*\\%
 PuOr-8-6!70!black, every mark/.append style={solid,fill=PuOr-8-6},mark=x\\%
 PuOr-8-7!70!black, every mark/.append style={solid,fill=PuOr-8-7},mark=+\\%
 PuOr-8-8!70!black, every mark/.append style={solid,fill=PuOr-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-9}{%
 PuOr-9-1!70!black, every mark/.append style={solid,fill=PuOr-9-1},mark=*\\%
 PuOr-9-2!70!black, every mark/.append style={solid,fill=PuOr-9-2},mark=square*\\%
 PuOr-9-3!70!black, every mark/.append style={solid,fill=PuOr-9-3},mark=triangle*\\%
 PuOr-9-4!70!black, every mark/.append style={solid,fill=PuOr-9-4},mark=diamond*\\%
 PuOr-9-5!70!black, every mark/.append style={solid,fill=PuOr-9-5},mark=pentagon*\\%
 PuOr-9-6!70!black, every mark/.append style={solid,fill=PuOr-9-6},mark=x\\%
 PuOr-9-7!70!black, every mark/.append style={solid,fill=PuOr-9-7},mark=+\\%
 PuOr-9-8!70!black, every mark/.append style={solid,fill=PuOr-9-8},mark=star\\%
 PuOr-9-9!70!black, every mark/.append style={solid,fill=PuOr-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-10}{%
 PuOr-10-1!70!black, every mark/.append style={solid,fill=PuOr-10-1},mark=*\\%
 PuOr-10-2!70!black, every mark/.append style={solid,fill=PuOr-10-2},mark=square*\\%
 PuOr-10-3!70!black, every mark/.append style={solid,fill=PuOr-10-3},mark=triangle*\\%
 PuOr-10-4!70!black, every mark/.append style={solid,fill=PuOr-10-4},mark=diamond*\\%
 PuOr-10-5!70!black, every mark/.append style={solid,fill=PuOr-10-5},mark=pentagon*\\%
 PuOr-10-6!70!black, every mark/.append style={solid,fill=PuOr-10-6},mark=x\\%
 PuOr-10-7!70!black, every mark/.append style={solid,fill=PuOr-10-7},mark=+\\%
 PuOr-10-8!70!black, every mark/.append style={solid,fill=PuOr-10-8},mark=star\\%
 PuOr-10-9!70!black, every mark/.append style={solid,fill=PuOr-10-9},mark=oplus*\\%
 PuOr-10-10!70!black, every mark/.append style={solid,fill=PuOr-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-PuOr-11}{%
 PuOr-11-1!70!black, every mark/.append style={solid,fill=PuOr-11-1},mark=*\\%
 PuOr-11-2!70!black, every mark/.append style={solid,fill=PuOr-11-2},mark=square*\\%
 PuOr-11-3!70!black, every mark/.append style={solid,fill=PuOr-11-3},mark=triangle*\\%
 PuOr-11-4!70!black, every mark/.append style={solid,fill=PuOr-11-4},mark=diamond*\\%
 PuOr-11-5!70!black, every mark/.append style={solid,fill=PuOr-11-5},mark=pentagon*\\%
 PuOr-11-6!70!black, every mark/.append style={solid,fill=PuOr-11-6},mark=x\\%
 PuOr-11-7!70!black, every mark/.append style={solid,fill=PuOr-11-7},mark=+\\%
 PuOr-11-8!70!black, every mark/.append style={solid,fill=PuOr-11-8},mark=star\\%
 PuOr-11-9!70!black, every mark/.append style={solid,fill=PuOr-11-9},mark=oplus*\\%
 PuOr-11-10!70!black, every mark/.append style={solid,fill=PuOr-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-3}{%
 BrBG-3-1!70!black, every mark/.append style={solid,fill=BrBG-3-1},mark=*\\%
 BrBG-3-2!70!black, every mark/.append style={solid,fill=BrBG-3-2},mark=square*\\%
 BrBG-3-3!70!black, every mark/.append style={solid,fill=BrBG-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-4}{%
 BrBG-4-1!70!black, every mark/.append style={solid,fill=BrBG-4-1},mark=*\\%
 BrBG-4-2!70!black, every mark/.append style={solid,fill=BrBG-4-2},mark=square*\\%
 BrBG-4-3!70!black, every mark/.append style={solid,fill=BrBG-4-3},mark=triangle*\\%
 BrBG-4-4!70!black, every mark/.append style={solid,fill=BrBG-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-5}{%
 BrBG-5-1!70!black, every mark/.append style={solid,fill=BrBG-5-1},mark=*\\%
 BrBG-5-2!70!black, every mark/.append style={solid,fill=BrBG-5-2},mark=square*\\%
 BrBG-5-3!70!black, every mark/.append style={solid,fill=BrBG-5-3},mark=triangle*\\%
 BrBG-5-4!70!black, every mark/.append style={solid,fill=BrBG-5-4},mark=diamond*\\%
 BrBG-5-5!70!black, every mark/.append style={solid,fill=BrBG-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-6}{%
 BrBG-6-1!70!black, every mark/.append style={solid,fill=BrBG-6-1},mark=*\\%
 BrBG-6-2!70!black, every mark/.append style={solid,fill=BrBG-6-2},mark=square*\\%
 BrBG-6-3!70!black, every mark/.append style={solid,fill=BrBG-6-3},mark=triangle*\\%
 BrBG-6-4!70!black, every mark/.append style={solid,fill=BrBG-6-4},mark=diamond*\\%
 BrBG-6-5!70!black, every mark/.append style={solid,fill=BrBG-6-5},mark=pentagon*\\%
 BrBG-6-6!70!black, every mark/.append style={solid,fill=BrBG-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-7}{%
 BrBG-7-1!70!black, every mark/.append style={solid,fill=BrBG-7-1},mark=*\\%
 BrBG-7-2!70!black, every mark/.append style={solid,fill=BrBG-7-2},mark=square*\\%
 BrBG-7-3!70!black, every mark/.append style={solid,fill=BrBG-7-3},mark=triangle*\\%
 BrBG-7-4!70!black, every mark/.append style={solid,fill=BrBG-7-4},mark=diamond*\\%
 BrBG-7-5!70!black, every mark/.append style={solid,fill=BrBG-7-5},mark=pentagon*\\%
 BrBG-7-6!70!black, every mark/.append style={solid,fill=BrBG-7-6},mark=x\\%
 BrBG-7-7!70!black, every mark/.append style={solid,fill=BrBG-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-8}{%
 BrBG-8-1!70!black, every mark/.append style={solid,fill=BrBG-8-1},mark=*\\%
 BrBG-8-2!70!black, every mark/.append style={solid,fill=BrBG-8-2},mark=square*\\%
 BrBG-8-3!70!black, every mark/.append style={solid,fill=BrBG-8-3},mark=triangle*\\%
 BrBG-8-4!70!black, every mark/.append style={solid,fill=BrBG-8-4},mark=diamond*\\%
 BrBG-8-5!70!black, every mark/.append style={solid,fill=BrBG-8-5},mark=pentagon*\\%
 BrBG-8-6!70!black, every mark/.append style={solid,fill=BrBG-8-6},mark=x\\%
 BrBG-8-7!70!black, every mark/.append style={solid,fill=BrBG-8-7},mark=+\\%
 BrBG-8-8!70!black, every mark/.append style={solid,fill=BrBG-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-9}{%
 BrBG-9-1!70!black, every mark/.append style={solid,fill=BrBG-9-1},mark=*\\%
 BrBG-9-2!70!black, every mark/.append style={solid,fill=BrBG-9-2},mark=square*\\%
 BrBG-9-3!70!black, every mark/.append style={solid,fill=BrBG-9-3},mark=triangle*\\%
 BrBG-9-4!70!black, every mark/.append style={solid,fill=BrBG-9-4},mark=diamond*\\%
 BrBG-9-5!70!black, every mark/.append style={solid,fill=BrBG-9-5},mark=pentagon*\\%
 BrBG-9-6!70!black, every mark/.append style={solid,fill=BrBG-9-6},mark=x\\%
 BrBG-9-7!70!black, every mark/.append style={solid,fill=BrBG-9-7},mark=+\\%
 BrBG-9-8!70!black, every mark/.append style={solid,fill=BrBG-9-8},mark=star\\%
 BrBG-9-9!70!black, every mark/.append style={solid,fill=BrBG-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-10}{%
 BrBG-10-1!70!black, every mark/.append style={solid,fill=BrBG-10-1},mark=*\\%
 BrBG-10-2!70!black, every mark/.append style={solid,fill=BrBG-10-2},mark=square*\\%
 BrBG-10-3!70!black, every mark/.append style={solid,fill=BrBG-10-3},mark=triangle*\\%
 BrBG-10-4!70!black, every mark/.append style={solid,fill=BrBG-10-4},mark=diamond*\\%
 BrBG-10-5!70!black, every mark/.append style={solid,fill=BrBG-10-5},mark=pentagon*\\%
 BrBG-10-6!70!black, every mark/.append style={solid,fill=BrBG-10-6},mark=x\\%
 BrBG-10-7!70!black, every mark/.append style={solid,fill=BrBG-10-7},mark=+\\%
 BrBG-10-8!70!black, every mark/.append style={solid,fill=BrBG-10-8},mark=star\\%
 BrBG-10-9!70!black, every mark/.append style={solid,fill=BrBG-10-9},mark=oplus*\\%
 BrBG-10-10!70!black, every mark/.append style={solid,fill=BrBG-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-BrBG-11}{%
 BrBG-11-1!70!black, every mark/.append style={solid,fill=BrBG-11-1},mark=*\\%
 BrBG-11-2!70!black, every mark/.append style={solid,fill=BrBG-11-2},mark=square*\\%
 BrBG-11-3!70!black, every mark/.append style={solid,fill=BrBG-11-3},mark=triangle*\\%
 BrBG-11-4!70!black, every mark/.append style={solid,fill=BrBG-11-4},mark=diamond*\\%
 BrBG-11-5!70!black, every mark/.append style={solid,fill=BrBG-11-5},mark=pentagon*\\%
 BrBG-11-6!70!black, every mark/.append style={solid,fill=BrBG-11-6},mark=x\\%
 BrBG-11-7!70!black, every mark/.append style={solid,fill=BrBG-11-7},mark=+\\%
 BrBG-11-8!70!black, every mark/.append style={solid,fill=BrBG-11-8},mark=star\\%
 BrBG-11-9!70!black, every mark/.append style={solid,fill=BrBG-11-9},mark=oplus*\\%
 BrBG-11-10!70!black, every mark/.append style={solid,fill=BrBG-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-3}{%
 PRGn-3-1!70!black, every mark/.append style={solid,fill=PRGn-3-1},mark=*\\%
 PRGn-3-2!70!black, every mark/.append style={solid,fill=PRGn-3-2},mark=square*\\%
 PRGn-3-3!70!black, every mark/.append style={solid,fill=PRGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-4}{%
 PRGn-4-1!70!black, every mark/.append style={solid,fill=PRGn-4-1},mark=*\\%
 PRGn-4-2!70!black, every mark/.append style={solid,fill=PRGn-4-2},mark=square*\\%
 PRGn-4-3!70!black, every mark/.append style={solid,fill=PRGn-4-3},mark=triangle*\\%
 PRGn-4-4!70!black, every mark/.append style={solid,fill=PRGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-5}{%
 PRGn-5-1!70!black, every mark/.append style={solid,fill=PRGn-5-1},mark=*\\%
 PRGn-5-2!70!black, every mark/.append style={solid,fill=PRGn-5-2},mark=square*\\%
 PRGn-5-3!70!black, every mark/.append style={solid,fill=PRGn-5-3},mark=triangle*\\%
 PRGn-5-4!70!black, every mark/.append style={solid,fill=PRGn-5-4},mark=diamond*\\%
 PRGn-5-5!70!black, every mark/.append style={solid,fill=PRGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-6}{%
 PRGn-6-1!70!black, every mark/.append style={solid,fill=PRGn-6-1},mark=*\\%
 PRGn-6-2!70!black, every mark/.append style={solid,fill=PRGn-6-2},mark=square*\\%
 PRGn-6-3!70!black, every mark/.append style={solid,fill=PRGn-6-3},mark=triangle*\\%
 PRGn-6-4!70!black, every mark/.append style={solid,fill=PRGn-6-4},mark=diamond*\\%
 PRGn-6-5!70!black, every mark/.append style={solid,fill=PRGn-6-5},mark=pentagon*\\%
 PRGn-6-6!70!black, every mark/.append style={solid,fill=PRGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-7}{%
 PRGn-7-1!70!black, every mark/.append style={solid,fill=PRGn-7-1},mark=*\\%
 PRGn-7-2!70!black, every mark/.append style={solid,fill=PRGn-7-2},mark=square*\\%
 PRGn-7-3!70!black, every mark/.append style={solid,fill=PRGn-7-3},mark=triangle*\\%
 PRGn-7-4!70!black, every mark/.append style={solid,fill=PRGn-7-4},mark=diamond*\\%
 PRGn-7-5!70!black, every mark/.append style={solid,fill=PRGn-7-5},mark=pentagon*\\%
 PRGn-7-6!70!black, every mark/.append style={solid,fill=PRGn-7-6},mark=x\\%
 PRGn-7-7!70!black, every mark/.append style={solid,fill=PRGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-8}{%
 PRGn-8-1!70!black, every mark/.append style={solid,fill=PRGn-8-1},mark=*\\%
 PRGn-8-2!70!black, every mark/.append style={solid,fill=PRGn-8-2},mark=square*\\%
 PRGn-8-3!70!black, every mark/.append style={solid,fill=PRGn-8-3},mark=triangle*\\%
 PRGn-8-4!70!black, every mark/.append style={solid,fill=PRGn-8-4},mark=diamond*\\%
 PRGn-8-5!70!black, every mark/.append style={solid,fill=PRGn-8-5},mark=pentagon*\\%
 PRGn-8-6!70!black, every mark/.append style={solid,fill=PRGn-8-6},mark=x\\%
 PRGn-8-7!70!black, every mark/.append style={solid,fill=PRGn-8-7},mark=+\\%
 PRGn-8-8!70!black, every mark/.append style={solid,fill=PRGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-9}{%
 PRGn-9-1!70!black, every mark/.append style={solid,fill=PRGn-9-1},mark=*\\%
 PRGn-9-2!70!black, every mark/.append style={solid,fill=PRGn-9-2},mark=square*\\%
 PRGn-9-3!70!black, every mark/.append style={solid,fill=PRGn-9-3},mark=triangle*\\%
 PRGn-9-4!70!black, every mark/.append style={solid,fill=PRGn-9-4},mark=diamond*\\%
 PRGn-9-5!70!black, every mark/.append style={solid,fill=PRGn-9-5},mark=pentagon*\\%
 PRGn-9-6!70!black, every mark/.append style={solid,fill=PRGn-9-6},mark=x\\%
 PRGn-9-7!70!black, every mark/.append style={solid,fill=PRGn-9-7},mark=+\\%
 PRGn-9-8!70!black, every mark/.append style={solid,fill=PRGn-9-8},mark=star\\%
 PRGn-9-9!70!black, every mark/.append style={solid,fill=PRGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-10}{%
 PRGn-10-1!70!black, every mark/.append style={solid,fill=PRGn-10-1},mark=*\\%
 PRGn-10-2!70!black, every mark/.append style={solid,fill=PRGn-10-2},mark=square*\\%
 PRGn-10-3!70!black, every mark/.append style={solid,fill=PRGn-10-3},mark=triangle*\\%
 PRGn-10-4!70!black, every mark/.append style={solid,fill=PRGn-10-4},mark=diamond*\\%
 PRGn-10-5!70!black, every mark/.append style={solid,fill=PRGn-10-5},mark=pentagon*\\%
 PRGn-10-6!70!black, every mark/.append style={solid,fill=PRGn-10-6},mark=x\\%
 PRGn-10-7!70!black, every mark/.append style={solid,fill=PRGn-10-7},mark=+\\%
 PRGn-10-8!70!black, every mark/.append style={solid,fill=PRGn-10-8},mark=star\\%
 PRGn-10-9!70!black, every mark/.append style={solid,fill=PRGn-10-9},mark=oplus*\\%
 PRGn-10-10!70!black, every mark/.append style={solid,fill=PRGn-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-PRGn-11}{%
 PRGn-11-1!70!black, every mark/.append style={solid,fill=PRGn-11-1},mark=*\\%
 PRGn-11-2!70!black, every mark/.append style={solid,fill=PRGn-11-2},mark=square*\\%
 PRGn-11-3!70!black, every mark/.append style={solid,fill=PRGn-11-3},mark=triangle*\\%
 PRGn-11-4!70!black, every mark/.append style={solid,fill=PRGn-11-4},mark=diamond*\\%
 PRGn-11-5!70!black, every mark/.append style={solid,fill=PRGn-11-5},mark=pentagon*\\%
 PRGn-11-6!70!black, every mark/.append style={solid,fill=PRGn-11-6},mark=x\\%
 PRGn-11-7!70!black, every mark/.append style={solid,fill=PRGn-11-7},mark=+\\%
 PRGn-11-8!70!black, every mark/.append style={solid,fill=PRGn-11-8},mark=star\\%
 PRGn-11-9!70!black, every mark/.append style={solid,fill=PRGn-11-9},mark=oplus*\\%
 PRGn-11-10!70!black, every mark/.append style={solid,fill=PRGn-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-3}{%
 PiYG-3-1!70!black, every mark/.append style={solid,fill=PiYG-3-1},mark=*\\%
 PiYG-3-2!70!black, every mark/.append style={solid,fill=PiYG-3-2},mark=square*\\%
 PiYG-3-3!70!black, every mark/.append style={solid,fill=PiYG-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-4}{%
 PiYG-4-1!70!black, every mark/.append style={solid,fill=PiYG-4-1},mark=*\\%
 PiYG-4-2!70!black, every mark/.append style={solid,fill=PiYG-4-2},mark=square*\\%
 PiYG-4-3!70!black, every mark/.append style={solid,fill=PiYG-4-3},mark=triangle*\\%
 PiYG-4-4!70!black, every mark/.append style={solid,fill=PiYG-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-5}{%
 PiYG-5-1!70!black, every mark/.append style={solid,fill=PiYG-5-1},mark=*\\%
 PiYG-5-2!70!black, every mark/.append style={solid,fill=PiYG-5-2},mark=square*\\%
 PiYG-5-3!70!black, every mark/.append style={solid,fill=PiYG-5-3},mark=triangle*\\%
 PiYG-5-4!70!black, every mark/.append style={solid,fill=PiYG-5-4},mark=diamond*\\%
 PiYG-5-5!70!black, every mark/.append style={solid,fill=PiYG-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-6}{%
 PiYG-6-1!70!black, every mark/.append style={solid,fill=PiYG-6-1},mark=*\\%
 PiYG-6-2!70!black, every mark/.append style={solid,fill=PiYG-6-2},mark=square*\\%
 PiYG-6-3!70!black, every mark/.append style={solid,fill=PiYG-6-3},mark=triangle*\\%
 PiYG-6-4!70!black, every mark/.append style={solid,fill=PiYG-6-4},mark=diamond*\\%
 PiYG-6-5!70!black, every mark/.append style={solid,fill=PiYG-6-5},mark=pentagon*\\%
 PiYG-6-6!70!black, every mark/.append style={solid,fill=PiYG-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-7}{%
 PiYG-7-1!70!black, every mark/.append style={solid,fill=PiYG-7-1},mark=*\\%
 PiYG-7-2!70!black, every mark/.append style={solid,fill=PiYG-7-2},mark=square*\\%
 PiYG-7-3!70!black, every mark/.append style={solid,fill=PiYG-7-3},mark=triangle*\\%
 PiYG-7-4!70!black, every mark/.append style={solid,fill=PiYG-7-4},mark=diamond*\\%
 PiYG-7-5!70!black, every mark/.append style={solid,fill=PiYG-7-5},mark=pentagon*\\%
 PiYG-7-6!70!black, every mark/.append style={solid,fill=PiYG-7-6},mark=x\\%
 PiYG-7-7!70!black, every mark/.append style={solid,fill=PiYG-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-8}{%
 PiYG-8-1!70!black, every mark/.append style={solid,fill=PiYG-8-1},mark=*\\%
 PiYG-8-2!70!black, every mark/.append style={solid,fill=PiYG-8-2},mark=square*\\%
 PiYG-8-3!70!black, every mark/.append style={solid,fill=PiYG-8-3},mark=triangle*\\%
 PiYG-8-4!70!black, every mark/.append style={solid,fill=PiYG-8-4},mark=diamond*\\%
 PiYG-8-5!70!black, every mark/.append style={solid,fill=PiYG-8-5},mark=pentagon*\\%
 PiYG-8-6!70!black, every mark/.append style={solid,fill=PiYG-8-6},mark=x\\%
 PiYG-8-7!70!black, every mark/.append style={solid,fill=PiYG-8-7},mark=+\\%
 PiYG-8-8!70!black, every mark/.append style={solid,fill=PiYG-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-9}{%
 PiYG-9-1!70!black, every mark/.append style={solid,fill=PiYG-9-1},mark=*\\%
 PiYG-9-2!70!black, every mark/.append style={solid,fill=PiYG-9-2},mark=square*\\%
 PiYG-9-3!70!black, every mark/.append style={solid,fill=PiYG-9-3},mark=triangle*\\%
 PiYG-9-4!70!black, every mark/.append style={solid,fill=PiYG-9-4},mark=diamond*\\%
 PiYG-9-5!70!black, every mark/.append style={solid,fill=PiYG-9-5},mark=pentagon*\\%
 PiYG-9-6!70!black, every mark/.append style={solid,fill=PiYG-9-6},mark=x\\%
 PiYG-9-7!70!black, every mark/.append style={solid,fill=PiYG-9-7},mark=+\\%
 PiYG-9-8!70!black, every mark/.append style={solid,fill=PiYG-9-8},mark=star\\%
 PiYG-9-9!70!black, every mark/.append style={solid,fill=PiYG-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-10}{%
 PiYG-10-1!70!black, every mark/.append style={solid,fill=PiYG-10-1},mark=*\\%
 PiYG-10-2!70!black, every mark/.append style={solid,fill=PiYG-10-2},mark=square*\\%
 PiYG-10-3!70!black, every mark/.append style={solid,fill=PiYG-10-3},mark=triangle*\\%
 PiYG-10-4!70!black, every mark/.append style={solid,fill=PiYG-10-4},mark=diamond*\\%
 PiYG-10-5!70!black, every mark/.append style={solid,fill=PiYG-10-5},mark=pentagon*\\%
 PiYG-10-6!70!black, every mark/.append style={solid,fill=PiYG-10-6},mark=x\\%
 PiYG-10-7!70!black, every mark/.append style={solid,fill=PiYG-10-7},mark=+\\%
 PiYG-10-8!70!black, every mark/.append style={solid,fill=PiYG-10-8},mark=star\\%
 PiYG-10-9!70!black, every mark/.append style={solid,fill=PiYG-10-9},mark=oplus*\\%
 PiYG-10-10!70!black, every mark/.append style={solid,fill=PiYG-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-PiYG-11}{%
 PiYG-11-1!70!black, every mark/.append style={solid,fill=PiYG-11-1},mark=*\\%
 PiYG-11-2!70!black, every mark/.append style={solid,fill=PiYG-11-2},mark=square*\\%
 PiYG-11-3!70!black, every mark/.append style={solid,fill=PiYG-11-3},mark=triangle*\\%
 PiYG-11-4!70!black, every mark/.append style={solid,fill=PiYG-11-4},mark=diamond*\\%
 PiYG-11-5!70!black, every mark/.append style={solid,fill=PiYG-11-5},mark=pentagon*\\%
 PiYG-11-6!70!black, every mark/.append style={solid,fill=PiYG-11-6},mark=x\\%
 PiYG-11-7!70!black, every mark/.append style={solid,fill=PiYG-11-7},mark=+\\%
 PiYG-11-8!70!black, every mark/.append style={solid,fill=PiYG-11-8},mark=star\\%
 PiYG-11-9!70!black, every mark/.append style={solid,fill=PiYG-11-9},mark=oplus*\\%
 PiYG-11-10!70!black, every mark/.append style={solid,fill=PiYG-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-3}{%
 RdBu-3-1!70!black, every mark/.append style={solid,fill=RdBu-3-1},mark=*\\%
 RdBu-3-2!70!black, every mark/.append style={solid,fill=RdBu-3-2},mark=square*\\%
 RdBu-3-3!70!black, every mark/.append style={solid,fill=RdBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-4}{%
 RdBu-4-1!70!black, every mark/.append style={solid,fill=RdBu-4-1},mark=*\\%
 RdBu-4-2!70!black, every mark/.append style={solid,fill=RdBu-4-2},mark=square*\\%
 RdBu-4-3!70!black, every mark/.append style={solid,fill=RdBu-4-3},mark=triangle*\\%
 RdBu-4-4!70!black, every mark/.append style={solid,fill=RdBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-5}{%
 RdBu-5-1!70!black, every mark/.append style={solid,fill=RdBu-5-1},mark=*\\%
 RdBu-5-2!70!black, every mark/.append style={solid,fill=RdBu-5-2},mark=square*\\%
 RdBu-5-3!70!black, every mark/.append style={solid,fill=RdBu-5-3},mark=triangle*\\%
 RdBu-5-4!70!black, every mark/.append style={solid,fill=RdBu-5-4},mark=diamond*\\%
 RdBu-5-5!70!black, every mark/.append style={solid,fill=RdBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-6}{%
 RdBu-6-1!70!black, every mark/.append style={solid,fill=RdBu-6-1},mark=*\\%
 RdBu-6-2!70!black, every mark/.append style={solid,fill=RdBu-6-2},mark=square*\\%
 RdBu-6-3!70!black, every mark/.append style={solid,fill=RdBu-6-3},mark=triangle*\\%
 RdBu-6-4!70!black, every mark/.append style={solid,fill=RdBu-6-4},mark=diamond*\\%
 RdBu-6-5!70!black, every mark/.append style={solid,fill=RdBu-6-5},mark=pentagon*\\%
 RdBu-6-6!70!black, every mark/.append style={solid,fill=RdBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-7}{%
 RdBu-7-1!70!black, every mark/.append style={solid,fill=RdBu-7-1},mark=*\\%
 RdBu-7-2!70!black, every mark/.append style={solid,fill=RdBu-7-2},mark=square*\\%
 RdBu-7-3!70!black, every mark/.append style={solid,fill=RdBu-7-3},mark=triangle*\\%
 RdBu-7-4!70!black, every mark/.append style={solid,fill=RdBu-7-4},mark=diamond*\\%
 RdBu-7-5!70!black, every mark/.append style={solid,fill=RdBu-7-5},mark=pentagon*\\%
 RdBu-7-6!70!black, every mark/.append style={solid,fill=RdBu-7-6},mark=x\\%
 RdBu-7-7!70!black, every mark/.append style={solid,fill=RdBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-8}{%
 RdBu-8-1!70!black, every mark/.append style={solid,fill=RdBu-8-1},mark=*\\%
 RdBu-8-2!70!black, every mark/.append style={solid,fill=RdBu-8-2},mark=square*\\%
 RdBu-8-3!70!black, every mark/.append style={solid,fill=RdBu-8-3},mark=triangle*\\%
 RdBu-8-4!70!black, every mark/.append style={solid,fill=RdBu-8-4},mark=diamond*\\%
 RdBu-8-5!70!black, every mark/.append style={solid,fill=RdBu-8-5},mark=pentagon*\\%
 RdBu-8-6!70!black, every mark/.append style={solid,fill=RdBu-8-6},mark=x\\%
 RdBu-8-7!70!black, every mark/.append style={solid,fill=RdBu-8-7},mark=+\\%
 RdBu-8-8!70!black, every mark/.append style={solid,fill=RdBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-9}{%
 RdBu-9-1!70!black, every mark/.append style={solid,fill=RdBu-9-1},mark=*\\%
 RdBu-9-2!70!black, every mark/.append style={solid,fill=RdBu-9-2},mark=square*\\%
 RdBu-9-3!70!black, every mark/.append style={solid,fill=RdBu-9-3},mark=triangle*\\%
 RdBu-9-4!70!black, every mark/.append style={solid,fill=RdBu-9-4},mark=diamond*\\%
 RdBu-9-5!70!black, every mark/.append style={solid,fill=RdBu-9-5},mark=pentagon*\\%
 RdBu-9-6!70!black, every mark/.append style={solid,fill=RdBu-9-6},mark=x\\%
 RdBu-9-7!70!black, every mark/.append style={solid,fill=RdBu-9-7},mark=+\\%
 RdBu-9-8!70!black, every mark/.append style={solid,fill=RdBu-9-8},mark=star\\%
 RdBu-9-9!70!black, every mark/.append style={solid,fill=RdBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-10}{%
 RdBu-10-1!70!black, every mark/.append style={solid,fill=RdBu-10-1},mark=*\\%
 RdBu-10-2!70!black, every mark/.append style={solid,fill=RdBu-10-2},mark=square*\\%
 RdBu-10-3!70!black, every mark/.append style={solid,fill=RdBu-10-3},mark=triangle*\\%
 RdBu-10-4!70!black, every mark/.append style={solid,fill=RdBu-10-4},mark=diamond*\\%
 RdBu-10-5!70!black, every mark/.append style={solid,fill=RdBu-10-5},mark=pentagon*\\%
 RdBu-10-6!70!black, every mark/.append style={solid,fill=RdBu-10-6},mark=x\\%
 RdBu-10-7!70!black, every mark/.append style={solid,fill=RdBu-10-7},mark=+\\%
 RdBu-10-8!70!black, every mark/.append style={solid,fill=RdBu-10-8},mark=star\\%
 RdBu-10-9!70!black, every mark/.append style={solid,fill=RdBu-10-9},mark=oplus*\\%
 RdBu-10-10!70!black, every mark/.append style={solid,fill=RdBu-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdBu-11}{%
 RdBu-11-1!70!black, every mark/.append style={solid,fill=RdBu-11-1},mark=*\\%
 RdBu-11-2!70!black, every mark/.append style={solid,fill=RdBu-11-2},mark=square*\\%
 RdBu-11-3!70!black, every mark/.append style={solid,fill=RdBu-11-3},mark=triangle*\\%
 RdBu-11-4!70!black, every mark/.append style={solid,fill=RdBu-11-4},mark=diamond*\\%
 RdBu-11-5!70!black, every mark/.append style={solid,fill=RdBu-11-5},mark=pentagon*\\%
 RdBu-11-6!70!black, every mark/.append style={solid,fill=RdBu-11-6},mark=x\\%
 RdBu-11-7!70!black, every mark/.append style={solid,fill=RdBu-11-7},mark=+\\%
 RdBu-11-8!70!black, every mark/.append style={solid,fill=RdBu-11-8},mark=star\\%
 RdBu-11-9!70!black, every mark/.append style={solid,fill=RdBu-11-9},mark=oplus*\\%
 RdBu-11-10!70!black, every mark/.append style={solid,fill=RdBu-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-3}{%
 RdGy-3-1!70!black, every mark/.append style={solid,fill=RdGy-3-1},mark=*\\%
 RdGy-3-2!70!black, every mark/.append style={solid,fill=RdGy-3-2},mark=square*\\%
 RdGy-3-3!70!black, every mark/.append style={solid,fill=RdGy-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-4}{%
 RdGy-4-1!70!black, every mark/.append style={solid,fill=RdGy-4-1},mark=*\\%
 RdGy-4-2!70!black, every mark/.append style={solid,fill=RdGy-4-2},mark=square*\\%
 RdGy-4-3!70!black, every mark/.append style={solid,fill=RdGy-4-3},mark=triangle*\\%
 RdGy-4-4!70!black, every mark/.append style={solid,fill=RdGy-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-5}{%
 RdGy-5-1!70!black, every mark/.append style={solid,fill=RdGy-5-1},mark=*\\%
 RdGy-5-2!70!black, every mark/.append style={solid,fill=RdGy-5-2},mark=square*\\%
 RdGy-5-3!70!black, every mark/.append style={solid,fill=RdGy-5-3},mark=triangle*\\%
 RdGy-5-4!70!black, every mark/.append style={solid,fill=RdGy-5-4},mark=diamond*\\%
 RdGy-5-5!70!black, every mark/.append style={solid,fill=RdGy-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-6}{%
 RdGy-6-1!70!black, every mark/.append style={solid,fill=RdGy-6-1},mark=*\\%
 RdGy-6-2!70!black, every mark/.append style={solid,fill=RdGy-6-2},mark=square*\\%
 RdGy-6-3!70!black, every mark/.append style={solid,fill=RdGy-6-3},mark=triangle*\\%
 RdGy-6-4!70!black, every mark/.append style={solid,fill=RdGy-6-4},mark=diamond*\\%
 RdGy-6-5!70!black, every mark/.append style={solid,fill=RdGy-6-5},mark=pentagon*\\%
 RdGy-6-6!70!black, every mark/.append style={solid,fill=RdGy-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-7}{%
 RdGy-7-1!70!black, every mark/.append style={solid,fill=RdGy-7-1},mark=*\\%
 RdGy-7-2!70!black, every mark/.append style={solid,fill=RdGy-7-2},mark=square*\\%
 RdGy-7-3!70!black, every mark/.append style={solid,fill=RdGy-7-3},mark=triangle*\\%
 RdGy-7-4!70!black, every mark/.append style={solid,fill=RdGy-7-4},mark=diamond*\\%
 RdGy-7-5!70!black, every mark/.append style={solid,fill=RdGy-7-5},mark=pentagon*\\%
 RdGy-7-6!70!black, every mark/.append style={solid,fill=RdGy-7-6},mark=x\\%
 RdGy-7-7!70!black, every mark/.append style={solid,fill=RdGy-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-8}{%
 RdGy-8-1!70!black, every mark/.append style={solid,fill=RdGy-8-1},mark=*\\%
 RdGy-8-2!70!black, every mark/.append style={solid,fill=RdGy-8-2},mark=square*\\%
 RdGy-8-3!70!black, every mark/.append style={solid,fill=RdGy-8-3},mark=triangle*\\%
 RdGy-8-4!70!black, every mark/.append style={solid,fill=RdGy-8-4},mark=diamond*\\%
 RdGy-8-5!70!black, every mark/.append style={solid,fill=RdGy-8-5},mark=pentagon*\\%
 RdGy-8-6!70!black, every mark/.append style={solid,fill=RdGy-8-6},mark=x\\%
 RdGy-8-7!70!black, every mark/.append style={solid,fill=RdGy-8-7},mark=+\\%
 RdGy-8-8!70!black, every mark/.append style={solid,fill=RdGy-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-9}{%
 RdGy-9-1!70!black, every mark/.append style={solid,fill=RdGy-9-1},mark=*\\%
 RdGy-9-2!70!black, every mark/.append style={solid,fill=RdGy-9-2},mark=square*\\%
 RdGy-9-3!70!black, every mark/.append style={solid,fill=RdGy-9-3},mark=triangle*\\%
 RdGy-9-4!70!black, every mark/.append style={solid,fill=RdGy-9-4},mark=diamond*\\%
 RdGy-9-5!70!black, every mark/.append style={solid,fill=RdGy-9-5},mark=pentagon*\\%
 RdGy-9-6!70!black, every mark/.append style={solid,fill=RdGy-9-6},mark=x\\%
 RdGy-9-7!70!black, every mark/.append style={solid,fill=RdGy-9-7},mark=+\\%
 RdGy-9-8!70!black, every mark/.append style={solid,fill=RdGy-9-8},mark=star\\%
 RdGy-9-9!70!black, every mark/.append style={solid,fill=RdGy-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-10}{%
 RdGy-10-1!70!black, every mark/.append style={solid,fill=RdGy-10-1},mark=*\\%
 RdGy-10-2!70!black, every mark/.append style={solid,fill=RdGy-10-2},mark=square*\\%
 RdGy-10-3!70!black, every mark/.append style={solid,fill=RdGy-10-3},mark=triangle*\\%
 RdGy-10-4!70!black, every mark/.append style={solid,fill=RdGy-10-4},mark=diamond*\\%
 RdGy-10-5!70!black, every mark/.append style={solid,fill=RdGy-10-5},mark=pentagon*\\%
 RdGy-10-6!70!black, every mark/.append style={solid,fill=RdGy-10-6},mark=x\\%
 RdGy-10-7!70!black, every mark/.append style={solid,fill=RdGy-10-7},mark=+\\%
 RdGy-10-8!70!black, every mark/.append style={solid,fill=RdGy-10-8},mark=star\\%
 RdGy-10-9!70!black, every mark/.append style={solid,fill=RdGy-10-9},mark=oplus*\\%
 RdGy-10-10!70!black, every mark/.append style={solid,fill=RdGy-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdGy-11}{%
 RdGy-11-1!70!black, every mark/.append style={solid,fill=RdGy-11-1},mark=*\\%
 RdGy-11-2!70!black, every mark/.append style={solid,fill=RdGy-11-2},mark=square*\\%
 RdGy-11-3!70!black, every mark/.append style={solid,fill=RdGy-11-3},mark=triangle*\\%
 RdGy-11-4!70!black, every mark/.append style={solid,fill=RdGy-11-4},mark=diamond*\\%
 RdGy-11-5!70!black, every mark/.append style={solid,fill=RdGy-11-5},mark=pentagon*\\%
 RdGy-11-6!70!black, every mark/.append style={solid,fill=RdGy-11-6},mark=x\\%
 RdGy-11-7!70!black, every mark/.append style={solid,fill=RdGy-11-7},mark=+\\%
 RdGy-11-8!70!black, every mark/.append style={solid,fill=RdGy-11-8},mark=star\\%
 RdGy-11-9!70!black, every mark/.append style={solid,fill=RdGy-11-9},mark=oplus*\\%
 RdGy-11-10!70!black, every mark/.append style={solid,fill=RdGy-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-3}{%
 RdYlBu-3-1!70!black, every mark/.append style={solid,fill=RdYlBu-3-1},mark=*\\%
 RdYlBu-3-2!70!black, every mark/.append style={solid,fill=RdYlBu-3-2},mark=square*\\%
 RdYlBu-3-3!70!black, every mark/.append style={solid,fill=RdYlBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-4}{%
 RdYlBu-4-1!70!black, every mark/.append style={solid,fill=RdYlBu-4-1},mark=*\\%
 RdYlBu-4-2!70!black, every mark/.append style={solid,fill=RdYlBu-4-2},mark=square*\\%
 RdYlBu-4-3!70!black, every mark/.append style={solid,fill=RdYlBu-4-3},mark=triangle*\\%
 RdYlBu-4-4!70!black, every mark/.append style={solid,fill=RdYlBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-5}{%
 RdYlBu-5-1!70!black, every mark/.append style={solid,fill=RdYlBu-5-1},mark=*\\%
 RdYlBu-5-2!70!black, every mark/.append style={solid,fill=RdYlBu-5-2},mark=square*\\%
 RdYlBu-5-3!70!black, every mark/.append style={solid,fill=RdYlBu-5-3},mark=triangle*\\%
 RdYlBu-5-4!70!black, every mark/.append style={solid,fill=RdYlBu-5-4},mark=diamond*\\%
 RdYlBu-5-5!70!black, every mark/.append style={solid,fill=RdYlBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-6}{%
 RdYlBu-6-1!70!black, every mark/.append style={solid,fill=RdYlBu-6-1},mark=*\\%
 RdYlBu-6-2!70!black, every mark/.append style={solid,fill=RdYlBu-6-2},mark=square*\\%
 RdYlBu-6-3!70!black, every mark/.append style={solid,fill=RdYlBu-6-3},mark=triangle*\\%
 RdYlBu-6-4!70!black, every mark/.append style={solid,fill=RdYlBu-6-4},mark=diamond*\\%
 RdYlBu-6-5!70!black, every mark/.append style={solid,fill=RdYlBu-6-5},mark=pentagon*\\%
 RdYlBu-6-6!70!black, every mark/.append style={solid,fill=RdYlBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-7}{%
 RdYlBu-7-1!70!black, every mark/.append style={solid,fill=RdYlBu-7-1},mark=*\\%
 RdYlBu-7-2!70!black, every mark/.append style={solid,fill=RdYlBu-7-2},mark=square*\\%
 RdYlBu-7-3!70!black, every mark/.append style={solid,fill=RdYlBu-7-3},mark=triangle*\\%
 RdYlBu-7-4!70!black, every mark/.append style={solid,fill=RdYlBu-7-4},mark=diamond*\\%
 RdYlBu-7-5!70!black, every mark/.append style={solid,fill=RdYlBu-7-5},mark=pentagon*\\%
 RdYlBu-7-6!70!black, every mark/.append style={solid,fill=RdYlBu-7-6},mark=x\\%
 RdYlBu-7-7!70!black, every mark/.append style={solid,fill=RdYlBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-8}{%
 RdYlBu-8-1!70!black, every mark/.append style={solid,fill=RdYlBu-8-1},mark=*\\%
 RdYlBu-8-2!70!black, every mark/.append style={solid,fill=RdYlBu-8-2},mark=square*\\%
 RdYlBu-8-3!70!black, every mark/.append style={solid,fill=RdYlBu-8-3},mark=triangle*\\%
 RdYlBu-8-4!70!black, every mark/.append style={solid,fill=RdYlBu-8-4},mark=diamond*\\%
 RdYlBu-8-5!70!black, every mark/.append style={solid,fill=RdYlBu-8-5},mark=pentagon*\\%
 RdYlBu-8-6!70!black, every mark/.append style={solid,fill=RdYlBu-8-6},mark=x\\%
 RdYlBu-8-7!70!black, every mark/.append style={solid,fill=RdYlBu-8-7},mark=+\\%
 RdYlBu-8-8!70!black, every mark/.append style={solid,fill=RdYlBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-9}{%
 RdYlBu-9-1!70!black, every mark/.append style={solid,fill=RdYlBu-9-1},mark=*\\%
 RdYlBu-9-2!70!black, every mark/.append style={solid,fill=RdYlBu-9-2},mark=square*\\%
 RdYlBu-9-3!70!black, every mark/.append style={solid,fill=RdYlBu-9-3},mark=triangle*\\%
 RdYlBu-9-4!70!black, every mark/.append style={solid,fill=RdYlBu-9-4},mark=diamond*\\%
 RdYlBu-9-5!70!black, every mark/.append style={solid,fill=RdYlBu-9-5},mark=pentagon*\\%
 RdYlBu-9-6!70!black, every mark/.append style={solid,fill=RdYlBu-9-6},mark=x\\%
 RdYlBu-9-7!70!black, every mark/.append style={solid,fill=RdYlBu-9-7},mark=+\\%
 RdYlBu-9-8!70!black, every mark/.append style={solid,fill=RdYlBu-9-8},mark=star\\%
 RdYlBu-9-9!70!black, every mark/.append style={solid,fill=RdYlBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-10}{%
 RdYlBu-10-1!70!black, every mark/.append style={solid,fill=RdYlBu-10-1},mark=*\\%
 RdYlBu-10-2!70!black, every mark/.append style={solid,fill=RdYlBu-10-2},mark=square*\\%
 RdYlBu-10-3!70!black, every mark/.append style={solid,fill=RdYlBu-10-3},mark=triangle*\\%
 RdYlBu-10-4!70!black, every mark/.append style={solid,fill=RdYlBu-10-4},mark=diamond*\\%
 RdYlBu-10-5!70!black, every mark/.append style={solid,fill=RdYlBu-10-5},mark=pentagon*\\%
 RdYlBu-10-6!70!black, every mark/.append style={solid,fill=RdYlBu-10-6},mark=x\\%
 RdYlBu-10-7!70!black, every mark/.append style={solid,fill=RdYlBu-10-7},mark=+\\%
 RdYlBu-10-8!70!black, every mark/.append style={solid,fill=RdYlBu-10-8},mark=star\\%
 RdYlBu-10-9!70!black, every mark/.append style={solid,fill=RdYlBu-10-9},mark=oplus*\\%
 RdYlBu-10-10!70!black, every mark/.append style={solid,fill=RdYlBu-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlBu-11}{%
 RdYlBu-11-1!70!black, every mark/.append style={solid,fill=RdYlBu-11-1},mark=*\\%
 RdYlBu-11-2!70!black, every mark/.append style={solid,fill=RdYlBu-11-2},mark=square*\\%
 RdYlBu-11-3!70!black, every mark/.append style={solid,fill=RdYlBu-11-3},mark=triangle*\\%
 RdYlBu-11-4!70!black, every mark/.append style={solid,fill=RdYlBu-11-4},mark=diamond*\\%
 RdYlBu-11-5!70!black, every mark/.append style={solid,fill=RdYlBu-11-5},mark=pentagon*\\%
 RdYlBu-11-6!70!black, every mark/.append style={solid,fill=RdYlBu-11-6},mark=x\\%
 RdYlBu-11-7!70!black, every mark/.append style={solid,fill=RdYlBu-11-7},mark=+\\%
 RdYlBu-11-8!70!black, every mark/.append style={solid,fill=RdYlBu-11-8},mark=star\\%
 RdYlBu-11-9!70!black, every mark/.append style={solid,fill=RdYlBu-11-9},mark=oplus*\\%
 RdYlBu-11-10!70!black, every mark/.append style={solid,fill=RdYlBu-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-3}{%
 Spectral-3-1!70!black, every mark/.append style={solid,fill=Spectral-3-1},mark=*\\%
 Spectral-3-2!70!black, every mark/.append style={solid,fill=Spectral-3-2},mark=square*\\%
 Spectral-3-3!70!black, every mark/.append style={solid,fill=Spectral-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-4}{%
 Spectral-4-1!70!black, every mark/.append style={solid,fill=Spectral-4-1},mark=*\\%
 Spectral-4-2!70!black, every mark/.append style={solid,fill=Spectral-4-2},mark=square*\\%
 Spectral-4-3!70!black, every mark/.append style={solid,fill=Spectral-4-3},mark=triangle*\\%
 Spectral-4-4!70!black, every mark/.append style={solid,fill=Spectral-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-5}{%
 Spectral-5-1!70!black, every mark/.append style={solid,fill=Spectral-5-1},mark=*\\%
 Spectral-5-2!70!black, every mark/.append style={solid,fill=Spectral-5-2},mark=square*\\%
 Spectral-5-3!70!black, every mark/.append style={solid,fill=Spectral-5-3},mark=triangle*\\%
 Spectral-5-4!70!black, every mark/.append style={solid,fill=Spectral-5-4},mark=diamond*\\%
 Spectral-5-5!70!black, every mark/.append style={solid,fill=Spectral-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-6}{%
 Spectral-6-1!70!black, every mark/.append style={solid,fill=Spectral-6-1},mark=*\\%
 Spectral-6-2!70!black, every mark/.append style={solid,fill=Spectral-6-2},mark=square*\\%
 Spectral-6-3!70!black, every mark/.append style={solid,fill=Spectral-6-3},mark=triangle*\\%
 Spectral-6-4!70!black, every mark/.append style={solid,fill=Spectral-6-4},mark=diamond*\\%
 Spectral-6-5!70!black, every mark/.append style={solid,fill=Spectral-6-5},mark=pentagon*\\%
 Spectral-6-6!70!black, every mark/.append style={solid,fill=Spectral-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-7}{%
 Spectral-7-1!70!black, every mark/.append style={solid,fill=Spectral-7-1},mark=*\\%
 Spectral-7-2!70!black, every mark/.append style={solid,fill=Spectral-7-2},mark=square*\\%
 Spectral-7-3!70!black, every mark/.append style={solid,fill=Spectral-7-3},mark=triangle*\\%
 Spectral-7-4!70!black, every mark/.append style={solid,fill=Spectral-7-4},mark=diamond*\\%
 Spectral-7-5!70!black, every mark/.append style={solid,fill=Spectral-7-5},mark=pentagon*\\%
 Spectral-7-6!70!black, every mark/.append style={solid,fill=Spectral-7-6},mark=x\\%
 Spectral-7-7!70!black, every mark/.append style={solid,fill=Spectral-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-8}{%
 Spectral-8-1!70!black, every mark/.append style={solid,fill=Spectral-8-1},mark=*\\%
 Spectral-8-2!70!black, every mark/.append style={solid,fill=Spectral-8-2},mark=square*\\%
 Spectral-8-3!70!black, every mark/.append style={solid,fill=Spectral-8-3},mark=triangle*\\%
 Spectral-8-4!70!black, every mark/.append style={solid,fill=Spectral-8-4},mark=diamond*\\%
 Spectral-8-5!70!black, every mark/.append style={solid,fill=Spectral-8-5},mark=pentagon*\\%
 Spectral-8-6!70!black, every mark/.append style={solid,fill=Spectral-8-6},mark=x\\%
 Spectral-8-7!70!black, every mark/.append style={solid,fill=Spectral-8-7},mark=+\\%
 Spectral-8-8!70!black, every mark/.append style={solid,fill=Spectral-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-9}{%
 Spectral-9-1!70!black, every mark/.append style={solid,fill=Spectral-9-1},mark=*\\%
 Spectral-9-2!70!black, every mark/.append style={solid,fill=Spectral-9-2},mark=square*\\%
 Spectral-9-3!70!black, every mark/.append style={solid,fill=Spectral-9-3},mark=triangle*\\%
 Spectral-9-4!70!black, every mark/.append style={solid,fill=Spectral-9-4},mark=diamond*\\%
 Spectral-9-5!70!black, every mark/.append style={solid,fill=Spectral-9-5},mark=pentagon*\\%
 Spectral-9-6!70!black, every mark/.append style={solid,fill=Spectral-9-6},mark=x\\%
 Spectral-9-7!70!black, every mark/.append style={solid,fill=Spectral-9-7},mark=+\\%
 Spectral-9-8!70!black, every mark/.append style={solid,fill=Spectral-9-8},mark=star\\%
 Spectral-9-9!70!black, every mark/.append style={solid,fill=Spectral-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-10}{%
 Spectral-10-1!70!black, every mark/.append style={solid,fill=Spectral-10-1},mark=*\\%
 Spectral-10-2!70!black, every mark/.append style={solid,fill=Spectral-10-2},mark=square*\\%
 Spectral-10-3!70!black, every mark/.append style={solid,fill=Spectral-10-3},mark=triangle*\\%
 Spectral-10-4!70!black, every mark/.append style={solid,fill=Spectral-10-4},mark=diamond*\\%
 Spectral-10-5!70!black, every mark/.append style={solid,fill=Spectral-10-5},mark=pentagon*\\%
 Spectral-10-6!70!black, every mark/.append style={solid,fill=Spectral-10-6},mark=x\\%
 Spectral-10-7!70!black, every mark/.append style={solid,fill=Spectral-10-7},mark=+\\%
 Spectral-10-8!70!black, every mark/.append style={solid,fill=Spectral-10-8},mark=star\\%
 Spectral-10-9!70!black, every mark/.append style={solid,fill=Spectral-10-9},mark=oplus*\\%
 Spectral-10-10!70!black, every mark/.append style={solid,fill=Spectral-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Spectral-11}{%
 Spectral-11-1!70!black, every mark/.append style={solid,fill=Spectral-11-1},mark=*\\%
 Spectral-11-2!70!black, every mark/.append style={solid,fill=Spectral-11-2},mark=square*\\%
 Spectral-11-3!70!black, every mark/.append style={solid,fill=Spectral-11-3},mark=triangle*\\%
 Spectral-11-4!70!black, every mark/.append style={solid,fill=Spectral-11-4},mark=diamond*\\%
 Spectral-11-5!70!black, every mark/.append style={solid,fill=Spectral-11-5},mark=pentagon*\\%
 Spectral-11-6!70!black, every mark/.append style={solid,fill=Spectral-11-6},mark=x\\%
 Spectral-11-7!70!black, every mark/.append style={solid,fill=Spectral-11-7},mark=+\\%
 Spectral-11-8!70!black, every mark/.append style={solid,fill=Spectral-11-8},mark=star\\%
 Spectral-11-9!70!black, every mark/.append style={solid,fill=Spectral-11-9},mark=oplus*\\%
 Spectral-11-10!70!black, every mark/.append style={solid,fill=Spectral-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-3}{%
 RdYlGn-3-1!70!black, every mark/.append style={solid,fill=RdYlGn-3-1},mark=*\\%
 RdYlGn-3-2!70!black, every mark/.append style={solid,fill=RdYlGn-3-2},mark=square*\\%
 RdYlGn-3-3!70!black, every mark/.append style={solid,fill=RdYlGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-4}{%
 RdYlGn-4-1!70!black, every mark/.append style={solid,fill=RdYlGn-4-1},mark=*\\%
 RdYlGn-4-2!70!black, every mark/.append style={solid,fill=RdYlGn-4-2},mark=square*\\%
 RdYlGn-4-3!70!black, every mark/.append style={solid,fill=RdYlGn-4-3},mark=triangle*\\%
 RdYlGn-4-4!70!black, every mark/.append style={solid,fill=RdYlGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-5}{%
 RdYlGn-5-1!70!black, every mark/.append style={solid,fill=RdYlGn-5-1},mark=*\\%
 RdYlGn-5-2!70!black, every mark/.append style={solid,fill=RdYlGn-5-2},mark=square*\\%
 RdYlGn-5-3!70!black, every mark/.append style={solid,fill=RdYlGn-5-3},mark=triangle*\\%
 RdYlGn-5-4!70!black, every mark/.append style={solid,fill=RdYlGn-5-4},mark=diamond*\\%
 RdYlGn-5-5!70!black, every mark/.append style={solid,fill=RdYlGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-6}{%
 RdYlGn-6-1!70!black, every mark/.append style={solid,fill=RdYlGn-6-1},mark=*\\%
 RdYlGn-6-2!70!black, every mark/.append style={solid,fill=RdYlGn-6-2},mark=square*\\%
 RdYlGn-6-3!70!black, every mark/.append style={solid,fill=RdYlGn-6-3},mark=triangle*\\%
 RdYlGn-6-4!70!black, every mark/.append style={solid,fill=RdYlGn-6-4},mark=diamond*\\%
 RdYlGn-6-5!70!black, every mark/.append style={solid,fill=RdYlGn-6-5},mark=pentagon*\\%
 RdYlGn-6-6!70!black, every mark/.append style={solid,fill=RdYlGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-7}{%
 RdYlGn-7-1!70!black, every mark/.append style={solid,fill=RdYlGn-7-1},mark=*\\%
 RdYlGn-7-2!70!black, every mark/.append style={solid,fill=RdYlGn-7-2},mark=square*\\%
 RdYlGn-7-3!70!black, every mark/.append style={solid,fill=RdYlGn-7-3},mark=triangle*\\%
 RdYlGn-7-4!70!black, every mark/.append style={solid,fill=RdYlGn-7-4},mark=diamond*\\%
 RdYlGn-7-5!70!black, every mark/.append style={solid,fill=RdYlGn-7-5},mark=pentagon*\\%
 RdYlGn-7-6!70!black, every mark/.append style={solid,fill=RdYlGn-7-6},mark=x\\%
 RdYlGn-7-7!70!black, every mark/.append style={solid,fill=RdYlGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-8}{%
 RdYlGn-8-1!70!black, every mark/.append style={solid,fill=RdYlGn-8-1},mark=*\\%
 RdYlGn-8-2!70!black, every mark/.append style={solid,fill=RdYlGn-8-2},mark=square*\\%
 RdYlGn-8-3!70!black, every mark/.append style={solid,fill=RdYlGn-8-3},mark=triangle*\\%
 RdYlGn-8-4!70!black, every mark/.append style={solid,fill=RdYlGn-8-4},mark=diamond*\\%
 RdYlGn-8-5!70!black, every mark/.append style={solid,fill=RdYlGn-8-5},mark=pentagon*\\%
 RdYlGn-8-6!70!black, every mark/.append style={solid,fill=RdYlGn-8-6},mark=x\\%
 RdYlGn-8-7!70!black, every mark/.append style={solid,fill=RdYlGn-8-7},mark=+\\%
 RdYlGn-8-8!70!black, every mark/.append style={solid,fill=RdYlGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-9}{%
 RdYlGn-9-1!70!black, every mark/.append style={solid,fill=RdYlGn-9-1},mark=*\\%
 RdYlGn-9-2!70!black, every mark/.append style={solid,fill=RdYlGn-9-2},mark=square*\\%
 RdYlGn-9-3!70!black, every mark/.append style={solid,fill=RdYlGn-9-3},mark=triangle*\\%
 RdYlGn-9-4!70!black, every mark/.append style={solid,fill=RdYlGn-9-4},mark=diamond*\\%
 RdYlGn-9-5!70!black, every mark/.append style={solid,fill=RdYlGn-9-5},mark=pentagon*\\%
 RdYlGn-9-6!70!black, every mark/.append style={solid,fill=RdYlGn-9-6},mark=x\\%
 RdYlGn-9-7!70!black, every mark/.append style={solid,fill=RdYlGn-9-7},mark=+\\%
 RdYlGn-9-8!70!black, every mark/.append style={solid,fill=RdYlGn-9-8},mark=star\\%
 RdYlGn-9-9!70!black, every mark/.append style={solid,fill=RdYlGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-10}{%
 RdYlGn-10-1!70!black, every mark/.append style={solid,fill=RdYlGn-10-1},mark=*\\%
 RdYlGn-10-2!70!black, every mark/.append style={solid,fill=RdYlGn-10-2},mark=square*\\%
 RdYlGn-10-3!70!black, every mark/.append style={solid,fill=RdYlGn-10-3},mark=triangle*\\%
 RdYlGn-10-4!70!black, every mark/.append style={solid,fill=RdYlGn-10-4},mark=diamond*\\%
 RdYlGn-10-5!70!black, every mark/.append style={solid,fill=RdYlGn-10-5},mark=pentagon*\\%
 RdYlGn-10-6!70!black, every mark/.append style={solid,fill=RdYlGn-10-6},mark=x\\%
 RdYlGn-10-7!70!black, every mark/.append style={solid,fill=RdYlGn-10-7},mark=+\\%
 RdYlGn-10-8!70!black, every mark/.append style={solid,fill=RdYlGn-10-8},mark=star\\%
 RdYlGn-10-9!70!black, every mark/.append style={solid,fill=RdYlGn-10-9},mark=oplus*\\%
 RdYlGn-10-10!70!black, every mark/.append style={solid,fill=RdYlGn-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-RdYlGn-11}{%
 RdYlGn-11-1!70!black, every mark/.append style={solid,fill=RdYlGn-11-1},mark=*\\%
 RdYlGn-11-2!70!black, every mark/.append style={solid,fill=RdYlGn-11-2},mark=square*\\%
 RdYlGn-11-3!70!black, every mark/.append style={solid,fill=RdYlGn-11-3},mark=triangle*\\%
 RdYlGn-11-4!70!black, every mark/.append style={solid,fill=RdYlGn-11-4},mark=diamond*\\%
 RdYlGn-11-5!70!black, every mark/.append style={solid,fill=RdYlGn-11-5},mark=pentagon*\\%
 RdYlGn-11-6!70!black, every mark/.append style={solid,fill=RdYlGn-11-6},mark=x\\%
 RdYlGn-11-7!70!black, every mark/.append style={solid,fill=RdYlGn-11-7},mark=+\\%
 RdYlGn-11-8!70!black, every mark/.append style={solid,fill=RdYlGn-11-8},mark=star\\%
 RdYlGn-11-9!70!black, every mark/.append style={solid,fill=RdYlGn-11-9},mark=oplus*\\%
 RdYlGn-11-10!70!black, every mark/.append style={solid,fill=RdYlGn-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-3}{%
 Set3-3-1!70!black, every mark/.append style={solid,fill=Set3-3-1},mark=*\\%
 Set3-3-2!70!black, every mark/.append style={solid,fill=Set3-3-2},mark=square*\\%
 Set3-3-3!70!black, every mark/.append style={solid,fill=Set3-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-4}{%
 Set3-4-1!70!black, every mark/.append style={solid,fill=Set3-4-1},mark=*\\%
 Set3-4-2!70!black, every mark/.append style={solid,fill=Set3-4-2},mark=square*\\%
 Set3-4-3!70!black, every mark/.append style={solid,fill=Set3-4-3},mark=triangle*\\%
 Set3-4-4!70!black, every mark/.append style={solid,fill=Set3-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-5}{%
 Set3-5-1!70!black, every mark/.append style={solid,fill=Set3-5-1},mark=*\\%
 Set3-5-2!70!black, every mark/.append style={solid,fill=Set3-5-2},mark=square*\\%
 Set3-5-3!70!black, every mark/.append style={solid,fill=Set3-5-3},mark=triangle*\\%
 Set3-5-4!70!black, every mark/.append style={solid,fill=Set3-5-4},mark=diamond*\\%
 Set3-5-5!70!black, every mark/.append style={solid,fill=Set3-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-6}{%
 Set3-6-1!70!black, every mark/.append style={solid,fill=Set3-6-1},mark=*\\%
 Set3-6-2!70!black, every mark/.append style={solid,fill=Set3-6-2},mark=square*\\%
 Set3-6-3!70!black, every mark/.append style={solid,fill=Set3-6-3},mark=triangle*\\%
 Set3-6-4!70!black, every mark/.append style={solid,fill=Set3-6-4},mark=diamond*\\%
 Set3-6-5!70!black, every mark/.append style={solid,fill=Set3-6-5},mark=pentagon*\\%
 Set3-6-6!70!black, every mark/.append style={solid,fill=Set3-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-7}{%
 Set3-7-1!70!black, every mark/.append style={solid,fill=Set3-7-1},mark=*\\%
 Set3-7-2!70!black, every mark/.append style={solid,fill=Set3-7-2},mark=square*\\%
 Set3-7-3!70!black, every mark/.append style={solid,fill=Set3-7-3},mark=triangle*\\%
 Set3-7-4!70!black, every mark/.append style={solid,fill=Set3-7-4},mark=diamond*\\%
 Set3-7-5!70!black, every mark/.append style={solid,fill=Set3-7-5},mark=pentagon*\\%
 Set3-7-6!70!black, every mark/.append style={solid,fill=Set3-7-6},mark=x\\%
 Set3-7-7!70!black, every mark/.append style={solid,fill=Set3-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-8}{%
 Set3-8-1!70!black, every mark/.append style={solid,fill=Set3-8-1},mark=*\\%
 Set3-8-2!70!black, every mark/.append style={solid,fill=Set3-8-2},mark=square*\\%
 Set3-8-3!70!black, every mark/.append style={solid,fill=Set3-8-3},mark=triangle*\\%
 Set3-8-4!70!black, every mark/.append style={solid,fill=Set3-8-4},mark=diamond*\\%
 Set3-8-5!70!black, every mark/.append style={solid,fill=Set3-8-5},mark=pentagon*\\%
 Set3-8-6!70!black, every mark/.append style={solid,fill=Set3-8-6},mark=x\\%
 Set3-8-7!70!black, every mark/.append style={solid,fill=Set3-8-7},mark=+\\%
 Set3-8-8!70!black, every mark/.append style={solid,fill=Set3-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-9}{%
 Set3-9-1!70!black, every mark/.append style={solid,fill=Set3-9-1},mark=*\\%
 Set3-9-2!70!black, every mark/.append style={solid,fill=Set3-9-2},mark=square*\\%
 Set3-9-3!70!black, every mark/.append style={solid,fill=Set3-9-3},mark=triangle*\\%
 Set3-9-4!70!black, every mark/.append style={solid,fill=Set3-9-4},mark=diamond*\\%
 Set3-9-5!70!black, every mark/.append style={solid,fill=Set3-9-5},mark=pentagon*\\%
 Set3-9-6!70!black, every mark/.append style={solid,fill=Set3-9-6},mark=x\\%
 Set3-9-7!70!black, every mark/.append style={solid,fill=Set3-9-7},mark=+\\%
 Set3-9-8!70!black, every mark/.append style={solid,fill=Set3-9-8},mark=star\\%
 Set3-9-9!70!black, every mark/.append style={solid,fill=Set3-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-10}{%
 Set3-10-1!70!black, every mark/.append style={solid,fill=Set3-10-1},mark=*\\%
 Set3-10-2!70!black, every mark/.append style={solid,fill=Set3-10-2},mark=square*\\%
 Set3-10-3!70!black, every mark/.append style={solid,fill=Set3-10-3},mark=triangle*\\%
 Set3-10-4!70!black, every mark/.append style={solid,fill=Set3-10-4},mark=diamond*\\%
 Set3-10-5!70!black, every mark/.append style={solid,fill=Set3-10-5},mark=pentagon*\\%
 Set3-10-6!70!black, every mark/.append style={solid,fill=Set3-10-6},mark=x\\%
 Set3-10-7!70!black, every mark/.append style={solid,fill=Set3-10-7},mark=+\\%
 Set3-10-8!70!black, every mark/.append style={solid,fill=Set3-10-8},mark=star\\%
 Set3-10-9!70!black, every mark/.append style={solid,fill=Set3-10-9},mark=oplus*\\%
 Set3-10-10!70!black, every mark/.append style={solid,fill=Set3-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-11}{%
 Set3-11-1!70!black, every mark/.append style={solid,fill=Set3-11-1},mark=*\\%
 Set3-11-2!70!black, every mark/.append style={solid,fill=Set3-11-2},mark=square*\\%
 Set3-11-3!70!black, every mark/.append style={solid,fill=Set3-11-3},mark=triangle*\\%
 Set3-11-4!70!black, every mark/.append style={solid,fill=Set3-11-4},mark=diamond*\\%
 Set3-11-5!70!black, every mark/.append style={solid,fill=Set3-11-5},mark=pentagon*\\%
 Set3-11-6!70!black, every mark/.append style={solid,fill=Set3-11-6},mark=x\\%
 Set3-11-7!70!black, every mark/.append style={solid,fill=Set3-11-7},mark=+\\%
 Set3-11-8!70!black, every mark/.append style={solid,fill=Set3-11-8},mark=star\\%
 Set3-11-9!70!black, every mark/.append style={solid,fill=Set3-11-9},mark=oplus*\\%
 Set3-11-10!70!black, every mark/.append style={solid,fill=Set3-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set3-12}{%
 Set3-12-1!70!black, every mark/.append style={solid,fill=Set3-12-1},mark=*\\%
 Set3-12-2!70!black, every mark/.append style={solid,fill=Set3-12-2},mark=square*\\%
 Set3-12-3!70!black, every mark/.append style={solid,fill=Set3-12-3},mark=triangle*\\%
 Set3-12-4!70!black, every mark/.append style={solid,fill=Set3-12-4},mark=diamond*\\%
 Set3-12-5!70!black, every mark/.append style={solid,fill=Set3-12-5},mark=pentagon*\\%
 Set3-12-6!70!black, every mark/.append style={solid,fill=Set3-12-6},mark=x\\%
 Set3-12-7!70!black, every mark/.append style={solid,fill=Set3-12-7},mark=+\\%
 Set3-12-8!70!black, every mark/.append style={solid,fill=Set3-12-8},mark=star\\%
 Set3-12-9!70!black, every mark/.append style={solid,fill=Set3-12-9},mark=oplus*\\%
 Set3-12-10!70!black, every mark/.append style={solid,fill=Set3-12-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-3}{%
 Pastel1-3-1!70!black, every mark/.append style={solid,fill=Pastel1-3-1},mark=*\\%
 Pastel1-3-2!70!black, every mark/.append style={solid,fill=Pastel1-3-2},mark=square*\\%
 Pastel1-3-3!70!black, every mark/.append style={solid,fill=Pastel1-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-4}{%
 Pastel1-4-1!70!black, every mark/.append style={solid,fill=Pastel1-4-1},mark=*\\%
 Pastel1-4-2!70!black, every mark/.append style={solid,fill=Pastel1-4-2},mark=square*\\%
 Pastel1-4-3!70!black, every mark/.append style={solid,fill=Pastel1-4-3},mark=triangle*\\%
 Pastel1-4-4!70!black, every mark/.append style={solid,fill=Pastel1-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-5}{%
 Pastel1-5-1!70!black, every mark/.append style={solid,fill=Pastel1-5-1},mark=*\\%
 Pastel1-5-2!70!black, every mark/.append style={solid,fill=Pastel1-5-2},mark=square*\\%
 Pastel1-5-3!70!black, every mark/.append style={solid,fill=Pastel1-5-3},mark=triangle*\\%
 Pastel1-5-4!70!black, every mark/.append style={solid,fill=Pastel1-5-4},mark=diamond*\\%
 Pastel1-5-5!70!black, every mark/.append style={solid,fill=Pastel1-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-6}{%
 Pastel1-6-1!70!black, every mark/.append style={solid,fill=Pastel1-6-1},mark=*\\%
 Pastel1-6-2!70!black, every mark/.append style={solid,fill=Pastel1-6-2},mark=square*\\%
 Pastel1-6-3!70!black, every mark/.append style={solid,fill=Pastel1-6-3},mark=triangle*\\%
 Pastel1-6-4!70!black, every mark/.append style={solid,fill=Pastel1-6-4},mark=diamond*\\%
 Pastel1-6-5!70!black, every mark/.append style={solid,fill=Pastel1-6-5},mark=pentagon*\\%
 Pastel1-6-6!70!black, every mark/.append style={solid,fill=Pastel1-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-7}{%
 Pastel1-7-1!70!black, every mark/.append style={solid,fill=Pastel1-7-1},mark=*\\%
 Pastel1-7-2!70!black, every mark/.append style={solid,fill=Pastel1-7-2},mark=square*\\%
 Pastel1-7-3!70!black, every mark/.append style={solid,fill=Pastel1-7-3},mark=triangle*\\%
 Pastel1-7-4!70!black, every mark/.append style={solid,fill=Pastel1-7-4},mark=diamond*\\%
 Pastel1-7-5!70!black, every mark/.append style={solid,fill=Pastel1-7-5},mark=pentagon*\\%
 Pastel1-7-6!70!black, every mark/.append style={solid,fill=Pastel1-7-6},mark=x\\%
 Pastel1-7-7!70!black, every mark/.append style={solid,fill=Pastel1-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-8}{%
 Pastel1-8-1!70!black, every mark/.append style={solid,fill=Pastel1-8-1},mark=*\\%
 Pastel1-8-2!70!black, every mark/.append style={solid,fill=Pastel1-8-2},mark=square*\\%
 Pastel1-8-3!70!black, every mark/.append style={solid,fill=Pastel1-8-3},mark=triangle*\\%
 Pastel1-8-4!70!black, every mark/.append style={solid,fill=Pastel1-8-4},mark=diamond*\\%
 Pastel1-8-5!70!black, every mark/.append style={solid,fill=Pastel1-8-5},mark=pentagon*\\%
 Pastel1-8-6!70!black, every mark/.append style={solid,fill=Pastel1-8-6},mark=x\\%
 Pastel1-8-7!70!black, every mark/.append style={solid,fill=Pastel1-8-7},mark=+\\%
 Pastel1-8-8!70!black, every mark/.append style={solid,fill=Pastel1-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel1-9}{%
 Pastel1-9-1!70!black, every mark/.append style={solid,fill=Pastel1-9-1},mark=*\\%
 Pastel1-9-2!70!black, every mark/.append style={solid,fill=Pastel1-9-2},mark=square*\\%
 Pastel1-9-3!70!black, every mark/.append style={solid,fill=Pastel1-9-3},mark=triangle*\\%
 Pastel1-9-4!70!black, every mark/.append style={solid,fill=Pastel1-9-4},mark=diamond*\\%
 Pastel1-9-5!70!black, every mark/.append style={solid,fill=Pastel1-9-5},mark=pentagon*\\%
 Pastel1-9-6!70!black, every mark/.append style={solid,fill=Pastel1-9-6},mark=x\\%
 Pastel1-9-7!70!black, every mark/.append style={solid,fill=Pastel1-9-7},mark=+\\%
 Pastel1-9-8!70!black, every mark/.append style={solid,fill=Pastel1-9-8},mark=star\\%
 Pastel1-9-9!70!black, every mark/.append style={solid,fill=Pastel1-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-3}{%
 Set1-3-1!70!black, every mark/.append style={solid,fill=Set1-3-1},mark=*\\%
 Set1-3-2!70!black, every mark/.append style={solid,fill=Set1-3-2},mark=square*\\%
 Set1-3-3!70!black, every mark/.append style={solid,fill=Set1-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-4}{%
 Set1-4-1!70!black, every mark/.append style={solid,fill=Set1-4-1},mark=*\\%
 Set1-4-2!70!black, every mark/.append style={solid,fill=Set1-4-2},mark=square*\\%
 Set1-4-3!70!black, every mark/.append style={solid,fill=Set1-4-3},mark=triangle*\\%
 Set1-4-4!70!black, every mark/.append style={solid,fill=Set1-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-5}{%
 Set1-5-1!70!black, every mark/.append style={solid,fill=Set1-5-1},mark=*\\%
 Set1-5-2!70!black, every mark/.append style={solid,fill=Set1-5-2},mark=square*\\%
 Set1-5-3!70!black, every mark/.append style={solid,fill=Set1-5-3},mark=triangle*\\%
 Set1-5-4!70!black, every mark/.append style={solid,fill=Set1-5-4},mark=diamond*\\%
 Set1-5-5!70!black, every mark/.append style={solid,fill=Set1-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-6}{%
 Set1-6-1!70!black, every mark/.append style={solid,fill=Set1-6-1},mark=*\\%
 Set1-6-2!70!black, every mark/.append style={solid,fill=Set1-6-2},mark=square*\\%
 Set1-6-3!70!black, every mark/.append style={solid,fill=Set1-6-3},mark=triangle*\\%
 Set1-6-4!70!black, every mark/.append style={solid,fill=Set1-6-4},mark=diamond*\\%
 Set1-6-5!70!black, every mark/.append style={solid,fill=Set1-6-5},mark=pentagon*\\%
 Set1-6-6!70!black, every mark/.append style={solid,fill=Set1-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-7}{%
 Set1-7-1!70!black, every mark/.append style={solid,fill=Set1-7-1},mark=*\\%
 Set1-7-2!70!black, every mark/.append style={solid,fill=Set1-7-2},mark=square*\\%
 Set1-7-3!70!black, every mark/.append style={solid,fill=Set1-7-3},mark=triangle*\\%
 Set1-7-4!70!black, every mark/.append style={solid,fill=Set1-7-4},mark=diamond*\\%
 Set1-7-5!70!black, every mark/.append style={solid,fill=Set1-7-5},mark=pentagon*\\%
 Set1-7-6!70!black, every mark/.append style={solid,fill=Set1-7-6},mark=x\\%
 Set1-7-7!70!black, every mark/.append style={solid,fill=Set1-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-8}{%
 Set1-8-1!70!black, every mark/.append style={solid,fill=Set1-8-1},mark=*\\%
 Set1-8-2!70!black, every mark/.append style={solid,fill=Set1-8-2},mark=square*\\%
 Set1-8-3!70!black, every mark/.append style={solid,fill=Set1-8-3},mark=triangle*\\%
 Set1-8-4!70!black, every mark/.append style={solid,fill=Set1-8-4},mark=diamond*\\%
 Set1-8-5!70!black, every mark/.append style={solid,fill=Set1-8-5},mark=pentagon*\\%
 Set1-8-6!70!black, every mark/.append style={solid,fill=Set1-8-6},mark=x\\%
 Set1-8-7!70!black, every mark/.append style={solid,fill=Set1-8-7},mark=+\\%
 Set1-8-8!70!black, every mark/.append style={solid,fill=Set1-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Set1-9}{%
 Set1-9-1!70!black, every mark/.append style={solid,fill=Set1-9-1},mark=*\\%
 Set1-9-2!70!black, every mark/.append style={solid,fill=Set1-9-2},mark=square*\\%
 Set1-9-3!70!black, every mark/.append style={solid,fill=Set1-9-3},mark=triangle*\\%
 Set1-9-4!70!black, every mark/.append style={solid,fill=Set1-9-4},mark=diamond*\\%
 Set1-9-5!70!black, every mark/.append style={solid,fill=Set1-9-5},mark=pentagon*\\%
 Set1-9-6!70!black, every mark/.append style={solid,fill=Set1-9-6},mark=x\\%
 Set1-9-7!70!black, every mark/.append style={solid,fill=Set1-9-7},mark=+\\%
 Set1-9-8!70!black, every mark/.append style={solid,fill=Set1-9-8},mark=star\\%
 Set1-9-9!70!black, every mark/.append style={solid,fill=Set1-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-3}{%
 Pastel2-3-1!70!black, every mark/.append style={solid,fill=Pastel2-3-1},mark=*\\%
 Pastel2-3-2!70!black, every mark/.append style={solid,fill=Pastel2-3-2},mark=square*\\%
 Pastel2-3-3!70!black, every mark/.append style={solid,fill=Pastel2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-4}{%
 Pastel2-4-1!70!black, every mark/.append style={solid,fill=Pastel2-4-1},mark=*\\%
 Pastel2-4-2!70!black, every mark/.append style={solid,fill=Pastel2-4-2},mark=square*\\%
 Pastel2-4-3!70!black, every mark/.append style={solid,fill=Pastel2-4-3},mark=triangle*\\%
 Pastel2-4-4!70!black, every mark/.append style={solid,fill=Pastel2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-5}{%
 Pastel2-5-1!70!black, every mark/.append style={solid,fill=Pastel2-5-1},mark=*\\%
 Pastel2-5-2!70!black, every mark/.append style={solid,fill=Pastel2-5-2},mark=square*\\%
 Pastel2-5-3!70!black, every mark/.append style={solid,fill=Pastel2-5-3},mark=triangle*\\%
 Pastel2-5-4!70!black, every mark/.append style={solid,fill=Pastel2-5-4},mark=diamond*\\%
 Pastel2-5-5!70!black, every mark/.append style={solid,fill=Pastel2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-6}{%
 Pastel2-6-1!70!black, every mark/.append style={solid,fill=Pastel2-6-1},mark=*\\%
 Pastel2-6-2!70!black, every mark/.append style={solid,fill=Pastel2-6-2},mark=square*\\%
 Pastel2-6-3!70!black, every mark/.append style={solid,fill=Pastel2-6-3},mark=triangle*\\%
 Pastel2-6-4!70!black, every mark/.append style={solid,fill=Pastel2-6-4},mark=diamond*\\%
 Pastel2-6-5!70!black, every mark/.append style={solid,fill=Pastel2-6-5},mark=pentagon*\\%
 Pastel2-6-6!70!black, every mark/.append style={solid,fill=Pastel2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-7}{%
 Pastel2-7-1!70!black, every mark/.append style={solid,fill=Pastel2-7-1},mark=*\\%
 Pastel2-7-2!70!black, every mark/.append style={solid,fill=Pastel2-7-2},mark=square*\\%
 Pastel2-7-3!70!black, every mark/.append style={solid,fill=Pastel2-7-3},mark=triangle*\\%
 Pastel2-7-4!70!black, every mark/.append style={solid,fill=Pastel2-7-4},mark=diamond*\\%
 Pastel2-7-5!70!black, every mark/.append style={solid,fill=Pastel2-7-5},mark=pentagon*\\%
 Pastel2-7-6!70!black, every mark/.append style={solid,fill=Pastel2-7-6},mark=x\\%
 Pastel2-7-7!70!black, every mark/.append style={solid,fill=Pastel2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Pastel2-8}{%
 Pastel2-8-1!70!black, every mark/.append style={solid,fill=Pastel2-8-1},mark=*\\%
 Pastel2-8-2!70!black, every mark/.append style={solid,fill=Pastel2-8-2},mark=square*\\%
 Pastel2-8-3!70!black, every mark/.append style={solid,fill=Pastel2-8-3},mark=triangle*\\%
 Pastel2-8-4!70!black, every mark/.append style={solid,fill=Pastel2-8-4},mark=diamond*\\%
 Pastel2-8-5!70!black, every mark/.append style={solid,fill=Pastel2-8-5},mark=pentagon*\\%
 Pastel2-8-6!70!black, every mark/.append style={solid,fill=Pastel2-8-6},mark=x\\%
 Pastel2-8-7!70!black, every mark/.append style={solid,fill=Pastel2-8-7},mark=+\\%
 Pastel2-8-8!70!black, every mark/.append style={solid,fill=Pastel2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-3}{%
 Set2-3-1!70!black, every mark/.append style={solid,fill=Set2-3-1},mark=*\\%
 Set2-3-2!70!black, every mark/.append style={solid,fill=Set2-3-2},mark=square*\\%
 Set2-3-3!70!black, every mark/.append style={solid,fill=Set2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-4}{%
 Set2-4-1!70!black, every mark/.append style={solid,fill=Set2-4-1},mark=*\\%
 Set2-4-2!70!black, every mark/.append style={solid,fill=Set2-4-2},mark=square*\\%
 Set2-4-3!70!black, every mark/.append style={solid,fill=Set2-4-3},mark=triangle*\\%
 Set2-4-4!70!black, every mark/.append style={solid,fill=Set2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-5}{%
 Set2-5-1!70!black, every mark/.append style={solid,fill=Set2-5-1},mark=*\\%
 Set2-5-2!70!black, every mark/.append style={solid,fill=Set2-5-2},mark=square*\\%
 Set2-5-3!70!black, every mark/.append style={solid,fill=Set2-5-3},mark=triangle*\\%
 Set2-5-4!70!black, every mark/.append style={solid,fill=Set2-5-4},mark=diamond*\\%
 Set2-5-5!70!black, every mark/.append style={solid,fill=Set2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-6}{%
 Set2-6-1!70!black, every mark/.append style={solid,fill=Set2-6-1},mark=*\\%
 Set2-6-2!70!black, every mark/.append style={solid,fill=Set2-6-2},mark=square*\\%
 Set2-6-3!70!black, every mark/.append style={solid,fill=Set2-6-3},mark=triangle*\\%
 Set2-6-4!70!black, every mark/.append style={solid,fill=Set2-6-4},mark=diamond*\\%
 Set2-6-5!70!black, every mark/.append style={solid,fill=Set2-6-5},mark=pentagon*\\%
 Set2-6-6!70!black, every mark/.append style={solid,fill=Set2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-7}{%
 Set2-7-1!70!black, every mark/.append style={solid,fill=Set2-7-1},mark=*\\%
 Set2-7-2!70!black, every mark/.append style={solid,fill=Set2-7-2},mark=square*\\%
 Set2-7-3!70!black, every mark/.append style={solid,fill=Set2-7-3},mark=triangle*\\%
 Set2-7-4!70!black, every mark/.append style={solid,fill=Set2-7-4},mark=diamond*\\%
 Set2-7-5!70!black, every mark/.append style={solid,fill=Set2-7-5},mark=pentagon*\\%
 Set2-7-6!70!black, every mark/.append style={solid,fill=Set2-7-6},mark=x\\%
 Set2-7-7!70!black, every mark/.append style={solid,fill=Set2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Set2-8}{%
 Set2-8-1!70!black, every mark/.append style={solid,fill=Set2-8-1},mark=*\\%
 Set2-8-2!70!black, every mark/.append style={solid,fill=Set2-8-2},mark=square*\\%
 Set2-8-3!70!black, every mark/.append style={solid,fill=Set2-8-3},mark=triangle*\\%
 Set2-8-4!70!black, every mark/.append style={solid,fill=Set2-8-4},mark=diamond*\\%
 Set2-8-5!70!black, every mark/.append style={solid,fill=Set2-8-5},mark=pentagon*\\%
 Set2-8-6!70!black, every mark/.append style={solid,fill=Set2-8-6},mark=x\\%
 Set2-8-7!70!black, every mark/.append style={solid,fill=Set2-8-7},mark=+\\%
 Set2-8-8!70!black, every mark/.append style={solid,fill=Set2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-3}{%
 Dark2-3-1!70!black, every mark/.append style={solid,fill=Dark2-3-1},mark=*\\%
 Dark2-3-2!70!black, every mark/.append style={solid,fill=Dark2-3-2},mark=square*\\%
 Dark2-3-3!70!black, every mark/.append style={solid,fill=Dark2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-4}{%
 Dark2-4-1!70!black, every mark/.append style={solid,fill=Dark2-4-1},mark=*\\%
 Dark2-4-2!70!black, every mark/.append style={solid,fill=Dark2-4-2},mark=square*\\%
 Dark2-4-3!70!black, every mark/.append style={solid,fill=Dark2-4-3},mark=triangle*\\%
 Dark2-4-4!70!black, every mark/.append style={solid,fill=Dark2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-5}{%
 Dark2-5-1!70!black, every mark/.append style={solid,fill=Dark2-5-1},mark=*\\%
 Dark2-5-2!70!black, every mark/.append style={solid,fill=Dark2-5-2},mark=square*\\%
 Dark2-5-3!70!black, every mark/.append style={solid,fill=Dark2-5-3},mark=triangle*\\%
 Dark2-5-4!70!black, every mark/.append style={solid,fill=Dark2-5-4},mark=diamond*\\%
 Dark2-5-5!70!black, every mark/.append style={solid,fill=Dark2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-6}{%
 Dark2-6-1!70!black, every mark/.append style={solid,fill=Dark2-6-1},mark=*\\%
 Dark2-6-2!70!black, every mark/.append style={solid,fill=Dark2-6-2},mark=square*\\%
 Dark2-6-3!70!black, every mark/.append style={solid,fill=Dark2-6-3},mark=triangle*\\%
 Dark2-6-4!70!black, every mark/.append style={solid,fill=Dark2-6-4},mark=diamond*\\%
 Dark2-6-5!70!black, every mark/.append style={solid,fill=Dark2-6-5},mark=pentagon*\\%
 Dark2-6-6!70!black, every mark/.append style={solid,fill=Dark2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-7}{%
 Dark2-7-1!70!black, every mark/.append style={solid,fill=Dark2-7-1},mark=*\\%
 Dark2-7-2!70!black, every mark/.append style={solid,fill=Dark2-7-2},mark=square*\\%
 Dark2-7-3!70!black, every mark/.append style={solid,fill=Dark2-7-3},mark=triangle*\\%
 Dark2-7-4!70!black, every mark/.append style={solid,fill=Dark2-7-4},mark=diamond*\\%
 Dark2-7-5!70!black, every mark/.append style={solid,fill=Dark2-7-5},mark=pentagon*\\%
 Dark2-7-6!70!black, every mark/.append style={solid,fill=Dark2-7-6},mark=x\\%
 Dark2-7-7!70!black, every mark/.append style={solid,fill=Dark2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Dark2-8}{%
 Dark2-8-1!70!black, every mark/.append style={solid,fill=Dark2-8-1},mark=*\\%
 Dark2-8-2!70!black, every mark/.append style={solid,fill=Dark2-8-2},mark=square*\\%
 Dark2-8-3!70!black, every mark/.append style={solid,fill=Dark2-8-3},mark=triangle*\\%
 Dark2-8-4!70!black, every mark/.append style={solid,fill=Dark2-8-4},mark=diamond*\\%
 Dark2-8-5!70!black, every mark/.append style={solid,fill=Dark2-8-5},mark=pentagon*\\%
 Dark2-8-6!70!black, every mark/.append style={solid,fill=Dark2-8-6},mark=x\\%
 Dark2-8-7!70!black, every mark/.append style={solid,fill=Dark2-8-7},mark=+\\%
 Dark2-8-8!70!black, every mark/.append style={solid,fill=Dark2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-3}{%
 Paired-3-1!70!black, every mark/.append style={solid,fill=Paired-3-1},mark=*\\%
 Paired-3-2!70!black, every mark/.append style={solid,fill=Paired-3-2},mark=square*\\%
 Paired-3-3!70!black, every mark/.append style={solid,fill=Paired-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-4}{%
 Paired-4-1!70!black, every mark/.append style={solid,fill=Paired-4-1},mark=*\\%
 Paired-4-2!70!black, every mark/.append style={solid,fill=Paired-4-2},mark=square*\\%
 Paired-4-3!70!black, every mark/.append style={solid,fill=Paired-4-3},mark=triangle*\\%
 Paired-4-4!70!black, every mark/.append style={solid,fill=Paired-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-5}{%
 Paired-5-1!70!black, every mark/.append style={solid,fill=Paired-5-1},mark=*\\%
 Paired-5-2!70!black, every mark/.append style={solid,fill=Paired-5-2},mark=square*\\%
 Paired-5-3!70!black, every mark/.append style={solid,fill=Paired-5-3},mark=triangle*\\%
 Paired-5-4!70!black, every mark/.append style={solid,fill=Paired-5-4},mark=diamond*\\%
 Paired-5-5!70!black, every mark/.append style={solid,fill=Paired-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-6}{%
 Paired-6-1!70!black, every mark/.append style={solid,fill=Paired-6-1},mark=*\\%
 Paired-6-2!70!black, every mark/.append style={solid,fill=Paired-6-2},mark=square*\\%
 Paired-6-3!70!black, every mark/.append style={solid,fill=Paired-6-3},mark=triangle*\\%
 Paired-6-4!70!black, every mark/.append style={solid,fill=Paired-6-4},mark=diamond*\\%
 Paired-6-5!70!black, every mark/.append style={solid,fill=Paired-6-5},mark=pentagon*\\%
 Paired-6-6!70!black, every mark/.append style={solid,fill=Paired-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-7}{%
 Paired-7-1!70!black, every mark/.append style={solid,fill=Paired-7-1},mark=*\\%
 Paired-7-2!70!black, every mark/.append style={solid,fill=Paired-7-2},mark=square*\\%
 Paired-7-3!70!black, every mark/.append style={solid,fill=Paired-7-3},mark=triangle*\\%
 Paired-7-4!70!black, every mark/.append style={solid,fill=Paired-7-4},mark=diamond*\\%
 Paired-7-5!70!black, every mark/.append style={solid,fill=Paired-7-5},mark=pentagon*\\%
 Paired-7-6!70!black, every mark/.append style={solid,fill=Paired-7-6},mark=x\\%
 Paired-7-7!70!black, every mark/.append style={solid,fill=Paired-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-8}{%
 Paired-8-1!70!black, every mark/.append style={solid,fill=Paired-8-1},mark=*\\%
 Paired-8-2!70!black, every mark/.append style={solid,fill=Paired-8-2},mark=square*\\%
 Paired-8-3!70!black, every mark/.append style={solid,fill=Paired-8-3},mark=triangle*\\%
 Paired-8-4!70!black, every mark/.append style={solid,fill=Paired-8-4},mark=diamond*\\%
 Paired-8-5!70!black, every mark/.append style={solid,fill=Paired-8-5},mark=pentagon*\\%
 Paired-8-6!70!black, every mark/.append style={solid,fill=Paired-8-6},mark=x\\%
 Paired-8-7!70!black, every mark/.append style={solid,fill=Paired-8-7},mark=+\\%
 Paired-8-8!70!black, every mark/.append style={solid,fill=Paired-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-9}{%
 Paired-9-1!70!black, every mark/.append style={solid,fill=Paired-9-1},mark=*\\%
 Paired-9-2!70!black, every mark/.append style={solid,fill=Paired-9-2},mark=square*\\%
 Paired-9-3!70!black, every mark/.append style={solid,fill=Paired-9-3},mark=triangle*\\%
 Paired-9-4!70!black, every mark/.append style={solid,fill=Paired-9-4},mark=diamond*\\%
 Paired-9-5!70!black, every mark/.append style={solid,fill=Paired-9-5},mark=pentagon*\\%
 Paired-9-6!70!black, every mark/.append style={solid,fill=Paired-9-6},mark=x\\%
 Paired-9-7!70!black, every mark/.append style={solid,fill=Paired-9-7},mark=+\\%
 Paired-9-8!70!black, every mark/.append style={solid,fill=Paired-9-8},mark=star\\%
 Paired-9-9!70!black, every mark/.append style={solid,fill=Paired-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-10}{%
 Paired-10-1!70!black, every mark/.append style={solid,fill=Paired-10-1},mark=*\\%
 Paired-10-2!70!black, every mark/.append style={solid,fill=Paired-10-2},mark=square*\\%
 Paired-10-3!70!black, every mark/.append style={solid,fill=Paired-10-3},mark=triangle*\\%
 Paired-10-4!70!black, every mark/.append style={solid,fill=Paired-10-4},mark=diamond*\\%
 Paired-10-5!70!black, every mark/.append style={solid,fill=Paired-10-5},mark=pentagon*\\%
 Paired-10-6!70!black, every mark/.append style={solid,fill=Paired-10-6},mark=x\\%
 Paired-10-7!70!black, every mark/.append style={solid,fill=Paired-10-7},mark=+\\%
 Paired-10-8!70!black, every mark/.append style={solid,fill=Paired-10-8},mark=star\\%
 Paired-10-9!70!black, every mark/.append style={solid,fill=Paired-10-9},mark=oplus*\\%
 Paired-10-10!70!black, every mark/.append style={solid,fill=Paired-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-11}{%
 Paired-11-1!70!black, every mark/.append style={solid,fill=Paired-11-1},mark=*\\%
 Paired-11-2!70!black, every mark/.append style={solid,fill=Paired-11-2},mark=square*\\%
 Paired-11-3!70!black, every mark/.append style={solid,fill=Paired-11-3},mark=triangle*\\%
 Paired-11-4!70!black, every mark/.append style={solid,fill=Paired-11-4},mark=diamond*\\%
 Paired-11-5!70!black, every mark/.append style={solid,fill=Paired-11-5},mark=pentagon*\\%
 Paired-11-6!70!black, every mark/.append style={solid,fill=Paired-11-6},mark=x\\%
 Paired-11-7!70!black, every mark/.append style={solid,fill=Paired-11-7},mark=+\\%
 Paired-11-8!70!black, every mark/.append style={solid,fill=Paired-11-8},mark=star\\%
 Paired-11-9!70!black, every mark/.append style={solid,fill=Paired-11-9},mark=oplus*\\%
 Paired-11-10!70!black, every mark/.append style={solid,fill=Paired-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Paired-12}{%
 Paired-12-1!70!black, every mark/.append style={solid,fill=Paired-12-1},mark=*\\%
 Paired-12-2!70!black, every mark/.append style={solid,fill=Paired-12-2},mark=square*\\%
 Paired-12-3!70!black, every mark/.append style={solid,fill=Paired-12-3},mark=triangle*\\%
 Paired-12-4!70!black, every mark/.append style={solid,fill=Paired-12-4},mark=diamond*\\%
 Paired-12-5!70!black, every mark/.append style={solid,fill=Paired-12-5},mark=pentagon*\\%
 Paired-12-6!70!black, every mark/.append style={solid,fill=Paired-12-6},mark=x\\%
 Paired-12-7!70!black, every mark/.append style={solid,fill=Paired-12-7},mark=+\\%
 Paired-12-8!70!black, every mark/.append style={solid,fill=Paired-12-8},mark=star\\%
 Paired-12-9!70!black, every mark/.append style={solid,fill=Paired-12-9},mark=oplus*\\%
 Paired-12-10!70!black, every mark/.append style={solid,fill=Paired-12-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-3}{%
 Accent-3-1!70!black, every mark/.append style={solid,fill=Accent-3-1},mark=*\\%
 Accent-3-2!70!black, every mark/.append style={solid,fill=Accent-3-2},mark=square*\\%
 Accent-3-3!70!black, every mark/.append style={solid,fill=Accent-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-4}{%
 Accent-4-1!70!black, every mark/.append style={solid,fill=Accent-4-1},mark=*\\%
 Accent-4-2!70!black, every mark/.append style={solid,fill=Accent-4-2},mark=square*\\%
 Accent-4-3!70!black, every mark/.append style={solid,fill=Accent-4-3},mark=triangle*\\%
 Accent-4-4!70!black, every mark/.append style={solid,fill=Accent-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-5}{%
 Accent-5-1!70!black, every mark/.append style={solid,fill=Accent-5-1},mark=*\\%
 Accent-5-2!70!black, every mark/.append style={solid,fill=Accent-5-2},mark=square*\\%
 Accent-5-3!70!black, every mark/.append style={solid,fill=Accent-5-3},mark=triangle*\\%
 Accent-5-4!70!black, every mark/.append style={solid,fill=Accent-5-4},mark=diamond*\\%
 Accent-5-5!70!black, every mark/.append style={solid,fill=Accent-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-6}{%
 Accent-6-1!70!black, every mark/.append style={solid,fill=Accent-6-1},mark=*\\%
 Accent-6-2!70!black, every mark/.append style={solid,fill=Accent-6-2},mark=square*\\%
 Accent-6-3!70!black, every mark/.append style={solid,fill=Accent-6-3},mark=triangle*\\%
 Accent-6-4!70!black, every mark/.append style={solid,fill=Accent-6-4},mark=diamond*\\%
 Accent-6-5!70!black, every mark/.append style={solid,fill=Accent-6-5},mark=pentagon*\\%
 Accent-6-6!70!black, every mark/.append style={solid,fill=Accent-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-7}{%
 Accent-7-1!70!black, every mark/.append style={solid,fill=Accent-7-1},mark=*\\%
 Accent-7-2!70!black, every mark/.append style={solid,fill=Accent-7-2},mark=square*\\%
 Accent-7-3!70!black, every mark/.append style={solid,fill=Accent-7-3},mark=triangle*\\%
 Accent-7-4!70!black, every mark/.append style={solid,fill=Accent-7-4},mark=diamond*\\%
 Accent-7-5!70!black, every mark/.append style={solid,fill=Accent-7-5},mark=pentagon*\\%
 Accent-7-6!70!black, every mark/.append style={solid,fill=Accent-7-6},mark=x\\%
 Accent-7-7!70!black, every mark/.append style={solid,fill=Accent-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{Mark-Accent-8}{%
 Accent-8-1!70!black, every mark/.append style={solid,fill=Accent-8-1},mark=*\\%
 Accent-8-2!70!black, every mark/.append style={solid,fill=Accent-8-2},mark=square*\\%
 Accent-8-3!70!black, every mark/.append style={solid,fill=Accent-8-3},mark=triangle*\\%
 Accent-8-4!70!black, every mark/.append style={solid,fill=Accent-8-4},mark=diamond*\\%
 Accent-8-5!70!black, every mark/.append style={solid,fill=Accent-8-5},mark=pentagon*\\%
 Accent-8-6!70!black, every mark/.append style={solid,fill=Accent-8-6},mark=x\\%
 Accent-8-7!70!black, every mark/.append style={solid,fill=Accent-8-7},mark=+\\%
 Accent-8-8!70!black, every mark/.append style={solid,fill=Accent-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-3}{%
 YlGn-3-1!70, every mark/.append style={solid,fill=YlGn-3-1},mark=*\\%
 YlGn-3-2!70, every mark/.append style={solid,fill=YlGn-3-2},mark=square*\\%
 YlGn-3-3!70, every mark/.append style={solid,fill=YlGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-4}{%
 YlGn-4-1!70, every mark/.append style={solid,fill=YlGn-4-1},mark=*\\%
 YlGn-4-2!70, every mark/.append style={solid,fill=YlGn-4-2},mark=square*\\%
 YlGn-4-3!70, every mark/.append style={solid,fill=YlGn-4-3},mark=triangle*\\%
 YlGn-4-4!70, every mark/.append style={solid,fill=YlGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-5}{%
 YlGn-5-1!70, every mark/.append style={solid,fill=YlGn-5-1},mark=*\\%
 YlGn-5-2!70, every mark/.append style={solid,fill=YlGn-5-2},mark=square*\\%
 YlGn-5-3!70, every mark/.append style={solid,fill=YlGn-5-3},mark=triangle*\\%
 YlGn-5-4!70, every mark/.append style={solid,fill=YlGn-5-4},mark=diamond*\\%
 YlGn-5-5!70, every mark/.append style={solid,fill=YlGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-6}{%
 YlGn-6-1!70, every mark/.append style={solid,fill=YlGn-6-1},mark=*\\%
 YlGn-6-2!70, every mark/.append style={solid,fill=YlGn-6-2},mark=square*\\%
 YlGn-6-3!70, every mark/.append style={solid,fill=YlGn-6-3},mark=triangle*\\%
 YlGn-6-4!70, every mark/.append style={solid,fill=YlGn-6-4},mark=diamond*\\%
 YlGn-6-5!70, every mark/.append style={solid,fill=YlGn-6-5},mark=pentagon*\\%
 YlGn-6-6!70, every mark/.append style={solid,fill=YlGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-7}{%
 YlGn-7-1!70, every mark/.append style={solid,fill=YlGn-7-1},mark=*\\%
 YlGn-7-2!70, every mark/.append style={solid,fill=YlGn-7-2},mark=square*\\%
 YlGn-7-3!70, every mark/.append style={solid,fill=YlGn-7-3},mark=triangle*\\%
 YlGn-7-4!70, every mark/.append style={solid,fill=YlGn-7-4},mark=diamond*\\%
 YlGn-7-5!70, every mark/.append style={solid,fill=YlGn-7-5},mark=pentagon*\\%
 YlGn-7-6!70, every mark/.append style={solid,fill=YlGn-7-6},mark=x\\%
 YlGn-7-7!70, every mark/.append style={solid,fill=YlGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-8}{%
 YlGn-8-1!70, every mark/.append style={solid,fill=YlGn-8-1},mark=*\\%
 YlGn-8-2!70, every mark/.append style={solid,fill=YlGn-8-2},mark=square*\\%
 YlGn-8-3!70, every mark/.append style={solid,fill=YlGn-8-3},mark=triangle*\\%
 YlGn-8-4!70, every mark/.append style={solid,fill=YlGn-8-4},mark=diamond*\\%
 YlGn-8-5!70, every mark/.append style={solid,fill=YlGn-8-5},mark=pentagon*\\%
 YlGn-8-6!70, every mark/.append style={solid,fill=YlGn-8-6},mark=x\\%
 YlGn-8-7!70, every mark/.append style={solid,fill=YlGn-8-7},mark=+\\%
 YlGn-8-8!70, every mark/.append style={solid,fill=YlGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGn-9}{%
 YlGn-9-1!70, every mark/.append style={solid,fill=YlGn-9-1},mark=*\\%
 YlGn-9-2!70, every mark/.append style={solid,fill=YlGn-9-2},mark=square*\\%
 YlGn-9-3!70, every mark/.append style={solid,fill=YlGn-9-3},mark=triangle*\\%
 YlGn-9-4!70, every mark/.append style={solid,fill=YlGn-9-4},mark=diamond*\\%
 YlGn-9-5!70, every mark/.append style={solid,fill=YlGn-9-5},mark=pentagon*\\%
 YlGn-9-6!70, every mark/.append style={solid,fill=YlGn-9-6},mark=x\\%
 YlGn-9-7!70, every mark/.append style={solid,fill=YlGn-9-7},mark=+\\%
 YlGn-9-8!70, every mark/.append style={solid,fill=YlGn-9-8},mark=star\\%
 YlGn-9-9!70, every mark/.append style={solid,fill=YlGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-3}{%
 YlGnBu-3-1!70, every mark/.append style={solid,fill=YlGnBu-3-1},mark=*\\%
 YlGnBu-3-2!70, every mark/.append style={solid,fill=YlGnBu-3-2},mark=square*\\%
 YlGnBu-3-3!70, every mark/.append style={solid,fill=YlGnBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-4}{%
 YlGnBu-4-1!70, every mark/.append style={solid,fill=YlGnBu-4-1},mark=*\\%
 YlGnBu-4-2!70, every mark/.append style={solid,fill=YlGnBu-4-2},mark=square*\\%
 YlGnBu-4-3!70, every mark/.append style={solid,fill=YlGnBu-4-3},mark=triangle*\\%
 YlGnBu-4-4!70, every mark/.append style={solid,fill=YlGnBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-5}{%
 YlGnBu-5-1!70, every mark/.append style={solid,fill=YlGnBu-5-1},mark=*\\%
 YlGnBu-5-2!70, every mark/.append style={solid,fill=YlGnBu-5-2},mark=square*\\%
 YlGnBu-5-3!70, every mark/.append style={solid,fill=YlGnBu-5-3},mark=triangle*\\%
 YlGnBu-5-4!70, every mark/.append style={solid,fill=YlGnBu-5-4},mark=diamond*\\%
 YlGnBu-5-5!70, every mark/.append style={solid,fill=YlGnBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-6}{%
 YlGnBu-6-1!70, every mark/.append style={solid,fill=YlGnBu-6-1},mark=*\\%
 YlGnBu-6-2!70, every mark/.append style={solid,fill=YlGnBu-6-2},mark=square*\\%
 YlGnBu-6-3!70, every mark/.append style={solid,fill=YlGnBu-6-3},mark=triangle*\\%
 YlGnBu-6-4!70, every mark/.append style={solid,fill=YlGnBu-6-4},mark=diamond*\\%
 YlGnBu-6-5!70, every mark/.append style={solid,fill=YlGnBu-6-5},mark=pentagon*\\%
 YlGnBu-6-6!70, every mark/.append style={solid,fill=YlGnBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-7}{%
 YlGnBu-7-1!70, every mark/.append style={solid,fill=YlGnBu-7-1},mark=*\\%
 YlGnBu-7-2!70, every mark/.append style={solid,fill=YlGnBu-7-2},mark=square*\\%
 YlGnBu-7-3!70, every mark/.append style={solid,fill=YlGnBu-7-3},mark=triangle*\\%
 YlGnBu-7-4!70, every mark/.append style={solid,fill=YlGnBu-7-4},mark=diamond*\\%
 YlGnBu-7-5!70, every mark/.append style={solid,fill=YlGnBu-7-5},mark=pentagon*\\%
 YlGnBu-7-6!70, every mark/.append style={solid,fill=YlGnBu-7-6},mark=x\\%
 YlGnBu-7-7!70, every mark/.append style={solid,fill=YlGnBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-8}{%
 YlGnBu-8-1!70, every mark/.append style={solid,fill=YlGnBu-8-1},mark=*\\%
 YlGnBu-8-2!70, every mark/.append style={solid,fill=YlGnBu-8-2},mark=square*\\%
 YlGnBu-8-3!70, every mark/.append style={solid,fill=YlGnBu-8-3},mark=triangle*\\%
 YlGnBu-8-4!70, every mark/.append style={solid,fill=YlGnBu-8-4},mark=diamond*\\%
 YlGnBu-8-5!70, every mark/.append style={solid,fill=YlGnBu-8-5},mark=pentagon*\\%
 YlGnBu-8-6!70, every mark/.append style={solid,fill=YlGnBu-8-6},mark=x\\%
 YlGnBu-8-7!70, every mark/.append style={solid,fill=YlGnBu-8-7},mark=+\\%
 YlGnBu-8-8!70, every mark/.append style={solid,fill=YlGnBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlGnBu-9}{%
 YlGnBu-9-1!70, every mark/.append style={solid,fill=YlGnBu-9-1},mark=*\\%
 YlGnBu-9-2!70, every mark/.append style={solid,fill=YlGnBu-9-2},mark=square*\\%
 YlGnBu-9-3!70, every mark/.append style={solid,fill=YlGnBu-9-3},mark=triangle*\\%
 YlGnBu-9-4!70, every mark/.append style={solid,fill=YlGnBu-9-4},mark=diamond*\\%
 YlGnBu-9-5!70, every mark/.append style={solid,fill=YlGnBu-9-5},mark=pentagon*\\%
 YlGnBu-9-6!70, every mark/.append style={solid,fill=YlGnBu-9-6},mark=x\\%
 YlGnBu-9-7!70, every mark/.append style={solid,fill=YlGnBu-9-7},mark=+\\%
 YlGnBu-9-8!70, every mark/.append style={solid,fill=YlGnBu-9-8},mark=star\\%
 YlGnBu-9-9!70, every mark/.append style={solid,fill=YlGnBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-3}{%
 GnBu-3-1!70, every mark/.append style={solid,fill=GnBu-3-1},mark=*\\%
 GnBu-3-2!70, every mark/.append style={solid,fill=GnBu-3-2},mark=square*\\%
 GnBu-3-3!70, every mark/.append style={solid,fill=GnBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-4}{%
 GnBu-4-1!70, every mark/.append style={solid,fill=GnBu-4-1},mark=*\\%
 GnBu-4-2!70, every mark/.append style={solid,fill=GnBu-4-2},mark=square*\\%
 GnBu-4-3!70, every mark/.append style={solid,fill=GnBu-4-3},mark=triangle*\\%
 GnBu-4-4!70, every mark/.append style={solid,fill=GnBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-5}{%
 GnBu-5-1!70, every mark/.append style={solid,fill=GnBu-5-1},mark=*\\%
 GnBu-5-2!70, every mark/.append style={solid,fill=GnBu-5-2},mark=square*\\%
 GnBu-5-3!70, every mark/.append style={solid,fill=GnBu-5-3},mark=triangle*\\%
 GnBu-5-4!70, every mark/.append style={solid,fill=GnBu-5-4},mark=diamond*\\%
 GnBu-5-5!70, every mark/.append style={solid,fill=GnBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-6}{%
 GnBu-6-1!70, every mark/.append style={solid,fill=GnBu-6-1},mark=*\\%
 GnBu-6-2!70, every mark/.append style={solid,fill=GnBu-6-2},mark=square*\\%
 GnBu-6-3!70, every mark/.append style={solid,fill=GnBu-6-3},mark=triangle*\\%
 GnBu-6-4!70, every mark/.append style={solid,fill=GnBu-6-4},mark=diamond*\\%
 GnBu-6-5!70, every mark/.append style={solid,fill=GnBu-6-5},mark=pentagon*\\%
 GnBu-6-6!70, every mark/.append style={solid,fill=GnBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-7}{%
 GnBu-7-1!70, every mark/.append style={solid,fill=GnBu-7-1},mark=*\\%
 GnBu-7-2!70, every mark/.append style={solid,fill=GnBu-7-2},mark=square*\\%
 GnBu-7-3!70, every mark/.append style={solid,fill=GnBu-7-3},mark=triangle*\\%
 GnBu-7-4!70, every mark/.append style={solid,fill=GnBu-7-4},mark=diamond*\\%
 GnBu-7-5!70, every mark/.append style={solid,fill=GnBu-7-5},mark=pentagon*\\%
 GnBu-7-6!70, every mark/.append style={solid,fill=GnBu-7-6},mark=x\\%
 GnBu-7-7!70, every mark/.append style={solid,fill=GnBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-8}{%
 GnBu-8-1!70, every mark/.append style={solid,fill=GnBu-8-1},mark=*\\%
 GnBu-8-2!70, every mark/.append style={solid,fill=GnBu-8-2},mark=square*\\%
 GnBu-8-3!70, every mark/.append style={solid,fill=GnBu-8-3},mark=triangle*\\%
 GnBu-8-4!70, every mark/.append style={solid,fill=GnBu-8-4},mark=diamond*\\%
 GnBu-8-5!70, every mark/.append style={solid,fill=GnBu-8-5},mark=pentagon*\\%
 GnBu-8-6!70, every mark/.append style={solid,fill=GnBu-8-6},mark=x\\%
 GnBu-8-7!70, every mark/.append style={solid,fill=GnBu-8-7},mark=+\\%
 GnBu-8-8!70, every mark/.append style={solid,fill=GnBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-GnBu-9}{%
 GnBu-9-1!70, every mark/.append style={solid,fill=GnBu-9-1},mark=*\\%
 GnBu-9-2!70, every mark/.append style={solid,fill=GnBu-9-2},mark=square*\\%
 GnBu-9-3!70, every mark/.append style={solid,fill=GnBu-9-3},mark=triangle*\\%
 GnBu-9-4!70, every mark/.append style={solid,fill=GnBu-9-4},mark=diamond*\\%
 GnBu-9-5!70, every mark/.append style={solid,fill=GnBu-9-5},mark=pentagon*\\%
 GnBu-9-6!70, every mark/.append style={solid,fill=GnBu-9-6},mark=x\\%
 GnBu-9-7!70, every mark/.append style={solid,fill=GnBu-9-7},mark=+\\%
 GnBu-9-8!70, every mark/.append style={solid,fill=GnBu-9-8},mark=star\\%
 GnBu-9-9!70, every mark/.append style={solid,fill=GnBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-3}{%
 BuGn-3-1!70, every mark/.append style={solid,fill=BuGn-3-1},mark=*\\%
 BuGn-3-2!70, every mark/.append style={solid,fill=BuGn-3-2},mark=square*\\%
 BuGn-3-3!70, every mark/.append style={solid,fill=BuGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-4}{%
 BuGn-4-1!70, every mark/.append style={solid,fill=BuGn-4-1},mark=*\\%
 BuGn-4-2!70, every mark/.append style={solid,fill=BuGn-4-2},mark=square*\\%
 BuGn-4-3!70, every mark/.append style={solid,fill=BuGn-4-3},mark=triangle*\\%
 BuGn-4-4!70, every mark/.append style={solid,fill=BuGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-5}{%
 BuGn-5-1!70, every mark/.append style={solid,fill=BuGn-5-1},mark=*\\%
 BuGn-5-2!70, every mark/.append style={solid,fill=BuGn-5-2},mark=square*\\%
 BuGn-5-3!70, every mark/.append style={solid,fill=BuGn-5-3},mark=triangle*\\%
 BuGn-5-4!70, every mark/.append style={solid,fill=BuGn-5-4},mark=diamond*\\%
 BuGn-5-5!70, every mark/.append style={solid,fill=BuGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-6}{%
 BuGn-6-1!70, every mark/.append style={solid,fill=BuGn-6-1},mark=*\\%
 BuGn-6-2!70, every mark/.append style={solid,fill=BuGn-6-2},mark=square*\\%
 BuGn-6-3!70, every mark/.append style={solid,fill=BuGn-6-3},mark=triangle*\\%
 BuGn-6-4!70, every mark/.append style={solid,fill=BuGn-6-4},mark=diamond*\\%
 BuGn-6-5!70, every mark/.append style={solid,fill=BuGn-6-5},mark=pentagon*\\%
 BuGn-6-6!70, every mark/.append style={solid,fill=BuGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-7}{%
 BuGn-7-1!70, every mark/.append style={solid,fill=BuGn-7-1},mark=*\\%
 BuGn-7-2!70, every mark/.append style={solid,fill=BuGn-7-2},mark=square*\\%
 BuGn-7-3!70, every mark/.append style={solid,fill=BuGn-7-3},mark=triangle*\\%
 BuGn-7-4!70, every mark/.append style={solid,fill=BuGn-7-4},mark=diamond*\\%
 BuGn-7-5!70, every mark/.append style={solid,fill=BuGn-7-5},mark=pentagon*\\%
 BuGn-7-6!70, every mark/.append style={solid,fill=BuGn-7-6},mark=x\\%
 BuGn-7-7!70, every mark/.append style={solid,fill=BuGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-8}{%
 BuGn-8-1!70, every mark/.append style={solid,fill=BuGn-8-1},mark=*\\%
 BuGn-8-2!70, every mark/.append style={solid,fill=BuGn-8-2},mark=square*\\%
 BuGn-8-3!70, every mark/.append style={solid,fill=BuGn-8-3},mark=triangle*\\%
 BuGn-8-4!70, every mark/.append style={solid,fill=BuGn-8-4},mark=diamond*\\%
 BuGn-8-5!70, every mark/.append style={solid,fill=BuGn-8-5},mark=pentagon*\\%
 BuGn-8-6!70, every mark/.append style={solid,fill=BuGn-8-6},mark=x\\%
 BuGn-8-7!70, every mark/.append style={solid,fill=BuGn-8-7},mark=+\\%
 BuGn-8-8!70, every mark/.append style={solid,fill=BuGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuGn-9}{%
 BuGn-9-1!70, every mark/.append style={solid,fill=BuGn-9-1},mark=*\\%
 BuGn-9-2!70, every mark/.append style={solid,fill=BuGn-9-2},mark=square*\\%
 BuGn-9-3!70, every mark/.append style={solid,fill=BuGn-9-3},mark=triangle*\\%
 BuGn-9-4!70, every mark/.append style={solid,fill=BuGn-9-4},mark=diamond*\\%
 BuGn-9-5!70, every mark/.append style={solid,fill=BuGn-9-5},mark=pentagon*\\%
 BuGn-9-6!70, every mark/.append style={solid,fill=BuGn-9-6},mark=x\\%
 BuGn-9-7!70, every mark/.append style={solid,fill=BuGn-9-7},mark=+\\%
 BuGn-9-8!70, every mark/.append style={solid,fill=BuGn-9-8},mark=star\\%
 BuGn-9-9!70, every mark/.append style={solid,fill=BuGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-3}{%
 PuBuGn-3-1!70, every mark/.append style={solid,fill=PuBuGn-3-1},mark=*\\%
 PuBuGn-3-2!70, every mark/.append style={solid,fill=PuBuGn-3-2},mark=square*\\%
 PuBuGn-3-3!70, every mark/.append style={solid,fill=PuBuGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-4}{%
 PuBuGn-4-1!70, every mark/.append style={solid,fill=PuBuGn-4-1},mark=*\\%
 PuBuGn-4-2!70, every mark/.append style={solid,fill=PuBuGn-4-2},mark=square*\\%
 PuBuGn-4-3!70, every mark/.append style={solid,fill=PuBuGn-4-3},mark=triangle*\\%
 PuBuGn-4-4!70, every mark/.append style={solid,fill=PuBuGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-5}{%
 PuBuGn-5-1!70, every mark/.append style={solid,fill=PuBuGn-5-1},mark=*\\%
 PuBuGn-5-2!70, every mark/.append style={solid,fill=PuBuGn-5-2},mark=square*\\%
 PuBuGn-5-3!70, every mark/.append style={solid,fill=PuBuGn-5-3},mark=triangle*\\%
 PuBuGn-5-4!70, every mark/.append style={solid,fill=PuBuGn-5-4},mark=diamond*\\%
 PuBuGn-5-5!70, every mark/.append style={solid,fill=PuBuGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-6}{%
 PuBuGn-6-1!70, every mark/.append style={solid,fill=PuBuGn-6-1},mark=*\\%
 PuBuGn-6-2!70, every mark/.append style={solid,fill=PuBuGn-6-2},mark=square*\\%
 PuBuGn-6-3!70, every mark/.append style={solid,fill=PuBuGn-6-3},mark=triangle*\\%
 PuBuGn-6-4!70, every mark/.append style={solid,fill=PuBuGn-6-4},mark=diamond*\\%
 PuBuGn-6-5!70, every mark/.append style={solid,fill=PuBuGn-6-5},mark=pentagon*\\%
 PuBuGn-6-6!70, every mark/.append style={solid,fill=PuBuGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-7}{%
 PuBuGn-7-1!70, every mark/.append style={solid,fill=PuBuGn-7-1},mark=*\\%
 PuBuGn-7-2!70, every mark/.append style={solid,fill=PuBuGn-7-2},mark=square*\\%
 PuBuGn-7-3!70, every mark/.append style={solid,fill=PuBuGn-7-3},mark=triangle*\\%
 PuBuGn-7-4!70, every mark/.append style={solid,fill=PuBuGn-7-4},mark=diamond*\\%
 PuBuGn-7-5!70, every mark/.append style={solid,fill=PuBuGn-7-5},mark=pentagon*\\%
 PuBuGn-7-6!70, every mark/.append style={solid,fill=PuBuGn-7-6},mark=x\\%
 PuBuGn-7-7!70, every mark/.append style={solid,fill=PuBuGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-8}{%
 PuBuGn-8-1!70, every mark/.append style={solid,fill=PuBuGn-8-1},mark=*\\%
 PuBuGn-8-2!70, every mark/.append style={solid,fill=PuBuGn-8-2},mark=square*\\%
 PuBuGn-8-3!70, every mark/.append style={solid,fill=PuBuGn-8-3},mark=triangle*\\%
 PuBuGn-8-4!70, every mark/.append style={solid,fill=PuBuGn-8-4},mark=diamond*\\%
 PuBuGn-8-5!70, every mark/.append style={solid,fill=PuBuGn-8-5},mark=pentagon*\\%
 PuBuGn-8-6!70, every mark/.append style={solid,fill=PuBuGn-8-6},mark=x\\%
 PuBuGn-8-7!70, every mark/.append style={solid,fill=PuBuGn-8-7},mark=+\\%
 PuBuGn-8-8!70, every mark/.append style={solid,fill=PuBuGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBuGn-9}{%
 PuBuGn-9-1!70, every mark/.append style={solid,fill=PuBuGn-9-1},mark=*\\%
 PuBuGn-9-2!70, every mark/.append style={solid,fill=PuBuGn-9-2},mark=square*\\%
 PuBuGn-9-3!70, every mark/.append style={solid,fill=PuBuGn-9-3},mark=triangle*\\%
 PuBuGn-9-4!70, every mark/.append style={solid,fill=PuBuGn-9-4},mark=diamond*\\%
 PuBuGn-9-5!70, every mark/.append style={solid,fill=PuBuGn-9-5},mark=pentagon*\\%
 PuBuGn-9-6!70, every mark/.append style={solid,fill=PuBuGn-9-6},mark=x\\%
 PuBuGn-9-7!70, every mark/.append style={solid,fill=PuBuGn-9-7},mark=+\\%
 PuBuGn-9-8!70, every mark/.append style={solid,fill=PuBuGn-9-8},mark=star\\%
 PuBuGn-9-9!70, every mark/.append style={solid,fill=PuBuGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-3}{%
 PuBu-3-1!70, every mark/.append style={solid,fill=PuBu-3-1},mark=*\\%
 PuBu-3-2!70, every mark/.append style={solid,fill=PuBu-3-2},mark=square*\\%
 PuBu-3-3!70, every mark/.append style={solid,fill=PuBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-4}{%
 PuBu-4-1!70, every mark/.append style={solid,fill=PuBu-4-1},mark=*\\%
 PuBu-4-2!70, every mark/.append style={solid,fill=PuBu-4-2},mark=square*\\%
 PuBu-4-3!70, every mark/.append style={solid,fill=PuBu-4-3},mark=triangle*\\%
 PuBu-4-4!70, every mark/.append style={solid,fill=PuBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-5}{%
 PuBu-5-1!70, every mark/.append style={solid,fill=PuBu-5-1},mark=*\\%
 PuBu-5-2!70, every mark/.append style={solid,fill=PuBu-5-2},mark=square*\\%
 PuBu-5-3!70, every mark/.append style={solid,fill=PuBu-5-3},mark=triangle*\\%
 PuBu-5-4!70, every mark/.append style={solid,fill=PuBu-5-4},mark=diamond*\\%
 PuBu-5-5!70, every mark/.append style={solid,fill=PuBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-6}{%
 PuBu-6-1!70, every mark/.append style={solid,fill=PuBu-6-1},mark=*\\%
 PuBu-6-2!70, every mark/.append style={solid,fill=PuBu-6-2},mark=square*\\%
 PuBu-6-3!70, every mark/.append style={solid,fill=PuBu-6-3},mark=triangle*\\%
 PuBu-6-4!70, every mark/.append style={solid,fill=PuBu-6-4},mark=diamond*\\%
 PuBu-6-5!70, every mark/.append style={solid,fill=PuBu-6-5},mark=pentagon*\\%
 PuBu-6-6!70, every mark/.append style={solid,fill=PuBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-7}{%
 PuBu-7-1!70, every mark/.append style={solid,fill=PuBu-7-1},mark=*\\%
 PuBu-7-2!70, every mark/.append style={solid,fill=PuBu-7-2},mark=square*\\%
 PuBu-7-3!70, every mark/.append style={solid,fill=PuBu-7-3},mark=triangle*\\%
 PuBu-7-4!70, every mark/.append style={solid,fill=PuBu-7-4},mark=diamond*\\%
 PuBu-7-5!70, every mark/.append style={solid,fill=PuBu-7-5},mark=pentagon*\\%
 PuBu-7-6!70, every mark/.append style={solid,fill=PuBu-7-6},mark=x\\%
 PuBu-7-7!70, every mark/.append style={solid,fill=PuBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-8}{%
 PuBu-8-1!70, every mark/.append style={solid,fill=PuBu-8-1},mark=*\\%
 PuBu-8-2!70, every mark/.append style={solid,fill=PuBu-8-2},mark=square*\\%
 PuBu-8-3!70, every mark/.append style={solid,fill=PuBu-8-3},mark=triangle*\\%
 PuBu-8-4!70, every mark/.append style={solid,fill=PuBu-8-4},mark=diamond*\\%
 PuBu-8-5!70, every mark/.append style={solid,fill=PuBu-8-5},mark=pentagon*\\%
 PuBu-8-6!70, every mark/.append style={solid,fill=PuBu-8-6},mark=x\\%
 PuBu-8-7!70, every mark/.append style={solid,fill=PuBu-8-7},mark=+\\%
 PuBu-8-8!70, every mark/.append style={solid,fill=PuBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuBu-9}{%
 PuBu-9-1!70, every mark/.append style={solid,fill=PuBu-9-1},mark=*\\%
 PuBu-9-2!70, every mark/.append style={solid,fill=PuBu-9-2},mark=square*\\%
 PuBu-9-3!70, every mark/.append style={solid,fill=PuBu-9-3},mark=triangle*\\%
 PuBu-9-4!70, every mark/.append style={solid,fill=PuBu-9-4},mark=diamond*\\%
 PuBu-9-5!70, every mark/.append style={solid,fill=PuBu-9-5},mark=pentagon*\\%
 PuBu-9-6!70, every mark/.append style={solid,fill=PuBu-9-6},mark=x\\%
 PuBu-9-7!70, every mark/.append style={solid,fill=PuBu-9-7},mark=+\\%
 PuBu-9-8!70, every mark/.append style={solid,fill=PuBu-9-8},mark=star\\%
 PuBu-9-9!70, every mark/.append style={solid,fill=PuBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-3}{%
 BuPu-3-1!70, every mark/.append style={solid,fill=BuPu-3-1},mark=*\\%
 BuPu-3-2!70, every mark/.append style={solid,fill=BuPu-3-2},mark=square*\\%
 BuPu-3-3!70, every mark/.append style={solid,fill=BuPu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-4}{%
 BuPu-4-1!70, every mark/.append style={solid,fill=BuPu-4-1},mark=*\\%
 BuPu-4-2!70, every mark/.append style={solid,fill=BuPu-4-2},mark=square*\\%
 BuPu-4-3!70, every mark/.append style={solid,fill=BuPu-4-3},mark=triangle*\\%
 BuPu-4-4!70, every mark/.append style={solid,fill=BuPu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-5}{%
 BuPu-5-1!70, every mark/.append style={solid,fill=BuPu-5-1},mark=*\\%
 BuPu-5-2!70, every mark/.append style={solid,fill=BuPu-5-2},mark=square*\\%
 BuPu-5-3!70, every mark/.append style={solid,fill=BuPu-5-3},mark=triangle*\\%
 BuPu-5-4!70, every mark/.append style={solid,fill=BuPu-5-4},mark=diamond*\\%
 BuPu-5-5!70, every mark/.append style={solid,fill=BuPu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-6}{%
 BuPu-6-1!70, every mark/.append style={solid,fill=BuPu-6-1},mark=*\\%
 BuPu-6-2!70, every mark/.append style={solid,fill=BuPu-6-2},mark=square*\\%
 BuPu-6-3!70, every mark/.append style={solid,fill=BuPu-6-3},mark=triangle*\\%
 BuPu-6-4!70, every mark/.append style={solid,fill=BuPu-6-4},mark=diamond*\\%
 BuPu-6-5!70, every mark/.append style={solid,fill=BuPu-6-5},mark=pentagon*\\%
 BuPu-6-6!70, every mark/.append style={solid,fill=BuPu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-7}{%
 BuPu-7-1!70, every mark/.append style={solid,fill=BuPu-7-1},mark=*\\%
 BuPu-7-2!70, every mark/.append style={solid,fill=BuPu-7-2},mark=square*\\%
 BuPu-7-3!70, every mark/.append style={solid,fill=BuPu-7-3},mark=triangle*\\%
 BuPu-7-4!70, every mark/.append style={solid,fill=BuPu-7-4},mark=diamond*\\%
 BuPu-7-5!70, every mark/.append style={solid,fill=BuPu-7-5},mark=pentagon*\\%
 BuPu-7-6!70, every mark/.append style={solid,fill=BuPu-7-6},mark=x\\%
 BuPu-7-7!70, every mark/.append style={solid,fill=BuPu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-8}{%
 BuPu-8-1!70, every mark/.append style={solid,fill=BuPu-8-1},mark=*\\%
 BuPu-8-2!70, every mark/.append style={solid,fill=BuPu-8-2},mark=square*\\%
 BuPu-8-3!70, every mark/.append style={solid,fill=BuPu-8-3},mark=triangle*\\%
 BuPu-8-4!70, every mark/.append style={solid,fill=BuPu-8-4},mark=diamond*\\%
 BuPu-8-5!70, every mark/.append style={solid,fill=BuPu-8-5},mark=pentagon*\\%
 BuPu-8-6!70, every mark/.append style={solid,fill=BuPu-8-6},mark=x\\%
 BuPu-8-7!70, every mark/.append style={solid,fill=BuPu-8-7},mark=+\\%
 BuPu-8-8!70, every mark/.append style={solid,fill=BuPu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-BuPu-9}{%
 BuPu-9-1!70, every mark/.append style={solid,fill=BuPu-9-1},mark=*\\%
 BuPu-9-2!70, every mark/.append style={solid,fill=BuPu-9-2},mark=square*\\%
 BuPu-9-3!70, every mark/.append style={solid,fill=BuPu-9-3},mark=triangle*\\%
 BuPu-9-4!70, every mark/.append style={solid,fill=BuPu-9-4},mark=diamond*\\%
 BuPu-9-5!70, every mark/.append style={solid,fill=BuPu-9-5},mark=pentagon*\\%
 BuPu-9-6!70, every mark/.append style={solid,fill=BuPu-9-6},mark=x\\%
 BuPu-9-7!70, every mark/.append style={solid,fill=BuPu-9-7},mark=+\\%
 BuPu-9-8!70, every mark/.append style={solid,fill=BuPu-9-8},mark=star\\%
 BuPu-9-9!70, every mark/.append style={solid,fill=BuPu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-3}{%
 RdPu-3-1!70, every mark/.append style={solid,fill=RdPu-3-1},mark=*\\%
 RdPu-3-2!70, every mark/.append style={solid,fill=RdPu-3-2},mark=square*\\%
 RdPu-3-3!70, every mark/.append style={solid,fill=RdPu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-4}{%
 RdPu-4-1!70, every mark/.append style={solid,fill=RdPu-4-1},mark=*\\%
 RdPu-4-2!70, every mark/.append style={solid,fill=RdPu-4-2},mark=square*\\%
 RdPu-4-3!70, every mark/.append style={solid,fill=RdPu-4-3},mark=triangle*\\%
 RdPu-4-4!70, every mark/.append style={solid,fill=RdPu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-5}{%
 RdPu-5-1!70, every mark/.append style={solid,fill=RdPu-5-1},mark=*\\%
 RdPu-5-2!70, every mark/.append style={solid,fill=RdPu-5-2},mark=square*\\%
 RdPu-5-3!70, every mark/.append style={solid,fill=RdPu-5-3},mark=triangle*\\%
 RdPu-5-4!70, every mark/.append style={solid,fill=RdPu-5-4},mark=diamond*\\%
 RdPu-5-5!70, every mark/.append style={solid,fill=RdPu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-6}{%
 RdPu-6-1!70, every mark/.append style={solid,fill=RdPu-6-1},mark=*\\%
 RdPu-6-2!70, every mark/.append style={solid,fill=RdPu-6-2},mark=square*\\%
 RdPu-6-3!70, every mark/.append style={solid,fill=RdPu-6-3},mark=triangle*\\%
 RdPu-6-4!70, every mark/.append style={solid,fill=RdPu-6-4},mark=diamond*\\%
 RdPu-6-5!70, every mark/.append style={solid,fill=RdPu-6-5},mark=pentagon*\\%
 RdPu-6-6!70, every mark/.append style={solid,fill=RdPu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-7}{%
 RdPu-7-1!70, every mark/.append style={solid,fill=RdPu-7-1},mark=*\\%
 RdPu-7-2!70, every mark/.append style={solid,fill=RdPu-7-2},mark=square*\\%
 RdPu-7-3!70, every mark/.append style={solid,fill=RdPu-7-3},mark=triangle*\\%
 RdPu-7-4!70, every mark/.append style={solid,fill=RdPu-7-4},mark=diamond*\\%
 RdPu-7-5!70, every mark/.append style={solid,fill=RdPu-7-5},mark=pentagon*\\%
 RdPu-7-6!70, every mark/.append style={solid,fill=RdPu-7-6},mark=x\\%
 RdPu-7-7!70, every mark/.append style={solid,fill=RdPu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-8}{%
 RdPu-8-1!70, every mark/.append style={solid,fill=RdPu-8-1},mark=*\\%
 RdPu-8-2!70, every mark/.append style={solid,fill=RdPu-8-2},mark=square*\\%
 RdPu-8-3!70, every mark/.append style={solid,fill=RdPu-8-3},mark=triangle*\\%
 RdPu-8-4!70, every mark/.append style={solid,fill=RdPu-8-4},mark=diamond*\\%
 RdPu-8-5!70, every mark/.append style={solid,fill=RdPu-8-5},mark=pentagon*\\%
 RdPu-8-6!70, every mark/.append style={solid,fill=RdPu-8-6},mark=x\\%
 RdPu-8-7!70, every mark/.append style={solid,fill=RdPu-8-7},mark=+\\%
 RdPu-8-8!70, every mark/.append style={solid,fill=RdPu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdPu-9}{%
 RdPu-9-1!70, every mark/.append style={solid,fill=RdPu-9-1},mark=*\\%
 RdPu-9-2!70, every mark/.append style={solid,fill=RdPu-9-2},mark=square*\\%
 RdPu-9-3!70, every mark/.append style={solid,fill=RdPu-9-3},mark=triangle*\\%
 RdPu-9-4!70, every mark/.append style={solid,fill=RdPu-9-4},mark=diamond*\\%
 RdPu-9-5!70, every mark/.append style={solid,fill=RdPu-9-5},mark=pentagon*\\%
 RdPu-9-6!70, every mark/.append style={solid,fill=RdPu-9-6},mark=x\\%
 RdPu-9-7!70, every mark/.append style={solid,fill=RdPu-9-7},mark=+\\%
 RdPu-9-8!70, every mark/.append style={solid,fill=RdPu-9-8},mark=star\\%
 RdPu-9-9!70, every mark/.append style={solid,fill=RdPu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-3}{%
 PuRd-3-1!70, every mark/.append style={solid,fill=PuRd-3-1},mark=*\\%
 PuRd-3-2!70, every mark/.append style={solid,fill=PuRd-3-2},mark=square*\\%
 PuRd-3-3!70, every mark/.append style={solid,fill=PuRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-4}{%
 PuRd-4-1!70, every mark/.append style={solid,fill=PuRd-4-1},mark=*\\%
 PuRd-4-2!70, every mark/.append style={solid,fill=PuRd-4-2},mark=square*\\%
 PuRd-4-3!70, every mark/.append style={solid,fill=PuRd-4-3},mark=triangle*\\%
 PuRd-4-4!70, every mark/.append style={solid,fill=PuRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-5}{%
 PuRd-5-1!70, every mark/.append style={solid,fill=PuRd-5-1},mark=*\\%
 PuRd-5-2!70, every mark/.append style={solid,fill=PuRd-5-2},mark=square*\\%
 PuRd-5-3!70, every mark/.append style={solid,fill=PuRd-5-3},mark=triangle*\\%
 PuRd-5-4!70, every mark/.append style={solid,fill=PuRd-5-4},mark=diamond*\\%
 PuRd-5-5!70, every mark/.append style={solid,fill=PuRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-6}{%
 PuRd-6-1!70, every mark/.append style={solid,fill=PuRd-6-1},mark=*\\%
 PuRd-6-2!70, every mark/.append style={solid,fill=PuRd-6-2},mark=square*\\%
 PuRd-6-3!70, every mark/.append style={solid,fill=PuRd-6-3},mark=triangle*\\%
 PuRd-6-4!70, every mark/.append style={solid,fill=PuRd-6-4},mark=diamond*\\%
 PuRd-6-5!70, every mark/.append style={solid,fill=PuRd-6-5},mark=pentagon*\\%
 PuRd-6-6!70, every mark/.append style={solid,fill=PuRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-7}{%
 PuRd-7-1!70, every mark/.append style={solid,fill=PuRd-7-1},mark=*\\%
 PuRd-7-2!70, every mark/.append style={solid,fill=PuRd-7-2},mark=square*\\%
 PuRd-7-3!70, every mark/.append style={solid,fill=PuRd-7-3},mark=triangle*\\%
 PuRd-7-4!70, every mark/.append style={solid,fill=PuRd-7-4},mark=diamond*\\%
 PuRd-7-5!70, every mark/.append style={solid,fill=PuRd-7-5},mark=pentagon*\\%
 PuRd-7-6!70, every mark/.append style={solid,fill=PuRd-7-6},mark=x\\%
 PuRd-7-7!70, every mark/.append style={solid,fill=PuRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-8}{%
 PuRd-8-1!70, every mark/.append style={solid,fill=PuRd-8-1},mark=*\\%
 PuRd-8-2!70, every mark/.append style={solid,fill=PuRd-8-2},mark=square*\\%
 PuRd-8-3!70, every mark/.append style={solid,fill=PuRd-8-3},mark=triangle*\\%
 PuRd-8-4!70, every mark/.append style={solid,fill=PuRd-8-4},mark=diamond*\\%
 PuRd-8-5!70, every mark/.append style={solid,fill=PuRd-8-5},mark=pentagon*\\%
 PuRd-8-6!70, every mark/.append style={solid,fill=PuRd-8-6},mark=x\\%
 PuRd-8-7!70, every mark/.append style={solid,fill=PuRd-8-7},mark=+\\%
 PuRd-8-8!70, every mark/.append style={solid,fill=PuRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuRd-9}{%
 PuRd-9-1!70, every mark/.append style={solid,fill=PuRd-9-1},mark=*\\%
 PuRd-9-2!70, every mark/.append style={solid,fill=PuRd-9-2},mark=square*\\%
 PuRd-9-3!70, every mark/.append style={solid,fill=PuRd-9-3},mark=triangle*\\%
 PuRd-9-4!70, every mark/.append style={solid,fill=PuRd-9-4},mark=diamond*\\%
 PuRd-9-5!70, every mark/.append style={solid,fill=PuRd-9-5},mark=pentagon*\\%
 PuRd-9-6!70, every mark/.append style={solid,fill=PuRd-9-6},mark=x\\%
 PuRd-9-7!70, every mark/.append style={solid,fill=PuRd-9-7},mark=+\\%
 PuRd-9-8!70, every mark/.append style={solid,fill=PuRd-9-8},mark=star\\%
 PuRd-9-9!70, every mark/.append style={solid,fill=PuRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-3}{%
 OrRd-3-1!70, every mark/.append style={solid,fill=OrRd-3-1},mark=*\\%
 OrRd-3-2!70, every mark/.append style={solid,fill=OrRd-3-2},mark=square*\\%
 OrRd-3-3!70, every mark/.append style={solid,fill=OrRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-4}{%
 OrRd-4-1!70, every mark/.append style={solid,fill=OrRd-4-1},mark=*\\%
 OrRd-4-2!70, every mark/.append style={solid,fill=OrRd-4-2},mark=square*\\%
 OrRd-4-3!70, every mark/.append style={solid,fill=OrRd-4-3},mark=triangle*\\%
 OrRd-4-4!70, every mark/.append style={solid,fill=OrRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-5}{%
 OrRd-5-1!70, every mark/.append style={solid,fill=OrRd-5-1},mark=*\\%
 OrRd-5-2!70, every mark/.append style={solid,fill=OrRd-5-2},mark=square*\\%
 OrRd-5-3!70, every mark/.append style={solid,fill=OrRd-5-3},mark=triangle*\\%
 OrRd-5-4!70, every mark/.append style={solid,fill=OrRd-5-4},mark=diamond*\\%
 OrRd-5-5!70, every mark/.append style={solid,fill=OrRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-6}{%
 OrRd-6-1!70, every mark/.append style={solid,fill=OrRd-6-1},mark=*\\%
 OrRd-6-2!70, every mark/.append style={solid,fill=OrRd-6-2},mark=square*\\%
 OrRd-6-3!70, every mark/.append style={solid,fill=OrRd-6-3},mark=triangle*\\%
 OrRd-6-4!70, every mark/.append style={solid,fill=OrRd-6-4},mark=diamond*\\%
 OrRd-6-5!70, every mark/.append style={solid,fill=OrRd-6-5},mark=pentagon*\\%
 OrRd-6-6!70, every mark/.append style={solid,fill=OrRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-7}{%
 OrRd-7-1!70, every mark/.append style={solid,fill=OrRd-7-1},mark=*\\%
 OrRd-7-2!70, every mark/.append style={solid,fill=OrRd-7-2},mark=square*\\%
 OrRd-7-3!70, every mark/.append style={solid,fill=OrRd-7-3},mark=triangle*\\%
 OrRd-7-4!70, every mark/.append style={solid,fill=OrRd-7-4},mark=diamond*\\%
 OrRd-7-5!70, every mark/.append style={solid,fill=OrRd-7-5},mark=pentagon*\\%
 OrRd-7-6!70, every mark/.append style={solid,fill=OrRd-7-6},mark=x\\%
 OrRd-7-7!70, every mark/.append style={solid,fill=OrRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-8}{%
 OrRd-8-1!70, every mark/.append style={solid,fill=OrRd-8-1},mark=*\\%
 OrRd-8-2!70, every mark/.append style={solid,fill=OrRd-8-2},mark=square*\\%
 OrRd-8-3!70, every mark/.append style={solid,fill=OrRd-8-3},mark=triangle*\\%
 OrRd-8-4!70, every mark/.append style={solid,fill=OrRd-8-4},mark=diamond*\\%
 OrRd-8-5!70, every mark/.append style={solid,fill=OrRd-8-5},mark=pentagon*\\%
 OrRd-8-6!70, every mark/.append style={solid,fill=OrRd-8-6},mark=x\\%
 OrRd-8-7!70, every mark/.append style={solid,fill=OrRd-8-7},mark=+\\%
 OrRd-8-8!70, every mark/.append style={solid,fill=OrRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-OrRd-9}{%
 OrRd-9-1!70, every mark/.append style={solid,fill=OrRd-9-1},mark=*\\%
 OrRd-9-2!70, every mark/.append style={solid,fill=OrRd-9-2},mark=square*\\%
 OrRd-9-3!70, every mark/.append style={solid,fill=OrRd-9-3},mark=triangle*\\%
 OrRd-9-4!70, every mark/.append style={solid,fill=OrRd-9-4},mark=diamond*\\%
 OrRd-9-5!70, every mark/.append style={solid,fill=OrRd-9-5},mark=pentagon*\\%
 OrRd-9-6!70, every mark/.append style={solid,fill=OrRd-9-6},mark=x\\%
 OrRd-9-7!70, every mark/.append style={solid,fill=OrRd-9-7},mark=+\\%
 OrRd-9-8!70, every mark/.append style={solid,fill=OrRd-9-8},mark=star\\%
 OrRd-9-9!70, every mark/.append style={solid,fill=OrRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-3}{%
 YlOrRd-3-1!70, every mark/.append style={solid,fill=YlOrRd-3-1},mark=*\\%
 YlOrRd-3-2!70, every mark/.append style={solid,fill=YlOrRd-3-2},mark=square*\\%
 YlOrRd-3-3!70, every mark/.append style={solid,fill=YlOrRd-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-4}{%
 YlOrRd-4-1!70, every mark/.append style={solid,fill=YlOrRd-4-1},mark=*\\%
 YlOrRd-4-2!70, every mark/.append style={solid,fill=YlOrRd-4-2},mark=square*\\%
 YlOrRd-4-3!70, every mark/.append style={solid,fill=YlOrRd-4-3},mark=triangle*\\%
 YlOrRd-4-4!70, every mark/.append style={solid,fill=YlOrRd-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-5}{%
 YlOrRd-5-1!70, every mark/.append style={solid,fill=YlOrRd-5-1},mark=*\\%
 YlOrRd-5-2!70, every mark/.append style={solid,fill=YlOrRd-5-2},mark=square*\\%
 YlOrRd-5-3!70, every mark/.append style={solid,fill=YlOrRd-5-3},mark=triangle*\\%
 YlOrRd-5-4!70, every mark/.append style={solid,fill=YlOrRd-5-4},mark=diamond*\\%
 YlOrRd-5-5!70, every mark/.append style={solid,fill=YlOrRd-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-6}{%
 YlOrRd-6-1!70, every mark/.append style={solid,fill=YlOrRd-6-1},mark=*\\%
 YlOrRd-6-2!70, every mark/.append style={solid,fill=YlOrRd-6-2},mark=square*\\%
 YlOrRd-6-3!70, every mark/.append style={solid,fill=YlOrRd-6-3},mark=triangle*\\%
 YlOrRd-6-4!70, every mark/.append style={solid,fill=YlOrRd-6-4},mark=diamond*\\%
 YlOrRd-6-5!70, every mark/.append style={solid,fill=YlOrRd-6-5},mark=pentagon*\\%
 YlOrRd-6-6!70, every mark/.append style={solid,fill=YlOrRd-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-7}{%
 YlOrRd-7-1!70, every mark/.append style={solid,fill=YlOrRd-7-1},mark=*\\%
 YlOrRd-7-2!70, every mark/.append style={solid,fill=YlOrRd-7-2},mark=square*\\%
 YlOrRd-7-3!70, every mark/.append style={solid,fill=YlOrRd-7-3},mark=triangle*\\%
 YlOrRd-7-4!70, every mark/.append style={solid,fill=YlOrRd-7-4},mark=diamond*\\%
 YlOrRd-7-5!70, every mark/.append style={solid,fill=YlOrRd-7-5},mark=pentagon*\\%
 YlOrRd-7-6!70, every mark/.append style={solid,fill=YlOrRd-7-6},mark=x\\%
 YlOrRd-7-7!70, every mark/.append style={solid,fill=YlOrRd-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-8}{%
 YlOrRd-8-1!70, every mark/.append style={solid,fill=YlOrRd-8-1},mark=*\\%
 YlOrRd-8-2!70, every mark/.append style={solid,fill=YlOrRd-8-2},mark=square*\\%
 YlOrRd-8-3!70, every mark/.append style={solid,fill=YlOrRd-8-3},mark=triangle*\\%
 YlOrRd-8-4!70, every mark/.append style={solid,fill=YlOrRd-8-4},mark=diamond*\\%
 YlOrRd-8-5!70, every mark/.append style={solid,fill=YlOrRd-8-5},mark=pentagon*\\%
 YlOrRd-8-6!70, every mark/.append style={solid,fill=YlOrRd-8-6},mark=x\\%
 YlOrRd-8-7!70, every mark/.append style={solid,fill=YlOrRd-8-7},mark=+\\%
 YlOrRd-8-8!70, every mark/.append style={solid,fill=YlOrRd-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrRd-9}{%
 YlOrRd-9-1!70, every mark/.append style={solid,fill=YlOrRd-9-1},mark=*\\%
 YlOrRd-9-2!70, every mark/.append style={solid,fill=YlOrRd-9-2},mark=square*\\%
 YlOrRd-9-3!70, every mark/.append style={solid,fill=YlOrRd-9-3},mark=triangle*\\%
 YlOrRd-9-4!70, every mark/.append style={solid,fill=YlOrRd-9-4},mark=diamond*\\%
 YlOrRd-9-5!70, every mark/.append style={solid,fill=YlOrRd-9-5},mark=pentagon*\\%
 YlOrRd-9-6!70, every mark/.append style={solid,fill=YlOrRd-9-6},mark=x\\%
 YlOrRd-9-7!70, every mark/.append style={solid,fill=YlOrRd-9-7},mark=+\\%
 YlOrRd-9-8!70, every mark/.append style={solid,fill=YlOrRd-9-8},mark=star\\%
 YlOrRd-9-9!70, every mark/.append style={solid,fill=YlOrRd-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-3}{%
 YlOrBr-3-1!70, every mark/.append style={solid,fill=YlOrBr-3-1},mark=*\\%
 YlOrBr-3-2!70, every mark/.append style={solid,fill=YlOrBr-3-2},mark=square*\\%
 YlOrBr-3-3!70, every mark/.append style={solid,fill=YlOrBr-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-4}{%
 YlOrBr-4-1!70, every mark/.append style={solid,fill=YlOrBr-4-1},mark=*\\%
 YlOrBr-4-2!70, every mark/.append style={solid,fill=YlOrBr-4-2},mark=square*\\%
 YlOrBr-4-3!70, every mark/.append style={solid,fill=YlOrBr-4-3},mark=triangle*\\%
 YlOrBr-4-4!70, every mark/.append style={solid,fill=YlOrBr-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-5}{%
 YlOrBr-5-1!70, every mark/.append style={solid,fill=YlOrBr-5-1},mark=*\\%
 YlOrBr-5-2!70, every mark/.append style={solid,fill=YlOrBr-5-2},mark=square*\\%
 YlOrBr-5-3!70, every mark/.append style={solid,fill=YlOrBr-5-3},mark=triangle*\\%
 YlOrBr-5-4!70, every mark/.append style={solid,fill=YlOrBr-5-4},mark=diamond*\\%
 YlOrBr-5-5!70, every mark/.append style={solid,fill=YlOrBr-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-6}{%
 YlOrBr-6-1!70, every mark/.append style={solid,fill=YlOrBr-6-1},mark=*\\%
 YlOrBr-6-2!70, every mark/.append style={solid,fill=YlOrBr-6-2},mark=square*\\%
 YlOrBr-6-3!70, every mark/.append style={solid,fill=YlOrBr-6-3},mark=triangle*\\%
 YlOrBr-6-4!70, every mark/.append style={solid,fill=YlOrBr-6-4},mark=diamond*\\%
 YlOrBr-6-5!70, every mark/.append style={solid,fill=YlOrBr-6-5},mark=pentagon*\\%
 YlOrBr-6-6!70, every mark/.append style={solid,fill=YlOrBr-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-7}{%
 YlOrBr-7-1!70, every mark/.append style={solid,fill=YlOrBr-7-1},mark=*\\%
 YlOrBr-7-2!70, every mark/.append style={solid,fill=YlOrBr-7-2},mark=square*\\%
 YlOrBr-7-3!70, every mark/.append style={solid,fill=YlOrBr-7-3},mark=triangle*\\%
 YlOrBr-7-4!70, every mark/.append style={solid,fill=YlOrBr-7-4},mark=diamond*\\%
 YlOrBr-7-5!70, every mark/.append style={solid,fill=YlOrBr-7-5},mark=pentagon*\\%
 YlOrBr-7-6!70, every mark/.append style={solid,fill=YlOrBr-7-6},mark=x\\%
 YlOrBr-7-7!70, every mark/.append style={solid,fill=YlOrBr-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-8}{%
 YlOrBr-8-1!70, every mark/.append style={solid,fill=YlOrBr-8-1},mark=*\\%
 YlOrBr-8-2!70, every mark/.append style={solid,fill=YlOrBr-8-2},mark=square*\\%
 YlOrBr-8-3!70, every mark/.append style={solid,fill=YlOrBr-8-3},mark=triangle*\\%
 YlOrBr-8-4!70, every mark/.append style={solid,fill=YlOrBr-8-4},mark=diamond*\\%
 YlOrBr-8-5!70, every mark/.append style={solid,fill=YlOrBr-8-5},mark=pentagon*\\%
 YlOrBr-8-6!70, every mark/.append style={solid,fill=YlOrBr-8-6},mark=x\\%
 YlOrBr-8-7!70, every mark/.append style={solid,fill=YlOrBr-8-7},mark=+\\%
 YlOrBr-8-8!70, every mark/.append style={solid,fill=YlOrBr-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-YlOrBr-9}{%
 YlOrBr-9-1!70, every mark/.append style={solid,fill=YlOrBr-9-1},mark=*\\%
 YlOrBr-9-2!70, every mark/.append style={solid,fill=YlOrBr-9-2},mark=square*\\%
 YlOrBr-9-3!70, every mark/.append style={solid,fill=YlOrBr-9-3},mark=triangle*\\%
 YlOrBr-9-4!70, every mark/.append style={solid,fill=YlOrBr-9-4},mark=diamond*\\%
 YlOrBr-9-5!70, every mark/.append style={solid,fill=YlOrBr-9-5},mark=pentagon*\\%
 YlOrBr-9-6!70, every mark/.append style={solid,fill=YlOrBr-9-6},mark=x\\%
 YlOrBr-9-7!70, every mark/.append style={solid,fill=YlOrBr-9-7},mark=+\\%
 YlOrBr-9-8!70, every mark/.append style={solid,fill=YlOrBr-9-8},mark=star\\%
 YlOrBr-9-9!70, every mark/.append style={solid,fill=YlOrBr-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-3}{%
 Purples-3-1!70, every mark/.append style={solid,fill=Purples-3-1},mark=*\\%
 Purples-3-2!70, every mark/.append style={solid,fill=Purples-3-2},mark=square*\\%
 Purples-3-3!70, every mark/.append style={solid,fill=Purples-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-4}{%
 Purples-4-1!70, every mark/.append style={solid,fill=Purples-4-1},mark=*\\%
 Purples-4-2!70, every mark/.append style={solid,fill=Purples-4-2},mark=square*\\%
 Purples-4-3!70, every mark/.append style={solid,fill=Purples-4-3},mark=triangle*\\%
 Purples-4-4!70, every mark/.append style={solid,fill=Purples-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-5}{%
 Purples-5-1!70, every mark/.append style={solid,fill=Purples-5-1},mark=*\\%
 Purples-5-2!70, every mark/.append style={solid,fill=Purples-5-2},mark=square*\\%
 Purples-5-3!70, every mark/.append style={solid,fill=Purples-5-3},mark=triangle*\\%
 Purples-5-4!70, every mark/.append style={solid,fill=Purples-5-4},mark=diamond*\\%
 Purples-5-5!70, every mark/.append style={solid,fill=Purples-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-6}{%
 Purples-6-1!70, every mark/.append style={solid,fill=Purples-6-1},mark=*\\%
 Purples-6-2!70, every mark/.append style={solid,fill=Purples-6-2},mark=square*\\%
 Purples-6-3!70, every mark/.append style={solid,fill=Purples-6-3},mark=triangle*\\%
 Purples-6-4!70, every mark/.append style={solid,fill=Purples-6-4},mark=diamond*\\%
 Purples-6-5!70, every mark/.append style={solid,fill=Purples-6-5},mark=pentagon*\\%
 Purples-6-6!70, every mark/.append style={solid,fill=Purples-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-7}{%
 Purples-7-1!70, every mark/.append style={solid,fill=Purples-7-1},mark=*\\%
 Purples-7-2!70, every mark/.append style={solid,fill=Purples-7-2},mark=square*\\%
 Purples-7-3!70, every mark/.append style={solid,fill=Purples-7-3},mark=triangle*\\%
 Purples-7-4!70, every mark/.append style={solid,fill=Purples-7-4},mark=diamond*\\%
 Purples-7-5!70, every mark/.append style={solid,fill=Purples-7-5},mark=pentagon*\\%
 Purples-7-6!70, every mark/.append style={solid,fill=Purples-7-6},mark=x\\%
 Purples-7-7!70, every mark/.append style={solid,fill=Purples-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-8}{%
 Purples-8-1!70, every mark/.append style={solid,fill=Purples-8-1},mark=*\\%
 Purples-8-2!70, every mark/.append style={solid,fill=Purples-8-2},mark=square*\\%
 Purples-8-3!70, every mark/.append style={solid,fill=Purples-8-3},mark=triangle*\\%
 Purples-8-4!70, every mark/.append style={solid,fill=Purples-8-4},mark=diamond*\\%
 Purples-8-5!70, every mark/.append style={solid,fill=Purples-8-5},mark=pentagon*\\%
 Purples-8-6!70, every mark/.append style={solid,fill=Purples-8-6},mark=x\\%
 Purples-8-7!70, every mark/.append style={solid,fill=Purples-8-7},mark=+\\%
 Purples-8-8!70, every mark/.append style={solid,fill=Purples-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Purples-9}{%
 Purples-9-1!70, every mark/.append style={solid,fill=Purples-9-1},mark=*\\%
 Purples-9-2!70, every mark/.append style={solid,fill=Purples-9-2},mark=square*\\%
 Purples-9-3!70, every mark/.append style={solid,fill=Purples-9-3},mark=triangle*\\%
 Purples-9-4!70, every mark/.append style={solid,fill=Purples-9-4},mark=diamond*\\%
 Purples-9-5!70, every mark/.append style={solid,fill=Purples-9-5},mark=pentagon*\\%
 Purples-9-6!70, every mark/.append style={solid,fill=Purples-9-6},mark=x\\%
 Purples-9-7!70, every mark/.append style={solid,fill=Purples-9-7},mark=+\\%
 Purples-9-8!70, every mark/.append style={solid,fill=Purples-9-8},mark=star\\%
 Purples-9-9!70, every mark/.append style={solid,fill=Purples-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-3}{%
 Blues-3-1!70, every mark/.append style={solid,fill=Blues-3-1},mark=*\\%
 Blues-3-2!70, every mark/.append style={solid,fill=Blues-3-2},mark=square*\\%
 Blues-3-3!70, every mark/.append style={solid,fill=Blues-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-4}{%
 Blues-4-1!70, every mark/.append style={solid,fill=Blues-4-1},mark=*\\%
 Blues-4-2!70, every mark/.append style={solid,fill=Blues-4-2},mark=square*\\%
 Blues-4-3!70, every mark/.append style={solid,fill=Blues-4-3},mark=triangle*\\%
 Blues-4-4!70, every mark/.append style={solid,fill=Blues-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-5}{%
 Blues-5-1!70, every mark/.append style={solid,fill=Blues-5-1},mark=*\\%
 Blues-5-2!70, every mark/.append style={solid,fill=Blues-5-2},mark=square*\\%
 Blues-5-3!70, every mark/.append style={solid,fill=Blues-5-3},mark=triangle*\\%
 Blues-5-4!70, every mark/.append style={solid,fill=Blues-5-4},mark=diamond*\\%
 Blues-5-5!70, every mark/.append style={solid,fill=Blues-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-6}{%
 Blues-6-1!70, every mark/.append style={solid,fill=Blues-6-1},mark=*\\%
 Blues-6-2!70, every mark/.append style={solid,fill=Blues-6-2},mark=square*\\%
 Blues-6-3!70, every mark/.append style={solid,fill=Blues-6-3},mark=triangle*\\%
 Blues-6-4!70, every mark/.append style={solid,fill=Blues-6-4},mark=diamond*\\%
 Blues-6-5!70, every mark/.append style={solid,fill=Blues-6-5},mark=pentagon*\\%
 Blues-6-6!70, every mark/.append style={solid,fill=Blues-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-7}{%
 Blues-7-1!70, every mark/.append style={solid,fill=Blues-7-1},mark=*\\%
 Blues-7-2!70, every mark/.append style={solid,fill=Blues-7-2},mark=square*\\%
 Blues-7-3!70, every mark/.append style={solid,fill=Blues-7-3},mark=triangle*\\%
 Blues-7-4!70, every mark/.append style={solid,fill=Blues-7-4},mark=diamond*\\%
 Blues-7-5!70, every mark/.append style={solid,fill=Blues-7-5},mark=pentagon*\\%
 Blues-7-6!70, every mark/.append style={solid,fill=Blues-7-6},mark=x\\%
 Blues-7-7!70, every mark/.append style={solid,fill=Blues-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-8}{%
 Blues-8-1!70, every mark/.append style={solid,fill=Blues-8-1},mark=*\\%
 Blues-8-2!70, every mark/.append style={solid,fill=Blues-8-2},mark=square*\\%
 Blues-8-3!70, every mark/.append style={solid,fill=Blues-8-3},mark=triangle*\\%
 Blues-8-4!70, every mark/.append style={solid,fill=Blues-8-4},mark=diamond*\\%
 Blues-8-5!70, every mark/.append style={solid,fill=Blues-8-5},mark=pentagon*\\%
 Blues-8-6!70, every mark/.append style={solid,fill=Blues-8-6},mark=x\\%
 Blues-8-7!70, every mark/.append style={solid,fill=Blues-8-7},mark=+\\%
 Blues-8-8!70, every mark/.append style={solid,fill=Blues-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Blues-9}{%
 Blues-9-1!70, every mark/.append style={solid,fill=Blues-9-1},mark=*\\%
 Blues-9-2!70, every mark/.append style={solid,fill=Blues-9-2},mark=square*\\%
 Blues-9-3!70, every mark/.append style={solid,fill=Blues-9-3},mark=triangle*\\%
 Blues-9-4!70, every mark/.append style={solid,fill=Blues-9-4},mark=diamond*\\%
 Blues-9-5!70, every mark/.append style={solid,fill=Blues-9-5},mark=pentagon*\\%
 Blues-9-6!70, every mark/.append style={solid,fill=Blues-9-6},mark=x\\%
 Blues-9-7!70, every mark/.append style={solid,fill=Blues-9-7},mark=+\\%
 Blues-9-8!70, every mark/.append style={solid,fill=Blues-9-8},mark=star\\%
 Blues-9-9!70, every mark/.append style={solid,fill=Blues-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-3}{%
 Greens-3-1!70, every mark/.append style={solid,fill=Greens-3-1},mark=*\\%
 Greens-3-2!70, every mark/.append style={solid,fill=Greens-3-2},mark=square*\\%
 Greens-3-3!70, every mark/.append style={solid,fill=Greens-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-4}{%
 Greens-4-1!70, every mark/.append style={solid,fill=Greens-4-1},mark=*\\%
 Greens-4-2!70, every mark/.append style={solid,fill=Greens-4-2},mark=square*\\%
 Greens-4-3!70, every mark/.append style={solid,fill=Greens-4-3},mark=triangle*\\%
 Greens-4-4!70, every mark/.append style={solid,fill=Greens-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-5}{%
 Greens-5-1!70, every mark/.append style={solid,fill=Greens-5-1},mark=*\\%
 Greens-5-2!70, every mark/.append style={solid,fill=Greens-5-2},mark=square*\\%
 Greens-5-3!70, every mark/.append style={solid,fill=Greens-5-3},mark=triangle*\\%
 Greens-5-4!70, every mark/.append style={solid,fill=Greens-5-4},mark=diamond*\\%
 Greens-5-5!70, every mark/.append style={solid,fill=Greens-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-6}{%
 Greens-6-1!70, every mark/.append style={solid,fill=Greens-6-1},mark=*\\%
 Greens-6-2!70, every mark/.append style={solid,fill=Greens-6-2},mark=square*\\%
 Greens-6-3!70, every mark/.append style={solid,fill=Greens-6-3},mark=triangle*\\%
 Greens-6-4!70, every mark/.append style={solid,fill=Greens-6-4},mark=diamond*\\%
 Greens-6-5!70, every mark/.append style={solid,fill=Greens-6-5},mark=pentagon*\\%
 Greens-6-6!70, every mark/.append style={solid,fill=Greens-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-7}{%
 Greens-7-1!70, every mark/.append style={solid,fill=Greens-7-1},mark=*\\%
 Greens-7-2!70, every mark/.append style={solid,fill=Greens-7-2},mark=square*\\%
 Greens-7-3!70, every mark/.append style={solid,fill=Greens-7-3},mark=triangle*\\%
 Greens-7-4!70, every mark/.append style={solid,fill=Greens-7-4},mark=diamond*\\%
 Greens-7-5!70, every mark/.append style={solid,fill=Greens-7-5},mark=pentagon*\\%
 Greens-7-6!70, every mark/.append style={solid,fill=Greens-7-6},mark=x\\%
 Greens-7-7!70, every mark/.append style={solid,fill=Greens-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-8}{%
 Greens-8-1!70, every mark/.append style={solid,fill=Greens-8-1},mark=*\\%
 Greens-8-2!70, every mark/.append style={solid,fill=Greens-8-2},mark=square*\\%
 Greens-8-3!70, every mark/.append style={solid,fill=Greens-8-3},mark=triangle*\\%
 Greens-8-4!70, every mark/.append style={solid,fill=Greens-8-4},mark=diamond*\\%
 Greens-8-5!70, every mark/.append style={solid,fill=Greens-8-5},mark=pentagon*\\%
 Greens-8-6!70, every mark/.append style={solid,fill=Greens-8-6},mark=x\\%
 Greens-8-7!70, every mark/.append style={solid,fill=Greens-8-7},mark=+\\%
 Greens-8-8!70, every mark/.append style={solid,fill=Greens-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greens-9}{%
 Greens-9-1!70, every mark/.append style={solid,fill=Greens-9-1},mark=*\\%
 Greens-9-2!70, every mark/.append style={solid,fill=Greens-9-2},mark=square*\\%
 Greens-9-3!70, every mark/.append style={solid,fill=Greens-9-3},mark=triangle*\\%
 Greens-9-4!70, every mark/.append style={solid,fill=Greens-9-4},mark=diamond*\\%
 Greens-9-5!70, every mark/.append style={solid,fill=Greens-9-5},mark=pentagon*\\%
 Greens-9-6!70, every mark/.append style={solid,fill=Greens-9-6},mark=x\\%
 Greens-9-7!70, every mark/.append style={solid,fill=Greens-9-7},mark=+\\%
 Greens-9-8!70, every mark/.append style={solid,fill=Greens-9-8},mark=star\\%
 Greens-9-9!70, every mark/.append style={solid,fill=Greens-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-3}{%
 Oranges-3-1!70, every mark/.append style={solid,fill=Oranges-3-1},mark=*\\%
 Oranges-3-2!70, every mark/.append style={solid,fill=Oranges-3-2},mark=square*\\%
 Oranges-3-3!70, every mark/.append style={solid,fill=Oranges-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-4}{%
 Oranges-4-1!70, every mark/.append style={solid,fill=Oranges-4-1},mark=*\\%
 Oranges-4-2!70, every mark/.append style={solid,fill=Oranges-4-2},mark=square*\\%
 Oranges-4-3!70, every mark/.append style={solid,fill=Oranges-4-3},mark=triangle*\\%
 Oranges-4-4!70, every mark/.append style={solid,fill=Oranges-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-5}{%
 Oranges-5-1!70, every mark/.append style={solid,fill=Oranges-5-1},mark=*\\%
 Oranges-5-2!70, every mark/.append style={solid,fill=Oranges-5-2},mark=square*\\%
 Oranges-5-3!70, every mark/.append style={solid,fill=Oranges-5-3},mark=triangle*\\%
 Oranges-5-4!70, every mark/.append style={solid,fill=Oranges-5-4},mark=diamond*\\%
 Oranges-5-5!70, every mark/.append style={solid,fill=Oranges-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-6}{%
 Oranges-6-1!70, every mark/.append style={solid,fill=Oranges-6-1},mark=*\\%
 Oranges-6-2!70, every mark/.append style={solid,fill=Oranges-6-2},mark=square*\\%
 Oranges-6-3!70, every mark/.append style={solid,fill=Oranges-6-3},mark=triangle*\\%
 Oranges-6-4!70, every mark/.append style={solid,fill=Oranges-6-4},mark=diamond*\\%
 Oranges-6-5!70, every mark/.append style={solid,fill=Oranges-6-5},mark=pentagon*\\%
 Oranges-6-6!70, every mark/.append style={solid,fill=Oranges-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-7}{%
 Oranges-7-1!70, every mark/.append style={solid,fill=Oranges-7-1},mark=*\\%
 Oranges-7-2!70, every mark/.append style={solid,fill=Oranges-7-2},mark=square*\\%
 Oranges-7-3!70, every mark/.append style={solid,fill=Oranges-7-3},mark=triangle*\\%
 Oranges-7-4!70, every mark/.append style={solid,fill=Oranges-7-4},mark=diamond*\\%
 Oranges-7-5!70, every mark/.append style={solid,fill=Oranges-7-5},mark=pentagon*\\%
 Oranges-7-6!70, every mark/.append style={solid,fill=Oranges-7-6},mark=x\\%
 Oranges-7-7!70, every mark/.append style={solid,fill=Oranges-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-8}{%
 Oranges-8-1!70, every mark/.append style={solid,fill=Oranges-8-1},mark=*\\%
 Oranges-8-2!70, every mark/.append style={solid,fill=Oranges-8-2},mark=square*\\%
 Oranges-8-3!70, every mark/.append style={solid,fill=Oranges-8-3},mark=triangle*\\%
 Oranges-8-4!70, every mark/.append style={solid,fill=Oranges-8-4},mark=diamond*\\%
 Oranges-8-5!70, every mark/.append style={solid,fill=Oranges-8-5},mark=pentagon*\\%
 Oranges-8-6!70, every mark/.append style={solid,fill=Oranges-8-6},mark=x\\%
 Oranges-8-7!70, every mark/.append style={solid,fill=Oranges-8-7},mark=+\\%
 Oranges-8-8!70, every mark/.append style={solid,fill=Oranges-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Oranges-9}{%
 Oranges-9-1!70, every mark/.append style={solid,fill=Oranges-9-1},mark=*\\%
 Oranges-9-2!70, every mark/.append style={solid,fill=Oranges-9-2},mark=square*\\%
 Oranges-9-3!70, every mark/.append style={solid,fill=Oranges-9-3},mark=triangle*\\%
 Oranges-9-4!70, every mark/.append style={solid,fill=Oranges-9-4},mark=diamond*\\%
 Oranges-9-5!70, every mark/.append style={solid,fill=Oranges-9-5},mark=pentagon*\\%
 Oranges-9-6!70, every mark/.append style={solid,fill=Oranges-9-6},mark=x\\%
 Oranges-9-7!70, every mark/.append style={solid,fill=Oranges-9-7},mark=+\\%
 Oranges-9-8!70, every mark/.append style={solid,fill=Oranges-9-8},mark=star\\%
 Oranges-9-9!70, every mark/.append style={solid,fill=Oranges-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-3}{%
 Reds-3-1!70, every mark/.append style={solid,fill=Reds-3-1},mark=*\\%
 Reds-3-2!70, every mark/.append style={solid,fill=Reds-3-2},mark=square*\\%
 Reds-3-3!70, every mark/.append style={solid,fill=Reds-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-4}{%
 Reds-4-1!70, every mark/.append style={solid,fill=Reds-4-1},mark=*\\%
 Reds-4-2!70, every mark/.append style={solid,fill=Reds-4-2},mark=square*\\%
 Reds-4-3!70, every mark/.append style={solid,fill=Reds-4-3},mark=triangle*\\%
 Reds-4-4!70, every mark/.append style={solid,fill=Reds-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-5}{%
 Reds-5-1!70, every mark/.append style={solid,fill=Reds-5-1},mark=*\\%
 Reds-5-2!70, every mark/.append style={solid,fill=Reds-5-2},mark=square*\\%
 Reds-5-3!70, every mark/.append style={solid,fill=Reds-5-3},mark=triangle*\\%
 Reds-5-4!70, every mark/.append style={solid,fill=Reds-5-4},mark=diamond*\\%
 Reds-5-5!70, every mark/.append style={solid,fill=Reds-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-6}{%
 Reds-6-1!70, every mark/.append style={solid,fill=Reds-6-1},mark=*\\%
 Reds-6-2!70, every mark/.append style={solid,fill=Reds-6-2},mark=square*\\%
 Reds-6-3!70, every mark/.append style={solid,fill=Reds-6-3},mark=triangle*\\%
 Reds-6-4!70, every mark/.append style={solid,fill=Reds-6-4},mark=diamond*\\%
 Reds-6-5!70, every mark/.append style={solid,fill=Reds-6-5},mark=pentagon*\\%
 Reds-6-6!70, every mark/.append style={solid,fill=Reds-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-7}{%
 Reds-7-1!70, every mark/.append style={solid,fill=Reds-7-1},mark=*\\%
 Reds-7-2!70, every mark/.append style={solid,fill=Reds-7-2},mark=square*\\%
 Reds-7-3!70, every mark/.append style={solid,fill=Reds-7-3},mark=triangle*\\%
 Reds-7-4!70, every mark/.append style={solid,fill=Reds-7-4},mark=diamond*\\%
 Reds-7-5!70, every mark/.append style={solid,fill=Reds-7-5},mark=pentagon*\\%
 Reds-7-6!70, every mark/.append style={solid,fill=Reds-7-6},mark=x\\%
 Reds-7-7!70, every mark/.append style={solid,fill=Reds-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-8}{%
 Reds-8-1!70, every mark/.append style={solid,fill=Reds-8-1},mark=*\\%
 Reds-8-2!70, every mark/.append style={solid,fill=Reds-8-2},mark=square*\\%
 Reds-8-3!70, every mark/.append style={solid,fill=Reds-8-3},mark=triangle*\\%
 Reds-8-4!70, every mark/.append style={solid,fill=Reds-8-4},mark=diamond*\\%
 Reds-8-5!70, every mark/.append style={solid,fill=Reds-8-5},mark=pentagon*\\%
 Reds-8-6!70, every mark/.append style={solid,fill=Reds-8-6},mark=x\\%
 Reds-8-7!70, every mark/.append style={solid,fill=Reds-8-7},mark=+\\%
 Reds-8-8!70, every mark/.append style={solid,fill=Reds-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Reds-9}{%
 Reds-9-1!70, every mark/.append style={solid,fill=Reds-9-1},mark=*\\%
 Reds-9-2!70, every mark/.append style={solid,fill=Reds-9-2},mark=square*\\%
 Reds-9-3!70, every mark/.append style={solid,fill=Reds-9-3},mark=triangle*\\%
 Reds-9-4!70, every mark/.append style={solid,fill=Reds-9-4},mark=diamond*\\%
 Reds-9-5!70, every mark/.append style={solid,fill=Reds-9-5},mark=pentagon*\\%
 Reds-9-6!70, every mark/.append style={solid,fill=Reds-9-6},mark=x\\%
 Reds-9-7!70, every mark/.append style={solid,fill=Reds-9-7},mark=+\\%
 Reds-9-8!70, every mark/.append style={solid,fill=Reds-9-8},mark=star\\%
 Reds-9-9!70, every mark/.append style={solid,fill=Reds-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-3}{%
 Greys-3-1!70, every mark/.append style={solid,fill=Greys-3-1},mark=*\\%
 Greys-3-2!70, every mark/.append style={solid,fill=Greys-3-2},mark=square*\\%
 Greys-3-3!70, every mark/.append style={solid,fill=Greys-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-4}{%
 Greys-4-1!70, every mark/.append style={solid,fill=Greys-4-1},mark=*\\%
 Greys-4-2!70, every mark/.append style={solid,fill=Greys-4-2},mark=square*\\%
 Greys-4-3!70, every mark/.append style={solid,fill=Greys-4-3},mark=triangle*\\%
 Greys-4-4!70, every mark/.append style={solid,fill=Greys-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-5}{%
 Greys-5-1!70, every mark/.append style={solid,fill=Greys-5-1},mark=*\\%
 Greys-5-2!70, every mark/.append style={solid,fill=Greys-5-2},mark=square*\\%
 Greys-5-3!70, every mark/.append style={solid,fill=Greys-5-3},mark=triangle*\\%
 Greys-5-4!70, every mark/.append style={solid,fill=Greys-5-4},mark=diamond*\\%
 Greys-5-5!70, every mark/.append style={solid,fill=Greys-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-6}{%
 Greys-6-1!70, every mark/.append style={solid,fill=Greys-6-1},mark=*\\%
 Greys-6-2!70, every mark/.append style={solid,fill=Greys-6-2},mark=square*\\%
 Greys-6-3!70, every mark/.append style={solid,fill=Greys-6-3},mark=triangle*\\%
 Greys-6-4!70, every mark/.append style={solid,fill=Greys-6-4},mark=diamond*\\%
 Greys-6-5!70, every mark/.append style={solid,fill=Greys-6-5},mark=pentagon*\\%
 Greys-6-6!70, every mark/.append style={solid,fill=Greys-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-7}{%
 Greys-7-1!70, every mark/.append style={solid,fill=Greys-7-1},mark=*\\%
 Greys-7-2!70, every mark/.append style={solid,fill=Greys-7-2},mark=square*\\%
 Greys-7-3!70, every mark/.append style={solid,fill=Greys-7-3},mark=triangle*\\%
 Greys-7-4!70, every mark/.append style={solid,fill=Greys-7-4},mark=diamond*\\%
 Greys-7-5!70, every mark/.append style={solid,fill=Greys-7-5},mark=pentagon*\\%
 Greys-7-6!70, every mark/.append style={solid,fill=Greys-7-6},mark=x\\%
 Greys-7-7!70, every mark/.append style={solid,fill=Greys-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-8}{%
 Greys-8-1!70, every mark/.append style={solid,fill=Greys-8-1},mark=*\\%
 Greys-8-2!70, every mark/.append style={solid,fill=Greys-8-2},mark=square*\\%
 Greys-8-3!70, every mark/.append style={solid,fill=Greys-8-3},mark=triangle*\\%
 Greys-8-4!70, every mark/.append style={solid,fill=Greys-8-4},mark=diamond*\\%
 Greys-8-5!70, every mark/.append style={solid,fill=Greys-8-5},mark=pentagon*\\%
 Greys-8-6!70, every mark/.append style={solid,fill=Greys-8-6},mark=x\\%
 Greys-8-7!70, every mark/.append style={solid,fill=Greys-8-7},mark=+\\%
 Greys-8-8!70, every mark/.append style={solid,fill=Greys-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Greys-9}{%
 Greys-9-1!70, every mark/.append style={solid,fill=Greys-9-1},mark=*\\%
 Greys-9-2!70, every mark/.append style={solid,fill=Greys-9-2},mark=square*\\%
 Greys-9-3!70, every mark/.append style={solid,fill=Greys-9-3},mark=triangle*\\%
 Greys-9-4!70, every mark/.append style={solid,fill=Greys-9-4},mark=diamond*\\%
 Greys-9-5!70, every mark/.append style={solid,fill=Greys-9-5},mark=pentagon*\\%
 Greys-9-6!70, every mark/.append style={solid,fill=Greys-9-6},mark=x\\%
 Greys-9-7!70, every mark/.append style={solid,fill=Greys-9-7},mark=+\\%
 Greys-9-8!70, every mark/.append style={solid,fill=Greys-9-8},mark=star\\%
 Greys-9-9!70, every mark/.append style={solid,fill=Greys-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-3}{%
 PuOr-3-1!70, every mark/.append style={solid,fill=PuOr-3-1},mark=*\\%
 PuOr-3-2!70, every mark/.append style={solid,fill=PuOr-3-2},mark=square*\\%
 PuOr-3-3!70, every mark/.append style={solid,fill=PuOr-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-4}{%
 PuOr-4-1!70, every mark/.append style={solid,fill=PuOr-4-1},mark=*\\%
 PuOr-4-2!70, every mark/.append style={solid,fill=PuOr-4-2},mark=square*\\%
 PuOr-4-3!70, every mark/.append style={solid,fill=PuOr-4-3},mark=triangle*\\%
 PuOr-4-4!70, every mark/.append style={solid,fill=PuOr-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-5}{%
 PuOr-5-1!70, every mark/.append style={solid,fill=PuOr-5-1},mark=*\\%
 PuOr-5-2!70, every mark/.append style={solid,fill=PuOr-5-2},mark=square*\\%
 PuOr-5-3!70, every mark/.append style={solid,fill=PuOr-5-3},mark=triangle*\\%
 PuOr-5-4!70, every mark/.append style={solid,fill=PuOr-5-4},mark=diamond*\\%
 PuOr-5-5!70, every mark/.append style={solid,fill=PuOr-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-6}{%
 PuOr-6-1!70, every mark/.append style={solid,fill=PuOr-6-1},mark=*\\%
 PuOr-6-2!70, every mark/.append style={solid,fill=PuOr-6-2},mark=square*\\%
 PuOr-6-3!70, every mark/.append style={solid,fill=PuOr-6-3},mark=triangle*\\%
 PuOr-6-4!70, every mark/.append style={solid,fill=PuOr-6-4},mark=diamond*\\%
 PuOr-6-5!70, every mark/.append style={solid,fill=PuOr-6-5},mark=pentagon*\\%
 PuOr-6-6!70, every mark/.append style={solid,fill=PuOr-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-7}{%
 PuOr-7-1!70, every mark/.append style={solid,fill=PuOr-7-1},mark=*\\%
 PuOr-7-2!70, every mark/.append style={solid,fill=PuOr-7-2},mark=square*\\%
 PuOr-7-3!70, every mark/.append style={solid,fill=PuOr-7-3},mark=triangle*\\%
 PuOr-7-4!70, every mark/.append style={solid,fill=PuOr-7-4},mark=diamond*\\%
 PuOr-7-5!70, every mark/.append style={solid,fill=PuOr-7-5},mark=pentagon*\\%
 PuOr-7-6!70, every mark/.append style={solid,fill=PuOr-7-6},mark=x\\%
 PuOr-7-7!70, every mark/.append style={solid,fill=PuOr-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-8}{%
 PuOr-8-1!70, every mark/.append style={solid,fill=PuOr-8-1},mark=*\\%
 PuOr-8-2!70, every mark/.append style={solid,fill=PuOr-8-2},mark=square*\\%
 PuOr-8-3!70, every mark/.append style={solid,fill=PuOr-8-3},mark=triangle*\\%
 PuOr-8-4!70, every mark/.append style={solid,fill=PuOr-8-4},mark=diamond*\\%
 PuOr-8-5!70, every mark/.append style={solid,fill=PuOr-8-5},mark=pentagon*\\%
 PuOr-8-6!70, every mark/.append style={solid,fill=PuOr-8-6},mark=x\\%
 PuOr-8-7!70, every mark/.append style={solid,fill=PuOr-8-7},mark=+\\%
 PuOr-8-8!70, every mark/.append style={solid,fill=PuOr-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-9}{%
 PuOr-9-1!70, every mark/.append style={solid,fill=PuOr-9-1},mark=*\\%
 PuOr-9-2!70, every mark/.append style={solid,fill=PuOr-9-2},mark=square*\\%
 PuOr-9-3!70, every mark/.append style={solid,fill=PuOr-9-3},mark=triangle*\\%
 PuOr-9-4!70, every mark/.append style={solid,fill=PuOr-9-4},mark=diamond*\\%
 PuOr-9-5!70, every mark/.append style={solid,fill=PuOr-9-5},mark=pentagon*\\%
 PuOr-9-6!70, every mark/.append style={solid,fill=PuOr-9-6},mark=x\\%
 PuOr-9-7!70, every mark/.append style={solid,fill=PuOr-9-7},mark=+\\%
 PuOr-9-8!70, every mark/.append style={solid,fill=PuOr-9-8},mark=star\\%
 PuOr-9-9!70, every mark/.append style={solid,fill=PuOr-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-10}{%
 PuOr-10-1!70, every mark/.append style={solid,fill=PuOr-10-1},mark=*\\%
 PuOr-10-2!70, every mark/.append style={solid,fill=PuOr-10-2},mark=square*\\%
 PuOr-10-3!70, every mark/.append style={solid,fill=PuOr-10-3},mark=triangle*\\%
 PuOr-10-4!70, every mark/.append style={solid,fill=PuOr-10-4},mark=diamond*\\%
 PuOr-10-5!70, every mark/.append style={solid,fill=PuOr-10-5},mark=pentagon*\\%
 PuOr-10-6!70, every mark/.append style={solid,fill=PuOr-10-6},mark=x\\%
 PuOr-10-7!70, every mark/.append style={solid,fill=PuOr-10-7},mark=+\\%
 PuOr-10-8!70, every mark/.append style={solid,fill=PuOr-10-8},mark=star\\%
 PuOr-10-9!70, every mark/.append style={solid,fill=PuOr-10-9},mark=oplus*\\%
 PuOr-10-10!70, every mark/.append style={solid,fill=PuOr-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PuOr-11}{%
 PuOr-11-1!70, every mark/.append style={solid,fill=PuOr-11-1},mark=*\\%
 PuOr-11-2!70, every mark/.append style={solid,fill=PuOr-11-2},mark=square*\\%
 PuOr-11-3!70, every mark/.append style={solid,fill=PuOr-11-3},mark=triangle*\\%
 PuOr-11-4!70, every mark/.append style={solid,fill=PuOr-11-4},mark=diamond*\\%
 PuOr-11-5!70, every mark/.append style={solid,fill=PuOr-11-5},mark=pentagon*\\%
 PuOr-11-6!70, every mark/.append style={solid,fill=PuOr-11-6},mark=x\\%
 PuOr-11-7!70, every mark/.append style={solid,fill=PuOr-11-7},mark=+\\%
 PuOr-11-8!70, every mark/.append style={solid,fill=PuOr-11-8},mark=star\\%
 PuOr-11-9!70, every mark/.append style={solid,fill=PuOr-11-9},mark=oplus*\\%
 PuOr-11-10!70, every mark/.append style={solid,fill=PuOr-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-3}{%
 BrBG-3-1!70, every mark/.append style={solid,fill=BrBG-3-1},mark=*\\%
 BrBG-3-2!70, every mark/.append style={solid,fill=BrBG-3-2},mark=square*\\%
 BrBG-3-3!70, every mark/.append style={solid,fill=BrBG-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-4}{%
 BrBG-4-1!70, every mark/.append style={solid,fill=BrBG-4-1},mark=*\\%
 BrBG-4-2!70, every mark/.append style={solid,fill=BrBG-4-2},mark=square*\\%
 BrBG-4-3!70, every mark/.append style={solid,fill=BrBG-4-3},mark=triangle*\\%
 BrBG-4-4!70, every mark/.append style={solid,fill=BrBG-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-5}{%
 BrBG-5-1!70, every mark/.append style={solid,fill=BrBG-5-1},mark=*\\%
 BrBG-5-2!70, every mark/.append style={solid,fill=BrBG-5-2},mark=square*\\%
 BrBG-5-3!70, every mark/.append style={solid,fill=BrBG-5-3},mark=triangle*\\%
 BrBG-5-4!70, every mark/.append style={solid,fill=BrBG-5-4},mark=diamond*\\%
 BrBG-5-5!70, every mark/.append style={solid,fill=BrBG-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-6}{%
 BrBG-6-1!70, every mark/.append style={solid,fill=BrBG-6-1},mark=*\\%
 BrBG-6-2!70, every mark/.append style={solid,fill=BrBG-6-2},mark=square*\\%
 BrBG-6-3!70, every mark/.append style={solid,fill=BrBG-6-3},mark=triangle*\\%
 BrBG-6-4!70, every mark/.append style={solid,fill=BrBG-6-4},mark=diamond*\\%
 BrBG-6-5!70, every mark/.append style={solid,fill=BrBG-6-5},mark=pentagon*\\%
 BrBG-6-6!70, every mark/.append style={solid,fill=BrBG-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-7}{%
 BrBG-7-1!70, every mark/.append style={solid,fill=BrBG-7-1},mark=*\\%
 BrBG-7-2!70, every mark/.append style={solid,fill=BrBG-7-2},mark=square*\\%
 BrBG-7-3!70, every mark/.append style={solid,fill=BrBG-7-3},mark=triangle*\\%
 BrBG-7-4!70, every mark/.append style={solid,fill=BrBG-7-4},mark=diamond*\\%
 BrBG-7-5!70, every mark/.append style={solid,fill=BrBG-7-5},mark=pentagon*\\%
 BrBG-7-6!70, every mark/.append style={solid,fill=BrBG-7-6},mark=x\\%
 BrBG-7-7!70, every mark/.append style={solid,fill=BrBG-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-8}{%
 BrBG-8-1!70, every mark/.append style={solid,fill=BrBG-8-1},mark=*\\%
 BrBG-8-2!70, every mark/.append style={solid,fill=BrBG-8-2},mark=square*\\%
 BrBG-8-3!70, every mark/.append style={solid,fill=BrBG-8-3},mark=triangle*\\%
 BrBG-8-4!70, every mark/.append style={solid,fill=BrBG-8-4},mark=diamond*\\%
 BrBG-8-5!70, every mark/.append style={solid,fill=BrBG-8-5},mark=pentagon*\\%
 BrBG-8-6!70, every mark/.append style={solid,fill=BrBG-8-6},mark=x\\%
 BrBG-8-7!70, every mark/.append style={solid,fill=BrBG-8-7},mark=+\\%
 BrBG-8-8!70, every mark/.append style={solid,fill=BrBG-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-9}{%
 BrBG-9-1!70, every mark/.append style={solid,fill=BrBG-9-1},mark=*\\%
 BrBG-9-2!70, every mark/.append style={solid,fill=BrBG-9-2},mark=square*\\%
 BrBG-9-3!70, every mark/.append style={solid,fill=BrBG-9-3},mark=triangle*\\%
 BrBG-9-4!70, every mark/.append style={solid,fill=BrBG-9-4},mark=diamond*\\%
 BrBG-9-5!70, every mark/.append style={solid,fill=BrBG-9-5},mark=pentagon*\\%
 BrBG-9-6!70, every mark/.append style={solid,fill=BrBG-9-6},mark=x\\%
 BrBG-9-7!70, every mark/.append style={solid,fill=BrBG-9-7},mark=+\\%
 BrBG-9-8!70, every mark/.append style={solid,fill=BrBG-9-8},mark=star\\%
 BrBG-9-9!70, every mark/.append style={solid,fill=BrBG-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-10}{%
 BrBG-10-1!70, every mark/.append style={solid,fill=BrBG-10-1},mark=*\\%
 BrBG-10-2!70, every mark/.append style={solid,fill=BrBG-10-2},mark=square*\\%
 BrBG-10-3!70, every mark/.append style={solid,fill=BrBG-10-3},mark=triangle*\\%
 BrBG-10-4!70, every mark/.append style={solid,fill=BrBG-10-4},mark=diamond*\\%
 BrBG-10-5!70, every mark/.append style={solid,fill=BrBG-10-5},mark=pentagon*\\%
 BrBG-10-6!70, every mark/.append style={solid,fill=BrBG-10-6},mark=x\\%
 BrBG-10-7!70, every mark/.append style={solid,fill=BrBG-10-7},mark=+\\%
 BrBG-10-8!70, every mark/.append style={solid,fill=BrBG-10-8},mark=star\\%
 BrBG-10-9!70, every mark/.append style={solid,fill=BrBG-10-9},mark=oplus*\\%
 BrBG-10-10!70, every mark/.append style={solid,fill=BrBG-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-BrBG-11}{%
 BrBG-11-1!70, every mark/.append style={solid,fill=BrBG-11-1},mark=*\\%
 BrBG-11-2!70, every mark/.append style={solid,fill=BrBG-11-2},mark=square*\\%
 BrBG-11-3!70, every mark/.append style={solid,fill=BrBG-11-3},mark=triangle*\\%
 BrBG-11-4!70, every mark/.append style={solid,fill=BrBG-11-4},mark=diamond*\\%
 BrBG-11-5!70, every mark/.append style={solid,fill=BrBG-11-5},mark=pentagon*\\%
 BrBG-11-6!70, every mark/.append style={solid,fill=BrBG-11-6},mark=x\\%
 BrBG-11-7!70, every mark/.append style={solid,fill=BrBG-11-7},mark=+\\%
 BrBG-11-8!70, every mark/.append style={solid,fill=BrBG-11-8},mark=star\\%
 BrBG-11-9!70, every mark/.append style={solid,fill=BrBG-11-9},mark=oplus*\\%
 BrBG-11-10!70, every mark/.append style={solid,fill=BrBG-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-3}{%
 PRGn-3-1!70, every mark/.append style={solid,fill=PRGn-3-1},mark=*\\%
 PRGn-3-2!70, every mark/.append style={solid,fill=PRGn-3-2},mark=square*\\%
 PRGn-3-3!70, every mark/.append style={solid,fill=PRGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-4}{%
 PRGn-4-1!70, every mark/.append style={solid,fill=PRGn-4-1},mark=*\\%
 PRGn-4-2!70, every mark/.append style={solid,fill=PRGn-4-2},mark=square*\\%
 PRGn-4-3!70, every mark/.append style={solid,fill=PRGn-4-3},mark=triangle*\\%
 PRGn-4-4!70, every mark/.append style={solid,fill=PRGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-5}{%
 PRGn-5-1!70, every mark/.append style={solid,fill=PRGn-5-1},mark=*\\%
 PRGn-5-2!70, every mark/.append style={solid,fill=PRGn-5-2},mark=square*\\%
 PRGn-5-3!70, every mark/.append style={solid,fill=PRGn-5-3},mark=triangle*\\%
 PRGn-5-4!70, every mark/.append style={solid,fill=PRGn-5-4},mark=diamond*\\%
 PRGn-5-5!70, every mark/.append style={solid,fill=PRGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-6}{%
 PRGn-6-1!70, every mark/.append style={solid,fill=PRGn-6-1},mark=*\\%
 PRGn-6-2!70, every mark/.append style={solid,fill=PRGn-6-2},mark=square*\\%
 PRGn-6-3!70, every mark/.append style={solid,fill=PRGn-6-3},mark=triangle*\\%
 PRGn-6-4!70, every mark/.append style={solid,fill=PRGn-6-4},mark=diamond*\\%
 PRGn-6-5!70, every mark/.append style={solid,fill=PRGn-6-5},mark=pentagon*\\%
 PRGn-6-6!70, every mark/.append style={solid,fill=PRGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-7}{%
 PRGn-7-1!70, every mark/.append style={solid,fill=PRGn-7-1},mark=*\\%
 PRGn-7-2!70, every mark/.append style={solid,fill=PRGn-7-2},mark=square*\\%
 PRGn-7-3!70, every mark/.append style={solid,fill=PRGn-7-3},mark=triangle*\\%
 PRGn-7-4!70, every mark/.append style={solid,fill=PRGn-7-4},mark=diamond*\\%
 PRGn-7-5!70, every mark/.append style={solid,fill=PRGn-7-5},mark=pentagon*\\%
 PRGn-7-6!70, every mark/.append style={solid,fill=PRGn-7-6},mark=x\\%
 PRGn-7-7!70, every mark/.append style={solid,fill=PRGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-8}{%
 PRGn-8-1!70, every mark/.append style={solid,fill=PRGn-8-1},mark=*\\%
 PRGn-8-2!70, every mark/.append style={solid,fill=PRGn-8-2},mark=square*\\%
 PRGn-8-3!70, every mark/.append style={solid,fill=PRGn-8-3},mark=triangle*\\%
 PRGn-8-4!70, every mark/.append style={solid,fill=PRGn-8-4},mark=diamond*\\%
 PRGn-8-5!70, every mark/.append style={solid,fill=PRGn-8-5},mark=pentagon*\\%
 PRGn-8-6!70, every mark/.append style={solid,fill=PRGn-8-6},mark=x\\%
 PRGn-8-7!70, every mark/.append style={solid,fill=PRGn-8-7},mark=+\\%
 PRGn-8-8!70, every mark/.append style={solid,fill=PRGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-9}{%
 PRGn-9-1!70, every mark/.append style={solid,fill=PRGn-9-1},mark=*\\%
 PRGn-9-2!70, every mark/.append style={solid,fill=PRGn-9-2},mark=square*\\%
 PRGn-9-3!70, every mark/.append style={solid,fill=PRGn-9-3},mark=triangle*\\%
 PRGn-9-4!70, every mark/.append style={solid,fill=PRGn-9-4},mark=diamond*\\%
 PRGn-9-5!70, every mark/.append style={solid,fill=PRGn-9-5},mark=pentagon*\\%
 PRGn-9-6!70, every mark/.append style={solid,fill=PRGn-9-6},mark=x\\%
 PRGn-9-7!70, every mark/.append style={solid,fill=PRGn-9-7},mark=+\\%
 PRGn-9-8!70, every mark/.append style={solid,fill=PRGn-9-8},mark=star\\%
 PRGn-9-9!70, every mark/.append style={solid,fill=PRGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-10}{%
 PRGn-10-1!70, every mark/.append style={solid,fill=PRGn-10-1},mark=*\\%
 PRGn-10-2!70, every mark/.append style={solid,fill=PRGn-10-2},mark=square*\\%
 PRGn-10-3!70, every mark/.append style={solid,fill=PRGn-10-3},mark=triangle*\\%
 PRGn-10-4!70, every mark/.append style={solid,fill=PRGn-10-4},mark=diamond*\\%
 PRGn-10-5!70, every mark/.append style={solid,fill=PRGn-10-5},mark=pentagon*\\%
 PRGn-10-6!70, every mark/.append style={solid,fill=PRGn-10-6},mark=x\\%
 PRGn-10-7!70, every mark/.append style={solid,fill=PRGn-10-7},mark=+\\%
 PRGn-10-8!70, every mark/.append style={solid,fill=PRGn-10-8},mark=star\\%
 PRGn-10-9!70, every mark/.append style={solid,fill=PRGn-10-9},mark=oplus*\\%
 PRGn-10-10!70, every mark/.append style={solid,fill=PRGn-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PRGn-11}{%
 PRGn-11-1!70, every mark/.append style={solid,fill=PRGn-11-1},mark=*\\%
 PRGn-11-2!70, every mark/.append style={solid,fill=PRGn-11-2},mark=square*\\%
 PRGn-11-3!70, every mark/.append style={solid,fill=PRGn-11-3},mark=triangle*\\%
 PRGn-11-4!70, every mark/.append style={solid,fill=PRGn-11-4},mark=diamond*\\%
 PRGn-11-5!70, every mark/.append style={solid,fill=PRGn-11-5},mark=pentagon*\\%
 PRGn-11-6!70, every mark/.append style={solid,fill=PRGn-11-6},mark=x\\%
 PRGn-11-7!70, every mark/.append style={solid,fill=PRGn-11-7},mark=+\\%
 PRGn-11-8!70, every mark/.append style={solid,fill=PRGn-11-8},mark=star\\%
 PRGn-11-9!70, every mark/.append style={solid,fill=PRGn-11-9},mark=oplus*\\%
 PRGn-11-10!70, every mark/.append style={solid,fill=PRGn-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-3}{%
 PiYG-3-1!70, every mark/.append style={solid,fill=PiYG-3-1},mark=*\\%
 PiYG-3-2!70, every mark/.append style={solid,fill=PiYG-3-2},mark=square*\\%
 PiYG-3-3!70, every mark/.append style={solid,fill=PiYG-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-4}{%
 PiYG-4-1!70, every mark/.append style={solid,fill=PiYG-4-1},mark=*\\%
 PiYG-4-2!70, every mark/.append style={solid,fill=PiYG-4-2},mark=square*\\%
 PiYG-4-3!70, every mark/.append style={solid,fill=PiYG-4-3},mark=triangle*\\%
 PiYG-4-4!70, every mark/.append style={solid,fill=PiYG-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-5}{%
 PiYG-5-1!70, every mark/.append style={solid,fill=PiYG-5-1},mark=*\\%
 PiYG-5-2!70, every mark/.append style={solid,fill=PiYG-5-2},mark=square*\\%
 PiYG-5-3!70, every mark/.append style={solid,fill=PiYG-5-3},mark=triangle*\\%
 PiYG-5-4!70, every mark/.append style={solid,fill=PiYG-5-4},mark=diamond*\\%
 PiYG-5-5!70, every mark/.append style={solid,fill=PiYG-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-6}{%
 PiYG-6-1!70, every mark/.append style={solid,fill=PiYG-6-1},mark=*\\%
 PiYG-6-2!70, every mark/.append style={solid,fill=PiYG-6-2},mark=square*\\%
 PiYG-6-3!70, every mark/.append style={solid,fill=PiYG-6-3},mark=triangle*\\%
 PiYG-6-4!70, every mark/.append style={solid,fill=PiYG-6-4},mark=diamond*\\%
 PiYG-6-5!70, every mark/.append style={solid,fill=PiYG-6-5},mark=pentagon*\\%
 PiYG-6-6!70, every mark/.append style={solid,fill=PiYG-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-7}{%
 PiYG-7-1!70, every mark/.append style={solid,fill=PiYG-7-1},mark=*\\%
 PiYG-7-2!70, every mark/.append style={solid,fill=PiYG-7-2},mark=square*\\%
 PiYG-7-3!70, every mark/.append style={solid,fill=PiYG-7-3},mark=triangle*\\%
 PiYG-7-4!70, every mark/.append style={solid,fill=PiYG-7-4},mark=diamond*\\%
 PiYG-7-5!70, every mark/.append style={solid,fill=PiYG-7-5},mark=pentagon*\\%
 PiYG-7-6!70, every mark/.append style={solid,fill=PiYG-7-6},mark=x\\%
 PiYG-7-7!70, every mark/.append style={solid,fill=PiYG-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-8}{%
 PiYG-8-1!70, every mark/.append style={solid,fill=PiYG-8-1},mark=*\\%
 PiYG-8-2!70, every mark/.append style={solid,fill=PiYG-8-2},mark=square*\\%
 PiYG-8-3!70, every mark/.append style={solid,fill=PiYG-8-3},mark=triangle*\\%
 PiYG-8-4!70, every mark/.append style={solid,fill=PiYG-8-4},mark=diamond*\\%
 PiYG-8-5!70, every mark/.append style={solid,fill=PiYG-8-5},mark=pentagon*\\%
 PiYG-8-6!70, every mark/.append style={solid,fill=PiYG-8-6},mark=x\\%
 PiYG-8-7!70, every mark/.append style={solid,fill=PiYG-8-7},mark=+\\%
 PiYG-8-8!70, every mark/.append style={solid,fill=PiYG-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-9}{%
 PiYG-9-1!70, every mark/.append style={solid,fill=PiYG-9-1},mark=*\\%
 PiYG-9-2!70, every mark/.append style={solid,fill=PiYG-9-2},mark=square*\\%
 PiYG-9-3!70, every mark/.append style={solid,fill=PiYG-9-3},mark=triangle*\\%
 PiYG-9-4!70, every mark/.append style={solid,fill=PiYG-9-4},mark=diamond*\\%
 PiYG-9-5!70, every mark/.append style={solid,fill=PiYG-9-5},mark=pentagon*\\%
 PiYG-9-6!70, every mark/.append style={solid,fill=PiYG-9-6},mark=x\\%
 PiYG-9-7!70, every mark/.append style={solid,fill=PiYG-9-7},mark=+\\%
 PiYG-9-8!70, every mark/.append style={solid,fill=PiYG-9-8},mark=star\\%
 PiYG-9-9!70, every mark/.append style={solid,fill=PiYG-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-10}{%
 PiYG-10-1!70, every mark/.append style={solid,fill=PiYG-10-1},mark=*\\%
 PiYG-10-2!70, every mark/.append style={solid,fill=PiYG-10-2},mark=square*\\%
 PiYG-10-3!70, every mark/.append style={solid,fill=PiYG-10-3},mark=triangle*\\%
 PiYG-10-4!70, every mark/.append style={solid,fill=PiYG-10-4},mark=diamond*\\%
 PiYG-10-5!70, every mark/.append style={solid,fill=PiYG-10-5},mark=pentagon*\\%
 PiYG-10-6!70, every mark/.append style={solid,fill=PiYG-10-6},mark=x\\%
 PiYG-10-7!70, every mark/.append style={solid,fill=PiYG-10-7},mark=+\\%
 PiYG-10-8!70, every mark/.append style={solid,fill=PiYG-10-8},mark=star\\%
 PiYG-10-9!70, every mark/.append style={solid,fill=PiYG-10-9},mark=oplus*\\%
 PiYG-10-10!70, every mark/.append style={solid,fill=PiYG-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-PiYG-11}{%
 PiYG-11-1!70, every mark/.append style={solid,fill=PiYG-11-1},mark=*\\%
 PiYG-11-2!70, every mark/.append style={solid,fill=PiYG-11-2},mark=square*\\%
 PiYG-11-3!70, every mark/.append style={solid,fill=PiYG-11-3},mark=triangle*\\%
 PiYG-11-4!70, every mark/.append style={solid,fill=PiYG-11-4},mark=diamond*\\%
 PiYG-11-5!70, every mark/.append style={solid,fill=PiYG-11-5},mark=pentagon*\\%
 PiYG-11-6!70, every mark/.append style={solid,fill=PiYG-11-6},mark=x\\%
 PiYG-11-7!70, every mark/.append style={solid,fill=PiYG-11-7},mark=+\\%
 PiYG-11-8!70, every mark/.append style={solid,fill=PiYG-11-8},mark=star\\%
 PiYG-11-9!70, every mark/.append style={solid,fill=PiYG-11-9},mark=oplus*\\%
 PiYG-11-10!70, every mark/.append style={solid,fill=PiYG-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-3}{%
 RdBu-3-1!70, every mark/.append style={solid,fill=RdBu-3-1},mark=*\\%
 RdBu-3-2!70, every mark/.append style={solid,fill=RdBu-3-2},mark=square*\\%
 RdBu-3-3!70, every mark/.append style={solid,fill=RdBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-4}{%
 RdBu-4-1!70, every mark/.append style={solid,fill=RdBu-4-1},mark=*\\%
 RdBu-4-2!70, every mark/.append style={solid,fill=RdBu-4-2},mark=square*\\%
 RdBu-4-3!70, every mark/.append style={solid,fill=RdBu-4-3},mark=triangle*\\%
 RdBu-4-4!70, every mark/.append style={solid,fill=RdBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-5}{%
 RdBu-5-1!70, every mark/.append style={solid,fill=RdBu-5-1},mark=*\\%
 RdBu-5-2!70, every mark/.append style={solid,fill=RdBu-5-2},mark=square*\\%
 RdBu-5-3!70, every mark/.append style={solid,fill=RdBu-5-3},mark=triangle*\\%
 RdBu-5-4!70, every mark/.append style={solid,fill=RdBu-5-4},mark=diamond*\\%
 RdBu-5-5!70, every mark/.append style={solid,fill=RdBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-6}{%
 RdBu-6-1!70, every mark/.append style={solid,fill=RdBu-6-1},mark=*\\%
 RdBu-6-2!70, every mark/.append style={solid,fill=RdBu-6-2},mark=square*\\%
 RdBu-6-3!70, every mark/.append style={solid,fill=RdBu-6-3},mark=triangle*\\%
 RdBu-6-4!70, every mark/.append style={solid,fill=RdBu-6-4},mark=diamond*\\%
 RdBu-6-5!70, every mark/.append style={solid,fill=RdBu-6-5},mark=pentagon*\\%
 RdBu-6-6!70, every mark/.append style={solid,fill=RdBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-7}{%
 RdBu-7-1!70, every mark/.append style={solid,fill=RdBu-7-1},mark=*\\%
 RdBu-7-2!70, every mark/.append style={solid,fill=RdBu-7-2},mark=square*\\%
 RdBu-7-3!70, every mark/.append style={solid,fill=RdBu-7-3},mark=triangle*\\%
 RdBu-7-4!70, every mark/.append style={solid,fill=RdBu-7-4},mark=diamond*\\%
 RdBu-7-5!70, every mark/.append style={solid,fill=RdBu-7-5},mark=pentagon*\\%
 RdBu-7-6!70, every mark/.append style={solid,fill=RdBu-7-6},mark=x\\%
 RdBu-7-7!70, every mark/.append style={solid,fill=RdBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-8}{%
 RdBu-8-1!70, every mark/.append style={solid,fill=RdBu-8-1},mark=*\\%
 RdBu-8-2!70, every mark/.append style={solid,fill=RdBu-8-2},mark=square*\\%
 RdBu-8-3!70, every mark/.append style={solid,fill=RdBu-8-3},mark=triangle*\\%
 RdBu-8-4!70, every mark/.append style={solid,fill=RdBu-8-4},mark=diamond*\\%
 RdBu-8-5!70, every mark/.append style={solid,fill=RdBu-8-5},mark=pentagon*\\%
 RdBu-8-6!70, every mark/.append style={solid,fill=RdBu-8-6},mark=x\\%
 RdBu-8-7!70, every mark/.append style={solid,fill=RdBu-8-7},mark=+\\%
 RdBu-8-8!70, every mark/.append style={solid,fill=RdBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-9}{%
 RdBu-9-1!70, every mark/.append style={solid,fill=RdBu-9-1},mark=*\\%
 RdBu-9-2!70, every mark/.append style={solid,fill=RdBu-9-2},mark=square*\\%
 RdBu-9-3!70, every mark/.append style={solid,fill=RdBu-9-3},mark=triangle*\\%
 RdBu-9-4!70, every mark/.append style={solid,fill=RdBu-9-4},mark=diamond*\\%
 RdBu-9-5!70, every mark/.append style={solid,fill=RdBu-9-5},mark=pentagon*\\%
 RdBu-9-6!70, every mark/.append style={solid,fill=RdBu-9-6},mark=x\\%
 RdBu-9-7!70, every mark/.append style={solid,fill=RdBu-9-7},mark=+\\%
 RdBu-9-8!70, every mark/.append style={solid,fill=RdBu-9-8},mark=star\\%
 RdBu-9-9!70, every mark/.append style={solid,fill=RdBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-10}{%
 RdBu-10-1!70, every mark/.append style={solid,fill=RdBu-10-1},mark=*\\%
 RdBu-10-2!70, every mark/.append style={solid,fill=RdBu-10-2},mark=square*\\%
 RdBu-10-3!70, every mark/.append style={solid,fill=RdBu-10-3},mark=triangle*\\%
 RdBu-10-4!70, every mark/.append style={solid,fill=RdBu-10-4},mark=diamond*\\%
 RdBu-10-5!70, every mark/.append style={solid,fill=RdBu-10-5},mark=pentagon*\\%
 RdBu-10-6!70, every mark/.append style={solid,fill=RdBu-10-6},mark=x\\%
 RdBu-10-7!70, every mark/.append style={solid,fill=RdBu-10-7},mark=+\\%
 RdBu-10-8!70, every mark/.append style={solid,fill=RdBu-10-8},mark=star\\%
 RdBu-10-9!70, every mark/.append style={solid,fill=RdBu-10-9},mark=oplus*\\%
 RdBu-10-10!70, every mark/.append style={solid,fill=RdBu-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdBu-11}{%
 RdBu-11-1!70, every mark/.append style={solid,fill=RdBu-11-1},mark=*\\%
 RdBu-11-2!70, every mark/.append style={solid,fill=RdBu-11-2},mark=square*\\%
 RdBu-11-3!70, every mark/.append style={solid,fill=RdBu-11-3},mark=triangle*\\%
 RdBu-11-4!70, every mark/.append style={solid,fill=RdBu-11-4},mark=diamond*\\%
 RdBu-11-5!70, every mark/.append style={solid,fill=RdBu-11-5},mark=pentagon*\\%
 RdBu-11-6!70, every mark/.append style={solid,fill=RdBu-11-6},mark=x\\%
 RdBu-11-7!70, every mark/.append style={solid,fill=RdBu-11-7},mark=+\\%
 RdBu-11-8!70, every mark/.append style={solid,fill=RdBu-11-8},mark=star\\%
 RdBu-11-9!70, every mark/.append style={solid,fill=RdBu-11-9},mark=oplus*\\%
 RdBu-11-10!70, every mark/.append style={solid,fill=RdBu-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-3}{%
 RdGy-3-1!70, every mark/.append style={solid,fill=RdGy-3-1},mark=*\\%
 RdGy-3-2!70, every mark/.append style={solid,fill=RdGy-3-2},mark=square*\\%
 RdGy-3-3!70, every mark/.append style={solid,fill=RdGy-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-4}{%
 RdGy-4-1!70, every mark/.append style={solid,fill=RdGy-4-1},mark=*\\%
 RdGy-4-2!70, every mark/.append style={solid,fill=RdGy-4-2},mark=square*\\%
 RdGy-4-3!70, every mark/.append style={solid,fill=RdGy-4-3},mark=triangle*\\%
 RdGy-4-4!70, every mark/.append style={solid,fill=RdGy-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-5}{%
 RdGy-5-1!70, every mark/.append style={solid,fill=RdGy-5-1},mark=*\\%
 RdGy-5-2!70, every mark/.append style={solid,fill=RdGy-5-2},mark=square*\\%
 RdGy-5-3!70, every mark/.append style={solid,fill=RdGy-5-3},mark=triangle*\\%
 RdGy-5-4!70, every mark/.append style={solid,fill=RdGy-5-4},mark=diamond*\\%
 RdGy-5-5!70, every mark/.append style={solid,fill=RdGy-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-6}{%
 RdGy-6-1!70, every mark/.append style={solid,fill=RdGy-6-1},mark=*\\%
 RdGy-6-2!70, every mark/.append style={solid,fill=RdGy-6-2},mark=square*\\%
 RdGy-6-3!70, every mark/.append style={solid,fill=RdGy-6-3},mark=triangle*\\%
 RdGy-6-4!70, every mark/.append style={solid,fill=RdGy-6-4},mark=diamond*\\%
 RdGy-6-5!70, every mark/.append style={solid,fill=RdGy-6-5},mark=pentagon*\\%
 RdGy-6-6!70, every mark/.append style={solid,fill=RdGy-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-7}{%
 RdGy-7-1!70, every mark/.append style={solid,fill=RdGy-7-1},mark=*\\%
 RdGy-7-2!70, every mark/.append style={solid,fill=RdGy-7-2},mark=square*\\%
 RdGy-7-3!70, every mark/.append style={solid,fill=RdGy-7-3},mark=triangle*\\%
 RdGy-7-4!70, every mark/.append style={solid,fill=RdGy-7-4},mark=diamond*\\%
 RdGy-7-5!70, every mark/.append style={solid,fill=RdGy-7-5},mark=pentagon*\\%
 RdGy-7-6!70, every mark/.append style={solid,fill=RdGy-7-6},mark=x\\%
 RdGy-7-7!70, every mark/.append style={solid,fill=RdGy-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-8}{%
 RdGy-8-1!70, every mark/.append style={solid,fill=RdGy-8-1},mark=*\\%
 RdGy-8-2!70, every mark/.append style={solid,fill=RdGy-8-2},mark=square*\\%
 RdGy-8-3!70, every mark/.append style={solid,fill=RdGy-8-3},mark=triangle*\\%
 RdGy-8-4!70, every mark/.append style={solid,fill=RdGy-8-4},mark=diamond*\\%
 RdGy-8-5!70, every mark/.append style={solid,fill=RdGy-8-5},mark=pentagon*\\%
 RdGy-8-6!70, every mark/.append style={solid,fill=RdGy-8-6},mark=x\\%
 RdGy-8-7!70, every mark/.append style={solid,fill=RdGy-8-7},mark=+\\%
 RdGy-8-8!70, every mark/.append style={solid,fill=RdGy-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-9}{%
 RdGy-9-1!70, every mark/.append style={solid,fill=RdGy-9-1},mark=*\\%
 RdGy-9-2!70, every mark/.append style={solid,fill=RdGy-9-2},mark=square*\\%
 RdGy-9-3!70, every mark/.append style={solid,fill=RdGy-9-3},mark=triangle*\\%
 RdGy-9-4!70, every mark/.append style={solid,fill=RdGy-9-4},mark=diamond*\\%
 RdGy-9-5!70, every mark/.append style={solid,fill=RdGy-9-5},mark=pentagon*\\%
 RdGy-9-6!70, every mark/.append style={solid,fill=RdGy-9-6},mark=x\\%
 RdGy-9-7!70, every mark/.append style={solid,fill=RdGy-9-7},mark=+\\%
 RdGy-9-8!70, every mark/.append style={solid,fill=RdGy-9-8},mark=star\\%
 RdGy-9-9!70, every mark/.append style={solid,fill=RdGy-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-10}{%
 RdGy-10-1!70, every mark/.append style={solid,fill=RdGy-10-1},mark=*\\%
 RdGy-10-2!70, every mark/.append style={solid,fill=RdGy-10-2},mark=square*\\%
 RdGy-10-3!70, every mark/.append style={solid,fill=RdGy-10-3},mark=triangle*\\%
 RdGy-10-4!70, every mark/.append style={solid,fill=RdGy-10-4},mark=diamond*\\%
 RdGy-10-5!70, every mark/.append style={solid,fill=RdGy-10-5},mark=pentagon*\\%
 RdGy-10-6!70, every mark/.append style={solid,fill=RdGy-10-6},mark=x\\%
 RdGy-10-7!70, every mark/.append style={solid,fill=RdGy-10-7},mark=+\\%
 RdGy-10-8!70, every mark/.append style={solid,fill=RdGy-10-8},mark=star\\%
 RdGy-10-9!70, every mark/.append style={solid,fill=RdGy-10-9},mark=oplus*\\%
 RdGy-10-10!70, every mark/.append style={solid,fill=RdGy-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdGy-11}{%
 RdGy-11-1!70, every mark/.append style={solid,fill=RdGy-11-1},mark=*\\%
 RdGy-11-2!70, every mark/.append style={solid,fill=RdGy-11-2},mark=square*\\%
 RdGy-11-3!70, every mark/.append style={solid,fill=RdGy-11-3},mark=triangle*\\%
 RdGy-11-4!70, every mark/.append style={solid,fill=RdGy-11-4},mark=diamond*\\%
 RdGy-11-5!70, every mark/.append style={solid,fill=RdGy-11-5},mark=pentagon*\\%
 RdGy-11-6!70, every mark/.append style={solid,fill=RdGy-11-6},mark=x\\%
 RdGy-11-7!70, every mark/.append style={solid,fill=RdGy-11-7},mark=+\\%
 RdGy-11-8!70, every mark/.append style={solid,fill=RdGy-11-8},mark=star\\%
 RdGy-11-9!70, every mark/.append style={solid,fill=RdGy-11-9},mark=oplus*\\%
 RdGy-11-10!70, every mark/.append style={solid,fill=RdGy-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-3}{%
 RdYlBu-3-1!70, every mark/.append style={solid,fill=RdYlBu-3-1},mark=*\\%
 RdYlBu-3-2!70, every mark/.append style={solid,fill=RdYlBu-3-2},mark=square*\\%
 RdYlBu-3-3!70, every mark/.append style={solid,fill=RdYlBu-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-4}{%
 RdYlBu-4-1!70, every mark/.append style={solid,fill=RdYlBu-4-1},mark=*\\%
 RdYlBu-4-2!70, every mark/.append style={solid,fill=RdYlBu-4-2},mark=square*\\%
 RdYlBu-4-3!70, every mark/.append style={solid,fill=RdYlBu-4-3},mark=triangle*\\%
 RdYlBu-4-4!70, every mark/.append style={solid,fill=RdYlBu-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-5}{%
 RdYlBu-5-1!70, every mark/.append style={solid,fill=RdYlBu-5-1},mark=*\\%
 RdYlBu-5-2!70, every mark/.append style={solid,fill=RdYlBu-5-2},mark=square*\\%
 RdYlBu-5-3!70, every mark/.append style={solid,fill=RdYlBu-5-3},mark=triangle*\\%
 RdYlBu-5-4!70, every mark/.append style={solid,fill=RdYlBu-5-4},mark=diamond*\\%
 RdYlBu-5-5!70, every mark/.append style={solid,fill=RdYlBu-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-6}{%
 RdYlBu-6-1!70, every mark/.append style={solid,fill=RdYlBu-6-1},mark=*\\%
 RdYlBu-6-2!70, every mark/.append style={solid,fill=RdYlBu-6-2},mark=square*\\%
 RdYlBu-6-3!70, every mark/.append style={solid,fill=RdYlBu-6-3},mark=triangle*\\%
 RdYlBu-6-4!70, every mark/.append style={solid,fill=RdYlBu-6-4},mark=diamond*\\%
 RdYlBu-6-5!70, every mark/.append style={solid,fill=RdYlBu-6-5},mark=pentagon*\\%
 RdYlBu-6-6!70, every mark/.append style={solid,fill=RdYlBu-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-7}{%
 RdYlBu-7-1!70, every mark/.append style={solid,fill=RdYlBu-7-1},mark=*\\%
 RdYlBu-7-2!70, every mark/.append style={solid,fill=RdYlBu-7-2},mark=square*\\%
 RdYlBu-7-3!70, every mark/.append style={solid,fill=RdYlBu-7-3},mark=triangle*\\%
 RdYlBu-7-4!70, every mark/.append style={solid,fill=RdYlBu-7-4},mark=diamond*\\%
 RdYlBu-7-5!70, every mark/.append style={solid,fill=RdYlBu-7-5},mark=pentagon*\\%
 RdYlBu-7-6!70, every mark/.append style={solid,fill=RdYlBu-7-6},mark=x\\%
 RdYlBu-7-7!70, every mark/.append style={solid,fill=RdYlBu-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-8}{%
 RdYlBu-8-1!70, every mark/.append style={solid,fill=RdYlBu-8-1},mark=*\\%
 RdYlBu-8-2!70, every mark/.append style={solid,fill=RdYlBu-8-2},mark=square*\\%
 RdYlBu-8-3!70, every mark/.append style={solid,fill=RdYlBu-8-3},mark=triangle*\\%
 RdYlBu-8-4!70, every mark/.append style={solid,fill=RdYlBu-8-4},mark=diamond*\\%
 RdYlBu-8-5!70, every mark/.append style={solid,fill=RdYlBu-8-5},mark=pentagon*\\%
 RdYlBu-8-6!70, every mark/.append style={solid,fill=RdYlBu-8-6},mark=x\\%
 RdYlBu-8-7!70, every mark/.append style={solid,fill=RdYlBu-8-7},mark=+\\%
 RdYlBu-8-8!70, every mark/.append style={solid,fill=RdYlBu-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-9}{%
 RdYlBu-9-1!70, every mark/.append style={solid,fill=RdYlBu-9-1},mark=*\\%
 RdYlBu-9-2!70, every mark/.append style={solid,fill=RdYlBu-9-2},mark=square*\\%
 RdYlBu-9-3!70, every mark/.append style={solid,fill=RdYlBu-9-3},mark=triangle*\\%
 RdYlBu-9-4!70, every mark/.append style={solid,fill=RdYlBu-9-4},mark=diamond*\\%
 RdYlBu-9-5!70, every mark/.append style={solid,fill=RdYlBu-9-5},mark=pentagon*\\%
 RdYlBu-9-6!70, every mark/.append style={solid,fill=RdYlBu-9-6},mark=x\\%
 RdYlBu-9-7!70, every mark/.append style={solid,fill=RdYlBu-9-7},mark=+\\%
 RdYlBu-9-8!70, every mark/.append style={solid,fill=RdYlBu-9-8},mark=star\\%
 RdYlBu-9-9!70, every mark/.append style={solid,fill=RdYlBu-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-10}{%
 RdYlBu-10-1!70, every mark/.append style={solid,fill=RdYlBu-10-1},mark=*\\%
 RdYlBu-10-2!70, every mark/.append style={solid,fill=RdYlBu-10-2},mark=square*\\%
 RdYlBu-10-3!70, every mark/.append style={solid,fill=RdYlBu-10-3},mark=triangle*\\%
 RdYlBu-10-4!70, every mark/.append style={solid,fill=RdYlBu-10-4},mark=diamond*\\%
 RdYlBu-10-5!70, every mark/.append style={solid,fill=RdYlBu-10-5},mark=pentagon*\\%
 RdYlBu-10-6!70, every mark/.append style={solid,fill=RdYlBu-10-6},mark=x\\%
 RdYlBu-10-7!70, every mark/.append style={solid,fill=RdYlBu-10-7},mark=+\\%
 RdYlBu-10-8!70, every mark/.append style={solid,fill=RdYlBu-10-8},mark=star\\%
 RdYlBu-10-9!70, every mark/.append style={solid,fill=RdYlBu-10-9},mark=oplus*\\%
 RdYlBu-10-10!70, every mark/.append style={solid,fill=RdYlBu-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlBu-11}{%
 RdYlBu-11-1!70, every mark/.append style={solid,fill=RdYlBu-11-1},mark=*\\%
 RdYlBu-11-2!70, every mark/.append style={solid,fill=RdYlBu-11-2},mark=square*\\%
 RdYlBu-11-3!70, every mark/.append style={solid,fill=RdYlBu-11-3},mark=triangle*\\%
 RdYlBu-11-4!70, every mark/.append style={solid,fill=RdYlBu-11-4},mark=diamond*\\%
 RdYlBu-11-5!70, every mark/.append style={solid,fill=RdYlBu-11-5},mark=pentagon*\\%
 RdYlBu-11-6!70, every mark/.append style={solid,fill=RdYlBu-11-6},mark=x\\%
 RdYlBu-11-7!70, every mark/.append style={solid,fill=RdYlBu-11-7},mark=+\\%
 RdYlBu-11-8!70, every mark/.append style={solid,fill=RdYlBu-11-8},mark=star\\%
 RdYlBu-11-9!70, every mark/.append style={solid,fill=RdYlBu-11-9},mark=oplus*\\%
 RdYlBu-11-10!70, every mark/.append style={solid,fill=RdYlBu-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-3}{%
 Spectral-3-1!70, every mark/.append style={solid,fill=Spectral-3-1},mark=*\\%
 Spectral-3-2!70, every mark/.append style={solid,fill=Spectral-3-2},mark=square*\\%
 Spectral-3-3!70, every mark/.append style={solid,fill=Spectral-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-4}{%
 Spectral-4-1!70, every mark/.append style={solid,fill=Spectral-4-1},mark=*\\%
 Spectral-4-2!70, every mark/.append style={solid,fill=Spectral-4-2},mark=square*\\%
 Spectral-4-3!70, every mark/.append style={solid,fill=Spectral-4-3},mark=triangle*\\%
 Spectral-4-4!70, every mark/.append style={solid,fill=Spectral-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-5}{%
 Spectral-5-1!70, every mark/.append style={solid,fill=Spectral-5-1},mark=*\\%
 Spectral-5-2!70, every mark/.append style={solid,fill=Spectral-5-2},mark=square*\\%
 Spectral-5-3!70, every mark/.append style={solid,fill=Spectral-5-3},mark=triangle*\\%
 Spectral-5-4!70, every mark/.append style={solid,fill=Spectral-5-4},mark=diamond*\\%
 Spectral-5-5!70, every mark/.append style={solid,fill=Spectral-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-6}{%
 Spectral-6-1!70, every mark/.append style={solid,fill=Spectral-6-1},mark=*\\%
 Spectral-6-2!70, every mark/.append style={solid,fill=Spectral-6-2},mark=square*\\%
 Spectral-6-3!70, every mark/.append style={solid,fill=Spectral-6-3},mark=triangle*\\%
 Spectral-6-4!70, every mark/.append style={solid,fill=Spectral-6-4},mark=diamond*\\%
 Spectral-6-5!70, every mark/.append style={solid,fill=Spectral-6-5},mark=pentagon*\\%
 Spectral-6-6!70, every mark/.append style={solid,fill=Spectral-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-7}{%
 Spectral-7-1!70, every mark/.append style={solid,fill=Spectral-7-1},mark=*\\%
 Spectral-7-2!70, every mark/.append style={solid,fill=Spectral-7-2},mark=square*\\%
 Spectral-7-3!70, every mark/.append style={solid,fill=Spectral-7-3},mark=triangle*\\%
 Spectral-7-4!70, every mark/.append style={solid,fill=Spectral-7-4},mark=diamond*\\%
 Spectral-7-5!70, every mark/.append style={solid,fill=Spectral-7-5},mark=pentagon*\\%
 Spectral-7-6!70, every mark/.append style={solid,fill=Spectral-7-6},mark=x\\%
 Spectral-7-7!70, every mark/.append style={solid,fill=Spectral-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-8}{%
 Spectral-8-1!70, every mark/.append style={solid,fill=Spectral-8-1},mark=*\\%
 Spectral-8-2!70, every mark/.append style={solid,fill=Spectral-8-2},mark=square*\\%
 Spectral-8-3!70, every mark/.append style={solid,fill=Spectral-8-3},mark=triangle*\\%
 Spectral-8-4!70, every mark/.append style={solid,fill=Spectral-8-4},mark=diamond*\\%
 Spectral-8-5!70, every mark/.append style={solid,fill=Spectral-8-5},mark=pentagon*\\%
 Spectral-8-6!70, every mark/.append style={solid,fill=Spectral-8-6},mark=x\\%
 Spectral-8-7!70, every mark/.append style={solid,fill=Spectral-8-7},mark=+\\%
 Spectral-8-8!70, every mark/.append style={solid,fill=Spectral-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-9}{%
 Spectral-9-1!70, every mark/.append style={solid,fill=Spectral-9-1},mark=*\\%
 Spectral-9-2!70, every mark/.append style={solid,fill=Spectral-9-2},mark=square*\\%
 Spectral-9-3!70, every mark/.append style={solid,fill=Spectral-9-3},mark=triangle*\\%
 Spectral-9-4!70, every mark/.append style={solid,fill=Spectral-9-4},mark=diamond*\\%
 Spectral-9-5!70, every mark/.append style={solid,fill=Spectral-9-5},mark=pentagon*\\%
 Spectral-9-6!70, every mark/.append style={solid,fill=Spectral-9-6},mark=x\\%
 Spectral-9-7!70, every mark/.append style={solid,fill=Spectral-9-7},mark=+\\%
 Spectral-9-8!70, every mark/.append style={solid,fill=Spectral-9-8},mark=star\\%
 Spectral-9-9!70, every mark/.append style={solid,fill=Spectral-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-10}{%
 Spectral-10-1!70, every mark/.append style={solid,fill=Spectral-10-1},mark=*\\%
 Spectral-10-2!70, every mark/.append style={solid,fill=Spectral-10-2},mark=square*\\%
 Spectral-10-3!70, every mark/.append style={solid,fill=Spectral-10-3},mark=triangle*\\%
 Spectral-10-4!70, every mark/.append style={solid,fill=Spectral-10-4},mark=diamond*\\%
 Spectral-10-5!70, every mark/.append style={solid,fill=Spectral-10-5},mark=pentagon*\\%
 Spectral-10-6!70, every mark/.append style={solid,fill=Spectral-10-6},mark=x\\%
 Spectral-10-7!70, every mark/.append style={solid,fill=Spectral-10-7},mark=+\\%
 Spectral-10-8!70, every mark/.append style={solid,fill=Spectral-10-8},mark=star\\%
 Spectral-10-9!70, every mark/.append style={solid,fill=Spectral-10-9},mark=oplus*\\%
 Spectral-10-10!70, every mark/.append style={solid,fill=Spectral-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Spectral-11}{%
 Spectral-11-1!70, every mark/.append style={solid,fill=Spectral-11-1},mark=*\\%
 Spectral-11-2!70, every mark/.append style={solid,fill=Spectral-11-2},mark=square*\\%
 Spectral-11-3!70, every mark/.append style={solid,fill=Spectral-11-3},mark=triangle*\\%
 Spectral-11-4!70, every mark/.append style={solid,fill=Spectral-11-4},mark=diamond*\\%
 Spectral-11-5!70, every mark/.append style={solid,fill=Spectral-11-5},mark=pentagon*\\%
 Spectral-11-6!70, every mark/.append style={solid,fill=Spectral-11-6},mark=x\\%
 Spectral-11-7!70, every mark/.append style={solid,fill=Spectral-11-7},mark=+\\%
 Spectral-11-8!70, every mark/.append style={solid,fill=Spectral-11-8},mark=star\\%
 Spectral-11-9!70, every mark/.append style={solid,fill=Spectral-11-9},mark=oplus*\\%
 Spectral-11-10!70, every mark/.append style={solid,fill=Spectral-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-3}{%
 RdYlGn-3-1!70, every mark/.append style={solid,fill=RdYlGn-3-1},mark=*\\%
 RdYlGn-3-2!70, every mark/.append style={solid,fill=RdYlGn-3-2},mark=square*\\%
 RdYlGn-3-3!70, every mark/.append style={solid,fill=RdYlGn-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-4}{%
 RdYlGn-4-1!70, every mark/.append style={solid,fill=RdYlGn-4-1},mark=*\\%
 RdYlGn-4-2!70, every mark/.append style={solid,fill=RdYlGn-4-2},mark=square*\\%
 RdYlGn-4-3!70, every mark/.append style={solid,fill=RdYlGn-4-3},mark=triangle*\\%
 RdYlGn-4-4!70, every mark/.append style={solid,fill=RdYlGn-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-5}{%
 RdYlGn-5-1!70, every mark/.append style={solid,fill=RdYlGn-5-1},mark=*\\%
 RdYlGn-5-2!70, every mark/.append style={solid,fill=RdYlGn-5-2},mark=square*\\%
 RdYlGn-5-3!70, every mark/.append style={solid,fill=RdYlGn-5-3},mark=triangle*\\%
 RdYlGn-5-4!70, every mark/.append style={solid,fill=RdYlGn-5-4},mark=diamond*\\%
 RdYlGn-5-5!70, every mark/.append style={solid,fill=RdYlGn-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-6}{%
 RdYlGn-6-1!70, every mark/.append style={solid,fill=RdYlGn-6-1},mark=*\\%
 RdYlGn-6-2!70, every mark/.append style={solid,fill=RdYlGn-6-2},mark=square*\\%
 RdYlGn-6-3!70, every mark/.append style={solid,fill=RdYlGn-6-3},mark=triangle*\\%
 RdYlGn-6-4!70, every mark/.append style={solid,fill=RdYlGn-6-4},mark=diamond*\\%
 RdYlGn-6-5!70, every mark/.append style={solid,fill=RdYlGn-6-5},mark=pentagon*\\%
 RdYlGn-6-6!70, every mark/.append style={solid,fill=RdYlGn-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-7}{%
 RdYlGn-7-1!70, every mark/.append style={solid,fill=RdYlGn-7-1},mark=*\\%
 RdYlGn-7-2!70, every mark/.append style={solid,fill=RdYlGn-7-2},mark=square*\\%
 RdYlGn-7-3!70, every mark/.append style={solid,fill=RdYlGn-7-3},mark=triangle*\\%
 RdYlGn-7-4!70, every mark/.append style={solid,fill=RdYlGn-7-4},mark=diamond*\\%
 RdYlGn-7-5!70, every mark/.append style={solid,fill=RdYlGn-7-5},mark=pentagon*\\%
 RdYlGn-7-6!70, every mark/.append style={solid,fill=RdYlGn-7-6},mark=x\\%
 RdYlGn-7-7!70, every mark/.append style={solid,fill=RdYlGn-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-8}{%
 RdYlGn-8-1!70, every mark/.append style={solid,fill=RdYlGn-8-1},mark=*\\%
 RdYlGn-8-2!70, every mark/.append style={solid,fill=RdYlGn-8-2},mark=square*\\%
 RdYlGn-8-3!70, every mark/.append style={solid,fill=RdYlGn-8-3},mark=triangle*\\%
 RdYlGn-8-4!70, every mark/.append style={solid,fill=RdYlGn-8-4},mark=diamond*\\%
 RdYlGn-8-5!70, every mark/.append style={solid,fill=RdYlGn-8-5},mark=pentagon*\\%
 RdYlGn-8-6!70, every mark/.append style={solid,fill=RdYlGn-8-6},mark=x\\%
 RdYlGn-8-7!70, every mark/.append style={solid,fill=RdYlGn-8-7},mark=+\\%
 RdYlGn-8-8!70, every mark/.append style={solid,fill=RdYlGn-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-9}{%
 RdYlGn-9-1!70, every mark/.append style={solid,fill=RdYlGn-9-1},mark=*\\%
 RdYlGn-9-2!70, every mark/.append style={solid,fill=RdYlGn-9-2},mark=square*\\%
 RdYlGn-9-3!70, every mark/.append style={solid,fill=RdYlGn-9-3},mark=triangle*\\%
 RdYlGn-9-4!70, every mark/.append style={solid,fill=RdYlGn-9-4},mark=diamond*\\%
 RdYlGn-9-5!70, every mark/.append style={solid,fill=RdYlGn-9-5},mark=pentagon*\\%
 RdYlGn-9-6!70, every mark/.append style={solid,fill=RdYlGn-9-6},mark=x\\%
 RdYlGn-9-7!70, every mark/.append style={solid,fill=RdYlGn-9-7},mark=+\\%
 RdYlGn-9-8!70, every mark/.append style={solid,fill=RdYlGn-9-8},mark=star\\%
 RdYlGn-9-9!70, every mark/.append style={solid,fill=RdYlGn-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-10}{%
 RdYlGn-10-1!70, every mark/.append style={solid,fill=RdYlGn-10-1},mark=*\\%
 RdYlGn-10-2!70, every mark/.append style={solid,fill=RdYlGn-10-2},mark=square*\\%
 RdYlGn-10-3!70, every mark/.append style={solid,fill=RdYlGn-10-3},mark=triangle*\\%
 RdYlGn-10-4!70, every mark/.append style={solid,fill=RdYlGn-10-4},mark=diamond*\\%
 RdYlGn-10-5!70, every mark/.append style={solid,fill=RdYlGn-10-5},mark=pentagon*\\%
 RdYlGn-10-6!70, every mark/.append style={solid,fill=RdYlGn-10-6},mark=x\\%
 RdYlGn-10-7!70, every mark/.append style={solid,fill=RdYlGn-10-7},mark=+\\%
 RdYlGn-10-8!70, every mark/.append style={solid,fill=RdYlGn-10-8},mark=star\\%
 RdYlGn-10-9!70, every mark/.append style={solid,fill=RdYlGn-10-9},mark=oplus*\\%
 RdYlGn-10-10!70, every mark/.append style={solid,fill=RdYlGn-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-RdYlGn-11}{%
 RdYlGn-11-1!70, every mark/.append style={solid,fill=RdYlGn-11-1},mark=*\\%
 RdYlGn-11-2!70, every mark/.append style={solid,fill=RdYlGn-11-2},mark=square*\\%
 RdYlGn-11-3!70, every mark/.append style={solid,fill=RdYlGn-11-3},mark=triangle*\\%
 RdYlGn-11-4!70, every mark/.append style={solid,fill=RdYlGn-11-4},mark=diamond*\\%
 RdYlGn-11-5!70, every mark/.append style={solid,fill=RdYlGn-11-5},mark=pentagon*\\%
 RdYlGn-11-6!70, every mark/.append style={solid,fill=RdYlGn-11-6},mark=x\\%
 RdYlGn-11-7!70, every mark/.append style={solid,fill=RdYlGn-11-7},mark=+\\%
 RdYlGn-11-8!70, every mark/.append style={solid,fill=RdYlGn-11-8},mark=star\\%
 RdYlGn-11-9!70, every mark/.append style={solid,fill=RdYlGn-11-9},mark=oplus*\\%
 RdYlGn-11-10!70, every mark/.append style={solid,fill=RdYlGn-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-3}{%
 Set3-3-1!70, every mark/.append style={solid,fill=Set3-3-1},mark=*\\%
 Set3-3-2!70, every mark/.append style={solid,fill=Set3-3-2},mark=square*\\%
 Set3-3-3!70, every mark/.append style={solid,fill=Set3-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-4}{%
 Set3-4-1!70, every mark/.append style={solid,fill=Set3-4-1},mark=*\\%
 Set3-4-2!70, every mark/.append style={solid,fill=Set3-4-2},mark=square*\\%
 Set3-4-3!70, every mark/.append style={solid,fill=Set3-4-3},mark=triangle*\\%
 Set3-4-4!70, every mark/.append style={solid,fill=Set3-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-5}{%
 Set3-5-1!70, every mark/.append style={solid,fill=Set3-5-1},mark=*\\%
 Set3-5-2!70, every mark/.append style={solid,fill=Set3-5-2},mark=square*\\%
 Set3-5-3!70, every mark/.append style={solid,fill=Set3-5-3},mark=triangle*\\%
 Set3-5-4!70, every mark/.append style={solid,fill=Set3-5-4},mark=diamond*\\%
 Set3-5-5!70, every mark/.append style={solid,fill=Set3-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-6}{%
 Set3-6-1!70, every mark/.append style={solid,fill=Set3-6-1},mark=*\\%
 Set3-6-2!70, every mark/.append style={solid,fill=Set3-6-2},mark=square*\\%
 Set3-6-3!70, every mark/.append style={solid,fill=Set3-6-3},mark=triangle*\\%
 Set3-6-4!70, every mark/.append style={solid,fill=Set3-6-4},mark=diamond*\\%
 Set3-6-5!70, every mark/.append style={solid,fill=Set3-6-5},mark=pentagon*\\%
 Set3-6-6!70, every mark/.append style={solid,fill=Set3-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-7}{%
 Set3-7-1!70, every mark/.append style={solid,fill=Set3-7-1},mark=*\\%
 Set3-7-2!70, every mark/.append style={solid,fill=Set3-7-2},mark=square*\\%
 Set3-7-3!70, every mark/.append style={solid,fill=Set3-7-3},mark=triangle*\\%
 Set3-7-4!70, every mark/.append style={solid,fill=Set3-7-4},mark=diamond*\\%
 Set3-7-5!70, every mark/.append style={solid,fill=Set3-7-5},mark=pentagon*\\%
 Set3-7-6!70, every mark/.append style={solid,fill=Set3-7-6},mark=x\\%
 Set3-7-7!70, every mark/.append style={solid,fill=Set3-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-8}{%
 Set3-8-1!70, every mark/.append style={solid,fill=Set3-8-1},mark=*\\%
 Set3-8-2!70, every mark/.append style={solid,fill=Set3-8-2},mark=square*\\%
 Set3-8-3!70, every mark/.append style={solid,fill=Set3-8-3},mark=triangle*\\%
 Set3-8-4!70, every mark/.append style={solid,fill=Set3-8-4},mark=diamond*\\%
 Set3-8-5!70, every mark/.append style={solid,fill=Set3-8-5},mark=pentagon*\\%
 Set3-8-6!70, every mark/.append style={solid,fill=Set3-8-6},mark=x\\%
 Set3-8-7!70, every mark/.append style={solid,fill=Set3-8-7},mark=+\\%
 Set3-8-8!70, every mark/.append style={solid,fill=Set3-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-9}{%
 Set3-9-1!70, every mark/.append style={solid,fill=Set3-9-1},mark=*\\%
 Set3-9-2!70, every mark/.append style={solid,fill=Set3-9-2},mark=square*\\%
 Set3-9-3!70, every mark/.append style={solid,fill=Set3-9-3},mark=triangle*\\%
 Set3-9-4!70, every mark/.append style={solid,fill=Set3-9-4},mark=diamond*\\%
 Set3-9-5!70, every mark/.append style={solid,fill=Set3-9-5},mark=pentagon*\\%
 Set3-9-6!70, every mark/.append style={solid,fill=Set3-9-6},mark=x\\%
 Set3-9-7!70, every mark/.append style={solid,fill=Set3-9-7},mark=+\\%
 Set3-9-8!70, every mark/.append style={solid,fill=Set3-9-8},mark=star\\%
 Set3-9-9!70, every mark/.append style={solid,fill=Set3-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-10}{%
 Set3-10-1!70, every mark/.append style={solid,fill=Set3-10-1},mark=*\\%
 Set3-10-2!70, every mark/.append style={solid,fill=Set3-10-2},mark=square*\\%
 Set3-10-3!70, every mark/.append style={solid,fill=Set3-10-3},mark=triangle*\\%
 Set3-10-4!70, every mark/.append style={solid,fill=Set3-10-4},mark=diamond*\\%
 Set3-10-5!70, every mark/.append style={solid,fill=Set3-10-5},mark=pentagon*\\%
 Set3-10-6!70, every mark/.append style={solid,fill=Set3-10-6},mark=x\\%
 Set3-10-7!70, every mark/.append style={solid,fill=Set3-10-7},mark=+\\%
 Set3-10-8!70, every mark/.append style={solid,fill=Set3-10-8},mark=star\\%
 Set3-10-9!70, every mark/.append style={solid,fill=Set3-10-9},mark=oplus*\\%
 Set3-10-10!70, every mark/.append style={solid,fill=Set3-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-11}{%
 Set3-11-1!70, every mark/.append style={solid,fill=Set3-11-1},mark=*\\%
 Set3-11-2!70, every mark/.append style={solid,fill=Set3-11-2},mark=square*\\%
 Set3-11-3!70, every mark/.append style={solid,fill=Set3-11-3},mark=triangle*\\%
 Set3-11-4!70, every mark/.append style={solid,fill=Set3-11-4},mark=diamond*\\%
 Set3-11-5!70, every mark/.append style={solid,fill=Set3-11-5},mark=pentagon*\\%
 Set3-11-6!70, every mark/.append style={solid,fill=Set3-11-6},mark=x\\%
 Set3-11-7!70, every mark/.append style={solid,fill=Set3-11-7},mark=+\\%
 Set3-11-8!70, every mark/.append style={solid,fill=Set3-11-8},mark=star\\%
 Set3-11-9!70, every mark/.append style={solid,fill=Set3-11-9},mark=oplus*\\%
 Set3-11-10!70, every mark/.append style={solid,fill=Set3-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set3-12}{%
 Set3-12-1!70, every mark/.append style={solid,fill=Set3-12-1},mark=*\\%
 Set3-12-2!70, every mark/.append style={solid,fill=Set3-12-2},mark=square*\\%
 Set3-12-3!70, every mark/.append style={solid,fill=Set3-12-3},mark=triangle*\\%
 Set3-12-4!70, every mark/.append style={solid,fill=Set3-12-4},mark=diamond*\\%
 Set3-12-5!70, every mark/.append style={solid,fill=Set3-12-5},mark=pentagon*\\%
 Set3-12-6!70, every mark/.append style={solid,fill=Set3-12-6},mark=x\\%
 Set3-12-7!70, every mark/.append style={solid,fill=Set3-12-7},mark=+\\%
 Set3-12-8!70, every mark/.append style={solid,fill=Set3-12-8},mark=star\\%
 Set3-12-9!70, every mark/.append style={solid,fill=Set3-12-9},mark=oplus*\\%
 Set3-12-10!70, every mark/.append style={solid,fill=Set3-12-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-3}{%
 Pastel1-3-1!70, every mark/.append style={solid,fill=Pastel1-3-1},mark=*\\%
 Pastel1-3-2!70, every mark/.append style={solid,fill=Pastel1-3-2},mark=square*\\%
 Pastel1-3-3!70, every mark/.append style={solid,fill=Pastel1-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-4}{%
 Pastel1-4-1!70, every mark/.append style={solid,fill=Pastel1-4-1},mark=*\\%
 Pastel1-4-2!70, every mark/.append style={solid,fill=Pastel1-4-2},mark=square*\\%
 Pastel1-4-3!70, every mark/.append style={solid,fill=Pastel1-4-3},mark=triangle*\\%
 Pastel1-4-4!70, every mark/.append style={solid,fill=Pastel1-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-5}{%
 Pastel1-5-1!70, every mark/.append style={solid,fill=Pastel1-5-1},mark=*\\%
 Pastel1-5-2!70, every mark/.append style={solid,fill=Pastel1-5-2},mark=square*\\%
 Pastel1-5-3!70, every mark/.append style={solid,fill=Pastel1-5-3},mark=triangle*\\%
 Pastel1-5-4!70, every mark/.append style={solid,fill=Pastel1-5-4},mark=diamond*\\%
 Pastel1-5-5!70, every mark/.append style={solid,fill=Pastel1-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-6}{%
 Pastel1-6-1!70, every mark/.append style={solid,fill=Pastel1-6-1},mark=*\\%
 Pastel1-6-2!70, every mark/.append style={solid,fill=Pastel1-6-2},mark=square*\\%
 Pastel1-6-3!70, every mark/.append style={solid,fill=Pastel1-6-3},mark=triangle*\\%
 Pastel1-6-4!70, every mark/.append style={solid,fill=Pastel1-6-4},mark=diamond*\\%
 Pastel1-6-5!70, every mark/.append style={solid,fill=Pastel1-6-5},mark=pentagon*\\%
 Pastel1-6-6!70, every mark/.append style={solid,fill=Pastel1-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-7}{%
 Pastel1-7-1!70, every mark/.append style={solid,fill=Pastel1-7-1},mark=*\\%
 Pastel1-7-2!70, every mark/.append style={solid,fill=Pastel1-7-2},mark=square*\\%
 Pastel1-7-3!70, every mark/.append style={solid,fill=Pastel1-7-3},mark=triangle*\\%
 Pastel1-7-4!70, every mark/.append style={solid,fill=Pastel1-7-4},mark=diamond*\\%
 Pastel1-7-5!70, every mark/.append style={solid,fill=Pastel1-7-5},mark=pentagon*\\%
 Pastel1-7-6!70, every mark/.append style={solid,fill=Pastel1-7-6},mark=x\\%
 Pastel1-7-7!70, every mark/.append style={solid,fill=Pastel1-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-8}{%
 Pastel1-8-1!70, every mark/.append style={solid,fill=Pastel1-8-1},mark=*\\%
 Pastel1-8-2!70, every mark/.append style={solid,fill=Pastel1-8-2},mark=square*\\%
 Pastel1-8-3!70, every mark/.append style={solid,fill=Pastel1-8-3},mark=triangle*\\%
 Pastel1-8-4!70, every mark/.append style={solid,fill=Pastel1-8-4},mark=diamond*\\%
 Pastel1-8-5!70, every mark/.append style={solid,fill=Pastel1-8-5},mark=pentagon*\\%
 Pastel1-8-6!70, every mark/.append style={solid,fill=Pastel1-8-6},mark=x\\%
 Pastel1-8-7!70, every mark/.append style={solid,fill=Pastel1-8-7},mark=+\\%
 Pastel1-8-8!70, every mark/.append style={solid,fill=Pastel1-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel1-9}{%
 Pastel1-9-1!70, every mark/.append style={solid,fill=Pastel1-9-1},mark=*\\%
 Pastel1-9-2!70, every mark/.append style={solid,fill=Pastel1-9-2},mark=square*\\%
 Pastel1-9-3!70, every mark/.append style={solid,fill=Pastel1-9-3},mark=triangle*\\%
 Pastel1-9-4!70, every mark/.append style={solid,fill=Pastel1-9-4},mark=diamond*\\%
 Pastel1-9-5!70, every mark/.append style={solid,fill=Pastel1-9-5},mark=pentagon*\\%
 Pastel1-9-6!70, every mark/.append style={solid,fill=Pastel1-9-6},mark=x\\%
 Pastel1-9-7!70, every mark/.append style={solid,fill=Pastel1-9-7},mark=+\\%
 Pastel1-9-8!70, every mark/.append style={solid,fill=Pastel1-9-8},mark=star\\%
 Pastel1-9-9!70, every mark/.append style={solid,fill=Pastel1-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-3}{%
 Set1-3-1!70, every mark/.append style={solid,fill=Set1-3-1},mark=*\\%
 Set1-3-2!70, every mark/.append style={solid,fill=Set1-3-2},mark=square*\\%
 Set1-3-3!70, every mark/.append style={solid,fill=Set1-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-4}{%
 Set1-4-1!70, every mark/.append style={solid,fill=Set1-4-1},mark=*\\%
 Set1-4-2!70, every mark/.append style={solid,fill=Set1-4-2},mark=square*\\%
 Set1-4-3!70, every mark/.append style={solid,fill=Set1-4-3},mark=triangle*\\%
 Set1-4-4!70, every mark/.append style={solid,fill=Set1-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-5}{%
 Set1-5-1!70, every mark/.append style={solid,fill=Set1-5-1},mark=*\\%
 Set1-5-2!70, every mark/.append style={solid,fill=Set1-5-2},mark=square*\\%
 Set1-5-3!70, every mark/.append style={solid,fill=Set1-5-3},mark=triangle*\\%
 Set1-5-4!70, every mark/.append style={solid,fill=Set1-5-4},mark=diamond*\\%
 Set1-5-5!70, every mark/.append style={solid,fill=Set1-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-6}{%
 Set1-6-1!70, every mark/.append style={solid,fill=Set1-6-1},mark=*\\%
 Set1-6-2!70, every mark/.append style={solid,fill=Set1-6-2},mark=square*\\%
 Set1-6-3!70, every mark/.append style={solid,fill=Set1-6-3},mark=triangle*\\%
 Set1-6-4!70, every mark/.append style={solid,fill=Set1-6-4},mark=diamond*\\%
 Set1-6-5!70, every mark/.append style={solid,fill=Set1-6-5},mark=pentagon*\\%
 Set1-6-6!70, every mark/.append style={solid,fill=Set1-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-7}{%
 Set1-7-1!70, every mark/.append style={solid,fill=Set1-7-1},mark=*\\%
 Set1-7-2!70, every mark/.append style={solid,fill=Set1-7-2},mark=square*\\%
 Set1-7-3!70, every mark/.append style={solid,fill=Set1-7-3},mark=triangle*\\%
 Set1-7-4!70, every mark/.append style={solid,fill=Set1-7-4},mark=diamond*\\%
 Set1-7-5!70, every mark/.append style={solid,fill=Set1-7-5},mark=pentagon*\\%
 Set1-7-6!70, every mark/.append style={solid,fill=Set1-7-6},mark=x\\%
 Set1-7-7!70, every mark/.append style={solid,fill=Set1-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-8}{%
 Set1-8-1!70, every mark/.append style={solid,fill=Set1-8-1},mark=*\\%
 Set1-8-2!70, every mark/.append style={solid,fill=Set1-8-2},mark=square*\\%
 Set1-8-3!70, every mark/.append style={solid,fill=Set1-8-3},mark=triangle*\\%
 Set1-8-4!70, every mark/.append style={solid,fill=Set1-8-4},mark=diamond*\\%
 Set1-8-5!70, every mark/.append style={solid,fill=Set1-8-5},mark=pentagon*\\%
 Set1-8-6!70, every mark/.append style={solid,fill=Set1-8-6},mark=x\\%
 Set1-8-7!70, every mark/.append style={solid,fill=Set1-8-7},mark=+\\%
 Set1-8-8!70, every mark/.append style={solid,fill=Set1-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set1-9}{%
 Set1-9-1!70, every mark/.append style={solid,fill=Set1-9-1},mark=*\\%
 Set1-9-2!70, every mark/.append style={solid,fill=Set1-9-2},mark=square*\\%
 Set1-9-3!70, every mark/.append style={solid,fill=Set1-9-3},mark=triangle*\\%
 Set1-9-4!70, every mark/.append style={solid,fill=Set1-9-4},mark=diamond*\\%
 Set1-9-5!70, every mark/.append style={solid,fill=Set1-9-5},mark=pentagon*\\%
 Set1-9-6!70, every mark/.append style={solid,fill=Set1-9-6},mark=x\\%
 Set1-9-7!70, every mark/.append style={solid,fill=Set1-9-7},mark=+\\%
 Set1-9-8!70, every mark/.append style={solid,fill=Set1-9-8},mark=star\\%
 Set1-9-9!70, every mark/.append style={solid,fill=Set1-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-3}{%
 Pastel2-3-1!70, every mark/.append style={solid,fill=Pastel2-3-1},mark=*\\%
 Pastel2-3-2!70, every mark/.append style={solid,fill=Pastel2-3-2},mark=square*\\%
 Pastel2-3-3!70, every mark/.append style={solid,fill=Pastel2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-4}{%
 Pastel2-4-1!70, every mark/.append style={solid,fill=Pastel2-4-1},mark=*\\%
 Pastel2-4-2!70, every mark/.append style={solid,fill=Pastel2-4-2},mark=square*\\%
 Pastel2-4-3!70, every mark/.append style={solid,fill=Pastel2-4-3},mark=triangle*\\%
 Pastel2-4-4!70, every mark/.append style={solid,fill=Pastel2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-5}{%
 Pastel2-5-1!70, every mark/.append style={solid,fill=Pastel2-5-1},mark=*\\%
 Pastel2-5-2!70, every mark/.append style={solid,fill=Pastel2-5-2},mark=square*\\%
 Pastel2-5-3!70, every mark/.append style={solid,fill=Pastel2-5-3},mark=triangle*\\%
 Pastel2-5-4!70, every mark/.append style={solid,fill=Pastel2-5-4},mark=diamond*\\%
 Pastel2-5-5!70, every mark/.append style={solid,fill=Pastel2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-6}{%
 Pastel2-6-1!70, every mark/.append style={solid,fill=Pastel2-6-1},mark=*\\%
 Pastel2-6-2!70, every mark/.append style={solid,fill=Pastel2-6-2},mark=square*\\%
 Pastel2-6-3!70, every mark/.append style={solid,fill=Pastel2-6-3},mark=triangle*\\%
 Pastel2-6-4!70, every mark/.append style={solid,fill=Pastel2-6-4},mark=diamond*\\%
 Pastel2-6-5!70, every mark/.append style={solid,fill=Pastel2-6-5},mark=pentagon*\\%
 Pastel2-6-6!70, every mark/.append style={solid,fill=Pastel2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-7}{%
 Pastel2-7-1!70, every mark/.append style={solid,fill=Pastel2-7-1},mark=*\\%
 Pastel2-7-2!70, every mark/.append style={solid,fill=Pastel2-7-2},mark=square*\\%
 Pastel2-7-3!70, every mark/.append style={solid,fill=Pastel2-7-3},mark=triangle*\\%
 Pastel2-7-4!70, every mark/.append style={solid,fill=Pastel2-7-4},mark=diamond*\\%
 Pastel2-7-5!70, every mark/.append style={solid,fill=Pastel2-7-5},mark=pentagon*\\%
 Pastel2-7-6!70, every mark/.append style={solid,fill=Pastel2-7-6},mark=x\\%
 Pastel2-7-7!70, every mark/.append style={solid,fill=Pastel2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Pastel2-8}{%
 Pastel2-8-1!70, every mark/.append style={solid,fill=Pastel2-8-1},mark=*\\%
 Pastel2-8-2!70, every mark/.append style={solid,fill=Pastel2-8-2},mark=square*\\%
 Pastel2-8-3!70, every mark/.append style={solid,fill=Pastel2-8-3},mark=triangle*\\%
 Pastel2-8-4!70, every mark/.append style={solid,fill=Pastel2-8-4},mark=diamond*\\%
 Pastel2-8-5!70, every mark/.append style={solid,fill=Pastel2-8-5},mark=pentagon*\\%
 Pastel2-8-6!70, every mark/.append style={solid,fill=Pastel2-8-6},mark=x\\%
 Pastel2-8-7!70, every mark/.append style={solid,fill=Pastel2-8-7},mark=+\\%
 Pastel2-8-8!70, every mark/.append style={solid,fill=Pastel2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-3}{%
 Set2-3-1!70, every mark/.append style={solid,fill=Set2-3-1},mark=*\\%
 Set2-3-2!70, every mark/.append style={solid,fill=Set2-3-2},mark=square*\\%
 Set2-3-3!70, every mark/.append style={solid,fill=Set2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-4}{%
 Set2-4-1!70, every mark/.append style={solid,fill=Set2-4-1},mark=*\\%
 Set2-4-2!70, every mark/.append style={solid,fill=Set2-4-2},mark=square*\\%
 Set2-4-3!70, every mark/.append style={solid,fill=Set2-4-3},mark=triangle*\\%
 Set2-4-4!70, every mark/.append style={solid,fill=Set2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-5}{%
 Set2-5-1!70, every mark/.append style={solid,fill=Set2-5-1},mark=*\\%
 Set2-5-2!70, every mark/.append style={solid,fill=Set2-5-2},mark=square*\\%
 Set2-5-3!70, every mark/.append style={solid,fill=Set2-5-3},mark=triangle*\\%
 Set2-5-4!70, every mark/.append style={solid,fill=Set2-5-4},mark=diamond*\\%
 Set2-5-5!70, every mark/.append style={solid,fill=Set2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-6}{%
 Set2-6-1!70, every mark/.append style={solid,fill=Set2-6-1},mark=*\\%
 Set2-6-2!70, every mark/.append style={solid,fill=Set2-6-2},mark=square*\\%
 Set2-6-3!70, every mark/.append style={solid,fill=Set2-6-3},mark=triangle*\\%
 Set2-6-4!70, every mark/.append style={solid,fill=Set2-6-4},mark=diamond*\\%
 Set2-6-5!70, every mark/.append style={solid,fill=Set2-6-5},mark=pentagon*\\%
 Set2-6-6!70, every mark/.append style={solid,fill=Set2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-7}{%
 Set2-7-1!70, every mark/.append style={solid,fill=Set2-7-1},mark=*\\%
 Set2-7-2!70, every mark/.append style={solid,fill=Set2-7-2},mark=square*\\%
 Set2-7-3!70, every mark/.append style={solid,fill=Set2-7-3},mark=triangle*\\%
 Set2-7-4!70, every mark/.append style={solid,fill=Set2-7-4},mark=diamond*\\%
 Set2-7-5!70, every mark/.append style={solid,fill=Set2-7-5},mark=pentagon*\\%
 Set2-7-6!70, every mark/.append style={solid,fill=Set2-7-6},mark=x\\%
 Set2-7-7!70, every mark/.append style={solid,fill=Set2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Set2-8}{%
 Set2-8-1!70, every mark/.append style={solid,fill=Set2-8-1},mark=*\\%
 Set2-8-2!70, every mark/.append style={solid,fill=Set2-8-2},mark=square*\\%
 Set2-8-3!70, every mark/.append style={solid,fill=Set2-8-3},mark=triangle*\\%
 Set2-8-4!70, every mark/.append style={solid,fill=Set2-8-4},mark=diamond*\\%
 Set2-8-5!70, every mark/.append style={solid,fill=Set2-8-5},mark=pentagon*\\%
 Set2-8-6!70, every mark/.append style={solid,fill=Set2-8-6},mark=x\\%
 Set2-8-7!70, every mark/.append style={solid,fill=Set2-8-7},mark=+\\%
 Set2-8-8!70, every mark/.append style={solid,fill=Set2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-3}{%
 Dark2-3-1!70, every mark/.append style={solid,fill=Dark2-3-1},mark=*\\%
 Dark2-3-2!70, every mark/.append style={solid,fill=Dark2-3-2},mark=square*\\%
 Dark2-3-3!70, every mark/.append style={solid,fill=Dark2-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-4}{%
 Dark2-4-1!70, every mark/.append style={solid,fill=Dark2-4-1},mark=*\\%
 Dark2-4-2!70, every mark/.append style={solid,fill=Dark2-4-2},mark=square*\\%
 Dark2-4-3!70, every mark/.append style={solid,fill=Dark2-4-3},mark=triangle*\\%
 Dark2-4-4!70, every mark/.append style={solid,fill=Dark2-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-5}{%
 Dark2-5-1!70, every mark/.append style={solid,fill=Dark2-5-1},mark=*\\%
 Dark2-5-2!70, every mark/.append style={solid,fill=Dark2-5-2},mark=square*\\%
 Dark2-5-3!70, every mark/.append style={solid,fill=Dark2-5-3},mark=triangle*\\%
 Dark2-5-4!70, every mark/.append style={solid,fill=Dark2-5-4},mark=diamond*\\%
 Dark2-5-5!70, every mark/.append style={solid,fill=Dark2-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-6}{%
 Dark2-6-1!70, every mark/.append style={solid,fill=Dark2-6-1},mark=*\\%
 Dark2-6-2!70, every mark/.append style={solid,fill=Dark2-6-2},mark=square*\\%
 Dark2-6-3!70, every mark/.append style={solid,fill=Dark2-6-3},mark=triangle*\\%
 Dark2-6-4!70, every mark/.append style={solid,fill=Dark2-6-4},mark=diamond*\\%
 Dark2-6-5!70, every mark/.append style={solid,fill=Dark2-6-5},mark=pentagon*\\%
 Dark2-6-6!70, every mark/.append style={solid,fill=Dark2-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-7}{%
 Dark2-7-1!70, every mark/.append style={solid,fill=Dark2-7-1},mark=*\\%
 Dark2-7-2!70, every mark/.append style={solid,fill=Dark2-7-2},mark=square*\\%
 Dark2-7-3!70, every mark/.append style={solid,fill=Dark2-7-3},mark=triangle*\\%
 Dark2-7-4!70, every mark/.append style={solid,fill=Dark2-7-4},mark=diamond*\\%
 Dark2-7-5!70, every mark/.append style={solid,fill=Dark2-7-5},mark=pentagon*\\%
 Dark2-7-6!70, every mark/.append style={solid,fill=Dark2-7-6},mark=x\\%
 Dark2-7-7!70, every mark/.append style={solid,fill=Dark2-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Dark2-8}{%
 Dark2-8-1!70, every mark/.append style={solid,fill=Dark2-8-1},mark=*\\%
 Dark2-8-2!70, every mark/.append style={solid,fill=Dark2-8-2},mark=square*\\%
 Dark2-8-3!70, every mark/.append style={solid,fill=Dark2-8-3},mark=triangle*\\%
 Dark2-8-4!70, every mark/.append style={solid,fill=Dark2-8-4},mark=diamond*\\%
 Dark2-8-5!70, every mark/.append style={solid,fill=Dark2-8-5},mark=pentagon*\\%
 Dark2-8-6!70, every mark/.append style={solid,fill=Dark2-8-6},mark=x\\%
 Dark2-8-7!70, every mark/.append style={solid,fill=Dark2-8-7},mark=+\\%
 Dark2-8-8!70, every mark/.append style={solid,fill=Dark2-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-3}{%
 Paired-3-1!70, every mark/.append style={solid,fill=Paired-3-1},mark=*\\%
 Paired-3-2!70, every mark/.append style={solid,fill=Paired-3-2},mark=square*\\%
 Paired-3-3!70, every mark/.append style={solid,fill=Paired-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-4}{%
 Paired-4-1!70, every mark/.append style={solid,fill=Paired-4-1},mark=*\\%
 Paired-4-2!70, every mark/.append style={solid,fill=Paired-4-2},mark=square*\\%
 Paired-4-3!70, every mark/.append style={solid,fill=Paired-4-3},mark=triangle*\\%
 Paired-4-4!70, every mark/.append style={solid,fill=Paired-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-5}{%
 Paired-5-1!70, every mark/.append style={solid,fill=Paired-5-1},mark=*\\%
 Paired-5-2!70, every mark/.append style={solid,fill=Paired-5-2},mark=square*\\%
 Paired-5-3!70, every mark/.append style={solid,fill=Paired-5-3},mark=triangle*\\%
 Paired-5-4!70, every mark/.append style={solid,fill=Paired-5-4},mark=diamond*\\%
 Paired-5-5!70, every mark/.append style={solid,fill=Paired-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-6}{%
 Paired-6-1!70, every mark/.append style={solid,fill=Paired-6-1},mark=*\\%
 Paired-6-2!70, every mark/.append style={solid,fill=Paired-6-2},mark=square*\\%
 Paired-6-3!70, every mark/.append style={solid,fill=Paired-6-3},mark=triangle*\\%
 Paired-6-4!70, every mark/.append style={solid,fill=Paired-6-4},mark=diamond*\\%
 Paired-6-5!70, every mark/.append style={solid,fill=Paired-6-5},mark=pentagon*\\%
 Paired-6-6!70, every mark/.append style={solid,fill=Paired-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-7}{%
 Paired-7-1!70, every mark/.append style={solid,fill=Paired-7-1},mark=*\\%
 Paired-7-2!70, every mark/.append style={solid,fill=Paired-7-2},mark=square*\\%
 Paired-7-3!70, every mark/.append style={solid,fill=Paired-7-3},mark=triangle*\\%
 Paired-7-4!70, every mark/.append style={solid,fill=Paired-7-4},mark=diamond*\\%
 Paired-7-5!70, every mark/.append style={solid,fill=Paired-7-5},mark=pentagon*\\%
 Paired-7-6!70, every mark/.append style={solid,fill=Paired-7-6},mark=x\\%
 Paired-7-7!70, every mark/.append style={solid,fill=Paired-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-8}{%
 Paired-8-1!70, every mark/.append style={solid,fill=Paired-8-1},mark=*\\%
 Paired-8-2!70, every mark/.append style={solid,fill=Paired-8-2},mark=square*\\%
 Paired-8-3!70, every mark/.append style={solid,fill=Paired-8-3},mark=triangle*\\%
 Paired-8-4!70, every mark/.append style={solid,fill=Paired-8-4},mark=diamond*\\%
 Paired-8-5!70, every mark/.append style={solid,fill=Paired-8-5},mark=pentagon*\\%
 Paired-8-6!70, every mark/.append style={solid,fill=Paired-8-6},mark=x\\%
 Paired-8-7!70, every mark/.append style={solid,fill=Paired-8-7},mark=+\\%
 Paired-8-8!70, every mark/.append style={solid,fill=Paired-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-9}{%
 Paired-9-1!70, every mark/.append style={solid,fill=Paired-9-1},mark=*\\%
 Paired-9-2!70, every mark/.append style={solid,fill=Paired-9-2},mark=square*\\%
 Paired-9-3!70, every mark/.append style={solid,fill=Paired-9-3},mark=triangle*\\%
 Paired-9-4!70, every mark/.append style={solid,fill=Paired-9-4},mark=diamond*\\%
 Paired-9-5!70, every mark/.append style={solid,fill=Paired-9-5},mark=pentagon*\\%
 Paired-9-6!70, every mark/.append style={solid,fill=Paired-9-6},mark=x\\%
 Paired-9-7!70, every mark/.append style={solid,fill=Paired-9-7},mark=+\\%
 Paired-9-8!70, every mark/.append style={solid,fill=Paired-9-8},mark=star\\%
 Paired-9-9!70, every mark/.append style={solid,fill=Paired-9-9},mark=oplus*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-10}{%
 Paired-10-1!70, every mark/.append style={solid,fill=Paired-10-1},mark=*\\%
 Paired-10-2!70, every mark/.append style={solid,fill=Paired-10-2},mark=square*\\%
 Paired-10-3!70, every mark/.append style={solid,fill=Paired-10-3},mark=triangle*\\%
 Paired-10-4!70, every mark/.append style={solid,fill=Paired-10-4},mark=diamond*\\%
 Paired-10-5!70, every mark/.append style={solid,fill=Paired-10-5},mark=pentagon*\\%
 Paired-10-6!70, every mark/.append style={solid,fill=Paired-10-6},mark=x\\%
 Paired-10-7!70, every mark/.append style={solid,fill=Paired-10-7},mark=+\\%
 Paired-10-8!70, every mark/.append style={solid,fill=Paired-10-8},mark=star\\%
 Paired-10-9!70, every mark/.append style={solid,fill=Paired-10-9},mark=oplus*\\%
 Paired-10-10!70, every mark/.append style={solid,fill=Paired-10-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-11}{%
 Paired-11-1!70, every mark/.append style={solid,fill=Paired-11-1},mark=*\\%
 Paired-11-2!70, every mark/.append style={solid,fill=Paired-11-2},mark=square*\\%
 Paired-11-3!70, every mark/.append style={solid,fill=Paired-11-3},mark=triangle*\\%
 Paired-11-4!70, every mark/.append style={solid,fill=Paired-11-4},mark=diamond*\\%
 Paired-11-5!70, every mark/.append style={solid,fill=Paired-11-5},mark=pentagon*\\%
 Paired-11-6!70, every mark/.append style={solid,fill=Paired-11-6},mark=x\\%
 Paired-11-7!70, every mark/.append style={solid,fill=Paired-11-7},mark=+\\%
 Paired-11-8!70, every mark/.append style={solid,fill=Paired-11-8},mark=star\\%
 Paired-11-9!70, every mark/.append style={solid,fill=Paired-11-9},mark=oplus*\\%
 Paired-11-10!70, every mark/.append style={solid,fill=Paired-11-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Paired-12}{%
 Paired-12-1!70, every mark/.append style={solid,fill=Paired-12-1},mark=*\\%
 Paired-12-2!70, every mark/.append style={solid,fill=Paired-12-2},mark=square*\\%
 Paired-12-3!70, every mark/.append style={solid,fill=Paired-12-3},mark=triangle*\\%
 Paired-12-4!70, every mark/.append style={solid,fill=Paired-12-4},mark=diamond*\\%
 Paired-12-5!70, every mark/.append style={solid,fill=Paired-12-5},mark=pentagon*\\%
 Paired-12-6!70, every mark/.append style={solid,fill=Paired-12-6},mark=x\\%
 Paired-12-7!70, every mark/.append style={solid,fill=Paired-12-7},mark=+\\%
 Paired-12-8!70, every mark/.append style={solid,fill=Paired-12-8},mark=star\\%
 Paired-12-9!70, every mark/.append style={solid,fill=Paired-12-9},mark=oplus*\\%
 Paired-12-10!70, every mark/.append style={solid,fill=Paired-12-10},mark=otimes*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-3}{%
 Accent-3-1!70, every mark/.append style={solid,fill=Accent-3-1},mark=*\\%
 Accent-3-2!70, every mark/.append style={solid,fill=Accent-3-2},mark=square*\\%
 Accent-3-3!70, every mark/.append style={solid,fill=Accent-3-3},mark=triangle*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-4}{%
 Accent-4-1!70, every mark/.append style={solid,fill=Accent-4-1},mark=*\\%
 Accent-4-2!70, every mark/.append style={solid,fill=Accent-4-2},mark=square*\\%
 Accent-4-3!70, every mark/.append style={solid,fill=Accent-4-3},mark=triangle*\\%
 Accent-4-4!70, every mark/.append style={solid,fill=Accent-4-4},mark=diamond*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-5}{%
 Accent-5-1!70, every mark/.append style={solid,fill=Accent-5-1},mark=*\\%
 Accent-5-2!70, every mark/.append style={solid,fill=Accent-5-2},mark=square*\\%
 Accent-5-3!70, every mark/.append style={solid,fill=Accent-5-3},mark=triangle*\\%
 Accent-5-4!70, every mark/.append style={solid,fill=Accent-5-4},mark=diamond*\\%
 Accent-5-5!70, every mark/.append style={solid,fill=Accent-5-5},mark=pentagon*\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-6}{%
 Accent-6-1!70, every mark/.append style={solid,fill=Accent-6-1},mark=*\\%
 Accent-6-2!70, every mark/.append style={solid,fill=Accent-6-2},mark=square*\\%
 Accent-6-3!70, every mark/.append style={solid,fill=Accent-6-3},mark=triangle*\\%
 Accent-6-4!70, every mark/.append style={solid,fill=Accent-6-4},mark=diamond*\\%
 Accent-6-5!70, every mark/.append style={solid,fill=Accent-6-5},mark=pentagon*\\%
 Accent-6-6!70, every mark/.append style={solid,fill=Accent-6-6},mark=x\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-7}{%
 Accent-7-1!70, every mark/.append style={solid,fill=Accent-7-1},mark=*\\%
 Accent-7-2!70, every mark/.append style={solid,fill=Accent-7-2},mark=square*\\%
 Accent-7-3!70, every mark/.append style={solid,fill=Accent-7-3},mark=triangle*\\%
 Accent-7-4!70, every mark/.append style={solid,fill=Accent-7-4},mark=diamond*\\%
 Accent-7-5!70, every mark/.append style={solid,fill=Accent-7-5},mark=pentagon*\\%
 Accent-7-6!70, every mark/.append style={solid,fill=Accent-7-6},mark=x\\%
 Accent-7-7!70, every mark/.append style={solid,fill=Accent-7-7},mark=+\\%
}
\pgfplotscreateplotcyclelist{LightMark-Accent-8}{%
 Accent-8-1!70, every mark/.append style={solid,fill=Accent-8-1},mark=*\\%
 Accent-8-2!70, every mark/.append style={solid,fill=Accent-8-2},mark=square*\\%
 Accent-8-3!70, every mark/.append style={solid,fill=Accent-8-3},mark=triangle*\\%
 Accent-8-4!70, every mark/.append style={solid,fill=Accent-8-4},mark=diamond*\\%
 Accent-8-5!70, every mark/.append style={solid,fill=Accent-8-5},mark=pentagon*\\%
 Accent-8-6!70, every mark/.append style={solid,fill=Accent-8-6},mark=x\\%
 Accent-8-7!70, every mark/.append style={solid,fill=Accent-8-7},mark=+\\%
 Accent-8-8!70, every mark/.append style={solid,fill=Accent-8-8},mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-3}{%
 YlGn-3-1,mark=x\\%
 YlGn-3-2,mark=+\\%
 YlGn-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-4}{%
 YlGn-4-1,mark=x\\%
 YlGn-4-2,mark=+\\%
 YlGn-4-3,mark=-\\%
 YlGn-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-5}{%
 YlGn-5-1,mark=x\\%
 YlGn-5-2,mark=+\\%
 YlGn-5-3,mark=-\\%
 YlGn-5-4,mark=|\\%
 YlGn-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-6}{%
 YlGn-6-1,mark=x\\%
 YlGn-6-2,mark=+\\%
 YlGn-6-3,mark=-\\%
 YlGn-6-4,mark=|\\%
 YlGn-6-5,mark=asterisk\\%
 YlGn-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-7}{%
 YlGn-7-1,mark=x\\%
 YlGn-7-2,mark=+\\%
 YlGn-7-3,mark=-\\%
 YlGn-7-4,mark=|\\%
 YlGn-7-5,mark=asterisk\\%
 YlGn-7-6,mark=star\\%
 YlGn-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-8}{%
 YlGn-8-1,mark=x\\%
 YlGn-8-2,mark=+\\%
 YlGn-8-3,mark=-\\%
 YlGn-8-4,mark=|\\%
 YlGn-8-5,mark=asterisk\\%
 YlGn-8-6,mark=star\\%
 YlGn-8-7,mark=10-pointed star\\%
 YlGn-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGn-9}{%
 YlGn-9-1,mark=x\\%
 YlGn-9-2,mark=+\\%
 YlGn-9-3,mark=-\\%
 YlGn-9-4,mark=|\\%
 YlGn-9-5,mark=asterisk\\%
 YlGn-9-6,mark=star\\%
 YlGn-9-7,mark=10-pointed star\\%
 YlGn-9-8,mark=Mercedes star\\%
 YlGn-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-3}{%
 YlGnBu-3-1,mark=x\\%
 YlGnBu-3-2,mark=+\\%
 YlGnBu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-4}{%
 YlGnBu-4-1,mark=x\\%
 YlGnBu-4-2,mark=+\\%
 YlGnBu-4-3,mark=-\\%
 YlGnBu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-5}{%
 YlGnBu-5-1,mark=x\\%
 YlGnBu-5-2,mark=+\\%
 YlGnBu-5-3,mark=-\\%
 YlGnBu-5-4,mark=|\\%
 YlGnBu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-6}{%
 YlGnBu-6-1,mark=x\\%
 YlGnBu-6-2,mark=+\\%
 YlGnBu-6-3,mark=-\\%
 YlGnBu-6-4,mark=|\\%
 YlGnBu-6-5,mark=asterisk\\%
 YlGnBu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-7}{%
 YlGnBu-7-1,mark=x\\%
 YlGnBu-7-2,mark=+\\%
 YlGnBu-7-3,mark=-\\%
 YlGnBu-7-4,mark=|\\%
 YlGnBu-7-5,mark=asterisk\\%
 YlGnBu-7-6,mark=star\\%
 YlGnBu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-8}{%
 YlGnBu-8-1,mark=x\\%
 YlGnBu-8-2,mark=+\\%
 YlGnBu-8-3,mark=-\\%
 YlGnBu-8-4,mark=|\\%
 YlGnBu-8-5,mark=asterisk\\%
 YlGnBu-8-6,mark=star\\%
 YlGnBu-8-7,mark=10-pointed star\\%
 YlGnBu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlGnBu-9}{%
 YlGnBu-9-1,mark=x\\%
 YlGnBu-9-2,mark=+\\%
 YlGnBu-9-3,mark=-\\%
 YlGnBu-9-4,mark=|\\%
 YlGnBu-9-5,mark=asterisk\\%
 YlGnBu-9-6,mark=star\\%
 YlGnBu-9-7,mark=10-pointed star\\%
 YlGnBu-9-8,mark=Mercedes star\\%
 YlGnBu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-3}{%
 GnBu-3-1,mark=x\\%
 GnBu-3-2,mark=+\\%
 GnBu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-4}{%
 GnBu-4-1,mark=x\\%
 GnBu-4-2,mark=+\\%
 GnBu-4-3,mark=-\\%
 GnBu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-5}{%
 GnBu-5-1,mark=x\\%
 GnBu-5-2,mark=+\\%
 GnBu-5-3,mark=-\\%
 GnBu-5-4,mark=|\\%
 GnBu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-6}{%
 GnBu-6-1,mark=x\\%
 GnBu-6-2,mark=+\\%
 GnBu-6-3,mark=-\\%
 GnBu-6-4,mark=|\\%
 GnBu-6-5,mark=asterisk\\%
 GnBu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-7}{%
 GnBu-7-1,mark=x\\%
 GnBu-7-2,mark=+\\%
 GnBu-7-3,mark=-\\%
 GnBu-7-4,mark=|\\%
 GnBu-7-5,mark=asterisk\\%
 GnBu-7-6,mark=star\\%
 GnBu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-8}{%
 GnBu-8-1,mark=x\\%
 GnBu-8-2,mark=+\\%
 GnBu-8-3,mark=-\\%
 GnBu-8-4,mark=|\\%
 GnBu-8-5,mark=asterisk\\%
 GnBu-8-6,mark=star\\%
 GnBu-8-7,mark=10-pointed star\\%
 GnBu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-GnBu-9}{%
 GnBu-9-1,mark=x\\%
 GnBu-9-2,mark=+\\%
 GnBu-9-3,mark=-\\%
 GnBu-9-4,mark=|\\%
 GnBu-9-5,mark=asterisk\\%
 GnBu-9-6,mark=star\\%
 GnBu-9-7,mark=10-pointed star\\%
 GnBu-9-8,mark=Mercedes star\\%
 GnBu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-3}{%
 BuGn-3-1,mark=x\\%
 BuGn-3-2,mark=+\\%
 BuGn-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-4}{%
 BuGn-4-1,mark=x\\%
 BuGn-4-2,mark=+\\%
 BuGn-4-3,mark=-\\%
 BuGn-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-5}{%
 BuGn-5-1,mark=x\\%
 BuGn-5-2,mark=+\\%
 BuGn-5-3,mark=-\\%
 BuGn-5-4,mark=|\\%
 BuGn-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-6}{%
 BuGn-6-1,mark=x\\%
 BuGn-6-2,mark=+\\%
 BuGn-6-3,mark=-\\%
 BuGn-6-4,mark=|\\%
 BuGn-6-5,mark=asterisk\\%
 BuGn-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-7}{%
 BuGn-7-1,mark=x\\%
 BuGn-7-2,mark=+\\%
 BuGn-7-3,mark=-\\%
 BuGn-7-4,mark=|\\%
 BuGn-7-5,mark=asterisk\\%
 BuGn-7-6,mark=star\\%
 BuGn-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-8}{%
 BuGn-8-1,mark=x\\%
 BuGn-8-2,mark=+\\%
 BuGn-8-3,mark=-\\%
 BuGn-8-4,mark=|\\%
 BuGn-8-5,mark=asterisk\\%
 BuGn-8-6,mark=star\\%
 BuGn-8-7,mark=10-pointed star\\%
 BuGn-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuGn-9}{%
 BuGn-9-1,mark=x\\%
 BuGn-9-2,mark=+\\%
 BuGn-9-3,mark=-\\%
 BuGn-9-4,mark=|\\%
 BuGn-9-5,mark=asterisk\\%
 BuGn-9-6,mark=star\\%
 BuGn-9-7,mark=10-pointed star\\%
 BuGn-9-8,mark=Mercedes star\\%
 BuGn-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-3}{%
 PuBuGn-3-1,mark=x\\%
 PuBuGn-3-2,mark=+\\%
 PuBuGn-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-4}{%
 PuBuGn-4-1,mark=x\\%
 PuBuGn-4-2,mark=+\\%
 PuBuGn-4-3,mark=-\\%
 PuBuGn-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-5}{%
 PuBuGn-5-1,mark=x\\%
 PuBuGn-5-2,mark=+\\%
 PuBuGn-5-3,mark=-\\%
 PuBuGn-5-4,mark=|\\%
 PuBuGn-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-6}{%
 PuBuGn-6-1,mark=x\\%
 PuBuGn-6-2,mark=+\\%
 PuBuGn-6-3,mark=-\\%
 PuBuGn-6-4,mark=|\\%
 PuBuGn-6-5,mark=asterisk\\%
 PuBuGn-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-7}{%
 PuBuGn-7-1,mark=x\\%
 PuBuGn-7-2,mark=+\\%
 PuBuGn-7-3,mark=-\\%
 PuBuGn-7-4,mark=|\\%
 PuBuGn-7-5,mark=asterisk\\%
 PuBuGn-7-6,mark=star\\%
 PuBuGn-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-8}{%
 PuBuGn-8-1,mark=x\\%
 PuBuGn-8-2,mark=+\\%
 PuBuGn-8-3,mark=-\\%
 PuBuGn-8-4,mark=|\\%
 PuBuGn-8-5,mark=asterisk\\%
 PuBuGn-8-6,mark=star\\%
 PuBuGn-8-7,mark=10-pointed star\\%
 PuBuGn-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBuGn-9}{%
 PuBuGn-9-1,mark=x\\%
 PuBuGn-9-2,mark=+\\%
 PuBuGn-9-3,mark=-\\%
 PuBuGn-9-4,mark=|\\%
 PuBuGn-9-5,mark=asterisk\\%
 PuBuGn-9-6,mark=star\\%
 PuBuGn-9-7,mark=10-pointed star\\%
 PuBuGn-9-8,mark=Mercedes star\\%
 PuBuGn-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-3}{%
 PuBu-3-1,mark=x\\%
 PuBu-3-2,mark=+\\%
 PuBu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-4}{%
 PuBu-4-1,mark=x\\%
 PuBu-4-2,mark=+\\%
 PuBu-4-3,mark=-\\%
 PuBu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-5}{%
 PuBu-5-1,mark=x\\%
 PuBu-5-2,mark=+\\%
 PuBu-5-3,mark=-\\%
 PuBu-5-4,mark=|\\%
 PuBu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-6}{%
 PuBu-6-1,mark=x\\%
 PuBu-6-2,mark=+\\%
 PuBu-6-3,mark=-\\%
 PuBu-6-4,mark=|\\%
 PuBu-6-5,mark=asterisk\\%
 PuBu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-7}{%
 PuBu-7-1,mark=x\\%
 PuBu-7-2,mark=+\\%
 PuBu-7-3,mark=-\\%
 PuBu-7-4,mark=|\\%
 PuBu-7-5,mark=asterisk\\%
 PuBu-7-6,mark=star\\%
 PuBu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-8}{%
 PuBu-8-1,mark=x\\%
 PuBu-8-2,mark=+\\%
 PuBu-8-3,mark=-\\%
 PuBu-8-4,mark=|\\%
 PuBu-8-5,mark=asterisk\\%
 PuBu-8-6,mark=star\\%
 PuBu-8-7,mark=10-pointed star\\%
 PuBu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuBu-9}{%
 PuBu-9-1,mark=x\\%
 PuBu-9-2,mark=+\\%
 PuBu-9-3,mark=-\\%
 PuBu-9-4,mark=|\\%
 PuBu-9-5,mark=asterisk\\%
 PuBu-9-6,mark=star\\%
 PuBu-9-7,mark=10-pointed star\\%
 PuBu-9-8,mark=Mercedes star\\%
 PuBu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-3}{%
 BuPu-3-1,mark=x\\%
 BuPu-3-2,mark=+\\%
 BuPu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-4}{%
 BuPu-4-1,mark=x\\%
 BuPu-4-2,mark=+\\%
 BuPu-4-3,mark=-\\%
 BuPu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-5}{%
 BuPu-5-1,mark=x\\%
 BuPu-5-2,mark=+\\%
 BuPu-5-3,mark=-\\%
 BuPu-5-4,mark=|\\%
 BuPu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-6}{%
 BuPu-6-1,mark=x\\%
 BuPu-6-2,mark=+\\%
 BuPu-6-3,mark=-\\%
 BuPu-6-4,mark=|\\%
 BuPu-6-5,mark=asterisk\\%
 BuPu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-7}{%
 BuPu-7-1,mark=x\\%
 BuPu-7-2,mark=+\\%
 BuPu-7-3,mark=-\\%
 BuPu-7-4,mark=|\\%
 BuPu-7-5,mark=asterisk\\%
 BuPu-7-6,mark=star\\%
 BuPu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-8}{%
 BuPu-8-1,mark=x\\%
 BuPu-8-2,mark=+\\%
 BuPu-8-3,mark=-\\%
 BuPu-8-4,mark=|\\%
 BuPu-8-5,mark=asterisk\\%
 BuPu-8-6,mark=star\\%
 BuPu-8-7,mark=10-pointed star\\%
 BuPu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BuPu-9}{%
 BuPu-9-1,mark=x\\%
 BuPu-9-2,mark=+\\%
 BuPu-9-3,mark=-\\%
 BuPu-9-4,mark=|\\%
 BuPu-9-5,mark=asterisk\\%
 BuPu-9-6,mark=star\\%
 BuPu-9-7,mark=10-pointed star\\%
 BuPu-9-8,mark=Mercedes star\\%
 BuPu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-3}{%
 RdPu-3-1,mark=x\\%
 RdPu-3-2,mark=+\\%
 RdPu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-4}{%
 RdPu-4-1,mark=x\\%
 RdPu-4-2,mark=+\\%
 RdPu-4-3,mark=-\\%
 RdPu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-5}{%
 RdPu-5-1,mark=x\\%
 RdPu-5-2,mark=+\\%
 RdPu-5-3,mark=-\\%
 RdPu-5-4,mark=|\\%
 RdPu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-6}{%
 RdPu-6-1,mark=x\\%
 RdPu-6-2,mark=+\\%
 RdPu-6-3,mark=-\\%
 RdPu-6-4,mark=|\\%
 RdPu-6-5,mark=asterisk\\%
 RdPu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-7}{%
 RdPu-7-1,mark=x\\%
 RdPu-7-2,mark=+\\%
 RdPu-7-3,mark=-\\%
 RdPu-7-4,mark=|\\%
 RdPu-7-5,mark=asterisk\\%
 RdPu-7-6,mark=star\\%
 RdPu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-8}{%
 RdPu-8-1,mark=x\\%
 RdPu-8-2,mark=+\\%
 RdPu-8-3,mark=-\\%
 RdPu-8-4,mark=|\\%
 RdPu-8-5,mark=asterisk\\%
 RdPu-8-6,mark=star\\%
 RdPu-8-7,mark=10-pointed star\\%
 RdPu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdPu-9}{%
 RdPu-9-1,mark=x\\%
 RdPu-9-2,mark=+\\%
 RdPu-9-3,mark=-\\%
 RdPu-9-4,mark=|\\%
 RdPu-9-5,mark=asterisk\\%
 RdPu-9-6,mark=star\\%
 RdPu-9-7,mark=10-pointed star\\%
 RdPu-9-8,mark=Mercedes star\\%
 RdPu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-3}{%
 PuRd-3-1,mark=x\\%
 PuRd-3-2,mark=+\\%
 PuRd-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-4}{%
 PuRd-4-1,mark=x\\%
 PuRd-4-2,mark=+\\%
 PuRd-4-3,mark=-\\%
 PuRd-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-5}{%
 PuRd-5-1,mark=x\\%
 PuRd-5-2,mark=+\\%
 PuRd-5-3,mark=-\\%
 PuRd-5-4,mark=|\\%
 PuRd-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-6}{%
 PuRd-6-1,mark=x\\%
 PuRd-6-2,mark=+\\%
 PuRd-6-3,mark=-\\%
 PuRd-6-4,mark=|\\%
 PuRd-6-5,mark=asterisk\\%
 PuRd-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-7}{%
 PuRd-7-1,mark=x\\%
 PuRd-7-2,mark=+\\%
 PuRd-7-3,mark=-\\%
 PuRd-7-4,mark=|\\%
 PuRd-7-5,mark=asterisk\\%
 PuRd-7-6,mark=star\\%
 PuRd-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-8}{%
 PuRd-8-1,mark=x\\%
 PuRd-8-2,mark=+\\%
 PuRd-8-3,mark=-\\%
 PuRd-8-4,mark=|\\%
 PuRd-8-5,mark=asterisk\\%
 PuRd-8-6,mark=star\\%
 PuRd-8-7,mark=10-pointed star\\%
 PuRd-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuRd-9}{%
 PuRd-9-1,mark=x\\%
 PuRd-9-2,mark=+\\%
 PuRd-9-3,mark=-\\%
 PuRd-9-4,mark=|\\%
 PuRd-9-5,mark=asterisk\\%
 PuRd-9-6,mark=star\\%
 PuRd-9-7,mark=10-pointed star\\%
 PuRd-9-8,mark=Mercedes star\\%
 PuRd-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-3}{%
 OrRd-3-1,mark=x\\%
 OrRd-3-2,mark=+\\%
 OrRd-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-4}{%
 OrRd-4-1,mark=x\\%
 OrRd-4-2,mark=+\\%
 OrRd-4-3,mark=-\\%
 OrRd-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-5}{%
 OrRd-5-1,mark=x\\%
 OrRd-5-2,mark=+\\%
 OrRd-5-3,mark=-\\%
 OrRd-5-4,mark=|\\%
 OrRd-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-6}{%
 OrRd-6-1,mark=x\\%
 OrRd-6-2,mark=+\\%
 OrRd-6-3,mark=-\\%
 OrRd-6-4,mark=|\\%
 OrRd-6-5,mark=asterisk\\%
 OrRd-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-7}{%
 OrRd-7-1,mark=x\\%
 OrRd-7-2,mark=+\\%
 OrRd-7-3,mark=-\\%
 OrRd-7-4,mark=|\\%
 OrRd-7-5,mark=asterisk\\%
 OrRd-7-6,mark=star\\%
 OrRd-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-8}{%
 OrRd-8-1,mark=x\\%
 OrRd-8-2,mark=+\\%
 OrRd-8-3,mark=-\\%
 OrRd-8-4,mark=|\\%
 OrRd-8-5,mark=asterisk\\%
 OrRd-8-6,mark=star\\%
 OrRd-8-7,mark=10-pointed star\\%
 OrRd-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-OrRd-9}{%
 OrRd-9-1,mark=x\\%
 OrRd-9-2,mark=+\\%
 OrRd-9-3,mark=-\\%
 OrRd-9-4,mark=|\\%
 OrRd-9-5,mark=asterisk\\%
 OrRd-9-6,mark=star\\%
 OrRd-9-7,mark=10-pointed star\\%
 OrRd-9-8,mark=Mercedes star\\%
 OrRd-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-3}{%
 YlOrRd-3-1,mark=x\\%
 YlOrRd-3-2,mark=+\\%
 YlOrRd-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-4}{%
 YlOrRd-4-1,mark=x\\%
 YlOrRd-4-2,mark=+\\%
 YlOrRd-4-3,mark=-\\%
 YlOrRd-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-5}{%
 YlOrRd-5-1,mark=x\\%
 YlOrRd-5-2,mark=+\\%
 YlOrRd-5-3,mark=-\\%
 YlOrRd-5-4,mark=|\\%
 YlOrRd-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-6}{%
 YlOrRd-6-1,mark=x\\%
 YlOrRd-6-2,mark=+\\%
 YlOrRd-6-3,mark=-\\%
 YlOrRd-6-4,mark=|\\%
 YlOrRd-6-5,mark=asterisk\\%
 YlOrRd-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-7}{%
 YlOrRd-7-1,mark=x\\%
 YlOrRd-7-2,mark=+\\%
 YlOrRd-7-3,mark=-\\%
 YlOrRd-7-4,mark=|\\%
 YlOrRd-7-5,mark=asterisk\\%
 YlOrRd-7-6,mark=star\\%
 YlOrRd-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-8}{%
 YlOrRd-8-1,mark=x\\%
 YlOrRd-8-2,mark=+\\%
 YlOrRd-8-3,mark=-\\%
 YlOrRd-8-4,mark=|\\%
 YlOrRd-8-5,mark=asterisk\\%
 YlOrRd-8-6,mark=star\\%
 YlOrRd-8-7,mark=10-pointed star\\%
 YlOrRd-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrRd-9}{%
 YlOrRd-9-1,mark=x\\%
 YlOrRd-9-2,mark=+\\%
 YlOrRd-9-3,mark=-\\%
 YlOrRd-9-4,mark=|\\%
 YlOrRd-9-5,mark=asterisk\\%
 YlOrRd-9-6,mark=star\\%
 YlOrRd-9-7,mark=10-pointed star\\%
 YlOrRd-9-8,mark=Mercedes star\\%
 YlOrRd-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-3}{%
 YlOrBr-3-1,mark=x\\%
 YlOrBr-3-2,mark=+\\%
 YlOrBr-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-4}{%
 YlOrBr-4-1,mark=x\\%
 YlOrBr-4-2,mark=+\\%
 YlOrBr-4-3,mark=-\\%
 YlOrBr-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-5}{%
 YlOrBr-5-1,mark=x\\%
 YlOrBr-5-2,mark=+\\%
 YlOrBr-5-3,mark=-\\%
 YlOrBr-5-4,mark=|\\%
 YlOrBr-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-6}{%
 YlOrBr-6-1,mark=x\\%
 YlOrBr-6-2,mark=+\\%
 YlOrBr-6-3,mark=-\\%
 YlOrBr-6-4,mark=|\\%
 YlOrBr-6-5,mark=asterisk\\%
 YlOrBr-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-7}{%
 YlOrBr-7-1,mark=x\\%
 YlOrBr-7-2,mark=+\\%
 YlOrBr-7-3,mark=-\\%
 YlOrBr-7-4,mark=|\\%
 YlOrBr-7-5,mark=asterisk\\%
 YlOrBr-7-6,mark=star\\%
 YlOrBr-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-8}{%
 YlOrBr-8-1,mark=x\\%
 YlOrBr-8-2,mark=+\\%
 YlOrBr-8-3,mark=-\\%
 YlOrBr-8-4,mark=|\\%
 YlOrBr-8-5,mark=asterisk\\%
 YlOrBr-8-6,mark=star\\%
 YlOrBr-8-7,mark=10-pointed star\\%
 YlOrBr-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-YlOrBr-9}{%
 YlOrBr-9-1,mark=x\\%
 YlOrBr-9-2,mark=+\\%
 YlOrBr-9-3,mark=-\\%
 YlOrBr-9-4,mark=|\\%
 YlOrBr-9-5,mark=asterisk\\%
 YlOrBr-9-6,mark=star\\%
 YlOrBr-9-7,mark=10-pointed star\\%
 YlOrBr-9-8,mark=Mercedes star\\%
 YlOrBr-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-3}{%
 Purples-3-1,mark=x\\%
 Purples-3-2,mark=+\\%
 Purples-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-4}{%
 Purples-4-1,mark=x\\%
 Purples-4-2,mark=+\\%
 Purples-4-3,mark=-\\%
 Purples-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-5}{%
 Purples-5-1,mark=x\\%
 Purples-5-2,mark=+\\%
 Purples-5-3,mark=-\\%
 Purples-5-4,mark=|\\%
 Purples-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-6}{%
 Purples-6-1,mark=x\\%
 Purples-6-2,mark=+\\%
 Purples-6-3,mark=-\\%
 Purples-6-4,mark=|\\%
 Purples-6-5,mark=asterisk\\%
 Purples-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-7}{%
 Purples-7-1,mark=x\\%
 Purples-7-2,mark=+\\%
 Purples-7-3,mark=-\\%
 Purples-7-4,mark=|\\%
 Purples-7-5,mark=asterisk\\%
 Purples-7-6,mark=star\\%
 Purples-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-8}{%
 Purples-8-1,mark=x\\%
 Purples-8-2,mark=+\\%
 Purples-8-3,mark=-\\%
 Purples-8-4,mark=|\\%
 Purples-8-5,mark=asterisk\\%
 Purples-8-6,mark=star\\%
 Purples-8-7,mark=10-pointed star\\%
 Purples-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Purples-9}{%
 Purples-9-1,mark=x\\%
 Purples-9-2,mark=+\\%
 Purples-9-3,mark=-\\%
 Purples-9-4,mark=|\\%
 Purples-9-5,mark=asterisk\\%
 Purples-9-6,mark=star\\%
 Purples-9-7,mark=10-pointed star\\%
 Purples-9-8,mark=Mercedes star\\%
 Purples-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-3}{%
 Blues-3-1,mark=x\\%
 Blues-3-2,mark=+\\%
 Blues-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-4}{%
 Blues-4-1,mark=x\\%
 Blues-4-2,mark=+\\%
 Blues-4-3,mark=-\\%
 Blues-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-5}{%
 Blues-5-1,mark=x\\%
 Blues-5-2,mark=+\\%
 Blues-5-3,mark=-\\%
 Blues-5-4,mark=|\\%
 Blues-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-6}{%
 Blues-6-1,mark=x\\%
 Blues-6-2,mark=+\\%
 Blues-6-3,mark=-\\%
 Blues-6-4,mark=|\\%
 Blues-6-5,mark=asterisk\\%
 Blues-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-7}{%
 Blues-7-1,mark=x\\%
 Blues-7-2,mark=+\\%
 Blues-7-3,mark=-\\%
 Blues-7-4,mark=|\\%
 Blues-7-5,mark=asterisk\\%
 Blues-7-6,mark=star\\%
 Blues-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-8}{%
 Blues-8-1,mark=x\\%
 Blues-8-2,mark=+\\%
 Blues-8-3,mark=-\\%
 Blues-8-4,mark=|\\%
 Blues-8-5,mark=asterisk\\%
 Blues-8-6,mark=star\\%
 Blues-8-7,mark=10-pointed star\\%
 Blues-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Blues-9}{%
 Blues-9-1,mark=x\\%
 Blues-9-2,mark=+\\%
 Blues-9-3,mark=-\\%
 Blues-9-4,mark=|\\%
 Blues-9-5,mark=asterisk\\%
 Blues-9-6,mark=star\\%
 Blues-9-7,mark=10-pointed star\\%
 Blues-9-8,mark=Mercedes star\\%
 Blues-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-3}{%
 Greens-3-1,mark=x\\%
 Greens-3-2,mark=+\\%
 Greens-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-4}{%
 Greens-4-1,mark=x\\%
 Greens-4-2,mark=+\\%
 Greens-4-3,mark=-\\%
 Greens-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-5}{%
 Greens-5-1,mark=x\\%
 Greens-5-2,mark=+\\%
 Greens-5-3,mark=-\\%
 Greens-5-4,mark=|\\%
 Greens-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-6}{%
 Greens-6-1,mark=x\\%
 Greens-6-2,mark=+\\%
 Greens-6-3,mark=-\\%
 Greens-6-4,mark=|\\%
 Greens-6-5,mark=asterisk\\%
 Greens-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-7}{%
 Greens-7-1,mark=x\\%
 Greens-7-2,mark=+\\%
 Greens-7-3,mark=-\\%
 Greens-7-4,mark=|\\%
 Greens-7-5,mark=asterisk\\%
 Greens-7-6,mark=star\\%
 Greens-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-8}{%
 Greens-8-1,mark=x\\%
 Greens-8-2,mark=+\\%
 Greens-8-3,mark=-\\%
 Greens-8-4,mark=|\\%
 Greens-8-5,mark=asterisk\\%
 Greens-8-6,mark=star\\%
 Greens-8-7,mark=10-pointed star\\%
 Greens-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greens-9}{%
 Greens-9-1,mark=x\\%
 Greens-9-2,mark=+\\%
 Greens-9-3,mark=-\\%
 Greens-9-4,mark=|\\%
 Greens-9-5,mark=asterisk\\%
 Greens-9-6,mark=star\\%
 Greens-9-7,mark=10-pointed star\\%
 Greens-9-8,mark=Mercedes star\\%
 Greens-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-3}{%
 Oranges-3-1,mark=x\\%
 Oranges-3-2,mark=+\\%
 Oranges-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-4}{%
 Oranges-4-1,mark=x\\%
 Oranges-4-2,mark=+\\%
 Oranges-4-3,mark=-\\%
 Oranges-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-5}{%
 Oranges-5-1,mark=x\\%
 Oranges-5-2,mark=+\\%
 Oranges-5-3,mark=-\\%
 Oranges-5-4,mark=|\\%
 Oranges-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-6}{%
 Oranges-6-1,mark=x\\%
 Oranges-6-2,mark=+\\%
 Oranges-6-3,mark=-\\%
 Oranges-6-4,mark=|\\%
 Oranges-6-5,mark=asterisk\\%
 Oranges-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-7}{%
 Oranges-7-1,mark=x\\%
 Oranges-7-2,mark=+\\%
 Oranges-7-3,mark=-\\%
 Oranges-7-4,mark=|\\%
 Oranges-7-5,mark=asterisk\\%
 Oranges-7-6,mark=star\\%
 Oranges-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-8}{%
 Oranges-8-1,mark=x\\%
 Oranges-8-2,mark=+\\%
 Oranges-8-3,mark=-\\%
 Oranges-8-4,mark=|\\%
 Oranges-8-5,mark=asterisk\\%
 Oranges-8-6,mark=star\\%
 Oranges-8-7,mark=10-pointed star\\%
 Oranges-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Oranges-9}{%
 Oranges-9-1,mark=x\\%
 Oranges-9-2,mark=+\\%
 Oranges-9-3,mark=-\\%
 Oranges-9-4,mark=|\\%
 Oranges-9-5,mark=asterisk\\%
 Oranges-9-6,mark=star\\%
 Oranges-9-7,mark=10-pointed star\\%
 Oranges-9-8,mark=Mercedes star\\%
 Oranges-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-3}{%
 Reds-3-1,mark=x\\%
 Reds-3-2,mark=+\\%
 Reds-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-4}{%
 Reds-4-1,mark=x\\%
 Reds-4-2,mark=+\\%
 Reds-4-3,mark=-\\%
 Reds-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-5}{%
 Reds-5-1,mark=x\\%
 Reds-5-2,mark=+\\%
 Reds-5-3,mark=-\\%
 Reds-5-4,mark=|\\%
 Reds-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-6}{%
 Reds-6-1,mark=x\\%
 Reds-6-2,mark=+\\%
 Reds-6-3,mark=-\\%
 Reds-6-4,mark=|\\%
 Reds-6-5,mark=asterisk\\%
 Reds-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-7}{%
 Reds-7-1,mark=x\\%
 Reds-7-2,mark=+\\%
 Reds-7-3,mark=-\\%
 Reds-7-4,mark=|\\%
 Reds-7-5,mark=asterisk\\%
 Reds-7-6,mark=star\\%
 Reds-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-8}{%
 Reds-8-1,mark=x\\%
 Reds-8-2,mark=+\\%
 Reds-8-3,mark=-\\%
 Reds-8-4,mark=|\\%
 Reds-8-5,mark=asterisk\\%
 Reds-8-6,mark=star\\%
 Reds-8-7,mark=10-pointed star\\%
 Reds-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Reds-9}{%
 Reds-9-1,mark=x\\%
 Reds-9-2,mark=+\\%
 Reds-9-3,mark=-\\%
 Reds-9-4,mark=|\\%
 Reds-9-5,mark=asterisk\\%
 Reds-9-6,mark=star\\%
 Reds-9-7,mark=10-pointed star\\%
 Reds-9-8,mark=Mercedes star\\%
 Reds-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-3}{%
 Greys-3-1,mark=x\\%
 Greys-3-2,mark=+\\%
 Greys-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-4}{%
 Greys-4-1,mark=x\\%
 Greys-4-2,mark=+\\%
 Greys-4-3,mark=-\\%
 Greys-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-5}{%
 Greys-5-1,mark=x\\%
 Greys-5-2,mark=+\\%
 Greys-5-3,mark=-\\%
 Greys-5-4,mark=|\\%
 Greys-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-6}{%
 Greys-6-1,mark=x\\%
 Greys-6-2,mark=+\\%
 Greys-6-3,mark=-\\%
 Greys-6-4,mark=|\\%
 Greys-6-5,mark=asterisk\\%
 Greys-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-7}{%
 Greys-7-1,mark=x\\%
 Greys-7-2,mark=+\\%
 Greys-7-3,mark=-\\%
 Greys-7-4,mark=|\\%
 Greys-7-5,mark=asterisk\\%
 Greys-7-6,mark=star\\%
 Greys-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-8}{%
 Greys-8-1,mark=x\\%
 Greys-8-2,mark=+\\%
 Greys-8-3,mark=-\\%
 Greys-8-4,mark=|\\%
 Greys-8-5,mark=asterisk\\%
 Greys-8-6,mark=star\\%
 Greys-8-7,mark=10-pointed star\\%
 Greys-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Greys-9}{%
 Greys-9-1,mark=x\\%
 Greys-9-2,mark=+\\%
 Greys-9-3,mark=-\\%
 Greys-9-4,mark=|\\%
 Greys-9-5,mark=asterisk\\%
 Greys-9-6,mark=star\\%
 Greys-9-7,mark=10-pointed star\\%
 Greys-9-8,mark=Mercedes star\\%
 Greys-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-3}{%
 PuOr-3-1,mark=x\\%
 PuOr-3-2,mark=+\\%
 PuOr-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-4}{%
 PuOr-4-1,mark=x\\%
 PuOr-4-2,mark=+\\%
 PuOr-4-3,mark=-\\%
 PuOr-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-5}{%
 PuOr-5-1,mark=x\\%
 PuOr-5-2,mark=+\\%
 PuOr-5-3,mark=-\\%
 PuOr-5-4,mark=|\\%
 PuOr-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-6}{%
 PuOr-6-1,mark=x\\%
 PuOr-6-2,mark=+\\%
 PuOr-6-3,mark=-\\%
 PuOr-6-4,mark=|\\%
 PuOr-6-5,mark=asterisk\\%
 PuOr-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-7}{%
 PuOr-7-1,mark=x\\%
 PuOr-7-2,mark=+\\%
 PuOr-7-3,mark=-\\%
 PuOr-7-4,mark=|\\%
 PuOr-7-5,mark=asterisk\\%
 PuOr-7-6,mark=star\\%
 PuOr-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-8}{%
 PuOr-8-1,mark=x\\%
 PuOr-8-2,mark=+\\%
 PuOr-8-3,mark=-\\%
 PuOr-8-4,mark=|\\%
 PuOr-8-5,mark=asterisk\\%
 PuOr-8-6,mark=star\\%
 PuOr-8-7,mark=10-pointed star\\%
 PuOr-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-9}{%
 PuOr-9-1,mark=x\\%
 PuOr-9-2,mark=+\\%
 PuOr-9-3,mark=-\\%
 PuOr-9-4,mark=|\\%
 PuOr-9-5,mark=asterisk\\%
 PuOr-9-6,mark=star\\%
 PuOr-9-7,mark=10-pointed star\\%
 PuOr-9-8,mark=Mercedes star\\%
 PuOr-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-10}{%
 PuOr-10-1,mark=x\\%
 PuOr-10-2,mark=+\\%
 PuOr-10-3,mark=-\\%
 PuOr-10-4,mark=|\\%
 PuOr-10-5,mark=asterisk\\%
 PuOr-10-6,mark=star\\%
 PuOr-10-7,mark=10-pointed star\\%
 PuOr-10-8,mark=Mercedes star\\%
 PuOr-10-9,mark=Mercedes star flipped\\%
 PuOr-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PuOr-11}{%
 PuOr-11-1,mark=x\\%
 PuOr-11-2,mark=+\\%
 PuOr-11-3,mark=-\\%
 PuOr-11-4,mark=|\\%
 PuOr-11-5,mark=asterisk\\%
 PuOr-11-6,mark=star\\%
 PuOr-11-7,mark=10-pointed star\\%
 PuOr-11-8,mark=Mercedes star\\%
 PuOr-11-9,mark=Mercedes star flipped\\%
 PuOr-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-3}{%
 BrBG-3-1,mark=x\\%
 BrBG-3-2,mark=+\\%
 BrBG-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-4}{%
 BrBG-4-1,mark=x\\%
 BrBG-4-2,mark=+\\%
 BrBG-4-3,mark=-\\%
 BrBG-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-5}{%
 BrBG-5-1,mark=x\\%
 BrBG-5-2,mark=+\\%
 BrBG-5-3,mark=-\\%
 BrBG-5-4,mark=|\\%
 BrBG-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-6}{%
 BrBG-6-1,mark=x\\%
 BrBG-6-2,mark=+\\%
 BrBG-6-3,mark=-\\%
 BrBG-6-4,mark=|\\%
 BrBG-6-5,mark=asterisk\\%
 BrBG-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-7}{%
 BrBG-7-1,mark=x\\%
 BrBG-7-2,mark=+\\%
 BrBG-7-3,mark=-\\%
 BrBG-7-4,mark=|\\%
 BrBG-7-5,mark=asterisk\\%
 BrBG-7-6,mark=star\\%
 BrBG-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-8}{%
 BrBG-8-1,mark=x\\%
 BrBG-8-2,mark=+\\%
 BrBG-8-3,mark=-\\%
 BrBG-8-4,mark=|\\%
 BrBG-8-5,mark=asterisk\\%
 BrBG-8-6,mark=star\\%
 BrBG-8-7,mark=10-pointed star\\%
 BrBG-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-9}{%
 BrBG-9-1,mark=x\\%
 BrBG-9-2,mark=+\\%
 BrBG-9-3,mark=-\\%
 BrBG-9-4,mark=|\\%
 BrBG-9-5,mark=asterisk\\%
 BrBG-9-6,mark=star\\%
 BrBG-9-7,mark=10-pointed star\\%
 BrBG-9-8,mark=Mercedes star\\%
 BrBG-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-10}{%
 BrBG-10-1,mark=x\\%
 BrBG-10-2,mark=+\\%
 BrBG-10-3,mark=-\\%
 BrBG-10-4,mark=|\\%
 BrBG-10-5,mark=asterisk\\%
 BrBG-10-6,mark=star\\%
 BrBG-10-7,mark=10-pointed star\\%
 BrBG-10-8,mark=Mercedes star\\%
 BrBG-10-9,mark=Mercedes star flipped\\%
 BrBG-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-BrBG-11}{%
 BrBG-11-1,mark=x\\%
 BrBG-11-2,mark=+\\%
 BrBG-11-3,mark=-\\%
 BrBG-11-4,mark=|\\%
 BrBG-11-5,mark=asterisk\\%
 BrBG-11-6,mark=star\\%
 BrBG-11-7,mark=10-pointed star\\%
 BrBG-11-8,mark=Mercedes star\\%
 BrBG-11-9,mark=Mercedes star flipped\\%
 BrBG-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-3}{%
 PRGn-3-1,mark=x\\%
 PRGn-3-2,mark=+\\%
 PRGn-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-4}{%
 PRGn-4-1,mark=x\\%
 PRGn-4-2,mark=+\\%
 PRGn-4-3,mark=-\\%
 PRGn-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-5}{%
 PRGn-5-1,mark=x\\%
 PRGn-5-2,mark=+\\%
 PRGn-5-3,mark=-\\%
 PRGn-5-4,mark=|\\%
 PRGn-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-6}{%
 PRGn-6-1,mark=x\\%
 PRGn-6-2,mark=+\\%
 PRGn-6-3,mark=-\\%
 PRGn-6-4,mark=|\\%
 PRGn-6-5,mark=asterisk\\%
 PRGn-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-7}{%
 PRGn-7-1,mark=x\\%
 PRGn-7-2,mark=+\\%
 PRGn-7-3,mark=-\\%
 PRGn-7-4,mark=|\\%
 PRGn-7-5,mark=asterisk\\%
 PRGn-7-6,mark=star\\%
 PRGn-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-8}{%
 PRGn-8-1,mark=x\\%
 PRGn-8-2,mark=+\\%
 PRGn-8-3,mark=-\\%
 PRGn-8-4,mark=|\\%
 PRGn-8-5,mark=asterisk\\%
 PRGn-8-6,mark=star\\%
 PRGn-8-7,mark=10-pointed star\\%
 PRGn-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-9}{%
 PRGn-9-1,mark=x\\%
 PRGn-9-2,mark=+\\%
 PRGn-9-3,mark=-\\%
 PRGn-9-4,mark=|\\%
 PRGn-9-5,mark=asterisk\\%
 PRGn-9-6,mark=star\\%
 PRGn-9-7,mark=10-pointed star\\%
 PRGn-9-8,mark=Mercedes star\\%
 PRGn-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-10}{%
 PRGn-10-1,mark=x\\%
 PRGn-10-2,mark=+\\%
 PRGn-10-3,mark=-\\%
 PRGn-10-4,mark=|\\%
 PRGn-10-5,mark=asterisk\\%
 PRGn-10-6,mark=star\\%
 PRGn-10-7,mark=10-pointed star\\%
 PRGn-10-8,mark=Mercedes star\\%
 PRGn-10-9,mark=Mercedes star flipped\\%
 PRGn-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PRGn-11}{%
 PRGn-11-1,mark=x\\%
 PRGn-11-2,mark=+\\%
 PRGn-11-3,mark=-\\%
 PRGn-11-4,mark=|\\%
 PRGn-11-5,mark=asterisk\\%
 PRGn-11-6,mark=star\\%
 PRGn-11-7,mark=10-pointed star\\%
 PRGn-11-8,mark=Mercedes star\\%
 PRGn-11-9,mark=Mercedes star flipped\\%
 PRGn-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-3}{%
 PiYG-3-1,mark=x\\%
 PiYG-3-2,mark=+\\%
 PiYG-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-4}{%
 PiYG-4-1,mark=x\\%
 PiYG-4-2,mark=+\\%
 PiYG-4-3,mark=-\\%
 PiYG-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-5}{%
 PiYG-5-1,mark=x\\%
 PiYG-5-2,mark=+\\%
 PiYG-5-3,mark=-\\%
 PiYG-5-4,mark=|\\%
 PiYG-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-6}{%
 PiYG-6-1,mark=x\\%
 PiYG-6-2,mark=+\\%
 PiYG-6-3,mark=-\\%
 PiYG-6-4,mark=|\\%
 PiYG-6-5,mark=asterisk\\%
 PiYG-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-7}{%
 PiYG-7-1,mark=x\\%
 PiYG-7-2,mark=+\\%
 PiYG-7-3,mark=-\\%
 PiYG-7-4,mark=|\\%
 PiYG-7-5,mark=asterisk\\%
 PiYG-7-6,mark=star\\%
 PiYG-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-8}{%
 PiYG-8-1,mark=x\\%
 PiYG-8-2,mark=+\\%
 PiYG-8-3,mark=-\\%
 PiYG-8-4,mark=|\\%
 PiYG-8-5,mark=asterisk\\%
 PiYG-8-6,mark=star\\%
 PiYG-8-7,mark=10-pointed star\\%
 PiYG-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-9}{%
 PiYG-9-1,mark=x\\%
 PiYG-9-2,mark=+\\%
 PiYG-9-3,mark=-\\%
 PiYG-9-4,mark=|\\%
 PiYG-9-5,mark=asterisk\\%
 PiYG-9-6,mark=star\\%
 PiYG-9-7,mark=10-pointed star\\%
 PiYG-9-8,mark=Mercedes star\\%
 PiYG-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-10}{%
 PiYG-10-1,mark=x\\%
 PiYG-10-2,mark=+\\%
 PiYG-10-3,mark=-\\%
 PiYG-10-4,mark=|\\%
 PiYG-10-5,mark=asterisk\\%
 PiYG-10-6,mark=star\\%
 PiYG-10-7,mark=10-pointed star\\%
 PiYG-10-8,mark=Mercedes star\\%
 PiYG-10-9,mark=Mercedes star flipped\\%
 PiYG-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-PiYG-11}{%
 PiYG-11-1,mark=x\\%
 PiYG-11-2,mark=+\\%
 PiYG-11-3,mark=-\\%
 PiYG-11-4,mark=|\\%
 PiYG-11-5,mark=asterisk\\%
 PiYG-11-6,mark=star\\%
 PiYG-11-7,mark=10-pointed star\\%
 PiYG-11-8,mark=Mercedes star\\%
 PiYG-11-9,mark=Mercedes star flipped\\%
 PiYG-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-3}{%
 RdBu-3-1,mark=x\\%
 RdBu-3-2,mark=+\\%
 RdBu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-4}{%
 RdBu-4-1,mark=x\\%
 RdBu-4-2,mark=+\\%
 RdBu-4-3,mark=-\\%
 RdBu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-5}{%
 RdBu-5-1,mark=x\\%
 RdBu-5-2,mark=+\\%
 RdBu-5-3,mark=-\\%
 RdBu-5-4,mark=|\\%
 RdBu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-6}{%
 RdBu-6-1,mark=x\\%
 RdBu-6-2,mark=+\\%
 RdBu-6-3,mark=-\\%
 RdBu-6-4,mark=|\\%
 RdBu-6-5,mark=asterisk\\%
 RdBu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-7}{%
 RdBu-7-1,mark=x\\%
 RdBu-7-2,mark=+\\%
 RdBu-7-3,mark=-\\%
 RdBu-7-4,mark=|\\%
 RdBu-7-5,mark=asterisk\\%
 RdBu-7-6,mark=star\\%
 RdBu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-8}{%
 RdBu-8-1,mark=x\\%
 RdBu-8-2,mark=+\\%
 RdBu-8-3,mark=-\\%
 RdBu-8-4,mark=|\\%
 RdBu-8-5,mark=asterisk\\%
 RdBu-8-6,mark=star\\%
 RdBu-8-7,mark=10-pointed star\\%
 RdBu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-9}{%
 RdBu-9-1,mark=x\\%
 RdBu-9-2,mark=+\\%
 RdBu-9-3,mark=-\\%
 RdBu-9-4,mark=|\\%
 RdBu-9-5,mark=asterisk\\%
 RdBu-9-6,mark=star\\%
 RdBu-9-7,mark=10-pointed star\\%
 RdBu-9-8,mark=Mercedes star\\%
 RdBu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-10}{%
 RdBu-10-1,mark=x\\%
 RdBu-10-2,mark=+\\%
 RdBu-10-3,mark=-\\%
 RdBu-10-4,mark=|\\%
 RdBu-10-5,mark=asterisk\\%
 RdBu-10-6,mark=star\\%
 RdBu-10-7,mark=10-pointed star\\%
 RdBu-10-8,mark=Mercedes star\\%
 RdBu-10-9,mark=Mercedes star flipped\\%
 RdBu-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdBu-11}{%
 RdBu-11-1,mark=x\\%
 RdBu-11-2,mark=+\\%
 RdBu-11-3,mark=-\\%
 RdBu-11-4,mark=|\\%
 RdBu-11-5,mark=asterisk\\%
 RdBu-11-6,mark=star\\%
 RdBu-11-7,mark=10-pointed star\\%
 RdBu-11-8,mark=Mercedes star\\%
 RdBu-11-9,mark=Mercedes star flipped\\%
 RdBu-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-3}{%
 RdGy-3-1,mark=x\\%
 RdGy-3-2,mark=+\\%
 RdGy-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-4}{%
 RdGy-4-1,mark=x\\%
 RdGy-4-2,mark=+\\%
 RdGy-4-3,mark=-\\%
 RdGy-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-5}{%
 RdGy-5-1,mark=x\\%
 RdGy-5-2,mark=+\\%
 RdGy-5-3,mark=-\\%
 RdGy-5-4,mark=|\\%
 RdGy-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-6}{%
 RdGy-6-1,mark=x\\%
 RdGy-6-2,mark=+\\%
 RdGy-6-3,mark=-\\%
 RdGy-6-4,mark=|\\%
 RdGy-6-5,mark=asterisk\\%
 RdGy-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-7}{%
 RdGy-7-1,mark=x\\%
 RdGy-7-2,mark=+\\%
 RdGy-7-3,mark=-\\%
 RdGy-7-4,mark=|\\%
 RdGy-7-5,mark=asterisk\\%
 RdGy-7-6,mark=star\\%
 RdGy-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-8}{%
 RdGy-8-1,mark=x\\%
 RdGy-8-2,mark=+\\%
 RdGy-8-3,mark=-\\%
 RdGy-8-4,mark=|\\%
 RdGy-8-5,mark=asterisk\\%
 RdGy-8-6,mark=star\\%
 RdGy-8-7,mark=10-pointed star\\%
 RdGy-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-9}{%
 RdGy-9-1,mark=x\\%
 RdGy-9-2,mark=+\\%
 RdGy-9-3,mark=-\\%
 RdGy-9-4,mark=|\\%
 RdGy-9-5,mark=asterisk\\%
 RdGy-9-6,mark=star\\%
 RdGy-9-7,mark=10-pointed star\\%
 RdGy-9-8,mark=Mercedes star\\%
 RdGy-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-10}{%
 RdGy-10-1,mark=x\\%
 RdGy-10-2,mark=+\\%
 RdGy-10-3,mark=-\\%
 RdGy-10-4,mark=|\\%
 RdGy-10-5,mark=asterisk\\%
 RdGy-10-6,mark=star\\%
 RdGy-10-7,mark=10-pointed star\\%
 RdGy-10-8,mark=Mercedes star\\%
 RdGy-10-9,mark=Mercedes star flipped\\%
 RdGy-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdGy-11}{%
 RdGy-11-1,mark=x\\%
 RdGy-11-2,mark=+\\%
 RdGy-11-3,mark=-\\%
 RdGy-11-4,mark=|\\%
 RdGy-11-5,mark=asterisk\\%
 RdGy-11-6,mark=star\\%
 RdGy-11-7,mark=10-pointed star\\%
 RdGy-11-8,mark=Mercedes star\\%
 RdGy-11-9,mark=Mercedes star flipped\\%
 RdGy-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-3}{%
 RdYlBu-3-1,mark=x\\%
 RdYlBu-3-2,mark=+\\%
 RdYlBu-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-4}{%
 RdYlBu-4-1,mark=x\\%
 RdYlBu-4-2,mark=+\\%
 RdYlBu-4-3,mark=-\\%
 RdYlBu-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-5}{%
 RdYlBu-5-1,mark=x\\%
 RdYlBu-5-2,mark=+\\%
 RdYlBu-5-3,mark=-\\%
 RdYlBu-5-4,mark=|\\%
 RdYlBu-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-6}{%
 RdYlBu-6-1,mark=x\\%
 RdYlBu-6-2,mark=+\\%
 RdYlBu-6-3,mark=-\\%
 RdYlBu-6-4,mark=|\\%
 RdYlBu-6-5,mark=asterisk\\%
 RdYlBu-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-7}{%
 RdYlBu-7-1,mark=x\\%
 RdYlBu-7-2,mark=+\\%
 RdYlBu-7-3,mark=-\\%
 RdYlBu-7-4,mark=|\\%
 RdYlBu-7-5,mark=asterisk\\%
 RdYlBu-7-6,mark=star\\%
 RdYlBu-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-8}{%
 RdYlBu-8-1,mark=x\\%
 RdYlBu-8-2,mark=+\\%
 RdYlBu-8-3,mark=-\\%
 RdYlBu-8-4,mark=|\\%
 RdYlBu-8-5,mark=asterisk\\%
 RdYlBu-8-6,mark=star\\%
 RdYlBu-8-7,mark=10-pointed star\\%
 RdYlBu-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-9}{%
 RdYlBu-9-1,mark=x\\%
 RdYlBu-9-2,mark=+\\%
 RdYlBu-9-3,mark=-\\%
 RdYlBu-9-4,mark=|\\%
 RdYlBu-9-5,mark=asterisk\\%
 RdYlBu-9-6,mark=star\\%
 RdYlBu-9-7,mark=10-pointed star\\%
 RdYlBu-9-8,mark=Mercedes star\\%
 RdYlBu-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-10}{%
 RdYlBu-10-1,mark=x\\%
 RdYlBu-10-2,mark=+\\%
 RdYlBu-10-3,mark=-\\%
 RdYlBu-10-4,mark=|\\%
 RdYlBu-10-5,mark=asterisk\\%
 RdYlBu-10-6,mark=star\\%
 RdYlBu-10-7,mark=10-pointed star\\%
 RdYlBu-10-8,mark=Mercedes star\\%
 RdYlBu-10-9,mark=Mercedes star flipped\\%
 RdYlBu-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlBu-11}{%
 RdYlBu-11-1,mark=x\\%
 RdYlBu-11-2,mark=+\\%
 RdYlBu-11-3,mark=-\\%
 RdYlBu-11-4,mark=|\\%
 RdYlBu-11-5,mark=asterisk\\%
 RdYlBu-11-6,mark=star\\%
 RdYlBu-11-7,mark=10-pointed star\\%
 RdYlBu-11-8,mark=Mercedes star\\%
 RdYlBu-11-9,mark=Mercedes star flipped\\%
 RdYlBu-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-3}{%
 Spectral-3-1,mark=x\\%
 Spectral-3-2,mark=+\\%
 Spectral-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-4}{%
 Spectral-4-1,mark=x\\%
 Spectral-4-2,mark=+\\%
 Spectral-4-3,mark=-\\%
 Spectral-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-5}{%
 Spectral-5-1,mark=x\\%
 Spectral-5-2,mark=+\\%
 Spectral-5-3,mark=-\\%
 Spectral-5-4,mark=|\\%
 Spectral-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-6}{%
 Spectral-6-1,mark=x\\%
 Spectral-6-2,mark=+\\%
 Spectral-6-3,mark=-\\%
 Spectral-6-4,mark=|\\%
 Spectral-6-5,mark=asterisk\\%
 Spectral-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-7}{%
 Spectral-7-1,mark=x\\%
 Spectral-7-2,mark=+\\%
 Spectral-7-3,mark=-\\%
 Spectral-7-4,mark=|\\%
 Spectral-7-5,mark=asterisk\\%
 Spectral-7-6,mark=star\\%
 Spectral-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-8}{%
 Spectral-8-1,mark=x\\%
 Spectral-8-2,mark=+\\%
 Spectral-8-3,mark=-\\%
 Spectral-8-4,mark=|\\%
 Spectral-8-5,mark=asterisk\\%
 Spectral-8-6,mark=star\\%
 Spectral-8-7,mark=10-pointed star\\%
 Spectral-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-9}{%
 Spectral-9-1,mark=x\\%
 Spectral-9-2,mark=+\\%
 Spectral-9-3,mark=-\\%
 Spectral-9-4,mark=|\\%
 Spectral-9-5,mark=asterisk\\%
 Spectral-9-6,mark=star\\%
 Spectral-9-7,mark=10-pointed star\\%
 Spectral-9-8,mark=Mercedes star\\%
 Spectral-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-10}{%
 Spectral-10-1,mark=x\\%
 Spectral-10-2,mark=+\\%
 Spectral-10-3,mark=-\\%
 Spectral-10-4,mark=|\\%
 Spectral-10-5,mark=asterisk\\%
 Spectral-10-6,mark=star\\%
 Spectral-10-7,mark=10-pointed star\\%
 Spectral-10-8,mark=Mercedes star\\%
 Spectral-10-9,mark=Mercedes star flipped\\%
 Spectral-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Spectral-11}{%
 Spectral-11-1,mark=x\\%
 Spectral-11-2,mark=+\\%
 Spectral-11-3,mark=-\\%
 Spectral-11-4,mark=|\\%
 Spectral-11-5,mark=asterisk\\%
 Spectral-11-6,mark=star\\%
 Spectral-11-7,mark=10-pointed star\\%
 Spectral-11-8,mark=Mercedes star\\%
 Spectral-11-9,mark=Mercedes star flipped\\%
 Spectral-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-3}{%
 RdYlGn-3-1,mark=x\\%
 RdYlGn-3-2,mark=+\\%
 RdYlGn-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-4}{%
 RdYlGn-4-1,mark=x\\%
 RdYlGn-4-2,mark=+\\%
 RdYlGn-4-3,mark=-\\%
 RdYlGn-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-5}{%
 RdYlGn-5-1,mark=x\\%
 RdYlGn-5-2,mark=+\\%
 RdYlGn-5-3,mark=-\\%
 RdYlGn-5-4,mark=|\\%
 RdYlGn-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-6}{%
 RdYlGn-6-1,mark=x\\%
 RdYlGn-6-2,mark=+\\%
 RdYlGn-6-3,mark=-\\%
 RdYlGn-6-4,mark=|\\%
 RdYlGn-6-5,mark=asterisk\\%
 RdYlGn-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-7}{%
 RdYlGn-7-1,mark=x\\%
 RdYlGn-7-2,mark=+\\%
 RdYlGn-7-3,mark=-\\%
 RdYlGn-7-4,mark=|\\%
 RdYlGn-7-5,mark=asterisk\\%
 RdYlGn-7-6,mark=star\\%
 RdYlGn-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-8}{%
 RdYlGn-8-1,mark=x\\%
 RdYlGn-8-2,mark=+\\%
 RdYlGn-8-3,mark=-\\%
 RdYlGn-8-4,mark=|\\%
 RdYlGn-8-5,mark=asterisk\\%
 RdYlGn-8-6,mark=star\\%
 RdYlGn-8-7,mark=10-pointed star\\%
 RdYlGn-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-9}{%
 RdYlGn-9-1,mark=x\\%
 RdYlGn-9-2,mark=+\\%
 RdYlGn-9-3,mark=-\\%
 RdYlGn-9-4,mark=|\\%
 RdYlGn-9-5,mark=asterisk\\%
 RdYlGn-9-6,mark=star\\%
 RdYlGn-9-7,mark=10-pointed star\\%
 RdYlGn-9-8,mark=Mercedes star\\%
 RdYlGn-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-10}{%
 RdYlGn-10-1,mark=x\\%
 RdYlGn-10-2,mark=+\\%
 RdYlGn-10-3,mark=-\\%
 RdYlGn-10-4,mark=|\\%
 RdYlGn-10-5,mark=asterisk\\%
 RdYlGn-10-6,mark=star\\%
 RdYlGn-10-7,mark=10-pointed star\\%
 RdYlGn-10-8,mark=Mercedes star\\%
 RdYlGn-10-9,mark=Mercedes star flipped\\%
 RdYlGn-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-RdYlGn-11}{%
 RdYlGn-11-1,mark=x\\%
 RdYlGn-11-2,mark=+\\%
 RdYlGn-11-3,mark=-\\%
 RdYlGn-11-4,mark=|\\%
 RdYlGn-11-5,mark=asterisk\\%
 RdYlGn-11-6,mark=star\\%
 RdYlGn-11-7,mark=10-pointed star\\%
 RdYlGn-11-8,mark=Mercedes star\\%
 RdYlGn-11-9,mark=Mercedes star flipped\\%
 RdYlGn-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-3}{%
 Set3-3-1,mark=x\\%
 Set3-3-2,mark=+\\%
 Set3-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-4}{%
 Set3-4-1,mark=x\\%
 Set3-4-2,mark=+\\%
 Set3-4-3,mark=-\\%
 Set3-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-5}{%
 Set3-5-1,mark=x\\%
 Set3-5-2,mark=+\\%
 Set3-5-3,mark=-\\%
 Set3-5-4,mark=|\\%
 Set3-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-6}{%
 Set3-6-1,mark=x\\%
 Set3-6-2,mark=+\\%
 Set3-6-3,mark=-\\%
 Set3-6-4,mark=|\\%
 Set3-6-5,mark=asterisk\\%
 Set3-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-7}{%
 Set3-7-1,mark=x\\%
 Set3-7-2,mark=+\\%
 Set3-7-3,mark=-\\%
 Set3-7-4,mark=|\\%
 Set3-7-5,mark=asterisk\\%
 Set3-7-6,mark=star\\%
 Set3-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-8}{%
 Set3-8-1,mark=x\\%
 Set3-8-2,mark=+\\%
 Set3-8-3,mark=-\\%
 Set3-8-4,mark=|\\%
 Set3-8-5,mark=asterisk\\%
 Set3-8-6,mark=star\\%
 Set3-8-7,mark=10-pointed star\\%
 Set3-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-9}{%
 Set3-9-1,mark=x\\%
 Set3-9-2,mark=+\\%
 Set3-9-3,mark=-\\%
 Set3-9-4,mark=|\\%
 Set3-9-5,mark=asterisk\\%
 Set3-9-6,mark=star\\%
 Set3-9-7,mark=10-pointed star\\%
 Set3-9-8,mark=Mercedes star\\%
 Set3-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-10}{%
 Set3-10-1,mark=x\\%
 Set3-10-2,mark=+\\%
 Set3-10-3,mark=-\\%
 Set3-10-4,mark=|\\%
 Set3-10-5,mark=asterisk\\%
 Set3-10-6,mark=star\\%
 Set3-10-7,mark=10-pointed star\\%
 Set3-10-8,mark=Mercedes star\\%
 Set3-10-9,mark=Mercedes star flipped\\%
 Set3-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-11}{%
 Set3-11-1,mark=x\\%
 Set3-11-2,mark=+\\%
 Set3-11-3,mark=-\\%
 Set3-11-4,mark=|\\%
 Set3-11-5,mark=asterisk\\%
 Set3-11-6,mark=star\\%
 Set3-11-7,mark=10-pointed star\\%
 Set3-11-8,mark=Mercedes star\\%
 Set3-11-9,mark=Mercedes star flipped\\%
 Set3-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set3-12}{%
 Set3-12-1,mark=x\\%
 Set3-12-2,mark=+\\%
 Set3-12-3,mark=-\\%
 Set3-12-4,mark=|\\%
 Set3-12-5,mark=asterisk\\%
 Set3-12-6,mark=star\\%
 Set3-12-7,mark=10-pointed star\\%
 Set3-12-8,mark=Mercedes star\\%
 Set3-12-9,mark=Mercedes star flipped\\%
 Set3-12-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-3}{%
 Pastel1-3-1,mark=x\\%
 Pastel1-3-2,mark=+\\%
 Pastel1-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-4}{%
 Pastel1-4-1,mark=x\\%
 Pastel1-4-2,mark=+\\%
 Pastel1-4-3,mark=-\\%
 Pastel1-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-5}{%
 Pastel1-5-1,mark=x\\%
 Pastel1-5-2,mark=+\\%
 Pastel1-5-3,mark=-\\%
 Pastel1-5-4,mark=|\\%
 Pastel1-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-6}{%
 Pastel1-6-1,mark=x\\%
 Pastel1-6-2,mark=+\\%
 Pastel1-6-3,mark=-\\%
 Pastel1-6-4,mark=|\\%
 Pastel1-6-5,mark=asterisk\\%
 Pastel1-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-7}{%
 Pastel1-7-1,mark=x\\%
 Pastel1-7-2,mark=+\\%
 Pastel1-7-3,mark=-\\%
 Pastel1-7-4,mark=|\\%
 Pastel1-7-5,mark=asterisk\\%
 Pastel1-7-6,mark=star\\%
 Pastel1-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-8}{%
 Pastel1-8-1,mark=x\\%
 Pastel1-8-2,mark=+\\%
 Pastel1-8-3,mark=-\\%
 Pastel1-8-4,mark=|\\%
 Pastel1-8-5,mark=asterisk\\%
 Pastel1-8-6,mark=star\\%
 Pastel1-8-7,mark=10-pointed star\\%
 Pastel1-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel1-9}{%
 Pastel1-9-1,mark=x\\%
 Pastel1-9-2,mark=+\\%
 Pastel1-9-3,mark=-\\%
 Pastel1-9-4,mark=|\\%
 Pastel1-9-5,mark=asterisk\\%
 Pastel1-9-6,mark=star\\%
 Pastel1-9-7,mark=10-pointed star\\%
 Pastel1-9-8,mark=Mercedes star\\%
 Pastel1-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-3}{%
 Set1-3-1,mark=x\\%
 Set1-3-2,mark=+\\%
 Set1-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-4}{%
 Set1-4-1,mark=x\\%
 Set1-4-2,mark=+\\%
 Set1-4-3,mark=-\\%
 Set1-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-5}{%
 Set1-5-1,mark=x\\%
 Set1-5-2,mark=+\\%
 Set1-5-3,mark=-\\%
 Set1-5-4,mark=|\\%
 Set1-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-6}{%
 Set1-6-1,mark=x\\%
 Set1-6-2,mark=+\\%
 Set1-6-3,mark=-\\%
 Set1-6-4,mark=|\\%
 Set1-6-5,mark=asterisk\\%
 Set1-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-7}{%
 Set1-7-1,mark=x\\%
 Set1-7-2,mark=+\\%
 Set1-7-3,mark=-\\%
 Set1-7-4,mark=|\\%
 Set1-7-5,mark=asterisk\\%
 Set1-7-6,mark=star\\%
 Set1-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-8}{%
 Set1-8-1,mark=x\\%
 Set1-8-2,mark=+\\%
 Set1-8-3,mark=-\\%
 Set1-8-4,mark=|\\%
 Set1-8-5,mark=asterisk\\%
 Set1-8-6,mark=star\\%
 Set1-8-7,mark=10-pointed star\\%
 Set1-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set1-9}{%
 Set1-9-1,mark=x\\%
 Set1-9-2,mark=+\\%
 Set1-9-3,mark=-\\%
 Set1-9-4,mark=|\\%
 Set1-9-5,mark=asterisk\\%
 Set1-9-6,mark=star\\%
 Set1-9-7,mark=10-pointed star\\%
 Set1-9-8,mark=Mercedes star\\%
 Set1-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-3}{%
 Pastel2-3-1,mark=x\\%
 Pastel2-3-2,mark=+\\%
 Pastel2-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-4}{%
 Pastel2-4-1,mark=x\\%
 Pastel2-4-2,mark=+\\%
 Pastel2-4-3,mark=-\\%
 Pastel2-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-5}{%
 Pastel2-5-1,mark=x\\%
 Pastel2-5-2,mark=+\\%
 Pastel2-5-3,mark=-\\%
 Pastel2-5-4,mark=|\\%
 Pastel2-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-6}{%
 Pastel2-6-1,mark=x\\%
 Pastel2-6-2,mark=+\\%
 Pastel2-6-3,mark=-\\%
 Pastel2-6-4,mark=|\\%
 Pastel2-6-5,mark=asterisk\\%
 Pastel2-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-7}{%
 Pastel2-7-1,mark=x\\%
 Pastel2-7-2,mark=+\\%
 Pastel2-7-3,mark=-\\%
 Pastel2-7-4,mark=|\\%
 Pastel2-7-5,mark=asterisk\\%
 Pastel2-7-6,mark=star\\%
 Pastel2-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Pastel2-8}{%
 Pastel2-8-1,mark=x\\%
 Pastel2-8-2,mark=+\\%
 Pastel2-8-3,mark=-\\%
 Pastel2-8-4,mark=|\\%
 Pastel2-8-5,mark=asterisk\\%
 Pastel2-8-6,mark=star\\%
 Pastel2-8-7,mark=10-pointed star\\%
 Pastel2-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-3}{%
 Set2-3-1,mark=x\\%
 Set2-3-2,mark=+\\%
 Set2-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-4}{%
 Set2-4-1,mark=x\\%
 Set2-4-2,mark=+\\%
 Set2-4-3,mark=-\\%
 Set2-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-5}{%
 Set2-5-1,mark=x\\%
 Set2-5-2,mark=+\\%
 Set2-5-3,mark=-\\%
 Set2-5-4,mark=|\\%
 Set2-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-6}{%
 Set2-6-1,mark=x\\%
 Set2-6-2,mark=+\\%
 Set2-6-3,mark=-\\%
 Set2-6-4,mark=|\\%
 Set2-6-5,mark=asterisk\\%
 Set2-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-7}{%
 Set2-7-1,mark=x\\%
 Set2-7-2,mark=+\\%
 Set2-7-3,mark=-\\%
 Set2-7-4,mark=|\\%
 Set2-7-5,mark=asterisk\\%
 Set2-7-6,mark=star\\%
 Set2-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Set2-8}{%
 Set2-8-1,mark=x\\%
 Set2-8-2,mark=+\\%
 Set2-8-3,mark=-\\%
 Set2-8-4,mark=|\\%
 Set2-8-5,mark=asterisk\\%
 Set2-8-6,mark=star\\%
 Set2-8-7,mark=10-pointed star\\%
 Set2-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-3}{%
 Dark2-3-1,mark=x\\%
 Dark2-3-2,mark=+\\%
 Dark2-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-4}{%
 Dark2-4-1,mark=x\\%
 Dark2-4-2,mark=+\\%
 Dark2-4-3,mark=-\\%
 Dark2-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-5}{%
 Dark2-5-1,mark=x\\%
 Dark2-5-2,mark=+\\%
 Dark2-5-3,mark=-\\%
 Dark2-5-4,mark=|\\%
 Dark2-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-6}{%
 Dark2-6-1,mark=x\\%
 Dark2-6-2,mark=+\\%
 Dark2-6-3,mark=-\\%
 Dark2-6-4,mark=|\\%
 Dark2-6-5,mark=asterisk\\%
 Dark2-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-7}{%
 Dark2-7-1,mark=x\\%
 Dark2-7-2,mark=+\\%
 Dark2-7-3,mark=-\\%
 Dark2-7-4,mark=|\\%
 Dark2-7-5,mark=asterisk\\%
 Dark2-7-6,mark=star\\%
 Dark2-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Dark2-8}{%
 Dark2-8-1,mark=x\\%
 Dark2-8-2,mark=+\\%
 Dark2-8-3,mark=-\\%
 Dark2-8-4,mark=|\\%
 Dark2-8-5,mark=asterisk\\%
 Dark2-8-6,mark=star\\%
 Dark2-8-7,mark=10-pointed star\\%
 Dark2-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-3}{%
 Paired-3-1,mark=x\\%
 Paired-3-2,mark=+\\%
 Paired-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-4}{%
 Paired-4-1,mark=x\\%
 Paired-4-2,mark=+\\%
 Paired-4-3,mark=-\\%
 Paired-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-5}{%
 Paired-5-1,mark=x\\%
 Paired-5-2,mark=+\\%
 Paired-5-3,mark=-\\%
 Paired-5-4,mark=|\\%
 Paired-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-6}{%
 Paired-6-1,mark=x\\%
 Paired-6-2,mark=+\\%
 Paired-6-3,mark=-\\%
 Paired-6-4,mark=|\\%
 Paired-6-5,mark=asterisk\\%
 Paired-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-7}{%
 Paired-7-1,mark=x\\%
 Paired-7-2,mark=+\\%
 Paired-7-3,mark=-\\%
 Paired-7-4,mark=|\\%
 Paired-7-5,mark=asterisk\\%
 Paired-7-6,mark=star\\%
 Paired-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-8}{%
 Paired-8-1,mark=x\\%
 Paired-8-2,mark=+\\%
 Paired-8-3,mark=-\\%
 Paired-8-4,mark=|\\%
 Paired-8-5,mark=asterisk\\%
 Paired-8-6,mark=star\\%
 Paired-8-7,mark=10-pointed star\\%
 Paired-8-8,mark=Mercedes star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-9}{%
 Paired-9-1,mark=x\\%
 Paired-9-2,mark=+\\%
 Paired-9-3,mark=-\\%
 Paired-9-4,mark=|\\%
 Paired-9-5,mark=asterisk\\%
 Paired-9-6,mark=star\\%
 Paired-9-7,mark=10-pointed star\\%
 Paired-9-8,mark=Mercedes star\\%
 Paired-9-9,mark=Mercedes star flipped\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-10}{%
 Paired-10-1,mark=x\\%
 Paired-10-2,mark=+\\%
 Paired-10-3,mark=-\\%
 Paired-10-4,mark=|\\%
 Paired-10-5,mark=asterisk\\%
 Paired-10-6,mark=star\\%
 Paired-10-7,mark=10-pointed star\\%
 Paired-10-8,mark=Mercedes star\\%
 Paired-10-9,mark=Mercedes star flipped\\%
 Paired-10-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-11}{%
 Paired-11-1,mark=x\\%
 Paired-11-2,mark=+\\%
 Paired-11-3,mark=-\\%
 Paired-11-4,mark=|\\%
 Paired-11-5,mark=asterisk\\%
 Paired-11-6,mark=star\\%
 Paired-11-7,mark=10-pointed star\\%
 Paired-11-8,mark=Mercedes star\\%
 Paired-11-9,mark=Mercedes star flipped\\%
 Paired-11-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Paired-12}{%
 Paired-12-1,mark=x\\%
 Paired-12-2,mark=+\\%
 Paired-12-3,mark=-\\%
 Paired-12-4,mark=|\\%
 Paired-12-5,mark=asterisk\\%
 Paired-12-6,mark=star\\%
 Paired-12-7,mark=10-pointed star\\%
 Paired-12-8,mark=Mercedes star\\%
 Paired-12-9,mark=Mercedes star flipped\\%
 Paired-12-10,mark=pentagon\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-3}{%
 Accent-3-1,mark=x\\%
 Accent-3-2,mark=+\\%
 Accent-3-3,mark=-\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-4}{%
 Accent-4-1,mark=x\\%
 Accent-4-2,mark=+\\%
 Accent-4-3,mark=-\\%
 Accent-4-4,mark=|\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-5}{%
 Accent-5-1,mark=x\\%
 Accent-5-2,mark=+\\%
 Accent-5-3,mark=-\\%
 Accent-5-4,mark=|\\%
 Accent-5-5,mark=asterisk\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-6}{%
 Accent-6-1,mark=x\\%
 Accent-6-2,mark=+\\%
 Accent-6-3,mark=-\\%
 Accent-6-4,mark=|\\%
 Accent-6-5,mark=asterisk\\%
 Accent-6-6,mark=star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-7}{%
 Accent-7-1,mark=x\\%
 Accent-7-2,mark=+\\%
 Accent-7-3,mark=-\\%
 Accent-7-4,mark=|\\%
 Accent-7-5,mark=asterisk\\%
 Accent-7-6,mark=star\\%
 Accent-7-7,mark=10-pointed star\\%
}
\pgfplotscreateplotcyclelist{ErrorMark-Accent-8}{%
 Accent-8-1,mark=x\\%
 Accent-8-2,mark=+\\%
 Accent-8-3,mark=-\\%
 Accent-8-4,mark=|\\%
 Accent-8-5,mark=asterisk\\%
 Accent-8-6,mark=star\\%
 Accent-8-7,mark=10-pointed star\\%
 Accent-8-8,mark=Mercedes star\\%
}
\pgfplotsset{
colormap={YlGn-3}{
  color=(YlGn-3-1);
  color=(YlGn-3-2);
  color=(YlGn-3-3);
},
colormap={YlGn-4}{
  color=(YlGn-4-1);
  color=(YlGn-4-2);
  color=(YlGn-4-3);
  color=(YlGn-4-4);
},
colormap={YlGn-5}{
  color=(YlGn-5-1);
  color=(YlGn-5-2);
  color=(YlGn-5-3);
  color=(YlGn-5-4);
  color=(YlGn-5-5);
},
colormap={YlGn-6}{
  color=(YlGn-6-1);
  color=(YlGn-6-2);
  color=(YlGn-6-3);
  color=(YlGn-6-4);
  color=(YlGn-6-5);
  color=(YlGn-6-6);
},
colormap={YlGn-7}{
  color=(YlGn-7-1);
  color=(YlGn-7-2);
  color=(YlGn-7-3);
  color=(YlGn-7-4);
  color=(YlGn-7-5);
  color=(YlGn-7-6);
  color=(YlGn-7-7);
},
colormap={YlGn-8}{
  color=(YlGn-8-1);
  color=(YlGn-8-2);
  color=(YlGn-8-3);
  color=(YlGn-8-4);
  color=(YlGn-8-5);
  color=(YlGn-8-6);
  color=(YlGn-8-7);
  color=(YlGn-8-8);
},
colormap={YlGn-9}{
  color=(YlGn-9-1);
  color=(YlGn-9-2);
  color=(YlGn-9-3);
  color=(YlGn-9-4);
  color=(YlGn-9-5);
  color=(YlGn-9-6);
  color=(YlGn-9-7);
  color=(YlGn-9-8);
  color=(YlGn-9-9);
},
colormap={YlGnBu-3}{
  color=(YlGnBu-3-1);
  color=(YlGnBu-3-2);
  color=(YlGnBu-3-3);
},
colormap={YlGnBu-4}{
  color=(YlGnBu-4-1);
  color=(YlGnBu-4-2);
  color=(YlGnBu-4-3);
  color=(YlGnBu-4-4);
},
colormap={YlGnBu-5}{
  color=(YlGnBu-5-1);
  color=(YlGnBu-5-2);
  color=(YlGnBu-5-3);
  color=(YlGnBu-5-4);
  color=(YlGnBu-5-5);
},
colormap={YlGnBu-6}{
  color=(YlGnBu-6-1);
  color=(YlGnBu-6-2);
  color=(YlGnBu-6-3);
  color=(YlGnBu-6-4);
  color=(YlGnBu-6-5);
  color=(YlGnBu-6-6);
},
colormap={YlGnBu-7}{
  color=(YlGnBu-7-1);
  color=(YlGnBu-7-2);
  color=(YlGnBu-7-3);
  color=(YlGnBu-7-4);
  color=(YlGnBu-7-5);
  color=(YlGnBu-7-6);
  color=(YlGnBu-7-7);
},
colormap={YlGnBu-8}{
  color=(YlGnBu-8-1);
  color=(YlGnBu-8-2);
  color=(YlGnBu-8-3);
  color=(YlGnBu-8-4);
  color=(YlGnBu-8-5);
  color=(YlGnBu-8-6);
  color=(YlGnBu-8-7);
  color=(YlGnBu-8-8);
},
colormap={YlGnBu-9}{
  color=(YlGnBu-9-1);
  color=(YlGnBu-9-2);
  color=(YlGnBu-9-3);
  color=(YlGnBu-9-4);
  color=(YlGnBu-9-5);
  color=(YlGnBu-9-6);
  color=(YlGnBu-9-7);
  color=(YlGnBu-9-8);
  color=(YlGnBu-9-9);
},
colormap={GnBu-3}{
  color=(GnBu-3-1);
  color=(GnBu-3-2);
  color=(GnBu-3-3);
},
colormap={GnBu-4}{
  color=(GnBu-4-1);
  color=(GnBu-4-2);
  color=(GnBu-4-3);
  color=(GnBu-4-4);
},
colormap={GnBu-5}{
  color=(GnBu-5-1);
  color=(GnBu-5-2);
  color=(GnBu-5-3);
  color=(GnBu-5-4);
  color=(GnBu-5-5);
},
colormap={GnBu-6}{
  color=(GnBu-6-1);
  color=(GnBu-6-2);
  color=(GnBu-6-3);
  color=(GnBu-6-4);
  color=(GnBu-6-5);
  color=(GnBu-6-6);
},
colormap={GnBu-7}{
  color=(GnBu-7-1);
  color=(GnBu-7-2);
  color=(GnBu-7-3);
  color=(GnBu-7-4);
  color=(GnBu-7-5);
  color=(GnBu-7-6);
  color=(GnBu-7-7);
},
colormap={GnBu-8}{
  color=(GnBu-8-1);
  color=(GnBu-8-2);
  color=(GnBu-8-3);
  color=(GnBu-8-4);
  color=(GnBu-8-5);
  color=(GnBu-8-6);
  color=(GnBu-8-7);
  color=(GnBu-8-8);
},
colormap={GnBu-9}{
  color=(GnBu-9-1);
  color=(GnBu-9-2);
  color=(GnBu-9-3);
  color=(GnBu-9-4);
  color=(GnBu-9-5);
  color=(GnBu-9-6);
  color=(GnBu-9-7);
  color=(GnBu-9-8);
  color=(GnBu-9-9);
},
colormap={BuGn-3}{
  color=(BuGn-3-1);
  color=(BuGn-3-2);
  color=(BuGn-3-3);
},
colormap={BuGn-4}{
  color=(BuGn-4-1);
  color=(BuGn-4-2);
  color=(BuGn-4-3);
  color=(BuGn-4-4);
},
colormap={BuGn-5}{
  color=(BuGn-5-1);
  color=(BuGn-5-2);
  color=(BuGn-5-3);
  color=(BuGn-5-4);
  color=(BuGn-5-5);
},
colormap={BuGn-6}{
  color=(BuGn-6-1);
  color=(BuGn-6-2);
  color=(BuGn-6-3);
  color=(BuGn-6-4);
  color=(BuGn-6-5);
  color=(BuGn-6-6);
},
colormap={BuGn-7}{
  color=(BuGn-7-1);
  color=(BuGn-7-2);
  color=(BuGn-7-3);
  color=(BuGn-7-4);
  color=(BuGn-7-5);
  color=(BuGn-7-6);
  color=(BuGn-7-7);
},
colormap={BuGn-8}{
  color=(BuGn-8-1);
  color=(BuGn-8-2);
  color=(BuGn-8-3);
  color=(BuGn-8-4);
  color=(BuGn-8-5);
  color=(BuGn-8-6);
  color=(BuGn-8-7);
  color=(BuGn-8-8);
},
colormap={BuGn-9}{
  color=(BuGn-9-1);
  color=(BuGn-9-2);
  color=(BuGn-9-3);
  color=(BuGn-9-4);
  color=(BuGn-9-5);
  color=(BuGn-9-6);
  color=(BuGn-9-7);
  color=(BuGn-9-8);
  color=(BuGn-9-9);
},
colormap={PuBuGn-3}{
  color=(PuBuGn-3-1);
  color=(PuBuGn-3-2);
  color=(PuBuGn-3-3);
},
colormap={PuBuGn-4}{
  color=(PuBuGn-4-1);
  color=(PuBuGn-4-2);
  color=(PuBuGn-4-3);
  color=(PuBuGn-4-4);
},
colormap={PuBuGn-5}{
  color=(PuBuGn-5-1);
  color=(PuBuGn-5-2);
  color=(PuBuGn-5-3);
  color=(PuBuGn-5-4);
  color=(PuBuGn-5-5);
},
colormap={PuBuGn-6}{
  color=(PuBuGn-6-1);
  color=(PuBuGn-6-2);
  color=(PuBuGn-6-3);
  color=(PuBuGn-6-4);
  color=(PuBuGn-6-5);
  color=(PuBuGn-6-6);
},
colormap={PuBuGn-7}{
  color=(PuBuGn-7-1);
  color=(PuBuGn-7-2);
  color=(PuBuGn-7-3);
  color=(PuBuGn-7-4);
  color=(PuBuGn-7-5);
  color=(PuBuGn-7-6);
  color=(PuBuGn-7-7);
},
colormap={PuBuGn-8}{
  color=(PuBuGn-8-1);
  color=(PuBuGn-8-2);
  color=(PuBuGn-8-3);
  color=(PuBuGn-8-4);
  color=(PuBuGn-8-5);
  color=(PuBuGn-8-6);
  color=(PuBuGn-8-7);
  color=(PuBuGn-8-8);
},
colormap={PuBuGn-9}{
  color=(PuBuGn-9-1);
  color=(PuBuGn-9-2);
  color=(PuBuGn-9-3);
  color=(PuBuGn-9-4);
  color=(PuBuGn-9-5);
  color=(PuBuGn-9-6);
  color=(PuBuGn-9-7);
  color=(PuBuGn-9-8);
  color=(PuBuGn-9-9);
},
colormap={PuBu-3}{
  color=(PuBu-3-1);
  color=(PuBu-3-2);
  color=(PuBu-3-3);
},
colormap={PuBu-4}{
  color=(PuBu-4-1);
  color=(PuBu-4-2);
  color=(PuBu-4-3);
  color=(PuBu-4-4);
},
colormap={PuBu-5}{
  color=(PuBu-5-1);
  color=(PuBu-5-2);
  color=(PuBu-5-3);
  color=(PuBu-5-4);
  color=(PuBu-5-5);
},
colormap={PuBu-6}{
  color=(PuBu-6-1);
  color=(PuBu-6-2);
  color=(PuBu-6-3);
  color=(PuBu-6-4);
  color=(PuBu-6-5);
  color=(PuBu-6-6);
},
colormap={PuBu-7}{
  color=(PuBu-7-1);
  color=(PuBu-7-2);
  color=(PuBu-7-3);
  color=(PuBu-7-4);
  color=(PuBu-7-5);
  color=(PuBu-7-6);
  color=(PuBu-7-7);
},
colormap={PuBu-8}{
  color=(PuBu-8-1);
  color=(PuBu-8-2);
  color=(PuBu-8-3);
  color=(PuBu-8-4);
  color=(PuBu-8-5);
  color=(PuBu-8-6);
  color=(PuBu-8-7);
  color=(PuBu-8-8);
},
colormap={PuBu-9}{
  color=(PuBu-9-1);
  color=(PuBu-9-2);
  color=(PuBu-9-3);
  color=(PuBu-9-4);
  color=(PuBu-9-5);
  color=(PuBu-9-6);
  color=(PuBu-9-7);
  color=(PuBu-9-8);
  color=(PuBu-9-9);
},
colormap={BuPu-3}{
  color=(BuPu-3-1);
  color=(BuPu-3-2);
  color=(BuPu-3-3);
},
colormap={BuPu-4}{
  color=(BuPu-4-1);
  color=(BuPu-4-2);
  color=(BuPu-4-3);
  color=(BuPu-4-4);
},
colormap={BuPu-5}{
  color=(BuPu-5-1);
  color=(BuPu-5-2);
  color=(BuPu-5-3);
  color=(BuPu-5-4);
  color=(BuPu-5-5);
},
colormap={BuPu-6}{
  color=(BuPu-6-1);
  color=(BuPu-6-2);
  color=(BuPu-6-3);
  color=(BuPu-6-4);
  color=(BuPu-6-5);
  color=(BuPu-6-6);
},
colormap={BuPu-7}{
  color=(BuPu-7-1);
  color=(BuPu-7-2);
  color=(BuPu-7-3);
  color=(BuPu-7-4);
  color=(BuPu-7-5);
  color=(BuPu-7-6);
  color=(BuPu-7-7);
},
colormap={BuPu-8}{
  color=(BuPu-8-1);
  color=(BuPu-8-2);
  color=(BuPu-8-3);
  color=(BuPu-8-4);
  color=(BuPu-8-5);
  color=(BuPu-8-6);
  color=(BuPu-8-7);
  color=(BuPu-8-8);
},
colormap={BuPu-9}{
  color=(BuPu-9-1);
  color=(BuPu-9-2);
  color=(BuPu-9-3);
  color=(BuPu-9-4);
  color=(BuPu-9-5);
  color=(BuPu-9-6);
  color=(BuPu-9-7);
  color=(BuPu-9-8);
  color=(BuPu-9-9);
},
colormap={RdPu-3}{
  color=(RdPu-3-1);
  color=(RdPu-3-2);
  color=(RdPu-3-3);
},
colormap={RdPu-4}{
  color=(RdPu-4-1);
  color=(RdPu-4-2);
  color=(RdPu-4-3);
  color=(RdPu-4-4);
},
colormap={RdPu-5}{
  color=(RdPu-5-1);
  color=(RdPu-5-2);
  color=(RdPu-5-3);
  color=(RdPu-5-4);
  color=(RdPu-5-5);
},
colormap={RdPu-6}{
  color=(RdPu-6-1);
  color=(RdPu-6-2);
  color=(RdPu-6-3);
  color=(RdPu-6-4);
  color=(RdPu-6-5);
  color=(RdPu-6-6);
},
colormap={RdPu-7}{
  color=(RdPu-7-1);
  color=(RdPu-7-2);
  color=(RdPu-7-3);
  color=(RdPu-7-4);
  color=(RdPu-7-5);
  color=(RdPu-7-6);
  color=(RdPu-7-7);
},
colormap={RdPu-8}{
  color=(RdPu-8-1);
  color=(RdPu-8-2);
  color=(RdPu-8-3);
  color=(RdPu-8-4);
  color=(RdPu-8-5);
  color=(RdPu-8-6);
  color=(RdPu-8-7);
  color=(RdPu-8-8);
},
colormap={RdPu-9}{
  color=(RdPu-9-1);
  color=(RdPu-9-2);
  color=(RdPu-9-3);
  color=(RdPu-9-4);
  color=(RdPu-9-5);
  color=(RdPu-9-6);
  color=(RdPu-9-7);
  color=(RdPu-9-8);
  color=(RdPu-9-9);
},
colormap={PuRd-3}{
  color=(PuRd-3-1);
  color=(PuRd-3-2);
  color=(PuRd-3-3);
},
colormap={PuRd-4}{
  color=(PuRd-4-1);
  color=(PuRd-4-2);
  color=(PuRd-4-3);
  color=(PuRd-4-4);
},
colormap={PuRd-5}{
  color=(PuRd-5-1);
  color=(PuRd-5-2);
  color=(PuRd-5-3);
  color=(PuRd-5-4);
  color=(PuRd-5-5);
},
colormap={PuRd-6}{
  color=(PuRd-6-1);
  color=(PuRd-6-2);
  color=(PuRd-6-3);
  color=(PuRd-6-4);
  color=(PuRd-6-5);
  color=(PuRd-6-6);
},
colormap={PuRd-7}{
  color=(PuRd-7-1);
  color=(PuRd-7-2);
  color=(PuRd-7-3);
  color=(PuRd-7-4);
  color=(PuRd-7-5);
  color=(PuRd-7-6);
  color=(PuRd-7-7);
},
colormap={PuRd-8}{
  color=(PuRd-8-1);
  color=(PuRd-8-2);
  color=(PuRd-8-3);
  color=(PuRd-8-4);
  color=(PuRd-8-5);
  color=(PuRd-8-6);
  color=(PuRd-8-7);
  color=(PuRd-8-8);
},
colormap={PuRd-9}{
  color=(PuRd-9-1);
  color=(PuRd-9-2);
  color=(PuRd-9-3);
  color=(PuRd-9-4);
  color=(PuRd-9-5);
  color=(PuRd-9-6);
  color=(PuRd-9-7);
  color=(PuRd-9-8);
  color=(PuRd-9-9);
},
colormap={OrRd-3}{
  color=(OrRd-3-1);
  color=(OrRd-3-2);
  color=(OrRd-3-3);
},
colormap={OrRd-4}{
  color=(OrRd-4-1);
  color=(OrRd-4-2);
  color=(OrRd-4-3);
  color=(OrRd-4-4);
},
colormap={OrRd-5}{
  color=(OrRd-5-1);
  color=(OrRd-5-2);
  color=(OrRd-5-3);
  color=(OrRd-5-4);
  color=(OrRd-5-5);
},
colormap={OrRd-6}{
  color=(OrRd-6-1);
  color=(OrRd-6-2);
  color=(OrRd-6-3);
  color=(OrRd-6-4);
  color=(OrRd-6-5);
  color=(OrRd-6-6);
},
colormap={OrRd-7}{
  color=(OrRd-7-1);
  color=(OrRd-7-2);
  color=(OrRd-7-3);
  color=(OrRd-7-4);
  color=(OrRd-7-5);
  color=(OrRd-7-6);
  color=(OrRd-7-7);
},
colormap={OrRd-8}{
  color=(OrRd-8-1);
  color=(OrRd-8-2);
  color=(OrRd-8-3);
  color=(OrRd-8-4);
  color=(OrRd-8-5);
  color=(OrRd-8-6);
  color=(OrRd-8-7);
  color=(OrRd-8-8);
},
colormap={OrRd-9}{
  color=(OrRd-9-1);
  color=(OrRd-9-2);
  color=(OrRd-9-3);
  color=(OrRd-9-4);
  color=(OrRd-9-5);
  color=(OrRd-9-6);
  color=(OrRd-9-7);
  color=(OrRd-9-8);
  color=(OrRd-9-9);
},
colormap={YlOrRd-3}{
  color=(YlOrRd-3-1);
  color=(YlOrRd-3-2);
  color=(YlOrRd-3-3);
},
colormap={YlOrRd-4}{
  color=(YlOrRd-4-1);
  color=(YlOrRd-4-2);
  color=(YlOrRd-4-3);
  color=(YlOrRd-4-4);
},
colormap={YlOrRd-5}{
  color=(YlOrRd-5-1);
  color=(YlOrRd-5-2);
  color=(YlOrRd-5-3);
  color=(YlOrRd-5-4);
  color=(YlOrRd-5-5);
},
colormap={YlOrRd-6}{
  color=(YlOrRd-6-1);
  color=(YlOrRd-6-2);
  color=(YlOrRd-6-3);
  color=(YlOrRd-6-4);
  color=(YlOrRd-6-5);
  color=(YlOrRd-6-6);
},
colormap={YlOrRd-7}{
  color=(YlOrRd-7-1);
  color=(YlOrRd-7-2);
  color=(YlOrRd-7-3);
  color=(YlOrRd-7-4);
  color=(YlOrRd-7-5);
  color=(YlOrRd-7-6);
  color=(YlOrRd-7-7);
},
colormap={YlOrRd-8}{
  color=(YlOrRd-8-1);
  color=(YlOrRd-8-2);
  color=(YlOrRd-8-3);
  color=(YlOrRd-8-4);
  color=(YlOrRd-8-5);
  color=(YlOrRd-8-6);
  color=(YlOrRd-8-7);
  color=(YlOrRd-8-8);
},
colormap={YlOrRd-9}{
  color=(YlOrRd-9-1);
  color=(YlOrRd-9-2);
  color=(YlOrRd-9-3);
  color=(YlOrRd-9-4);
  color=(YlOrRd-9-5);
  color=(YlOrRd-9-6);
  color=(YlOrRd-9-7);
  color=(YlOrRd-9-8);
  color=(YlOrRd-9-9);
},
colormap={YlOrBr-3}{
  color=(YlOrBr-3-1);
  color=(YlOrBr-3-2);
  color=(YlOrBr-3-3);
},
colormap={YlOrBr-4}{
  color=(YlOrBr-4-1);
  color=(YlOrBr-4-2);
  color=(YlOrBr-4-3);
  color=(YlOrBr-4-4);
},
colormap={YlOrBr-5}{
  color=(YlOrBr-5-1);
  color=(YlOrBr-5-2);
  color=(YlOrBr-5-3);
  color=(YlOrBr-5-4);
  color=(YlOrBr-5-5);
},
colormap={YlOrBr-6}{
  color=(YlOrBr-6-1);
  color=(YlOrBr-6-2);
  color=(YlOrBr-6-3);
  color=(YlOrBr-6-4);
  color=(YlOrBr-6-5);
  color=(YlOrBr-6-6);
},
colormap={YlOrBr-7}{
  color=(YlOrBr-7-1);
  color=(YlOrBr-7-2);
  color=(YlOrBr-7-3);
  color=(YlOrBr-7-4);
  color=(YlOrBr-7-5);
  color=(YlOrBr-7-6);
  color=(YlOrBr-7-7);
},
colormap={YlOrBr-8}{
  color=(YlOrBr-8-1);
  color=(YlOrBr-8-2);
  color=(YlOrBr-8-3);
  color=(YlOrBr-8-4);
  color=(YlOrBr-8-5);
  color=(YlOrBr-8-6);
  color=(YlOrBr-8-7);
  color=(YlOrBr-8-8);
},
colormap={YlOrBr-9}{
  color=(YlOrBr-9-1);
  color=(YlOrBr-9-2);
  color=(YlOrBr-9-3);
  color=(YlOrBr-9-4);
  color=(YlOrBr-9-5);
  color=(YlOrBr-9-6);
  color=(YlOrBr-9-7);
  color=(YlOrBr-9-8);
  color=(YlOrBr-9-9);
},
colormap={Purples-3}{
  color=(Purples-3-1);
  color=(Purples-3-2);
  color=(Purples-3-3);
},
colormap={Purples-4}{
  color=(Purples-4-1);
  color=(Purples-4-2);
  color=(Purples-4-3);
  color=(Purples-4-4);
},
colormap={Purples-5}{
  color=(Purples-5-1);
  color=(Purples-5-2);
  color=(Purples-5-3);
  color=(Purples-5-4);
  color=(Purples-5-5);
},
colormap={Purples-6}{
  color=(Purples-6-1);
  color=(Purples-6-2);
  color=(Purples-6-3);
  color=(Purples-6-4);
  color=(Purples-6-5);
  color=(Purples-6-6);
},
colormap={Purples-7}{
  color=(Purples-7-1);
  color=(Purples-7-2);
  color=(Purples-7-3);
  color=(Purples-7-4);
  color=(Purples-7-5);
  color=(Purples-7-6);
  color=(Purples-7-7);
},
colormap={Purples-8}{
  color=(Purples-8-1);
  color=(Purples-8-2);
  color=(Purples-8-3);
  color=(Purples-8-4);
  color=(Purples-8-5);
  color=(Purples-8-6);
  color=(Purples-8-7);
  color=(Purples-8-8);
},
colormap={Purples-9}{
  color=(Purples-9-1);
  color=(Purples-9-2);
  color=(Purples-9-3);
  color=(Purples-9-4);
  color=(Purples-9-5);
  color=(Purples-9-6);
  color=(Purples-9-7);
  color=(Purples-9-8);
  color=(Purples-9-9);
},
colormap={Blues-3}{
  color=(Blues-3-1);
  color=(Blues-3-2);
  color=(Blues-3-3);
},
colormap={Blues-4}{
  color=(Blues-4-1);
  color=(Blues-4-2);
  color=(Blues-4-3);
  color=(Blues-4-4);
},
colormap={Blues-5}{
  color=(Blues-5-1);
  color=(Blues-5-2);
  color=(Blues-5-3);
  color=(Blues-5-4);
  color=(Blues-5-5);
},
colormap={Blues-6}{
  color=(Blues-6-1);
  color=(Blues-6-2);
  color=(Blues-6-3);
  color=(Blues-6-4);
  color=(Blues-6-5);
  color=(Blues-6-6);
},
colormap={Blues-7}{
  color=(Blues-7-1);
  color=(Blues-7-2);
  color=(Blues-7-3);
  color=(Blues-7-4);
  color=(Blues-7-5);
  color=(Blues-7-6);
  color=(Blues-7-7);
},
colormap={Blues-8}{
  color=(Blues-8-1);
  color=(Blues-8-2);
  color=(Blues-8-3);
  color=(Blues-8-4);
  color=(Blues-8-5);
  color=(Blues-8-6);
  color=(Blues-8-7);
  color=(Blues-8-8);
},
colormap={Blues-9}{
  color=(Blues-9-1);
  color=(Blues-9-2);
  color=(Blues-9-3);
  color=(Blues-9-4);
  color=(Blues-9-5);
  color=(Blues-9-6);
  color=(Blues-9-7);
  color=(Blues-9-8);
  color=(Blues-9-9);
},
colormap={Greens-3}{
  color=(Greens-3-1);
  color=(Greens-3-2);
  color=(Greens-3-3);
},
colormap={Greens-4}{
  color=(Greens-4-1);
  color=(Greens-4-2);
  color=(Greens-4-3);
  color=(Greens-4-4);
},
colormap={Greens-5}{
  color=(Greens-5-1);
  color=(Greens-5-2);
  color=(Greens-5-3);
  color=(Greens-5-4);
  color=(Greens-5-5);
},
colormap={Greens-6}{
  color=(Greens-6-1);
  color=(Greens-6-2);
  color=(Greens-6-3);
  color=(Greens-6-4);
  color=(Greens-6-5);
  color=(Greens-6-6);
},
colormap={Greens-7}{
  color=(Greens-7-1);
  color=(Greens-7-2);
  color=(Greens-7-3);
  color=(Greens-7-4);
  color=(Greens-7-5);
  color=(Greens-7-6);
  color=(Greens-7-7);
},
colormap={Greens-8}{
  color=(Greens-8-1);
  color=(Greens-8-2);
  color=(Greens-8-3);
  color=(Greens-8-4);
  color=(Greens-8-5);
  color=(Greens-8-6);
  color=(Greens-8-7);
  color=(Greens-8-8);
},
colormap={Greens-9}{
  color=(Greens-9-1);
  color=(Greens-9-2);
  color=(Greens-9-3);
  color=(Greens-9-4);
  color=(Greens-9-5);
  color=(Greens-9-6);
  color=(Greens-9-7);
  color=(Greens-9-8);
  color=(Greens-9-9);
},
colormap={Oranges-3}{
  color=(Oranges-3-1);
  color=(Oranges-3-2);
  color=(Oranges-3-3);
},
colormap={Oranges-4}{
  color=(Oranges-4-1);
  color=(Oranges-4-2);
  color=(Oranges-4-3);
  color=(Oranges-4-4);
},
colormap={Oranges-5}{
  color=(Oranges-5-1);
  color=(Oranges-5-2);
  color=(Oranges-5-3);
  color=(Oranges-5-4);
  color=(Oranges-5-5);
},
colormap={Oranges-6}{
  color=(Oranges-6-1);
  color=(Oranges-6-2);
  color=(Oranges-6-3);
  color=(Oranges-6-4);
  color=(Oranges-6-5);
  color=(Oranges-6-6);
},
colormap={Oranges-7}{
  color=(Oranges-7-1);
  color=(Oranges-7-2);
  color=(Oranges-7-3);
  color=(Oranges-7-4);
  color=(Oranges-7-5);
  color=(Oranges-7-6);
  color=(Oranges-7-7);
},
colormap={Oranges-8}{
  color=(Oranges-8-1);
  color=(Oranges-8-2);
  color=(Oranges-8-3);
  color=(Oranges-8-4);
  color=(Oranges-8-5);
  color=(Oranges-8-6);
  color=(Oranges-8-7);
  color=(Oranges-8-8);
},
colormap={Oranges-9}{
  color=(Oranges-9-1);
  color=(Oranges-9-2);
  color=(Oranges-9-3);
  color=(Oranges-9-4);
  color=(Oranges-9-5);
  color=(Oranges-9-6);
  color=(Oranges-9-7);
  color=(Oranges-9-8);
  color=(Oranges-9-9);
},
colormap={Reds-3}{
  color=(Reds-3-1);
  color=(Reds-3-2);
  color=(Reds-3-3);
},
colormap={Reds-4}{
  color=(Reds-4-1);
  color=(Reds-4-2);
  color=(Reds-4-3);
  color=(Reds-4-4);
},
colormap={Reds-5}{
  color=(Reds-5-1);
  color=(Reds-5-2);
  color=(Reds-5-3);
  color=(Reds-5-4);
  color=(Reds-5-5);
},
colormap={Reds-6}{
  color=(Reds-6-1);
  color=(Reds-6-2);
  color=(Reds-6-3);
  color=(Reds-6-4);
  color=(Reds-6-5);
  color=(Reds-6-6);
},
colormap={Reds-7}{
  color=(Reds-7-1);
  color=(Reds-7-2);
  color=(Reds-7-3);
  color=(Reds-7-4);
  color=(Reds-7-5);
  color=(Reds-7-6);
  color=(Reds-7-7);
},
colormap={Reds-8}{
  color=(Reds-8-1);
  color=(Reds-8-2);
  color=(Reds-8-3);
  color=(Reds-8-4);
  color=(Reds-8-5);
  color=(Reds-8-6);
  color=(Reds-8-7);
  color=(Reds-8-8);
},
colormap={Reds-9}{
  color=(Reds-9-1);
  color=(Reds-9-2);
  color=(Reds-9-3);
  color=(Reds-9-4);
  color=(Reds-9-5);
  color=(Reds-9-6);
  color=(Reds-9-7);
  color=(Reds-9-8);
  color=(Reds-9-9);
},
colormap={Greys-3}{
  color=(Greys-3-1);
  color=(Greys-3-2);
  color=(Greys-3-3);
},
colormap={Greys-4}{
  color=(Greys-4-1);
  color=(Greys-4-2);
  color=(Greys-4-3);
  color=(Greys-4-4);
},
colormap={Greys-5}{
  color=(Greys-5-1);
  color=(Greys-5-2);
  color=(Greys-5-3);
  color=(Greys-5-4);
  color=(Greys-5-5);
},
colormap={Greys-6}{
  color=(Greys-6-1);
  color=(Greys-6-2);
  color=(Greys-6-3);
  color=(Greys-6-4);
  color=(Greys-6-5);
  color=(Greys-6-6);
},
colormap={Greys-7}{
  color=(Greys-7-1);
  color=(Greys-7-2);
  color=(Greys-7-3);
  color=(Greys-7-4);
  color=(Greys-7-5);
  color=(Greys-7-6);
  color=(Greys-7-7);
},
colormap={Greys-8}{
  color=(Greys-8-1);
  color=(Greys-8-2);
  color=(Greys-8-3);
  color=(Greys-8-4);
  color=(Greys-8-5);
  color=(Greys-8-6);
  color=(Greys-8-7);
  color=(Greys-8-8);
},
colormap={Greys-9}{
  color=(Greys-9-1);
  color=(Greys-9-2);
  color=(Greys-9-3);
  color=(Greys-9-4);
  color=(Greys-9-5);
  color=(Greys-9-6);
  color=(Greys-9-7);
  color=(Greys-9-8);
  color=(Greys-9-9);
},
colormap={PuOr-3}{
  color=(PuOr-3-1);
  color=(PuOr-3-2);
  color=(PuOr-3-3);
},
colormap={PuOr-4}{
  color=(PuOr-4-1);
  color=(PuOr-4-2);
  color=(PuOr-4-3);
  color=(PuOr-4-4);
},
colormap={PuOr-5}{
  color=(PuOr-5-1);
  color=(PuOr-5-2);
  color=(PuOr-5-3);
  color=(PuOr-5-4);
  color=(PuOr-5-5);
},
colormap={PuOr-6}{
  color=(PuOr-6-1);
  color=(PuOr-6-2);
  color=(PuOr-6-3);
  color=(PuOr-6-4);
  color=(PuOr-6-5);
  color=(PuOr-6-6);
},
colormap={PuOr-7}{
  color=(PuOr-7-1);
  color=(PuOr-7-2);
  color=(PuOr-7-3);
  color=(PuOr-7-4);
  color=(PuOr-7-5);
  color=(PuOr-7-6);
  color=(PuOr-7-7);
},
colormap={PuOr-8}{
  color=(PuOr-8-1);
  color=(PuOr-8-2);
  color=(PuOr-8-3);
  color=(PuOr-8-4);
  color=(PuOr-8-5);
  color=(PuOr-8-6);
  color=(PuOr-8-7);
  color=(PuOr-8-8);
},
colormap={PuOr-9}{
  color=(PuOr-9-1);
  color=(PuOr-9-2);
  color=(PuOr-9-3);
  color=(PuOr-9-4);
  color=(PuOr-9-5);
  color=(PuOr-9-6);
  color=(PuOr-9-7);
  color=(PuOr-9-8);
  color=(PuOr-9-9);
},
colormap={PuOr-10}{
  color=(PuOr-10-1);
  color=(PuOr-10-2);
  color=(PuOr-10-3);
  color=(PuOr-10-4);
  color=(PuOr-10-5);
  color=(PuOr-10-6);
  color=(PuOr-10-7);
  color=(PuOr-10-8);
  color=(PuOr-10-9);
  color=(PuOr-10-10);
},
colormap={PuOr-11}{
  color=(PuOr-11-1);
  color=(PuOr-11-2);
  color=(PuOr-11-3);
  color=(PuOr-11-4);
  color=(PuOr-11-5);
  color=(PuOr-11-6);
  color=(PuOr-11-7);
  color=(PuOr-11-8);
  color=(PuOr-11-9);
  color=(PuOr-11-10);
  color=(PuOr-11-11);
},
colormap={BrBG-3}{
  color=(BrBG-3-1);
  color=(BrBG-3-2);
  color=(BrBG-3-3);
},
colormap={BrBG-4}{
  color=(BrBG-4-1);
  color=(BrBG-4-2);
  color=(BrBG-4-3);
  color=(BrBG-4-4);
},
colormap={BrBG-5}{
  color=(BrBG-5-1);
  color=(BrBG-5-2);
  color=(BrBG-5-3);
  color=(BrBG-5-4);
  color=(BrBG-5-5);
},
colormap={BrBG-6}{
  color=(BrBG-6-1);
  color=(BrBG-6-2);
  color=(BrBG-6-3);
  color=(BrBG-6-4);
  color=(BrBG-6-5);
  color=(BrBG-6-6);
},
colormap={BrBG-7}{
  color=(BrBG-7-1);
  color=(BrBG-7-2);
  color=(BrBG-7-3);
  color=(BrBG-7-4);
  color=(BrBG-7-5);
  color=(BrBG-7-6);
  color=(BrBG-7-7);
},
colormap={BrBG-8}{
  color=(BrBG-8-1);
  color=(BrBG-8-2);
  color=(BrBG-8-3);
  color=(BrBG-8-4);
  color=(BrBG-8-5);
  color=(BrBG-8-6);
  color=(BrBG-8-7);
  color=(BrBG-8-8);
},
colormap={BrBG-9}{
  color=(BrBG-9-1);
  color=(BrBG-9-2);
  color=(BrBG-9-3);
  color=(BrBG-9-4);
  color=(BrBG-9-5);
  color=(BrBG-9-6);
  color=(BrBG-9-7);
  color=(BrBG-9-8);
  color=(BrBG-9-9);
},
colormap={BrBG-10}{
  color=(BrBG-10-1);
  color=(BrBG-10-2);
  color=(BrBG-10-3);
  color=(BrBG-10-4);
  color=(BrBG-10-5);
  color=(BrBG-10-6);
  color=(BrBG-10-7);
  color=(BrBG-10-8);
  color=(BrBG-10-9);
  color=(BrBG-10-10);
},
colormap={BrBG-11}{
  color=(BrBG-11-1);
  color=(BrBG-11-2);
  color=(BrBG-11-3);
  color=(BrBG-11-4);
  color=(BrBG-11-5);
  color=(BrBG-11-6);
  color=(BrBG-11-7);
  color=(BrBG-11-8);
  color=(BrBG-11-9);
  color=(BrBG-11-10);
  color=(BrBG-11-11);
},
colormap={PRGn-3}{
  color=(PRGn-3-1);
  color=(PRGn-3-2);
  color=(PRGn-3-3);
},
colormap={PRGn-4}{
  color=(PRGn-4-1);
  color=(PRGn-4-2);
  color=(PRGn-4-3);
  color=(PRGn-4-4);
},
colormap={PRGn-5}{
  color=(PRGn-5-1);
  color=(PRGn-5-2);
  color=(PRGn-5-3);
  color=(PRGn-5-4);
  color=(PRGn-5-5);
},
colormap={PRGn-6}{
  color=(PRGn-6-1);
  color=(PRGn-6-2);
  color=(PRGn-6-3);
  color=(PRGn-6-4);
  color=(PRGn-6-5);
  color=(PRGn-6-6);
},
colormap={PRGn-7}{
  color=(PRGn-7-1);
  color=(PRGn-7-2);
  color=(PRGn-7-3);
  color=(PRGn-7-4);
  color=(PRGn-7-5);
  color=(PRGn-7-6);
  color=(PRGn-7-7);
},
colormap={PRGn-8}{
  color=(PRGn-8-1);
  color=(PRGn-8-2);
  color=(PRGn-8-3);
  color=(PRGn-8-4);
  color=(PRGn-8-5);
  color=(PRGn-8-6);
  color=(PRGn-8-7);
  color=(PRGn-8-8);
},
colormap={PRGn-9}{
  color=(PRGn-9-1);
  color=(PRGn-9-2);
  color=(PRGn-9-3);
  color=(PRGn-9-4);
  color=(PRGn-9-5);
  color=(PRGn-9-6);
  color=(PRGn-9-7);
  color=(PRGn-9-8);
  color=(PRGn-9-9);
},
colormap={PRGn-10}{
  color=(PRGn-10-1);
  color=(PRGn-10-2);
  color=(PRGn-10-3);
  color=(PRGn-10-4);
  color=(PRGn-10-5);
  color=(PRGn-10-6);
  color=(PRGn-10-7);
  color=(PRGn-10-8);
  color=(PRGn-10-9);
  color=(PRGn-10-10);
},
colormap={PRGn-11}{
  color=(PRGn-11-1);
  color=(PRGn-11-2);
  color=(PRGn-11-3);
  color=(PRGn-11-4);
  color=(PRGn-11-5);
  color=(PRGn-11-6);
  color=(PRGn-11-7);
  color=(PRGn-11-8);
  color=(PRGn-11-9);
  color=(PRGn-11-10);
  color=(PRGn-11-11);
},
colormap={PiYG-3}{
  color=(PiYG-3-1);
  color=(PiYG-3-2);
  color=(PiYG-3-3);
},
colormap={PiYG-4}{
  color=(PiYG-4-1);
  color=(PiYG-4-2);
  color=(PiYG-4-3);
  color=(PiYG-4-4);
},
colormap={PiYG-5}{
  color=(PiYG-5-1);
  color=(PiYG-5-2);
  color=(PiYG-5-3);
  color=(PiYG-5-4);
  color=(PiYG-5-5);
},
colormap={PiYG-6}{
  color=(PiYG-6-1);
  color=(PiYG-6-2);
  color=(PiYG-6-3);
  color=(PiYG-6-4);
  color=(PiYG-6-5);
  color=(PiYG-6-6);
},
colormap={PiYG-7}{
  color=(PiYG-7-1);
  color=(PiYG-7-2);
  color=(PiYG-7-3);
  color=(PiYG-7-4);
  color=(PiYG-7-5);
  color=(PiYG-7-6);
  color=(PiYG-7-7);
},
colormap={PiYG-8}{
  color=(PiYG-8-1);
  color=(PiYG-8-2);
  color=(PiYG-8-3);
  color=(PiYG-8-4);
  color=(PiYG-8-5);
  color=(PiYG-8-6);
  color=(PiYG-8-7);
  color=(PiYG-8-8);
},
colormap={PiYG-9}{
  color=(PiYG-9-1);
  color=(PiYG-9-2);
  color=(PiYG-9-3);
  color=(PiYG-9-4);
  color=(PiYG-9-5);
  color=(PiYG-9-6);
  color=(PiYG-9-7);
  color=(PiYG-9-8);
  color=(PiYG-9-9);
},
colormap={PiYG-10}{
  color=(PiYG-10-1);
  color=(PiYG-10-2);
  color=(PiYG-10-3);
  color=(PiYG-10-4);
  color=(PiYG-10-5);
  color=(PiYG-10-6);
  color=(PiYG-10-7);
  color=(PiYG-10-8);
  color=(PiYG-10-9);
  color=(PiYG-10-10);
},
colormap={PiYG-11}{
  color=(PiYG-11-1);
  color=(PiYG-11-2);
  color=(PiYG-11-3);
  color=(PiYG-11-4);
  color=(PiYG-11-5);
  color=(PiYG-11-6);
  color=(PiYG-11-7);
  color=(PiYG-11-8);
  color=(PiYG-11-9);
  color=(PiYG-11-10);
  color=(PiYG-11-11);
},
colormap={RdBu-3}{
  color=(RdBu-3-1);
  color=(RdBu-3-2);
  color=(RdBu-3-3);
},
colormap={RdBu-4}{
  color=(RdBu-4-1);
  color=(RdBu-4-2);
  color=(RdBu-4-3);
  color=(RdBu-4-4);
},
colormap={RdBu-5}{
  color=(RdBu-5-1);
  color=(RdBu-5-2);
  color=(RdBu-5-3);
  color=(RdBu-5-4);
  color=(RdBu-5-5);
},
colormap={RdBu-6}{
  color=(RdBu-6-1);
  color=(RdBu-6-2);
  color=(RdBu-6-3);
  color=(RdBu-6-4);
  color=(RdBu-6-5);
  color=(RdBu-6-6);
},
colormap={RdBu-7}{
  color=(RdBu-7-1);
  color=(RdBu-7-2);
  color=(RdBu-7-3);
  color=(RdBu-7-4);
  color=(RdBu-7-5);
  color=(RdBu-7-6);
  color=(RdBu-7-7);
},
colormap={RdBu-8}{
  color=(RdBu-8-1);
  color=(RdBu-8-2);
  color=(RdBu-8-3);
  color=(RdBu-8-4);
  color=(RdBu-8-5);
  color=(RdBu-8-6);
  color=(RdBu-8-7);
  color=(RdBu-8-8);
},
colormap={RdBu-9}{
  color=(RdBu-9-1);
  color=(RdBu-9-2);
  color=(RdBu-9-3);
  color=(RdBu-9-4);
  color=(RdBu-9-5);
  color=(RdBu-9-6);
  color=(RdBu-9-7);
  color=(RdBu-9-8);
  color=(RdBu-9-9);
},
colormap={RdBu-10}{
  color=(RdBu-10-1);
  color=(RdBu-10-2);
  color=(RdBu-10-3);
  color=(RdBu-10-4);
  color=(RdBu-10-5);
  color=(RdBu-10-6);
  color=(RdBu-10-7);
  color=(RdBu-10-8);
  color=(RdBu-10-9);
  color=(RdBu-10-10);
},
colormap={RdBu-11}{
  color=(RdBu-11-1);
  color=(RdBu-11-2);
  color=(RdBu-11-3);
  color=(RdBu-11-4);
  color=(RdBu-11-5);
  color=(RdBu-11-6);
  color=(RdBu-11-7);
  color=(RdBu-11-8);
  color=(RdBu-11-9);
  color=(RdBu-11-10);
  color=(RdBu-11-11);
},
colormap={RdGy-3}{
  color=(RdGy-3-1);
  color=(RdGy-3-2);
  color=(RdGy-3-3);
},
colormap={RdGy-4}{
  color=(RdGy-4-1);
  color=(RdGy-4-2);
  color=(RdGy-4-3);
  color=(RdGy-4-4);
},
colormap={RdGy-5}{
  color=(RdGy-5-1);
  color=(RdGy-5-2);
  color=(RdGy-5-3);
  color=(RdGy-5-4);
  color=(RdGy-5-5);
},
colormap={RdGy-6}{
  color=(RdGy-6-1);
  color=(RdGy-6-2);
  color=(RdGy-6-3);
  color=(RdGy-6-4);
  color=(RdGy-6-5);
  color=(RdGy-6-6);
},
colormap={RdGy-7}{
  color=(RdGy-7-1);
  color=(RdGy-7-2);
  color=(RdGy-7-3);
  color=(RdGy-7-4);
  color=(RdGy-7-5);
  color=(RdGy-7-6);
  color=(RdGy-7-7);
},
colormap={RdGy-8}{
  color=(RdGy-8-1);
  color=(RdGy-8-2);
  color=(RdGy-8-3);
  color=(RdGy-8-4);
  color=(RdGy-8-5);
  color=(RdGy-8-6);
  color=(RdGy-8-7);
  color=(RdGy-8-8);
},
colormap={RdGy-9}{
  color=(RdGy-9-1);
  color=(RdGy-9-2);
  color=(RdGy-9-3);
  color=(RdGy-9-4);
  color=(RdGy-9-5);
  color=(RdGy-9-6);
  color=(RdGy-9-7);
  color=(RdGy-9-8);
  color=(RdGy-9-9);
},
colormap={RdGy-10}{
  color=(RdGy-10-1);
  color=(RdGy-10-2);
  color=(RdGy-10-3);
  color=(RdGy-10-4);
  color=(RdGy-10-5);
  color=(RdGy-10-6);
  color=(RdGy-10-7);
  color=(RdGy-10-8);
  color=(RdGy-10-9);
  color=(RdGy-10-10);
},
colormap={RdGy-11}{
  color=(RdGy-11-1);
  color=(RdGy-11-2);
  color=(RdGy-11-3);
  color=(RdGy-11-4);
  color=(RdGy-11-5);
  color=(RdGy-11-6);
  color=(RdGy-11-7);
  color=(RdGy-11-8);
  color=(RdGy-11-9);
  color=(RdGy-11-10);
  color=(RdGy-11-11);
},
colormap={RdYlBu-3}{
  color=(RdYlBu-3-1);
  color=(RdYlBu-3-2);
  color=(RdYlBu-3-3);
},
colormap={RdYlBu-4}{
  color=(RdYlBu-4-1);
  color=(RdYlBu-4-2);
  color=(RdYlBu-4-3);
  color=(RdYlBu-4-4);
},
colormap={RdYlBu-5}{
  color=(RdYlBu-5-1);
  color=(RdYlBu-5-2);
  color=(RdYlBu-5-3);
  color=(RdYlBu-5-4);
  color=(RdYlBu-5-5);
},
colormap={RdYlBu-6}{
  color=(RdYlBu-6-1);
  color=(RdYlBu-6-2);
  color=(RdYlBu-6-3);
  color=(RdYlBu-6-4);
  color=(RdYlBu-6-5);
  color=(RdYlBu-6-6);
},
colormap={RdYlBu-7}{
  color=(RdYlBu-7-1);
  color=(RdYlBu-7-2);
  color=(RdYlBu-7-3);
  color=(RdYlBu-7-4);
  color=(RdYlBu-7-5);
  color=(RdYlBu-7-6);
  color=(RdYlBu-7-7);
},
colormap={RdYlBu-8}{
  color=(RdYlBu-8-1);
  color=(RdYlBu-8-2);
  color=(RdYlBu-8-3);
  color=(RdYlBu-8-4);
  color=(RdYlBu-8-5);
  color=(RdYlBu-8-6);
  color=(RdYlBu-8-7);
  color=(RdYlBu-8-8);
},
colormap={RdYlBu-9}{
  color=(RdYlBu-9-1);
  color=(RdYlBu-9-2);
  color=(RdYlBu-9-3);
  color=(RdYlBu-9-4);
  color=(RdYlBu-9-5);
  color=(RdYlBu-9-6);
  color=(RdYlBu-9-7);
  color=(RdYlBu-9-8);
  color=(RdYlBu-9-9);
},
colormap={RdYlBu-10}{
  color=(RdYlBu-10-1);
  color=(RdYlBu-10-2);
  color=(RdYlBu-10-3);
  color=(RdYlBu-10-4);
  color=(RdYlBu-10-5);
  color=(RdYlBu-10-6);
  color=(RdYlBu-10-7);
  color=(RdYlBu-10-8);
  color=(RdYlBu-10-9);
  color=(RdYlBu-10-10);
},
colormap={RdYlBu-11}{
  color=(RdYlBu-11-1);
  color=(RdYlBu-11-2);
  color=(RdYlBu-11-3);
  color=(RdYlBu-11-4);
  color=(RdYlBu-11-5);
  color=(RdYlBu-11-6);
  color=(RdYlBu-11-7);
  color=(RdYlBu-11-8);
  color=(RdYlBu-11-9);
  color=(RdYlBu-11-10);
  color=(RdYlBu-11-11);
},
colormap={Spectral-3}{
  color=(Spectral-3-1);
  color=(Spectral-3-2);
  color=(Spectral-3-3);
},
colormap={Spectral-4}{
  color=(Spectral-4-1);
  color=(Spectral-4-2);
  color=(Spectral-4-3);
  color=(Spectral-4-4);
},
colormap={Spectral-5}{
  color=(Spectral-5-1);
  color=(Spectral-5-2);
  color=(Spectral-5-3);
  color=(Spectral-5-4);
  color=(Spectral-5-5);
},
colormap={Spectral-6}{
  color=(Spectral-6-1);
  color=(Spectral-6-2);
  color=(Spectral-6-3);
  color=(Spectral-6-4);
  color=(Spectral-6-5);
  color=(Spectral-6-6);
},
colormap={Spectral-7}{
  color=(Spectral-7-1);
  color=(Spectral-7-2);
  color=(Spectral-7-3);
  color=(Spectral-7-4);
  color=(Spectral-7-5);
  color=(Spectral-7-6);
  color=(Spectral-7-7);
},
colormap={Spectral-8}{
  color=(Spectral-8-1);
  color=(Spectral-8-2);
  color=(Spectral-8-3);
  color=(Spectral-8-4);
  color=(Spectral-8-5);
  color=(Spectral-8-6);
  color=(Spectral-8-7);
  color=(Spectral-8-8);
},
colormap={Spectral-9}{
  color=(Spectral-9-1);
  color=(Spectral-9-2);
  color=(Spectral-9-3);
  color=(Spectral-9-4);
  color=(Spectral-9-5);
  color=(Spectral-9-6);
  color=(Spectral-9-7);
  color=(Spectral-9-8);
  color=(Spectral-9-9);
},
colormap={Spectral-10}{
  color=(Spectral-10-1);
  color=(Spectral-10-2);
  color=(Spectral-10-3);
  color=(Spectral-10-4);
  color=(Spectral-10-5);
  color=(Spectral-10-6);
  color=(Spectral-10-7);
  color=(Spectral-10-8);
  color=(Spectral-10-9);
  color=(Spectral-10-10);
},
colormap={Spectral-11}{
  color=(Spectral-11-1);
  color=(Spectral-11-2);
  color=(Spectral-11-3);
  color=(Spectral-11-4);
  color=(Spectral-11-5);
  color=(Spectral-11-6);
  color=(Spectral-11-7);
  color=(Spectral-11-8);
  color=(Spectral-11-9);
  color=(Spectral-11-10);
  color=(Spectral-11-11);
},
colormap={RdYlGn-3}{
  color=(RdYlGn-3-1);
  color=(RdYlGn-3-2);
  color=(RdYlGn-3-3);
},
colormap={RdYlGn-4}{
  color=(RdYlGn-4-1);
  color=(RdYlGn-4-2);
  color=(RdYlGn-4-3);
  color=(RdYlGn-4-4);
},
colormap={RdYlGn-5}{
  color=(RdYlGn-5-1);
  color=(RdYlGn-5-2);
  color=(RdYlGn-5-3);
  color=(RdYlGn-5-4);
  color=(RdYlGn-5-5);
},
colormap={RdYlGn-6}{
  color=(RdYlGn-6-1);
  color=(RdYlGn-6-2);
  color=(RdYlGn-6-3);
  color=(RdYlGn-6-4);
  color=(RdYlGn-6-5);
  color=(RdYlGn-6-6);
},
colormap={RdYlGn-7}{
  color=(RdYlGn-7-1);
  color=(RdYlGn-7-2);
  color=(RdYlGn-7-3);
  color=(RdYlGn-7-4);
  color=(RdYlGn-7-5);
  color=(RdYlGn-7-6);
  color=(RdYlGn-7-7);
},
colormap={RdYlGn-8}{
  color=(RdYlGn-8-1);
  color=(RdYlGn-8-2);
  color=(RdYlGn-8-3);
  color=(RdYlGn-8-4);
  color=(RdYlGn-8-5);
  color=(RdYlGn-8-6);
  color=(RdYlGn-8-7);
  color=(RdYlGn-8-8);
},
colormap={RdYlGn-9}{
  color=(RdYlGn-9-1);
  color=(RdYlGn-9-2);
  color=(RdYlGn-9-3);
  color=(RdYlGn-9-4);
  color=(RdYlGn-9-5);
  color=(RdYlGn-9-6);
  color=(RdYlGn-9-7);
  color=(RdYlGn-9-8);
  color=(RdYlGn-9-9);
},
colormap={RdYlGn-10}{
  color=(RdYlGn-10-1);
  color=(RdYlGn-10-2);
  color=(RdYlGn-10-3);
  color=(RdYlGn-10-4);
  color=(RdYlGn-10-5);
  color=(RdYlGn-10-6);
  color=(RdYlGn-10-7);
  color=(RdYlGn-10-8);
  color=(RdYlGn-10-9);
  color=(RdYlGn-10-10);
},
colormap={RdYlGn-11}{
  color=(RdYlGn-11-1);
  color=(RdYlGn-11-2);
  color=(RdYlGn-11-3);
  color=(RdYlGn-11-4);
  color=(RdYlGn-11-5);
  color=(RdYlGn-11-6);
  color=(RdYlGn-11-7);
  color=(RdYlGn-11-8);
  color=(RdYlGn-11-9);
  color=(RdYlGn-11-10);
  color=(RdYlGn-11-11);
},
colormap={Set3-3}{
  color=(Set3-3-1);
  color=(Set3-3-2);
  color=(Set3-3-3);
},
colormap={Set3-4}{
  color=(Set3-4-1);
  color=(Set3-4-2);
  color=(Set3-4-3);
  color=(Set3-4-4);
},
colormap={Set3-5}{
  color=(Set3-5-1);
  color=(Set3-5-2);
  color=(Set3-5-3);
  color=(Set3-5-4);
  color=(Set3-5-5);
},
colormap={Set3-6}{
  color=(Set3-6-1);
  color=(Set3-6-2);
  color=(Set3-6-3);
  color=(Set3-6-4);
  color=(Set3-6-5);
  color=(Set3-6-6);
},
colormap={Set3-7}{
  color=(Set3-7-1);
  color=(Set3-7-2);
  color=(Set3-7-3);
  color=(Set3-7-4);
  color=(Set3-7-5);
  color=(Set3-7-6);
  color=(Set3-7-7);
},
colormap={Set3-8}{
  color=(Set3-8-1);
  color=(Set3-8-2);
  color=(Set3-8-3);
  color=(Set3-8-4);
  color=(Set3-8-5);
  color=(Set3-8-6);
  color=(Set3-8-7);
  color=(Set3-8-8);
},
colormap={Set3-9}{
  color=(Set3-9-1);
  color=(Set3-9-2);
  color=(Set3-9-3);
  color=(Set3-9-4);
  color=(Set3-9-5);
  color=(Set3-9-6);
  color=(Set3-9-7);
  color=(Set3-9-8);
  color=(Set3-9-9);
},
colormap={Set3-10}{
  color=(Set3-10-1);
  color=(Set3-10-2);
  color=(Set3-10-3);
  color=(Set3-10-4);
  color=(Set3-10-5);
  color=(Set3-10-6);
  color=(Set3-10-7);
  color=(Set3-10-8);
  color=(Set3-10-9);
  color=(Set3-10-10);
},
colormap={Set3-11}{
  color=(Set3-11-1);
  color=(Set3-11-2);
  color=(Set3-11-3);
  color=(Set3-11-4);
  color=(Set3-11-5);
  color=(Set3-11-6);
  color=(Set3-11-7);
  color=(Set3-11-8);
  color=(Set3-11-9);
  color=(Set3-11-10);
  color=(Set3-11-11);
},
colormap={Set3-12}{
  color=(Set3-12-1);
  color=(Set3-12-2);
  color=(Set3-12-3);
  color=(Set3-12-4);
  color=(Set3-12-5);
  color=(Set3-12-6);
  color=(Set3-12-7);
  color=(Set3-12-8);
  color=(Set3-12-9);
  color=(Set3-12-10);
  color=(Set3-12-11);
  color=(Set3-12-12);
},
colormap={Pastel1-3}{
  color=(Pastel1-3-1);
  color=(Pastel1-3-2);
  color=(Pastel1-3-3);
},
colormap={Pastel1-4}{
  color=(Pastel1-4-1);
  color=(Pastel1-4-2);
  color=(Pastel1-4-3);
  color=(Pastel1-4-4);
},
colormap={Pastel1-5}{
  color=(Pastel1-5-1);
  color=(Pastel1-5-2);
  color=(Pastel1-5-3);
  color=(Pastel1-5-4);
  color=(Pastel1-5-5);
},
colormap={Pastel1-6}{
  color=(Pastel1-6-1);
  color=(Pastel1-6-2);
  color=(Pastel1-6-3);
  color=(Pastel1-6-4);
  color=(Pastel1-6-5);
  color=(Pastel1-6-6);
},
colormap={Pastel1-7}{
  color=(Pastel1-7-1);
  color=(Pastel1-7-2);
  color=(Pastel1-7-3);
  color=(Pastel1-7-4);
  color=(Pastel1-7-5);
  color=(Pastel1-7-6);
  color=(Pastel1-7-7);
},
colormap={Pastel1-8}{
  color=(Pastel1-8-1);
  color=(Pastel1-8-2);
  color=(Pastel1-8-3);
  color=(Pastel1-8-4);
  color=(Pastel1-8-5);
  color=(Pastel1-8-6);
  color=(Pastel1-8-7);
  color=(Pastel1-8-8);
},
colormap={Pastel1-9}{
  color=(Pastel1-9-1);
  color=(Pastel1-9-2);
  color=(Pastel1-9-3);
  color=(Pastel1-9-4);
  color=(Pastel1-9-5);
  color=(Pastel1-9-6);
  color=(Pastel1-9-7);
  color=(Pastel1-9-8);
  color=(Pastel1-9-9);
},
colormap={Set1-3}{
  color=(Set1-3-1);
  color=(Set1-3-2);
  color=(Set1-3-3);
},
colormap={Set1-4}{
  color=(Set1-4-1);
  color=(Set1-4-2);
  color=(Set1-4-3);
  color=(Set1-4-4);
},
colormap={Set1-5}{
  color=(Set1-5-1);
  color=(Set1-5-2);
  color=(Set1-5-3);
  color=(Set1-5-4);
  color=(Set1-5-5);
},
colormap={Set1-6}{
  color=(Set1-6-1);
  color=(Set1-6-2);
  color=(Set1-6-3);
  color=(Set1-6-4);
  color=(Set1-6-5);
  color=(Set1-6-6);
},
colormap={Set1-7}{
  color=(Set1-7-1);
  color=(Set1-7-2);
  color=(Set1-7-3);
  color=(Set1-7-4);
  color=(Set1-7-5);
  color=(Set1-7-6);
  color=(Set1-7-7);
},
colormap={Set1-8}{
  color=(Set1-8-1);
  color=(Set1-8-2);
  color=(Set1-8-3);
  color=(Set1-8-4);
  color=(Set1-8-5);
  color=(Set1-8-6);
  color=(Set1-8-7);
  color=(Set1-8-8);
},
colormap={Set1-9}{
  color=(Set1-9-1);
  color=(Set1-9-2);
  color=(Set1-9-3);
  color=(Set1-9-4);
  color=(Set1-9-5);
  color=(Set1-9-6);
  color=(Set1-9-7);
  color=(Set1-9-8);
  color=(Set1-9-9);
},
colormap={Pastel2-3}{
  color=(Pastel2-3-1);
  color=(Pastel2-3-2);
  color=(Pastel2-3-3);
},
colormap={Pastel2-4}{
  color=(Pastel2-4-1);
  color=(Pastel2-4-2);
  color=(Pastel2-4-3);
  color=(Pastel2-4-4);
},
colormap={Pastel2-5}{
  color=(Pastel2-5-1);
  color=(Pastel2-5-2);
  color=(Pastel2-5-3);
  color=(Pastel2-5-4);
  color=(Pastel2-5-5);
},
colormap={Pastel2-6}{
  color=(Pastel2-6-1);
  color=(Pastel2-6-2);
  color=(Pastel2-6-3);
  color=(Pastel2-6-4);
  color=(Pastel2-6-5);
  color=(Pastel2-6-6);
},
colormap={Pastel2-7}{
  color=(Pastel2-7-1);
  color=(Pastel2-7-2);
  color=(Pastel2-7-3);
  color=(Pastel2-7-4);
  color=(Pastel2-7-5);
  color=(Pastel2-7-6);
  color=(Pastel2-7-7);
},
colormap={Pastel2-8}{
  color=(Pastel2-8-1);
  color=(Pastel2-8-2);
  color=(Pastel2-8-3);
  color=(Pastel2-8-4);
  color=(Pastel2-8-5);
  color=(Pastel2-8-6);
  color=(Pastel2-8-7);
  color=(Pastel2-8-8);
},
colormap={Set2-3}{
  color=(Set2-3-1);
  color=(Set2-3-2);
  color=(Set2-3-3);
},
colormap={Set2-4}{
  color=(Set2-4-1);
  color=(Set2-4-2);
  color=(Set2-4-3);
  color=(Set2-4-4);
},
colormap={Set2-5}{
  color=(Set2-5-1);
  color=(Set2-5-2);
  color=(Set2-5-3);
  color=(Set2-5-4);
  color=(Set2-5-5);
},
colormap={Set2-6}{
  color=(Set2-6-1);
  color=(Set2-6-2);
  color=(Set2-6-3);
  color=(Set2-6-4);
  color=(Set2-6-5);
  color=(Set2-6-6);
},
colormap={Set2-7}{
  color=(Set2-7-1);
  color=(Set2-7-2);
  color=(Set2-7-3);
  color=(Set2-7-4);
  color=(Set2-7-5);
  color=(Set2-7-6);
  color=(Set2-7-7);
},
colormap={Set2-8}{
  color=(Set2-8-1);
  color=(Set2-8-2);
  color=(Set2-8-3);
  color=(Set2-8-4);
  color=(Set2-8-5);
  color=(Set2-8-6);
  color=(Set2-8-7);
  color=(Set2-8-8);
},
colormap={Dark2-3}{
  color=(Dark2-3-1);
  color=(Dark2-3-2);
  color=(Dark2-3-3);
},
colormap={Dark2-4}{
  color=(Dark2-4-1);
  color=(Dark2-4-2);
  color=(Dark2-4-3);
  color=(Dark2-4-4);
},
colormap={Dark2-5}{
  color=(Dark2-5-1);
  color=(Dark2-5-2);
  color=(Dark2-5-3);
  color=(Dark2-5-4);
  color=(Dark2-5-5);
},
colormap={Dark2-6}{
  color=(Dark2-6-1);
  color=(Dark2-6-2);
  color=(Dark2-6-3);
  color=(Dark2-6-4);
  color=(Dark2-6-5);
  color=(Dark2-6-6);
},
colormap={Dark2-7}{
  color=(Dark2-7-1);
  color=(Dark2-7-2);
  color=(Dark2-7-3);
  color=(Dark2-7-4);
  color=(Dark2-7-5);
  color=(Dark2-7-6);
  color=(Dark2-7-7);
},
colormap={Dark2-8}{
  color=(Dark2-8-1);
  color=(Dark2-8-2);
  color=(Dark2-8-3);
  color=(Dark2-8-4);
  color=(Dark2-8-5);
  color=(Dark2-8-6);
  color=(Dark2-8-7);
  color=(Dark2-8-8);
},
colormap={Paired-3}{
  color=(Paired-3-1);
  color=(Paired-3-2);
  color=(Paired-3-3);
},
colormap={Paired-4}{
  color=(Paired-4-1);
  color=(Paired-4-2);
  color=(Paired-4-3);
  color=(Paired-4-4);
},
colormap={Paired-5}{
  color=(Paired-5-1);
  color=(Paired-5-2);
  color=(Paired-5-3);
  color=(Paired-5-4);
  color=(Paired-5-5);
},
colormap={Paired-6}{
  color=(Paired-6-1);
  color=(Paired-6-2);
  color=(Paired-6-3);
  color=(Paired-6-4);
  color=(Paired-6-5);
  color=(Paired-6-6);
},
colormap={Paired-7}{
  color=(Paired-7-1);
  color=(Paired-7-2);
  color=(Paired-7-3);
  color=(Paired-7-4);
  color=(Paired-7-5);
  color=(Paired-7-6);
  color=(Paired-7-7);
},
colormap={Paired-8}{
  color=(Paired-8-1);
  color=(Paired-8-2);
  color=(Paired-8-3);
  color=(Paired-8-4);
  color=(Paired-8-5);
  color=(Paired-8-6);
  color=(Paired-8-7);
  color=(Paired-8-8);
},
colormap={Paired-9}{
  color=(Paired-9-1);
  color=(Paired-9-2);
  color=(Paired-9-3);
  color=(Paired-9-4);
  color=(Paired-9-5);
  color=(Paired-9-6);
  color=(Paired-9-7);
  color=(Paired-9-8);
  color=(Paired-9-9);
},
colormap={Paired-10}{
  color=(Paired-10-1);
  color=(Paired-10-2);
  color=(Paired-10-3);
  color=(Paired-10-4);
  color=(Paired-10-5);
  color=(Paired-10-6);
  color=(Paired-10-7);
  color=(Paired-10-8);
  color=(Paired-10-9);
  color=(Paired-10-10);
},
colormap={Paired-11}{
  color=(Paired-11-1);
  color=(Paired-11-2);
  color=(Paired-11-3);
  color=(Paired-11-4);
  color=(Paired-11-5);
  color=(Paired-11-6);
  color=(Paired-11-7);
  color=(Paired-11-8);
  color=(Paired-11-9);
  color=(Paired-11-10);
  color=(Paired-11-11);
},
colormap={Paired-12}{
  color=(Paired-12-1);
  color=(Paired-12-2);
  color=(Paired-12-3);
  color=(Paired-12-4);
  color=(Paired-12-5);
  color=(Paired-12-6);
  color=(Paired-12-7);
  color=(Paired-12-8);
  color=(Paired-12-9);
  color=(Paired-12-10);
  color=(Paired-12-11);
  color=(Paired-12-12);
},
colormap={Accent-3}{
  color=(Accent-3-1);
  color=(Accent-3-2);
  color=(Accent-3-3);
},
colormap={Accent-4}{
  color=(Accent-4-1);
  color=(Accent-4-2);
  color=(Accent-4-3);
  color=(Accent-4-4);
},
colormap={Accent-5}{
  color=(Accent-5-1);
  color=(Accent-5-2);
  color=(Accent-5-3);
  color=(Accent-5-4);
  color=(Accent-5-5);
},
colormap={Accent-6}{
  color=(Accent-6-1);
  color=(Accent-6-2);
  color=(Accent-6-3);
  color=(Accent-6-4);
  color=(Accent-6-5);
  color=(Accent-6-6);
},
colormap={Accent-7}{
  color=(Accent-7-1);
  color=(Accent-7-2);
  color=(Accent-7-3);
  color=(Accent-7-4);
  color=(Accent-7-5);
  color=(Accent-7-6);
  color=(Accent-7-7);
},
colormap={Accent-8}{
  color=(Accent-8-1);
  color=(Accent-8-2);
  color=(Accent-8-3);
  color=(Accent-8-4);
  color=(Accent-8-5);
  color=(Accent-8-6);
  color=(Accent-8-7);
  color=(Accent-8-8);
}
}


==> ignore/strassen_1_abc_2.tex <==
\begin{tikzpicture}[scale=.52]
%\begin{tikzpicture}
\begin{axis}[
%width=5cm,
%height=5cm,
title={$m=k=n$, 1 core},
xlabel={ $m = k = n$ },
%ylabel={\emph{Effective} GFLOPS},
  xmin=0,
  xmax=10000,
  ymin=20,
  ymax=34,
  xtick={1000,2000,3000,4000,5000,6000,7000,8000,9000,10000},
  ytick={5, 10, 15, 20, 25, 28.36, 30, 34},
  scaled x ticks=false,
  scaled x ticks=base 10:-3,
  grid=major,
  %scaled y ticks = false
  %x tick label style={/pgf/number format/1000 sep = \thinspace}
%/pgf/number format/fixed,
  %mark=square*,blue
  %axis background/.style={fill=blue!10},
  axis background/.style={fill=lightgray!20},
]

\addplot[
  %dotted,
  %dashed,
  red,
  %mark=*,
  %mark=x,
  %mark=triangle*,
  %only marks,
  %mark=diamond*,
  %mark=*,
  %mark=none,
  %mark=pentagon*,
  %mark=otimes,
  %mark=diamond*,
  %mark size=2.0pt,
  %mark options={scale=0.5,fill=white},
  %thick,
  %solid,
  line width=1pt,
] file {plotdata/strassen_1_abc.dat};


%\pgfplotsset{
%cycle list={%
%{red, mark=*}, {blue,mark=*},
%{red, mark=x}, {blue,mark=x},
%{red, mark=square*}, {blue,mark=square*},
%{red, mark=triangle*}, {blue,mark=triangle*},
%{red, mark=diamond*}, {blue,mark=diamond*},
%{red, mark=pentagon*}, {blue,mark=pentagon*}
%},
%legend style={
%at={(0.5,-0.2)},
%anchor=north,
%legend columns=2,
%cells={anchor=west},
%font=\footnotesize,
%rounded corners=2pt,
%},
%xlabel=$x$,ylabel=$f(x)$
%}
\addlegendentry{$a$}

\end{axis}
\end{tikzpicture}


==> ignore/strassen_uvw.tex <==

\begin{figure}[tb!]
{
\footnotesize%
\begin{equation*}
\begin{array}{l @{\hspace{1pt}} c @{\hspace{1pt}} l l r}  
M_0 &=& \alpha ( A_{0} + A_{3} ) ( B_{0} + B_{3} ); 
% \\ & 
& 
C_{0} +\!\!= M_0;  C_{3} +\!\!= M_0;  \\   
M_1 &=& \alpha ( A_{2} + A_{3} ) B_{0}; 
% \\ & 
& 
C_{2} +\!\!= M_1 ;  C_{3} -\!\!= M_1 ; \\  
M_2 &=& \alpha A_{0} ( B_{1} - B_{3} ); 
% \\ & 
&  
C_{1} +\!\!= M_2 ;  C_{3} +\!\!= M_2 ;
\\  
M_3 &=& \alpha A_{3}( B_{2} - B_{0} ); 
% \\ & 
&  
C_{0} +\!\!= M_3 ;  C_{2} +\!\!= M_3 ;
\\  
M_4 &=& \alpha ( A_{0} + A_{1}) B_{3};  
% \\ & 
& 
C_{1} +\!\!=  M_4 ;   C_{0} -\!\!= M_4;
\\  
M_5&=& \alpha (A_{2} - A_{0} )( B_{0} + B_{1} ); 
% \\ & 
& 
C_{3} +\!\!= M_5;  
\\  
M_6&=& \alpha (A_{1} - A_{3} )( B_{2} + B_{3} );  
% \\ & 
& 
C_{0} +\!\!= M_6 ; 
\end{array}
\label{eqn:allops}
\end{equation*} 


\[
\mathbf{U}=
\begin{bmatrix}
1 & 0 & 1 & 0 & 1 & -1 & 0 \\
0 & 0 & 0 & 0 & 1 & 0  & 1 \\
0 & 1 & 0 & 0 & 0 & 1  & 0 \\
1 & 1 & 0 & 1 & 0 & 0  & -1 \\
\end{bmatrix}
\]
\[
\mathbf{V}=
\begin{bmatrix}
1 & 1 & 0  & -1 & 0 & 1 & 0 \\
0 & 0 & 1  & 0  & 0 & 1 & 0 \\
0 & 0 & 0  & 1  & 0 & 0 & 1 \\
1 & 0 & -1 & 0  & 1 & 0 & 1 \\
\end{bmatrix}
\]
\[
\mathbf{W}=
\begin{bmatrix}
1 & 0 & 0 & 1 & -1 & 0 & 1 \\
0 & 0 & 1 & 0 & 1 & 0 & 0 \\
0 & 1 & 0 & 1 & 0 & 0 & 0 \\
1 & -1 & 1 & 0 & 0 & 1 & 0 \\
\end{bmatrix}
\]

} 
\caption{ $ \llbracket \bm{U}, \bm{V}, \bm{W} \rrbracket $ representation of
one-level $ \langle 2, 2, 2 \rangle $
Strassen's algorithm}

\label{fig:strassen_uvw}
\end{figure}




==> ignore/tikzlibrarypgfplots.colorbrewer.code.tex <==
\usepackage{pgfplotstable}

% Macro for creating a cycle list from a table.
% Makes it easier to define only as many cycle list entries as
% there are colorbrewer values
\newcommand\pgfplotscreatecolorbrewercyclelist{	\pgfmathtruncatemacro\maxindex{\pgfkeysvalueof{/pgfplots/colorbrewer values}-1}
	\pgfplotstabletypeset[
		begin table={},
		end table={},
		skip coltypes,
		string type,
		col sep=semicolon,
		write to macro=\listmacro,
		skip rows between index={\maxindex}{99},
		typeset=false,
		row sep=crcr
	]{
	colorbrewer1, thick, mark=*\\
	colorbrewer2, thick, mark=square*, mark size=1.75\\
	colorbrewer3, thick, mark=triangle*, mark size=2.5\\
	colorbrewer4, thick, mark=x, mark size=3, mark options={line width=2\pgflinewidth}\\
	colorbrewer5, thick, mark=*, mark options={fill=white}\\
	colorbrewer6, thick, mark=square*, mark size=1.75, mark options={fill=white}\\
	colorbrewer7, thick, mark=triangle*, mark size=2.5, mark options={fill=white}\\
	colorbrewer8, thick, mark=+, mark size=3, mark options={line width=2\pgflinewidth}\\
	}
	\begingroup
    \edef\A{\noexpand\global\noexpand\pgfplotscreateplotcyclelist{colorbrewer}{\unexpanded\expandafter{\listmacro}}}%
    \expandafter
    \endgroup\A
}

\pgfplotsset{
	colorbrewer values/.initial=8,
	colorbrewer scheme/.code={
		\pgfplotsset{colorbrewer scheme/#1}
		\pgfplotsset{colorbrewer values/\pgfkeysvalueof{/pgfplots/colorbrewer values}}
	},
	colorbrewer cycle list/.style={
		colorbrewer create cycle list,
		cycle list name=colorbrewer,
		/pgfplots/execute at begin axis={
			\pgfplotsset{
				colorbrewer scheme/#1,
				colorbrewer values/\pgfkeysvalueof{/pgfplots/colorbrewer values}
			}
		}
	},
	colorbrewer cycle list/.default=Dark2,
	colorbrewer create cycle list/.code={
		\pgfplotscreatecolorbrewercyclelist
	}
}



%%% The color schemes

\pgfplotsset{
	colorbrewer scheme/.is choice, 
	colorbrewer scheme/Accent/.style={
		colorbrewer values/.is choice,
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{127,201,127}
			\definecolor{colorbrewer2}{RGB}{190,174,212}
			\definecolor{colorbrewer3}{RGB}{253,192,134}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{127,201,127}
			\definecolor{colorbrewer2}{RGB}{190,174,212}
			\definecolor{colorbrewer3}{RGB}{253,192,134}
			\definecolor{colorbrewer4}{RGB}{255,255,153}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{127,201,127}
			\definecolor{colorbrewer2}{RGB}{190,174,212}
			\definecolor{colorbrewer3}{RGB}{253,192,134}
			\definecolor{colorbrewer4}{RGB}{255,255,153}
			\definecolor{colorbrewer5}{RGB}{56,108,176}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{127,201,127}
			\definecolor{colorbrewer2}{RGB}{190,174,212}
			\definecolor{colorbrewer3}{RGB}{253,192,134}
			\definecolor{colorbrewer4}{RGB}{255,255,153}
			\definecolor{colorbrewer5}{RGB}{56,108,176}
			\definecolor{colorbrewer6}{RGB}{240,2,127}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{127,201,127}
			\definecolor{colorbrewer2}{RGB}{190,174,212}
			\definecolor{colorbrewer3}{RGB}{253,192,134}
			\definecolor{colorbrewer4}{RGB}{255,255,153}
			\definecolor{colorbrewer5}{RGB}{56,108,176}
			\definecolor{colorbrewer6}{RGB}{240,2,127}
			\definecolor{colorbrewer7}{RGB}{191,91,23}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{127,201,127}
			\definecolor{colorbrewer2}{RGB}{190,174,212}
			\definecolor{colorbrewer3}{RGB}{253,192,134}
			\definecolor{colorbrewer4}{RGB}{255,255,153}
			\definecolor{colorbrewer5}{RGB}{56,108,176}
			\definecolor{colorbrewer6}{RGB}{240,2,127}
			\definecolor{colorbrewer7}{RGB}{191,91,23}
			\definecolor{colorbrewer8}{RGB}{102,102,102}
		},
		colorbrewer values/.unknown/.style={/errors/unknown choice value=\pgfkeyscurrentkey\pgfkeyscurrentvalue}
	},
	colorbrewer scheme/Blues/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{222,235,247}
			\definecolor{colorbrewer2}{RGB}{158,202,225}
			\definecolor{colorbrewer3}{RGB}{49,130,189}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{239,243,255}
			\definecolor{colorbrewer2}{RGB}{189,215,231}
			\definecolor{colorbrewer3}{RGB}{107,174,214}
			\definecolor{colorbrewer4}{RGB}{33,113,181}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{239,243,255}
			\definecolor{colorbrewer2}{RGB}{189,215,231}
			\definecolor{colorbrewer3}{RGB}{107,174,214}
			\definecolor{colorbrewer4}{RGB}{49,130,189}
			\definecolor{colorbrewer5}{RGB}{8,81,156}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{239,243,255}
			\definecolor{colorbrewer2}{RGB}{198,219,239}
			\definecolor{colorbrewer3}{RGB}{158,202,225}
			\definecolor{colorbrewer4}{RGB}{107,174,214}
			\definecolor{colorbrewer5}{RGB}{49,130,189}
			\definecolor{colorbrewer6}{RGB}{8,81,156}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{239,243,255}
			\definecolor{colorbrewer2}{RGB}{198,219,239}
			\definecolor{colorbrewer3}{RGB}{158,202,225}
			\definecolor{colorbrewer4}{RGB}{107,174,214}
			\definecolor{colorbrewer5}{RGB}{66,146,198}
			\definecolor{colorbrewer6}{RGB}{33,113,181}
			\definecolor{colorbrewer7}{RGB}{8,69,148}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{247,251,255}
			\definecolor{colorbrewer2}{RGB}{222,235,247}
			\definecolor{colorbrewer3}{RGB}{198,219,239}
			\definecolor{colorbrewer4}{RGB}{158,202,225}
			\definecolor{colorbrewer5}{RGB}{107,174,214}
			\definecolor{colorbrewer6}{RGB}{66,146,198}
			\definecolor{colorbrewer7}{RGB}{33,113,181}
			\definecolor{colorbrewer8}{RGB}{8,69,148}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{247,251,255}
			\definecolor{colorbrewer2}{RGB}{222,235,247}
			\definecolor{colorbrewer3}{RGB}{198,219,239}
			\definecolor{colorbrewer4}{RGB}{158,202,225}
			\definecolor{colorbrewer5}{RGB}{107,174,214}
			\definecolor{colorbrewer6}{RGB}{66,146,198}
			\definecolor{colorbrewer7}{RGB}{33,113,181}
			\definecolor{colorbrewer8}{RGB}{8,81,156}
			\definecolor{colorbrewer9}{RGB}{8,48,107}
		}
	},
	colorbrewer scheme/BrBG/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{216,179,101}
			\definecolor{colorbrewer2}{RGB}{245,245,245}
			\definecolor{colorbrewer3}{RGB}{90,180,172}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{166,97,26}
			\definecolor{colorbrewer2}{RGB}{223,194,125}
			\definecolor{colorbrewer3}{RGB}{128,205,193}
			\definecolor{colorbrewer4}{RGB}{1,133,113}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{166,97,26}
			\definecolor{colorbrewer2}{RGB}{223,194,125}
			\definecolor{colorbrewer3}{RGB}{245,245,245}
			\definecolor{colorbrewer4}{RGB}{128,205,193}
			\definecolor{colorbrewer5}{RGB}{1,133,113}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{140,81,10}
			\definecolor{colorbrewer2}{RGB}{216,179,101}
			\definecolor{colorbrewer3}{RGB}{246,232,195}
			\definecolor{colorbrewer4}{RGB}{199,234,229}
			\definecolor{colorbrewer5}{RGB}{90,180,172}
			\definecolor{colorbrewer6}{RGB}{1,102,94}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{140,81,10}
			\definecolor{colorbrewer2}{RGB}{216,179,101}
			\definecolor{colorbrewer3}{RGB}{246,232,195}
			\definecolor{colorbrewer4}{RGB}{245,245,245}
			\definecolor{colorbrewer5}{RGB}{199,234,229}
			\definecolor{colorbrewer6}{RGB}{90,180,172}
			\definecolor{colorbrewer7}{RGB}{1,102,94}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{140,81,10}
			\definecolor{colorbrewer2}{RGB}{191,129,45}
			\definecolor{colorbrewer3}{RGB}{223,194,125}
			\definecolor{colorbrewer4}{RGB}{246,232,195}
			\definecolor{colorbrewer5}{RGB}{199,234,229}
			\definecolor{colorbrewer6}{RGB}{128,205,193}
			\definecolor{colorbrewer7}{RGB}{53,151,143}
			\definecolor{colorbrewer8}{RGB}{1,102,94}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{140,81,10}
			\definecolor{colorbrewer2}{RGB}{191,129,45}
			\definecolor{colorbrewer3}{RGB}{223,194,125}
			\definecolor{colorbrewer4}{RGB}{246,232,195}
			\definecolor{colorbrewer5}{RGB}{245,245,245}
			\definecolor{colorbrewer6}{RGB}{199,234,229}
			\definecolor{colorbrewer7}{RGB}{128,205,193}
			\definecolor{colorbrewer8}{RGB}{53,151,143}
			\definecolor{colorbrewer9}{RGB}{1,102,94}
		},
		colorbrewer values/10/.code={
			\definecolor{colorbrewer1}{RGB}{84,48,5}
			\definecolor{colorbrewer2}{RGB}{140,81,10}
			\definecolor{colorbrewer3}{RGB}{191,129,45}
			\definecolor{colorbrewer4}{RGB}{223,194,125}
			\definecolor{colorbrewer5}{RGB}{246,232,195}
			\definecolor{colorbrewer6}{RGB}{199,234,229}
			\definecolor{colorbrewer7}{RGB}{128,205,193}
			\definecolor{colorbrewer8}{RGB}{53,151,143}
			\definecolor{colorbrewer9}{RGB}{1,102,94}
			\definecolor{colorbrewer10}{RGB}{0,60,48}
		},
		colorbrewer values/11/.code={
			\definecolor{colorbrewer1}{RGB}{84,48,5}
			\definecolor{colorbrewer2}{RGB}{140,81,10}
			\definecolor{colorbrewer3}{RGB}{191,129,45}
			\definecolor{colorbrewer4}{RGB}{223,194,125}
			\definecolor{colorbrewer5}{RGB}{246,232,195}
			\definecolor{colorbrewer6}{RGB}{245,245,245}
			\definecolor{colorbrewer7}{RGB}{199,234,229}
			\definecolor{colorbrewer8}{RGB}{128,205,193}
			\definecolor{colorbrewer9}{RGB}{53,151,143}
			\definecolor{colorbrewer10}{RGB}{1,102,94}
			\definecolor{colorbrewer11}{RGB}{0,60,48}
		}
	},
	colorbrewer scheme/BuGn/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{229,245,249}
			\definecolor{colorbrewer2}{RGB}{153,216,201}
			\definecolor{colorbrewer3}{RGB}{44,162,95}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{237,248,251}
			\definecolor{colorbrewer2}{RGB}{178,226,226}
			\definecolor{colorbrewer3}{RGB}{102,194,164}
			\definecolor{colorbrewer4}{RGB}{35,139,69}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{237,248,251}
			\definecolor{colorbrewer2}{RGB}{178,226,226}
			\definecolor{colorbrewer3}{RGB}{102,194,164}
			\definecolor{colorbrewer4}{RGB}{44,162,95}
			\definecolor{colorbrewer5}{RGB}{0,109,44}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{237,248,251}
			\definecolor{colorbrewer2}{RGB}{204,236,230}
			\definecolor{colorbrewer3}{RGB}{153,216,201}
			\definecolor{colorbrewer4}{RGB}{102,194,164}
			\definecolor{colorbrewer5}{RGB}{44,162,95}
			\definecolor{colorbrewer6}{RGB}{0,109,44}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{237,248,251}
			\definecolor{colorbrewer2}{RGB}{204,236,230}
			\definecolor{colorbrewer3}{RGB}{153,216,201}
			\definecolor{colorbrewer4}{RGB}{102,194,164}
			\definecolor{colorbrewer5}{RGB}{65,174,118}
			\definecolor{colorbrewer6}{RGB}{35,139,69}
			\definecolor{colorbrewer7}{RGB}{0,88,36}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{247,252,253}
			\definecolor{colorbrewer2}{RGB}{229,245,249}
			\definecolor{colorbrewer3}{RGB}{204,236,230}
			\definecolor{colorbrewer4}{RGB}{153,216,201}
			\definecolor{colorbrewer5}{RGB}{102,194,164}
			\definecolor{colorbrewer6}{RGB}{65,174,118}
			\definecolor{colorbrewer7}{RGB}{35,139,69}
			\definecolor{colorbrewer8}{RGB}{0,88,36}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{247,252,253}
			\definecolor{colorbrewer2}{RGB}{229,245,249}
			\definecolor{colorbrewer3}{RGB}{204,236,230}
			\definecolor{colorbrewer4}{RGB}{153,216,201}
			\definecolor{colorbrewer5}{RGB}{102,194,164}
			\definecolor{colorbrewer6}{RGB}{65,174,118}
			\definecolor{colorbrewer7}{RGB}{35,139,69}
			\definecolor{colorbrewer8}{RGB}{0,109,44}
			\definecolor{colorbrewer9}{RGB}{0,68,27}
		}
	},
	colorbrewer scheme/BuPu/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{224,236,244}
			\definecolor{colorbrewer2}{RGB}{158,188,218}
			\definecolor{colorbrewer3}{RGB}{136,86,167}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{237,248,251}
			\definecolor{colorbrewer2}{RGB}{179,205,227}
			\definecolor{colorbrewer3}{RGB}{140,150,198}
			\definecolor{colorbrewer4}{RGB}{136,65,157}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{237,248,251}
			\definecolor{colorbrewer2}{RGB}{179,205,227}
			\definecolor{colorbrewer3}{RGB}{140,150,198}
			\definecolor{colorbrewer4}{RGB}{136,86,167}
			\definecolor{colorbrewer5}{RGB}{129,15,124}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{237,248,251}
			\definecolor{colorbrewer2}{RGB}{191,211,230}
			\definecolor{colorbrewer3}{RGB}{158,188,218}
			\definecolor{colorbrewer4}{RGB}{140,150,198}
			\definecolor{colorbrewer5}{RGB}{136,86,167}
			\definecolor{colorbrewer6}{RGB}{129,15,124}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{237,248,251}
			\definecolor{colorbrewer2}{RGB}{191,211,230}
			\definecolor{colorbrewer3}{RGB}{158,188,218}
			\definecolor{colorbrewer4}{RGB}{140,150,198}
			\definecolor{colorbrewer5}{RGB}{140,107,177}
			\definecolor{colorbrewer6}{RGB}{136,65,157}
			\definecolor{colorbrewer7}{RGB}{110,1,107}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{247,252,253}
			\definecolor{colorbrewer2}{RGB}{224,236,244}
			\definecolor{colorbrewer3}{RGB}{191,211,230}
			\definecolor{colorbrewer4}{RGB}{158,188,218}
			\definecolor{colorbrewer5}{RGB}{140,150,198}
			\definecolor{colorbrewer6}{RGB}{140,107,177}
			\definecolor{colorbrewer7}{RGB}{136,65,157}
			\definecolor{colorbrewer8}{RGB}{110,1,107}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{247,252,253}
			\definecolor{colorbrewer2}{RGB}{224,236,244}
			\definecolor{colorbrewer3}{RGB}{191,211,230}
			\definecolor{colorbrewer4}{RGB}{158,188,218}
			\definecolor{colorbrewer5}{RGB}{140,150,198}
			\definecolor{colorbrewer6}{RGB}{140,107,177}
			\definecolor{colorbrewer7}{RGB}{136,65,157}
			\definecolor{colorbrewer8}{RGB}{129,15,124}
			\definecolor{colorbrewer9}{RGB}{77,0,75}
		}
	},
	colorbrewer scheme/Dark2/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{27,158,119}
			\definecolor{colorbrewer2}{RGB}{217,95,2}
			\definecolor{colorbrewer3}{RGB}{117,112,179}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{27,158,119}
			\definecolor{colorbrewer2}{RGB}{217,95,2}
			\definecolor{colorbrewer3}{RGB}{117,112,179}
			\definecolor{colorbrewer4}{RGB}{231,41,138}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{27,158,119}
			\definecolor{colorbrewer2}{RGB}{217,95,2}
			\definecolor{colorbrewer3}{RGB}{117,112,179}
			\definecolor{colorbrewer4}{RGB}{231,41,138}
			\definecolor{colorbrewer5}{RGB}{102,166,30}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{27,158,119}
			\definecolor{colorbrewer2}{RGB}{217,95,2}
			\definecolor{colorbrewer3}{RGB}{117,112,179}
			\definecolor{colorbrewer4}{RGB}{231,41,138}
			\definecolor{colorbrewer5}{RGB}{102,166,30}
			\definecolor{colorbrewer6}{RGB}{230,171,2}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{27,158,119}
			\definecolor{colorbrewer2}{RGB}{217,95,2}
			\definecolor{colorbrewer3}{RGB}{117,112,179}
			\definecolor{colorbrewer4}{RGB}{231,41,138}
			\definecolor{colorbrewer5}{RGB}{102,166,30}
			\definecolor{colorbrewer6}{RGB}{230,171,2}
			\definecolor{colorbrewer7}{RGB}{166,118,29}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{27,158,119}
			\definecolor{colorbrewer2}{RGB}{217,95,2}
			\definecolor{colorbrewer3}{RGB}{117,112,179}
			\definecolor{colorbrewer4}{RGB}{231,41,138}
			\definecolor{colorbrewer5}{RGB}{102,166,30}
			\definecolor{colorbrewer6}{RGB}{230,171,2}
			\definecolor{colorbrewer7}{RGB}{166,118,29}
			\definecolor{colorbrewer8}{RGB}{102,102,102}
		}
	},
	colorbrewer scheme/GnBu/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{224,243,219}
			\definecolor{colorbrewer2}{RGB}{168,221,181}
			\definecolor{colorbrewer3}{RGB}{67,162,202}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{240,249,232}
			\definecolor{colorbrewer2}{RGB}{186,228,188}
			\definecolor{colorbrewer3}{RGB}{123,204,196}
			\definecolor{colorbrewer4}{RGB}{43,140,190}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{240,249,232}
			\definecolor{colorbrewer2}{RGB}{186,228,188}
			\definecolor{colorbrewer3}{RGB}{123,204,196}
			\definecolor{colorbrewer4}{RGB}{67,162,202}
			\definecolor{colorbrewer5}{RGB}{8,104,172}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{240,249,232}
			\definecolor{colorbrewer2}{RGB}{204,235,197}
			\definecolor{colorbrewer3}{RGB}{168,221,181}
			\definecolor{colorbrewer4}{RGB}{123,204,196}
			\definecolor{colorbrewer5}{RGB}{67,162,202}
			\definecolor{colorbrewer6}{RGB}{8,104,172}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{240,249,232}
			\definecolor{colorbrewer2}{RGB}{204,235,197}
			\definecolor{colorbrewer3}{RGB}{168,221,181}
			\definecolor{colorbrewer4}{RGB}{123,204,196}
			\definecolor{colorbrewer5}{RGB}{78,179,211}
			\definecolor{colorbrewer6}{RGB}{43,140,190}
			\definecolor{colorbrewer7}{RGB}{8,88,158}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{247,252,240}
			\definecolor{colorbrewer2}{RGB}{224,243,219}
			\definecolor{colorbrewer3}{RGB}{204,235,197}
			\definecolor{colorbrewer4}{RGB}{168,221,181}
			\definecolor{colorbrewer5}{RGB}{123,204,196}
			\definecolor{colorbrewer6}{RGB}{78,179,211}
			\definecolor{colorbrewer7}{RGB}{43,140,190}
			\definecolor{colorbrewer8}{RGB}{8,88,158}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{247,252,240}
			\definecolor{colorbrewer2}{RGB}{224,243,219}
			\definecolor{colorbrewer3}{RGB}{204,235,197}
			\definecolor{colorbrewer4}{RGB}{168,221,181}
			\definecolor{colorbrewer5}{RGB}{123,204,196}
			\definecolor{colorbrewer6}{RGB}{78,179,211}
			\definecolor{colorbrewer7}{RGB}{43,140,190}
			\definecolor{colorbrewer8}{RGB}{8,104,172}
			\definecolor{colorbrewer9}{RGB}{8,64,129}
		}
	},
	colorbrewer scheme/Greens/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{229,245,224}
			\definecolor{colorbrewer2}{RGB}{161,217,155}
			\definecolor{colorbrewer3}{RGB}{49,163,84}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{237,248,233}
			\definecolor{colorbrewer2}{RGB}{186,228,179}
			\definecolor{colorbrewer3}{RGB}{116,196,118}
			\definecolor{colorbrewer4}{RGB}{35,139,69}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{237,248,233}
			\definecolor{colorbrewer2}{RGB}{186,228,179}
			\definecolor{colorbrewer3}{RGB}{116,196,118}
			\definecolor{colorbrewer4}{RGB}{49,163,84}
			\definecolor{colorbrewer5}{RGB}{0,109,44}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{237,248,233}
			\definecolor{colorbrewer2}{RGB}{199,233,192}
			\definecolor{colorbrewer3}{RGB}{161,217,155}
			\definecolor{colorbrewer4}{RGB}{116,196,118}
			\definecolor{colorbrewer5}{RGB}{49,163,84}
			\definecolor{colorbrewer6}{RGB}{0,109,44}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{237,248,233}
			\definecolor{colorbrewer2}{RGB}{199,233,192}
			\definecolor{colorbrewer3}{RGB}{161,217,155}
			\definecolor{colorbrewer4}{RGB}{116,196,118}
			\definecolor{colorbrewer5}{RGB}{65,171,93}
			\definecolor{colorbrewer6}{RGB}{35,139,69}
			\definecolor{colorbrewer7}{RGB}{0,90,50}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{247,252,245}
			\definecolor{colorbrewer2}{RGB}{229,245,224}
			\definecolor{colorbrewer3}{RGB}{199,233,192}
			\definecolor{colorbrewer4}{RGB}{161,217,155}
			\definecolor{colorbrewer5}{RGB}{116,196,118}
			\definecolor{colorbrewer6}{RGB}{65,171,93}
			\definecolor{colorbrewer7}{RGB}{35,139,69}
			\definecolor{colorbrewer8}{RGB}{0,90,50}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{247,252,245}
			\definecolor{colorbrewer2}{RGB}{229,245,224}
			\definecolor{colorbrewer3}{RGB}{199,233,192}
			\definecolor{colorbrewer4}{RGB}{161,217,155}
			\definecolor{colorbrewer5}{RGB}{116,196,118}
			\definecolor{colorbrewer6}{RGB}{65,171,93}
			\definecolor{colorbrewer7}{RGB}{35,139,69}
			\definecolor{colorbrewer8}{RGB}{0,109,44}
			\definecolor{colorbrewer9}{RGB}{0,68,27}
		}
	},
	colorbrewer scheme/Greys/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{240,240,240}
			\definecolor{colorbrewer2}{RGB}{189,189,189}
			\definecolor{colorbrewer3}{RGB}{99,99,99}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{247,247,247}
			\definecolor{colorbrewer2}{RGB}{204,204,204}
			\definecolor{colorbrewer3}{RGB}{150,150,150}
			\definecolor{colorbrewer4}{RGB}{82,82,82}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{247,247,247}
			\definecolor{colorbrewer2}{RGB}{204,204,204}
			\definecolor{colorbrewer3}{RGB}{150,150,150}
			\definecolor{colorbrewer4}{RGB}{99,99,99}
			\definecolor{colorbrewer5}{RGB}{37,37,37}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{247,247,247}
			\definecolor{colorbrewer2}{RGB}{217,217,217}
			\definecolor{colorbrewer3}{RGB}{189,189,189}
			\definecolor{colorbrewer4}{RGB}{150,150,150}
			\definecolor{colorbrewer5}{RGB}{99,99,99}
			\definecolor{colorbrewer6}{RGB}{37,37,37}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{247,247,247}
			\definecolor{colorbrewer2}{RGB}{217,217,217}
			\definecolor{colorbrewer3}{RGB}{189,189,189}
			\definecolor{colorbrewer4}{RGB}{150,150,150}
			\definecolor{colorbrewer5}{RGB}{115,115,115}
			\definecolor{colorbrewer6}{RGB}{82,82,82}
			\definecolor{colorbrewer7}{RGB}{37,37,37}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,255}
			\definecolor{colorbrewer2}{RGB}{240,240,240}
			\definecolor{colorbrewer3}{RGB}{217,217,217}
			\definecolor{colorbrewer4}{RGB}{189,189,189}
			\definecolor{colorbrewer5}{RGB}{150,150,150}
			\definecolor{colorbrewer6}{RGB}{115,115,115}
			\definecolor{colorbrewer7}{RGB}{82,82,82}
			\definecolor{colorbrewer8}{RGB}{37,37,37}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,255}
			\definecolor{colorbrewer2}{RGB}{240,240,240}
			\definecolor{colorbrewer3}{RGB}{217,217,217}
			\definecolor{colorbrewer4}{RGB}{189,189,189}
			\definecolor{colorbrewer5}{RGB}{150,150,150}
			\definecolor{colorbrewer6}{RGB}{115,115,115}
			\definecolor{colorbrewer7}{RGB}{82,82,82}
			\definecolor{colorbrewer8}{RGB}{37,37,37}
			\definecolor{colorbrewer9}{RGB}{0,0,0}
		}
	},
	colorbrewer scheme/Oranges/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{254,230,206}
			\definecolor{colorbrewer2}{RGB}{253,174,107}
			\definecolor{colorbrewer3}{RGB}{230,85,13}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{254,237,222}
			\definecolor{colorbrewer2}{RGB}{253,190,133}
			\definecolor{colorbrewer3}{RGB}{253,141,60}
			\definecolor{colorbrewer4}{RGB}{217,71,1}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{254,237,222}
			\definecolor{colorbrewer2}{RGB}{253,190,133}
			\definecolor{colorbrewer3}{RGB}{253,141,60}
			\definecolor{colorbrewer4}{RGB}{230,85,13}
			\definecolor{colorbrewer5}{RGB}{166,54,3}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{254,237,222}
			\definecolor{colorbrewer2}{RGB}{253,208,162}
			\definecolor{colorbrewer3}{RGB}{253,174,107}
			\definecolor{colorbrewer4}{RGB}{253,141,60}
			\definecolor{colorbrewer5}{RGB}{230,85,13}
			\definecolor{colorbrewer6}{RGB}{166,54,3}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{254,237,222}
			\definecolor{colorbrewer2}{RGB}{253,208,162}
			\definecolor{colorbrewer3}{RGB}{253,174,107}
			\definecolor{colorbrewer4}{RGB}{253,141,60}
			\definecolor{colorbrewer5}{RGB}{241,105,19}
			\definecolor{colorbrewer6}{RGB}{217,72,1}
			\definecolor{colorbrewer7}{RGB}{140,45,4}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{255,245,235}
			\definecolor{colorbrewer2}{RGB}{254,230,206}
			\definecolor{colorbrewer3}{RGB}{253,208,162}
			\definecolor{colorbrewer4}{RGB}{253,174,107}
			\definecolor{colorbrewer5}{RGB}{253,141,60}
			\definecolor{colorbrewer6}{RGB}{241,105,19}
			\definecolor{colorbrewer7}{RGB}{217,72,1}
			\definecolor{colorbrewer8}{RGB}{140,45,4}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{255,245,235}
			\definecolor{colorbrewer2}{RGB}{254,230,206}
			\definecolor{colorbrewer3}{RGB}{253,208,162}
			\definecolor{colorbrewer4}{RGB}{253,174,107}
			\definecolor{colorbrewer5}{RGB}{253,141,60}
			\definecolor{colorbrewer6}{RGB}{241,105,19}
			\definecolor{colorbrewer7}{RGB}{217,72,1}
			\definecolor{colorbrewer8}{RGB}{166,54,3}
			\definecolor{colorbrewer9}{RGB}{127,39,4}
		}
	},
	colorbrewer scheme/OrRd/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{254,232,200}
			\definecolor{colorbrewer2}{RGB}{253,187,132}
			\definecolor{colorbrewer3}{RGB}{227,74,51}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{254,240,217}
			\definecolor{colorbrewer2}{RGB}{253,204,138}
			\definecolor{colorbrewer3}{RGB}{252,141,89}
			\definecolor{colorbrewer4}{RGB}{215,48,31}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{254,240,217}
			\definecolor{colorbrewer2}{RGB}{253,204,138}
			\definecolor{colorbrewer3}{RGB}{252,141,89}
			\definecolor{colorbrewer4}{RGB}{227,74,51}
			\definecolor{colorbrewer5}{RGB}{179,0,0}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{254,240,217}
			\definecolor{colorbrewer2}{RGB}{253,212,158}
			\definecolor{colorbrewer3}{RGB}{253,187,132}
			\definecolor{colorbrewer4}{RGB}{252,141,89}
			\definecolor{colorbrewer5}{RGB}{227,74,51}
			\definecolor{colorbrewer6}{RGB}{179,0,0}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{254,240,217}
			\definecolor{colorbrewer2}{RGB}{253,212,158}
			\definecolor{colorbrewer3}{RGB}{253,187,132}
			\definecolor{colorbrewer4}{RGB}{252,141,89}
			\definecolor{colorbrewer5}{RGB}{239,101,72}
			\definecolor{colorbrewer6}{RGB}{215,48,31}
			\definecolor{colorbrewer7}{RGB}{153,0,0}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{255,247,236}
			\definecolor{colorbrewer2}{RGB}{254,232,200}
			\definecolor{colorbrewer3}{RGB}{253,212,158}
			\definecolor{colorbrewer4}{RGB}{253,187,132}
			\definecolor{colorbrewer5}{RGB}{252,141,89}
			\definecolor{colorbrewer6}{RGB}{239,101,72}
			\definecolor{colorbrewer7}{RGB}{215,48,31}
			\definecolor{colorbrewer8}{RGB}{153,0,0}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{255,247,236}
			\definecolor{colorbrewer2}{RGB}{254,232,200}
			\definecolor{colorbrewer3}{RGB}{253,212,158}
			\definecolor{colorbrewer4}{RGB}{253,187,132}
			\definecolor{colorbrewer5}{RGB}{252,141,89}
			\definecolor{colorbrewer6}{RGB}{239,101,72}
			\definecolor{colorbrewer7}{RGB}{215,48,31}
			\definecolor{colorbrewer8}{RGB}{179,0,0}
			\definecolor{colorbrewer9}{RGB}{127,0,0}
		}
	},
	colorbrewer scheme/Paired/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{166,206,227}
			\definecolor{colorbrewer2}{RGB}{31,120,180}
			\definecolor{colorbrewer3}{RGB}{178,223,138}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{166,206,227}
			\definecolor{colorbrewer2}{RGB}{31,120,180}
			\definecolor{colorbrewer3}{RGB}{178,223,138}
			\definecolor{colorbrewer4}{RGB}{51,160,44}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{166,206,227}
			\definecolor{colorbrewer2}{RGB}{31,120,180}
			\definecolor{colorbrewer3}{RGB}{178,223,138}
			\definecolor{colorbrewer4}{RGB}{51,160,44}
			\definecolor{colorbrewer5}{RGB}{251,154,153}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{166,206,227}
			\definecolor{colorbrewer2}{RGB}{31,120,180}
			\definecolor{colorbrewer3}{RGB}{178,223,138}
			\definecolor{colorbrewer4}{RGB}{51,160,44}
			\definecolor{colorbrewer5}{RGB}{251,154,153}
			\definecolor{colorbrewer6}{RGB}{227,26,28}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{166,206,227}
			\definecolor{colorbrewer2}{RGB}{31,120,180}
			\definecolor{colorbrewer3}{RGB}{178,223,138}
			\definecolor{colorbrewer4}{RGB}{51,160,44}
			\definecolor{colorbrewer5}{RGB}{251,154,153}
			\definecolor{colorbrewer6}{RGB}{227,26,28}
			\definecolor{colorbrewer7}{RGB}{253,191,111}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{166,206,227}
			\definecolor{colorbrewer2}{RGB}{31,120,180}
			\definecolor{colorbrewer3}{RGB}{178,223,138}
			\definecolor{colorbrewer4}{RGB}{51,160,44}
			\definecolor{colorbrewer5}{RGB}{251,154,153}
			\definecolor{colorbrewer6}{RGB}{227,26,28}
			\definecolor{colorbrewer7}{RGB}{253,191,111}
			\definecolor{colorbrewer8}{RGB}{255,127,0}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{166,206,227}
			\definecolor{colorbrewer2}{RGB}{31,120,180}
			\definecolor{colorbrewer3}{RGB}{178,223,138}
			\definecolor{colorbrewer4}{RGB}{51,160,44}
			\definecolor{colorbrewer5}{RGB}{251,154,153}
			\definecolor{colorbrewer6}{RGB}{227,26,28}
			\definecolor{colorbrewer7}{RGB}{253,191,111}
			\definecolor{colorbrewer8}{RGB}{255,127,0}
			\definecolor{colorbrewer9}{RGB}{202,178,214}
		},
		colorbrewer values/10/.code={
			\definecolor{colorbrewer1}{RGB}{166,206,227}
			\definecolor{colorbrewer2}{RGB}{31,120,180}
			\definecolor{colorbrewer3}{RGB}{178,223,138}
			\definecolor{colorbrewer4}{RGB}{51,160,44}
			\definecolor{colorbrewer5}{RGB}{251,154,153}
			\definecolor{colorbrewer6}{RGB}{227,26,28}
			\definecolor{colorbrewer7}{RGB}{253,191,111}
			\definecolor{colorbrewer8}{RGB}{255,127,0}
			\definecolor{colorbrewer9}{RGB}{202,178,214}
			\definecolor{colorbrewer10}{RGB}{106,61,154}
		},
		colorbrewer values/11/.code={
			\definecolor{colorbrewer1}{RGB}{166,206,227}
			\definecolor{colorbrewer2}{RGB}{31,120,180}
			\definecolor{colorbrewer3}{RGB}{178,223,138}
			\definecolor{colorbrewer4}{RGB}{51,160,44}
			\definecolor{colorbrewer5}{RGB}{251,154,153}
			\definecolor{colorbrewer6}{RGB}{227,26,28}
			\definecolor{colorbrewer7}{RGB}{253,191,111}
			\definecolor{colorbrewer8}{RGB}{255,127,0}
			\definecolor{colorbrewer9}{RGB}{202,178,214}
			\definecolor{colorbrewer10}{RGB}{106,61,154}
			\definecolor{colorbrewer11}{RGB}{255,255,153}
		},
		colorbrewer values/12/.code={
			\definecolor{colorbrewer1}{RGB}{166,206,227}
			\definecolor{colorbrewer2}{RGB}{31,120,180}
			\definecolor{colorbrewer3}{RGB}{178,223,138}
			\definecolor{colorbrewer4}{RGB}{51,160,44}
			\definecolor{colorbrewer5}{RGB}{251,154,153}
			\definecolor{colorbrewer6}{RGB}{227,26,28}
			\definecolor{colorbrewer7}{RGB}{253,191,111}
			\definecolor{colorbrewer8}{RGB}{255,127,0}
			\definecolor{colorbrewer9}{RGB}{202,178,214}
			\definecolor{colorbrewer10}{RGB}{106,61,154}
			\definecolor{colorbrewer11}{RGB}{255,255,153}
			\definecolor{colorbrewer12}{RGB}{177,89,40}
		}
	},
	colorbrewer scheme/Pastel1/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{251,180,174}
			\definecolor{colorbrewer2}{RGB}{179,205,227}
			\definecolor{colorbrewer3}{RGB}{204,235,197}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{251,180,174}
			\definecolor{colorbrewer2}{RGB}{179,205,227}
			\definecolor{colorbrewer3}{RGB}{204,235,197}
			\definecolor{colorbrewer4}{RGB}{222,203,228}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{251,180,174}
			\definecolor{colorbrewer2}{RGB}{179,205,227}
			\definecolor{colorbrewer3}{RGB}{204,235,197}
			\definecolor{colorbrewer4}{RGB}{222,203,228}
			\definecolor{colorbrewer5}{RGB}{254,217,166}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{251,180,174}
			\definecolor{colorbrewer2}{RGB}{179,205,227}
			\definecolor{colorbrewer3}{RGB}{204,235,197}
			\definecolor{colorbrewer4}{RGB}{222,203,228}
			\definecolor{colorbrewer5}{RGB}{254,217,166}
			\definecolor{colorbrewer6}{RGB}{255,255,204}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{251,180,174}
			\definecolor{colorbrewer2}{RGB}{179,205,227}
			\definecolor{colorbrewer3}{RGB}{204,235,197}
			\definecolor{colorbrewer4}{RGB}{222,203,228}
			\definecolor{colorbrewer5}{RGB}{254,217,166}
			\definecolor{colorbrewer6}{RGB}{255,255,204}
			\definecolor{colorbrewer7}{RGB}{229,216,189}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{251,180,174}
			\definecolor{colorbrewer2}{RGB}{179,205,227}
			\definecolor{colorbrewer3}{RGB}{204,235,197}
			\definecolor{colorbrewer4}{RGB}{222,203,228}
			\definecolor{colorbrewer5}{RGB}{254,217,166}
			\definecolor{colorbrewer6}{RGB}{255,255,204}
			\definecolor{colorbrewer7}{RGB}{229,216,189}
			\definecolor{colorbrewer8}{RGB}{253,218,236}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{251,180,174}
			\definecolor{colorbrewer2}{RGB}{179,205,227}
			\definecolor{colorbrewer3}{RGB}{204,235,197}
			\definecolor{colorbrewer4}{RGB}{222,203,228}
			\definecolor{colorbrewer5}{RGB}{254,217,166}
			\definecolor{colorbrewer6}{RGB}{255,255,204}
			\definecolor{colorbrewer7}{RGB}{229,216,189}
			\definecolor{colorbrewer8}{RGB}{253,218,236}
			\definecolor{colorbrewer9}{RGB}{242,242,242}
		}
	},
	colorbrewer scheme/Pastel2/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{179,226,205}
			\definecolor{colorbrewer2}{RGB}{253,205,172}
			\definecolor{colorbrewer3}{RGB}{203,213,232}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{179,226,205}
			\definecolor{colorbrewer2}{RGB}{253,205,172}
			\definecolor{colorbrewer3}{RGB}{203,213,232}
			\definecolor{colorbrewer4}{RGB}{244,202,228}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{179,226,205}
			\definecolor{colorbrewer2}{RGB}{253,205,172}
			\definecolor{colorbrewer3}{RGB}{203,213,232}
			\definecolor{colorbrewer4}{RGB}{244,202,228}
			\definecolor{colorbrewer5}{RGB}{230,245,201}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{179,226,205}
			\definecolor{colorbrewer2}{RGB}{253,205,172}
			\definecolor{colorbrewer3}{RGB}{203,213,232}
			\definecolor{colorbrewer4}{RGB}{244,202,228}
			\definecolor{colorbrewer5}{RGB}{230,245,201}
			\definecolor{colorbrewer6}{RGB}{255,242,174}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{179,226,205}
			\definecolor{colorbrewer2}{RGB}{253,205,172}
			\definecolor{colorbrewer3}{RGB}{203,213,232}
			\definecolor{colorbrewer4}{RGB}{244,202,228}
			\definecolor{colorbrewer5}{RGB}{230,245,201}
			\definecolor{colorbrewer6}{RGB}{255,242,174}
			\definecolor{colorbrewer7}{RGB}{241,226,204}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{179,226,205}
			\definecolor{colorbrewer2}{RGB}{253,205,172}
			\definecolor{colorbrewer3}{RGB}{203,213,232}
			\definecolor{colorbrewer4}{RGB}{244,202,228}
			\definecolor{colorbrewer5}{RGB}{230,245,201}
			\definecolor{colorbrewer6}{RGB}{255,242,174}
			\definecolor{colorbrewer7}{RGB}{241,226,204}
			\definecolor{colorbrewer8}{RGB}{204,204,204}
		}
	},
	colorbrewer scheme/PiYG/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{233,163,201}
			\definecolor{colorbrewer2}{RGB}{247,247,247}
			\definecolor{colorbrewer3}{RGB}{161,215,106}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{208,28,139}
			\definecolor{colorbrewer2}{RGB}{241,182,218}
			\definecolor{colorbrewer3}{RGB}{184,225,134}
			\definecolor{colorbrewer4}{RGB}{77,172,38}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{208,28,139}
			\definecolor{colorbrewer2}{RGB}{241,182,218}
			\definecolor{colorbrewer3}{RGB}{247,247,247}
			\definecolor{colorbrewer4}{RGB}{184,225,134}
			\definecolor{colorbrewer5}{RGB}{77,172,38}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{197,27,125}
			\definecolor{colorbrewer2}{RGB}{233,163,201}
			\definecolor{colorbrewer3}{RGB}{253,224,239}
			\definecolor{colorbrewer4}{RGB}{230,245,208}
			\definecolor{colorbrewer5}{RGB}{161,215,106}
			\definecolor{colorbrewer6}{RGB}{77,146,33}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{197,27,125}
			\definecolor{colorbrewer2}{RGB}{233,163,201}
			\definecolor{colorbrewer3}{RGB}{253,224,239}
			\definecolor{colorbrewer4}{RGB}{247,247,247}
			\definecolor{colorbrewer5}{RGB}{230,245,208}
			\definecolor{colorbrewer6}{RGB}{161,215,106}
			\definecolor{colorbrewer7}{RGB}{77,146,33}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{197,27,125}
			\definecolor{colorbrewer2}{RGB}{222,119,174}
			\definecolor{colorbrewer3}{RGB}{241,182,218}
			\definecolor{colorbrewer4}{RGB}{253,224,239}
			\definecolor{colorbrewer5}{RGB}{230,245,208}
			\definecolor{colorbrewer6}{RGB}{184,225,134}
			\definecolor{colorbrewer7}{RGB}{127,188,65}
			\definecolor{colorbrewer8}{RGB}{77,146,33}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{197,27,125}
			\definecolor{colorbrewer2}{RGB}{222,119,174}
			\definecolor{colorbrewer3}{RGB}{241,182,218}
			\definecolor{colorbrewer4}{RGB}{253,224,239}
			\definecolor{colorbrewer5}{RGB}{247,247,247}
			\definecolor{colorbrewer6}{RGB}{230,245,208}
			\definecolor{colorbrewer7}{RGB}{184,225,134}
			\definecolor{colorbrewer8}{RGB}{127,188,65}
			\definecolor{colorbrewer9}{RGB}{77,146,33}
		},
		colorbrewer values/10/.code={
			\definecolor{colorbrewer1}{RGB}{142,1,82}
			\definecolor{colorbrewer2}{RGB}{197,27,125}
			\definecolor{colorbrewer3}{RGB}{222,119,174}
			\definecolor{colorbrewer4}{RGB}{241,182,218}
			\definecolor{colorbrewer5}{RGB}{253,224,239}
			\definecolor{colorbrewer6}{RGB}{230,245,208}
			\definecolor{colorbrewer7}{RGB}{184,225,134}
			\definecolor{colorbrewer8}{RGB}{127,188,65}
			\definecolor{colorbrewer9}{RGB}{77,146,33}
			\definecolor{colorbrewer10}{RGB}{39,100,25}
		},
		colorbrewer values/11/.code={
			\definecolor{colorbrewer1}{RGB}{142,1,82}
			\definecolor{colorbrewer2}{RGB}{197,27,125}
			\definecolor{colorbrewer3}{RGB}{222,119,174}
			\definecolor{colorbrewer4}{RGB}{241,182,218}
			\definecolor{colorbrewer5}{RGB}{253,224,239}
			\definecolor{colorbrewer6}{RGB}{247,247,247}
			\definecolor{colorbrewer7}{RGB}{230,245,208}
			\definecolor{colorbrewer8}{RGB}{184,225,134}
			\definecolor{colorbrewer9}{RGB}{127,188,65}
			\definecolor{colorbrewer10}{RGB}{77,146,33}
			\definecolor{colorbrewer11}{RGB}{39,100,25}
		}
	},
	colorbrewer scheme/PRGn/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{175,141,195}
			\definecolor{colorbrewer2}{RGB}{247,247,247}
			\definecolor{colorbrewer3}{RGB}{127,191,123}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{123,50,148}
			\definecolor{colorbrewer2}{RGB}{194,165,207}
			\definecolor{colorbrewer3}{RGB}{166,219,160}
			\definecolor{colorbrewer4}{RGB}{0,136,55}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{123,50,148}
			\definecolor{colorbrewer2}{RGB}{194,165,207}
			\definecolor{colorbrewer3}{RGB}{247,247,247}
			\definecolor{colorbrewer4}{RGB}{166,219,160}
			\definecolor{colorbrewer5}{RGB}{0,136,55}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{118,42,131}
			\definecolor{colorbrewer2}{RGB}{175,141,195}
			\definecolor{colorbrewer3}{RGB}{231,212,232}
			\definecolor{colorbrewer4}{RGB}{217,240,211}
			\definecolor{colorbrewer5}{RGB}{127,191,123}
			\definecolor{colorbrewer6}{RGB}{27,120,55}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{118,42,131}
			\definecolor{colorbrewer2}{RGB}{175,141,195}
			\definecolor{colorbrewer3}{RGB}{231,212,232}
			\definecolor{colorbrewer4}{RGB}{247,247,247}
			\definecolor{colorbrewer5}{RGB}{217,240,211}
			\definecolor{colorbrewer6}{RGB}{127,191,123}
			\definecolor{colorbrewer7}{RGB}{27,120,55}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{118,42,131}
			\definecolor{colorbrewer2}{RGB}{153,112,171}
			\definecolor{colorbrewer3}{RGB}{194,165,207}
			\definecolor{colorbrewer4}{RGB}{231,212,232}
			\definecolor{colorbrewer5}{RGB}{217,240,211}
			\definecolor{colorbrewer6}{RGB}{166,219,160}
			\definecolor{colorbrewer7}{RGB}{90,174,97}
			\definecolor{colorbrewer8}{RGB}{27,120,55}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{118,42,131}
			\definecolor{colorbrewer2}{RGB}{153,112,171}
			\definecolor{colorbrewer3}{RGB}{194,165,207}
			\definecolor{colorbrewer4}{RGB}{231,212,232}
			\definecolor{colorbrewer5}{RGB}{247,247,247}
			\definecolor{colorbrewer6}{RGB}{217,240,211}
			\definecolor{colorbrewer7}{RGB}{166,219,160}
			\definecolor{colorbrewer8}{RGB}{90,174,97}
			\definecolor{colorbrewer9}{RGB}{27,120,55}
		},
		colorbrewer values/10/.code={
			\definecolor{colorbrewer1}{RGB}{64,0,75}
			\definecolor{colorbrewer2}{RGB}{118,42,131}
			\definecolor{colorbrewer3}{RGB}{153,112,171}
			\definecolor{colorbrewer4}{RGB}{194,165,207}
			\definecolor{colorbrewer5}{RGB}{231,212,232}
			\definecolor{colorbrewer6}{RGB}{217,240,211}
			\definecolor{colorbrewer7}{RGB}{166,219,160}
			\definecolor{colorbrewer8}{RGB}{90,174,97}
			\definecolor{colorbrewer9}{RGB}{27,120,55}
			\definecolor{colorbrewer10}{RGB}{0,68,27}
		},
		colorbrewer values/11/.code={
			\definecolor{colorbrewer1}{RGB}{64,0,75}
			\definecolor{colorbrewer2}{RGB}{118,42,131}
			\definecolor{colorbrewer3}{RGB}{153,112,171}
			\definecolor{colorbrewer4}{RGB}{194,165,207}
			\definecolor{colorbrewer5}{RGB}{231,212,232}
			\definecolor{colorbrewer6}{RGB}{247,247,247}
			\definecolor{colorbrewer7}{RGB}{217,240,211}
			\definecolor{colorbrewer8}{RGB}{166,219,160}
			\definecolor{colorbrewer9}{RGB}{90,174,97}
			\definecolor{colorbrewer10}{RGB}{27,120,55}
			\definecolor{colorbrewer11}{RGB}{0,68,27}
		}
	},
	colorbrewer scheme/PuBu/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{236,231,242}
			\definecolor{colorbrewer2}{RGB}{166,189,219}
			\definecolor{colorbrewer3}{RGB}{43,140,190}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{241,238,246}
			\definecolor{colorbrewer2}{RGB}{189,201,225}
			\definecolor{colorbrewer3}{RGB}{116,169,207}
			\definecolor{colorbrewer4}{RGB}{5,112,176}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{241,238,246}
			\definecolor{colorbrewer2}{RGB}{189,201,225}
			\definecolor{colorbrewer3}{RGB}{116,169,207}
			\definecolor{colorbrewer4}{RGB}{43,140,190}
			\definecolor{colorbrewer5}{RGB}{4,90,141}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{241,238,246}
			\definecolor{colorbrewer2}{RGB}{208,209,230}
			\definecolor{colorbrewer3}{RGB}{166,189,219}
			\definecolor{colorbrewer4}{RGB}{116,169,207}
			\definecolor{colorbrewer5}{RGB}{43,140,190}
			\definecolor{colorbrewer6}{RGB}{4,90,141}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{241,238,246}
			\definecolor{colorbrewer2}{RGB}{208,209,230}
			\definecolor{colorbrewer3}{RGB}{166,189,219}
			\definecolor{colorbrewer4}{RGB}{116,169,207}
			\definecolor{colorbrewer5}{RGB}{54,144,192}
			\definecolor{colorbrewer6}{RGB}{5,112,176}
			\definecolor{colorbrewer7}{RGB}{3,78,123}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{255,247,251}
			\definecolor{colorbrewer2}{RGB}{236,231,242}
			\definecolor{colorbrewer3}{RGB}{208,209,230}
			\definecolor{colorbrewer4}{RGB}{166,189,219}
			\definecolor{colorbrewer5}{RGB}{116,169,207}
			\definecolor{colorbrewer6}{RGB}{54,144,192}
			\definecolor{colorbrewer7}{RGB}{5,112,176}
			\definecolor{colorbrewer8}{RGB}{3,78,123}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{255,247,251}
			\definecolor{colorbrewer2}{RGB}{236,231,242}
			\definecolor{colorbrewer3}{RGB}{208,209,230}
			\definecolor{colorbrewer4}{RGB}{166,189,219}
			\definecolor{colorbrewer5}{RGB}{116,169,207}
			\definecolor{colorbrewer6}{RGB}{54,144,192}
			\definecolor{colorbrewer7}{RGB}{5,112,176}
			\definecolor{colorbrewer8}{RGB}{4,90,141}
			\definecolor{colorbrewer9}{RGB}{2,56,88}
		}
	},
	colorbrewer scheme/PuBuGn/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{236,226,240}
			\definecolor{colorbrewer2}{RGB}{166,189,219}
			\definecolor{colorbrewer3}{RGB}{28,144,153}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{246,239,247}
			\definecolor{colorbrewer2}{RGB}{189,201,225}
			\definecolor{colorbrewer3}{RGB}{103,169,207}
			\definecolor{colorbrewer4}{RGB}{2,129,138}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{246,239,247}
			\definecolor{colorbrewer2}{RGB}{189,201,225}
			\definecolor{colorbrewer3}{RGB}{103,169,207}
			\definecolor{colorbrewer4}{RGB}{28,144,153}
			\definecolor{colorbrewer5}{RGB}{1,108,89}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{246,239,247}
			\definecolor{colorbrewer2}{RGB}{208,209,230}
			\definecolor{colorbrewer3}{RGB}{166,189,219}
			\definecolor{colorbrewer4}{RGB}{103,169,207}
			\definecolor{colorbrewer5}{RGB}{28,144,153}
			\definecolor{colorbrewer6}{RGB}{1,108,89}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{246,239,247}
			\definecolor{colorbrewer2}{RGB}{208,209,230}
			\definecolor{colorbrewer3}{RGB}{166,189,219}
			\definecolor{colorbrewer4}{RGB}{103,169,207}
			\definecolor{colorbrewer5}{RGB}{54,144,192}
			\definecolor{colorbrewer6}{RGB}{2,129,138}
			\definecolor{colorbrewer7}{RGB}{1,100,80}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{255,247,251}
			\definecolor{colorbrewer2}{RGB}{236,226,240}
			\definecolor{colorbrewer3}{RGB}{208,209,230}
			\definecolor{colorbrewer4}{RGB}{166,189,219}
			\definecolor{colorbrewer5}{RGB}{103,169,207}
			\definecolor{colorbrewer6}{RGB}{54,144,192}
			\definecolor{colorbrewer7}{RGB}{2,129,138}
			\definecolor{colorbrewer8}{RGB}{1,100,80}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{255,247,251}
			\definecolor{colorbrewer2}{RGB}{236,226,240}
			\definecolor{colorbrewer3}{RGB}{208,209,230}
			\definecolor{colorbrewer4}{RGB}{166,189,219}
			\definecolor{colorbrewer5}{RGB}{103,169,207}
			\definecolor{colorbrewer6}{RGB}{54,144,192}
			\definecolor{colorbrewer7}{RGB}{2,129,138}
			\definecolor{colorbrewer8}{RGB}{1,108,89}
			\definecolor{colorbrewer9}{RGB}{1,70,54}
		}
	},
	colorbrewer scheme/PuOr/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{241,163,64}
			\definecolor{colorbrewer2}{RGB}{247,247,247}
			\definecolor{colorbrewer3}{RGB}{153,142,195}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{230,97,1}
			\definecolor{colorbrewer2}{RGB}{253,184,99}
			\definecolor{colorbrewer3}{RGB}{178,171,210}
			\definecolor{colorbrewer4}{RGB}{94,60,153}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{230,97,1}
			\definecolor{colorbrewer2}{RGB}{253,184,99}
			\definecolor{colorbrewer3}{RGB}{247,247,247}
			\definecolor{colorbrewer4}{RGB}{178,171,210}
			\definecolor{colorbrewer5}{RGB}{94,60,153}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{179,88,6}
			\definecolor{colorbrewer2}{RGB}{241,163,64}
			\definecolor{colorbrewer3}{RGB}{254,224,182}
			\definecolor{colorbrewer4}{RGB}{216,218,235}
			\definecolor{colorbrewer5}{RGB}{153,142,195}
			\definecolor{colorbrewer6}{RGB}{84,39,136}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{179,88,6}
			\definecolor{colorbrewer2}{RGB}{241,163,64}
			\definecolor{colorbrewer3}{RGB}{254,224,182}
			\definecolor{colorbrewer4}{RGB}{247,247,247}
			\definecolor{colorbrewer5}{RGB}{216,218,235}
			\definecolor{colorbrewer6}{RGB}{153,142,195}
			\definecolor{colorbrewer7}{RGB}{84,39,136}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{179,88,6}
			\definecolor{colorbrewer2}{RGB}{224,130,20}
			\definecolor{colorbrewer3}{RGB}{253,184,99}
			\definecolor{colorbrewer4}{RGB}{254,224,182}
			\definecolor{colorbrewer5}{RGB}{216,218,235}
			\definecolor{colorbrewer6}{RGB}{178,171,210}
			\definecolor{colorbrewer7}{RGB}{128,115,172}
			\definecolor{colorbrewer8}{RGB}{84,39,136}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{179,88,6}
			\definecolor{colorbrewer2}{RGB}{224,130,20}
			\definecolor{colorbrewer3}{RGB}{253,184,99}
			\definecolor{colorbrewer4}{RGB}{254,224,182}
			\definecolor{colorbrewer5}{RGB}{247,247,247}
			\definecolor{colorbrewer6}{RGB}{216,218,235}
			\definecolor{colorbrewer7}{RGB}{178,171,210}
			\definecolor{colorbrewer8}{RGB}{128,115,172}
			\definecolor{colorbrewer9}{RGB}{84,39,136}
		},
		colorbrewer values/10/.code={
			\definecolor{colorbrewer1}{RGB}{127,59,8}
			\definecolor{colorbrewer2}{RGB}{179,88,6}
			\definecolor{colorbrewer3}{RGB}{224,130,20}
			\definecolor{colorbrewer4}{RGB}{253,184,99}
			\definecolor{colorbrewer5}{RGB}{254,224,182}
			\definecolor{colorbrewer6}{RGB}{216,218,235}
			\definecolor{colorbrewer7}{RGB}{178,171,210}
			\definecolor{colorbrewer8}{RGB}{128,115,172}
			\definecolor{colorbrewer9}{RGB}{84,39,136}
			\definecolor{colorbrewer10}{RGB}{45,0,75}
		},
		colorbrewer values/11/.code={
			\definecolor{colorbrewer1}{RGB}{127,59,8}
			\definecolor{colorbrewer2}{RGB}{179,88,6}
			\definecolor{colorbrewer3}{RGB}{224,130,20}
			\definecolor{colorbrewer4}{RGB}{253,184,99}
			\definecolor{colorbrewer5}{RGB}{254,224,182}
			\definecolor{colorbrewer6}{RGB}{247,247,247}
			\definecolor{colorbrewer7}{RGB}{216,218,235}
			\definecolor{colorbrewer8}{RGB}{178,171,210}
			\definecolor{colorbrewer9}{RGB}{128,115,172}
			\definecolor{colorbrewer10}{RGB}{84,39,136}
			\definecolor{colorbrewer11}{RGB}{45,0,75}
		}
	},
	colorbrewer scheme/PuRd/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{231,225,239}
			\definecolor{colorbrewer2}{RGB}{201,148,199}
			\definecolor{colorbrewer3}{RGB}{221,28,119}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{241,238,246}
			\definecolor{colorbrewer2}{RGB}{215,181,216}
			\definecolor{colorbrewer3}{RGB}{223,101,176}
			\definecolor{colorbrewer4}{RGB}{206,18,86}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{241,238,246}
			\definecolor{colorbrewer2}{RGB}{215,181,216}
			\definecolor{colorbrewer3}{RGB}{223,101,176}
			\definecolor{colorbrewer4}{RGB}{221,28,119}
			\definecolor{colorbrewer5}{RGB}{152,0,67}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{241,238,246}
			\definecolor{colorbrewer2}{RGB}{212,185,218}
			\definecolor{colorbrewer3}{RGB}{201,148,199}
			\definecolor{colorbrewer4}{RGB}{223,101,176}
			\definecolor{colorbrewer5}{RGB}{221,28,119}
			\definecolor{colorbrewer6}{RGB}{152,0,67}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{241,238,246}
			\definecolor{colorbrewer2}{RGB}{212,185,218}
			\definecolor{colorbrewer3}{RGB}{201,148,199}
			\definecolor{colorbrewer4}{RGB}{223,101,176}
			\definecolor{colorbrewer5}{RGB}{231,41,138}
			\definecolor{colorbrewer6}{RGB}{206,18,86}
			\definecolor{colorbrewer7}{RGB}{145,0,63}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{247,244,249}
			\definecolor{colorbrewer2}{RGB}{231,225,239}
			\definecolor{colorbrewer3}{RGB}{212,185,218}
			\definecolor{colorbrewer4}{RGB}{201,148,199}
			\definecolor{colorbrewer5}{RGB}{223,101,176}
			\definecolor{colorbrewer6}{RGB}{231,41,138}
			\definecolor{colorbrewer7}{RGB}{206,18,86}
			\definecolor{colorbrewer8}{RGB}{145,0,63}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{247,244,249}
			\definecolor{colorbrewer2}{RGB}{231,225,239}
			\definecolor{colorbrewer3}{RGB}{212,185,218}
			\definecolor{colorbrewer4}{RGB}{201,148,199}
			\definecolor{colorbrewer5}{RGB}{223,101,176}
			\definecolor{colorbrewer6}{RGB}{231,41,138}
			\definecolor{colorbrewer7}{RGB}{206,18,86}
			\definecolor{colorbrewer8}{RGB}{152,0,67}
			\definecolor{colorbrewer9}{RGB}{103,0,31}
		}
	},
	colorbrewer scheme/Purples/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{239,237,245}
			\definecolor{colorbrewer2}{RGB}{188,189,220}
			\definecolor{colorbrewer3}{RGB}{117,107,177}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{242,240,247}
			\definecolor{colorbrewer2}{RGB}{203,201,226}
			\definecolor{colorbrewer3}{RGB}{158,154,200}
			\definecolor{colorbrewer4}{RGB}{106,81,163}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{242,240,247}
			\definecolor{colorbrewer2}{RGB}{203,201,226}
			\definecolor{colorbrewer3}{RGB}{158,154,200}
			\definecolor{colorbrewer4}{RGB}{117,107,177}
			\definecolor{colorbrewer5}{RGB}{84,39,143}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{242,240,247}
			\definecolor{colorbrewer2}{RGB}{218,218,235}
			\definecolor{colorbrewer3}{RGB}{188,189,220}
			\definecolor{colorbrewer4}{RGB}{158,154,200}
			\definecolor{colorbrewer5}{RGB}{117,107,177}
			\definecolor{colorbrewer6}{RGB}{84,39,143}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{242,240,247}
			\definecolor{colorbrewer2}{RGB}{218,218,235}
			\definecolor{colorbrewer3}{RGB}{188,189,220}
			\definecolor{colorbrewer4}{RGB}{158,154,200}
			\definecolor{colorbrewer5}{RGB}{128,125,186}
			\definecolor{colorbrewer6}{RGB}{106,81,163}
			\definecolor{colorbrewer7}{RGB}{74,20,134}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{252,251,253}
			\definecolor{colorbrewer2}{RGB}{239,237,245}
			\definecolor{colorbrewer3}{RGB}{218,218,235}
			\definecolor{colorbrewer4}{RGB}{188,189,220}
			\definecolor{colorbrewer5}{RGB}{158,154,200}
			\definecolor{colorbrewer6}{RGB}{128,125,186}
			\definecolor{colorbrewer7}{RGB}{106,81,163}
			\definecolor{colorbrewer8}{RGB}{74,20,134}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{252,251,253}
			\definecolor{colorbrewer2}{RGB}{239,237,245}
			\definecolor{colorbrewer3}{RGB}{218,218,235}
			\definecolor{colorbrewer4}{RGB}{188,189,220}
			\definecolor{colorbrewer5}{RGB}{158,154,200}
			\definecolor{colorbrewer6}{RGB}{128,125,186}
			\definecolor{colorbrewer7}{RGB}{106,81,163}
			\definecolor{colorbrewer8}{RGB}{84,39,143}
			\definecolor{colorbrewer9}{RGB}{63,0,125}
		}
	},
	colorbrewer scheme/RdBu/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{239,138,98}
			\definecolor{colorbrewer2}{RGB}{247,247,247}
			\definecolor{colorbrewer3}{RGB}{103,169,207}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{202,0,32}
			\definecolor{colorbrewer2}{RGB}{244,165,130}
			\definecolor{colorbrewer3}{RGB}{146,197,222}
			\definecolor{colorbrewer4}{RGB}{5,113,176}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{202,0,32}
			\definecolor{colorbrewer2}{RGB}{244,165,130}
			\definecolor{colorbrewer3}{RGB}{247,247,247}
			\definecolor{colorbrewer4}{RGB}{146,197,222}
			\definecolor{colorbrewer5}{RGB}{5,113,176}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{178,24,43}
			\definecolor{colorbrewer2}{RGB}{239,138,98}
			\definecolor{colorbrewer3}{RGB}{253,219,199}
			\definecolor{colorbrewer4}{RGB}{209,229,240}
			\definecolor{colorbrewer5}{RGB}{103,169,207}
			\definecolor{colorbrewer6}{RGB}{33,102,172}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{178,24,43}
			\definecolor{colorbrewer2}{RGB}{239,138,98}
			\definecolor{colorbrewer3}{RGB}{253,219,199}
			\definecolor{colorbrewer4}{RGB}{247,247,247}
			\definecolor{colorbrewer5}{RGB}{209,229,240}
			\definecolor{colorbrewer6}{RGB}{103,169,207}
			\definecolor{colorbrewer7}{RGB}{33,102,172}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{178,24,43}
			\definecolor{colorbrewer2}{RGB}{214,96,77}
			\definecolor{colorbrewer3}{RGB}{244,165,130}
			\definecolor{colorbrewer4}{RGB}{253,219,199}
			\definecolor{colorbrewer5}{RGB}{209,229,240}
			\definecolor{colorbrewer6}{RGB}{146,197,222}
			\definecolor{colorbrewer7}{RGB}{67,147,195}
			\definecolor{colorbrewer8}{RGB}{33,102,172}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{178,24,43}
			\definecolor{colorbrewer2}{RGB}{214,96,77}
			\definecolor{colorbrewer3}{RGB}{244,165,130}
			\definecolor{colorbrewer4}{RGB}{253,219,199}
			\definecolor{colorbrewer5}{RGB}{247,247,247}
			\definecolor{colorbrewer6}{RGB}{209,229,240}
			\definecolor{colorbrewer7}{RGB}{146,197,222}
			\definecolor{colorbrewer8}{RGB}{67,147,195}
			\definecolor{colorbrewer9}{RGB}{33,102,172}
		},
		colorbrewer values/10/.code={
			\definecolor{colorbrewer1}{RGB}{103,0,31}
			\definecolor{colorbrewer2}{RGB}{178,24,43}
			\definecolor{colorbrewer3}{RGB}{214,96,77}
			\definecolor{colorbrewer4}{RGB}{244,165,130}
			\definecolor{colorbrewer5}{RGB}{253,219,199}
			\definecolor{colorbrewer6}{RGB}{209,229,240}
			\definecolor{colorbrewer7}{RGB}{146,197,222}
			\definecolor{colorbrewer8}{RGB}{67,147,195}
			\definecolor{colorbrewer9}{RGB}{33,102,172}
			\definecolor{colorbrewer10}{RGB}{5,48,97}
		},
		colorbrewer values/11/.code={
			\definecolor{colorbrewer1}{RGB}{103,0,31}
			\definecolor{colorbrewer2}{RGB}{178,24,43}
			\definecolor{colorbrewer3}{RGB}{214,96,77}
			\definecolor{colorbrewer4}{RGB}{244,165,130}
			\definecolor{colorbrewer5}{RGB}{253,219,199}
			\definecolor{colorbrewer6}{RGB}{247,247,247}
			\definecolor{colorbrewer7}{RGB}{209,229,240}
			\definecolor{colorbrewer8}{RGB}{146,197,222}
			\definecolor{colorbrewer9}{RGB}{67,147,195}
			\definecolor{colorbrewer10}{RGB}{33,102,172}
			\definecolor{colorbrewer11}{RGB}{5,48,97}
		}
	},
	colorbrewer scheme/RdGy/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{239,138,98}
			\definecolor{colorbrewer2}{RGB}{255,255,255}
			\definecolor{colorbrewer3}{RGB}{153,153,153}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{202,0,32}
			\definecolor{colorbrewer2}{RGB}{244,165,130}
			\definecolor{colorbrewer3}{RGB}{186,186,186}
			\definecolor{colorbrewer4}{RGB}{64,64,64}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{202,0,32}
			\definecolor{colorbrewer2}{RGB}{244,165,130}
			\definecolor{colorbrewer3}{RGB}{255,255,255}
			\definecolor{colorbrewer4}{RGB}{186,186,186}
			\definecolor{colorbrewer5}{RGB}{64,64,64}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{178,24,43}
			\definecolor{colorbrewer2}{RGB}{239,138,98}
			\definecolor{colorbrewer3}{RGB}{253,219,199}
			\definecolor{colorbrewer4}{RGB}{224,224,224}
			\definecolor{colorbrewer5}{RGB}{153,153,153}
			\definecolor{colorbrewer6}{RGB}{77,77,77}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{178,24,43}
			\definecolor{colorbrewer2}{RGB}{239,138,98}
			\definecolor{colorbrewer3}{RGB}{253,219,199}
			\definecolor{colorbrewer4}{RGB}{255,255,255}
			\definecolor{colorbrewer5}{RGB}{224,224,224}
			\definecolor{colorbrewer6}{RGB}{153,153,153}
			\definecolor{colorbrewer7}{RGB}{77,77,77}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{178,24,43}
			\definecolor{colorbrewer2}{RGB}{214,96,77}
			\definecolor{colorbrewer3}{RGB}{244,165,130}
			\definecolor{colorbrewer4}{RGB}{253,219,199}
			\definecolor{colorbrewer5}{RGB}{224,224,224}
			\definecolor{colorbrewer6}{RGB}{186,186,186}
			\definecolor{colorbrewer7}{RGB}{135,135,135}
			\definecolor{colorbrewer8}{RGB}{77,77,77}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{178,24,43}
			\definecolor{colorbrewer2}{RGB}{214,96,77}
			\definecolor{colorbrewer3}{RGB}{244,165,130}
			\definecolor{colorbrewer4}{RGB}{253,219,199}
			\definecolor{colorbrewer5}{RGB}{255,255,255}
			\definecolor{colorbrewer6}{RGB}{224,224,224}
			\definecolor{colorbrewer7}{RGB}{186,186,186}
			\definecolor{colorbrewer8}{RGB}{135,135,135}
			\definecolor{colorbrewer9}{RGB}{77,77,77}
		},
		colorbrewer values/10/.code={
			\definecolor{colorbrewer1}{RGB}{103,0,31}
			\definecolor{colorbrewer2}{RGB}{178,24,43}
			\definecolor{colorbrewer3}{RGB}{214,96,77}
			\definecolor{colorbrewer4}{RGB}{244,165,130}
			\definecolor{colorbrewer5}{RGB}{253,219,199}
			\definecolor{colorbrewer6}{RGB}{224,224,224}
			\definecolor{colorbrewer7}{RGB}{186,186,186}
			\definecolor{colorbrewer8}{RGB}{135,135,135}
			\definecolor{colorbrewer9}{RGB}{77,77,77}
			\definecolor{colorbrewer10}{RGB}{26,26,26}
		},
		colorbrewer values/11/.code={
			\definecolor{colorbrewer1}{RGB}{103,0,31}
			\definecolor{colorbrewer2}{RGB}{178,24,43}
			\definecolor{colorbrewer3}{RGB}{214,96,77}
			\definecolor{colorbrewer4}{RGB}{244,165,130}
			\definecolor{colorbrewer5}{RGB}{253,219,199}
			\definecolor{colorbrewer6}{RGB}{255,255,255}
			\definecolor{colorbrewer7}{RGB}{224,224,224}
			\definecolor{colorbrewer8}{RGB}{186,186,186}
			\definecolor{colorbrewer9}{RGB}{135,135,135}
			\definecolor{colorbrewer10}{RGB}{77,77,77}
			\definecolor{colorbrewer11}{RGB}{26,26,26}
		}
	},
	colorbrewer scheme/RdPu/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{253,224,221}
			\definecolor{colorbrewer2}{RGB}{250,159,181}
			\definecolor{colorbrewer3}{RGB}{197,27,138}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{254,235,226}
			\definecolor{colorbrewer2}{RGB}{251,180,185}
			\definecolor{colorbrewer3}{RGB}{247,104,161}
			\definecolor{colorbrewer4}{RGB}{174,1,126}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{254,235,226}
			\definecolor{colorbrewer2}{RGB}{251,180,185}
			\definecolor{colorbrewer3}{RGB}{247,104,161}
			\definecolor{colorbrewer4}{RGB}{197,27,138}
			\definecolor{colorbrewer5}{RGB}{122,1,119}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{254,235,226}
			\definecolor{colorbrewer2}{RGB}{252,197,192}
			\definecolor{colorbrewer3}{RGB}{250,159,181}
			\definecolor{colorbrewer4}{RGB}{247,104,161}
			\definecolor{colorbrewer5}{RGB}{197,27,138}
			\definecolor{colorbrewer6}{RGB}{122,1,119}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{254,235,226}
			\definecolor{colorbrewer2}{RGB}{252,197,192}
			\definecolor{colorbrewer3}{RGB}{250,159,181}
			\definecolor{colorbrewer4}{RGB}{247,104,161}
			\definecolor{colorbrewer5}{RGB}{221,52,151}
			\definecolor{colorbrewer6}{RGB}{174,1,126}
			\definecolor{colorbrewer7}{RGB}{122,1,119}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{255,247,243}
			\definecolor{colorbrewer2}{RGB}{253,224,221}
			\definecolor{colorbrewer3}{RGB}{252,197,192}
			\definecolor{colorbrewer4}{RGB}{250,159,181}
			\definecolor{colorbrewer5}{RGB}{247,104,161}
			\definecolor{colorbrewer6}{RGB}{221,52,151}
			\definecolor{colorbrewer7}{RGB}{174,1,126}
			\definecolor{colorbrewer8}{RGB}{122,1,119}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{255,247,243}
			\definecolor{colorbrewer2}{RGB}{253,224,221}
			\definecolor{colorbrewer3}{RGB}{252,197,192}
			\definecolor{colorbrewer4}{RGB}{250,159,181}
			\definecolor{colorbrewer5}{RGB}{247,104,161}
			\definecolor{colorbrewer6}{RGB}{221,52,151}
			\definecolor{colorbrewer7}{RGB}{174,1,126}
			\definecolor{colorbrewer8}{RGB}{122,1,119}
			\definecolor{colorbrewer9}{RGB}{73,0,106}
		}
	},
	colorbrewer scheme/Reds/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{254,224,210}
			\definecolor{colorbrewer2}{RGB}{252,146,114}
			\definecolor{colorbrewer3}{RGB}{222,45,38}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{254,229,217}
			\definecolor{colorbrewer2}{RGB}{252,174,145}
			\definecolor{colorbrewer3}{RGB}{251,106,74}
			\definecolor{colorbrewer4}{RGB}{203,24,29}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{254,229,217}
			\definecolor{colorbrewer2}{RGB}{252,174,145}
			\definecolor{colorbrewer3}{RGB}{251,106,74}
			\definecolor{colorbrewer4}{RGB}{222,45,38}
			\definecolor{colorbrewer5}{RGB}{165,15,21}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{254,229,217}
			\definecolor{colorbrewer2}{RGB}{252,187,161}
			\definecolor{colorbrewer3}{RGB}{252,146,114}
			\definecolor{colorbrewer4}{RGB}{251,106,74}
			\definecolor{colorbrewer5}{RGB}{222,45,38}
			\definecolor{colorbrewer6}{RGB}{165,15,21}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{254,229,217}
			\definecolor{colorbrewer2}{RGB}{252,187,161}
			\definecolor{colorbrewer3}{RGB}{252,146,114}
			\definecolor{colorbrewer4}{RGB}{251,106,74}
			\definecolor{colorbrewer5}{RGB}{239,59,44}
			\definecolor{colorbrewer6}{RGB}{203,24,29}
			\definecolor{colorbrewer7}{RGB}{153,0,13}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{255,245,240}
			\definecolor{colorbrewer2}{RGB}{254,224,210}
			\definecolor{colorbrewer3}{RGB}{252,187,161}
			\definecolor{colorbrewer4}{RGB}{252,146,114}
			\definecolor{colorbrewer5}{RGB}{251,106,74}
			\definecolor{colorbrewer6}{RGB}{239,59,44}
			\definecolor{colorbrewer7}{RGB}{203,24,29}
			\definecolor{colorbrewer8}{RGB}{153,0,13}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{255,245,240}
			\definecolor{colorbrewer2}{RGB}{254,224,210}
			\definecolor{colorbrewer3}{RGB}{252,187,161}
			\definecolor{colorbrewer4}{RGB}{252,146,114}
			\definecolor{colorbrewer5}{RGB}{251,106,74}
			\definecolor{colorbrewer6}{RGB}{239,59,44}
			\definecolor{colorbrewer7}{RGB}{203,24,29}
			\definecolor{colorbrewer8}{RGB}{165,15,21}
			\definecolor{colorbrewer9}{RGB}{103,0,13}
		}
	},
	colorbrewer scheme/RdYlBu/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{252,141,89}
			\definecolor{colorbrewer2}{RGB}{255,255,191}
			\definecolor{colorbrewer3}{RGB}{145,191,219}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{215,25,28}
			\definecolor{colorbrewer2}{RGB}{253,174,97}
			\definecolor{colorbrewer3}{RGB}{171,217,233}
			\definecolor{colorbrewer4}{RGB}{44,123,182}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{215,25,28}
			\definecolor{colorbrewer2}{RGB}{253,174,97}
			\definecolor{colorbrewer3}{RGB}{255,255,191}
			\definecolor{colorbrewer4}{RGB}{171,217,233}
			\definecolor{colorbrewer5}{RGB}{44,123,182}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{215,48,39}
			\definecolor{colorbrewer2}{RGB}{252,141,89}
			\definecolor{colorbrewer3}{RGB}{254,224,144}
			\definecolor{colorbrewer4}{RGB}{224,243,248}
			\definecolor{colorbrewer5}{RGB}{145,191,219}
			\definecolor{colorbrewer6}{RGB}{69,117,180}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{215,48,39}
			\definecolor{colorbrewer2}{RGB}{252,141,89}
			\definecolor{colorbrewer3}{RGB}{254,224,144}
			\definecolor{colorbrewer4}{RGB}{255,255,191}
			\definecolor{colorbrewer5}{RGB}{224,243,248}
			\definecolor{colorbrewer6}{RGB}{145,191,219}
			\definecolor{colorbrewer7}{RGB}{69,117,180}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{215,48,39}
			\definecolor{colorbrewer2}{RGB}{244,109,67}
			\definecolor{colorbrewer3}{RGB}{253,174,97}
			\definecolor{colorbrewer4}{RGB}{254,224,144}
			\definecolor{colorbrewer5}{RGB}{224,243,248}
			\definecolor{colorbrewer6}{RGB}{171,217,233}
			\definecolor{colorbrewer7}{RGB}{116,173,209}
			\definecolor{colorbrewer8}{RGB}{69,117,180}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{215,48,39}
			\definecolor{colorbrewer2}{RGB}{244,109,67}
			\definecolor{colorbrewer3}{RGB}{253,174,97}
			\definecolor{colorbrewer4}{RGB}{254,224,144}
			\definecolor{colorbrewer5}{RGB}{255,255,191}
			\definecolor{colorbrewer6}{RGB}{224,243,248}
			\definecolor{colorbrewer7}{RGB}{171,217,233}
			\definecolor{colorbrewer8}{RGB}{116,173,209}
			\definecolor{colorbrewer9}{RGB}{69,117,180}
		},
		colorbrewer values/10/.code={
			\definecolor{colorbrewer1}{RGB}{165,0,38}
			\definecolor{colorbrewer2}{RGB}{215,48,39}
			\definecolor{colorbrewer3}{RGB}{244,109,67}
			\definecolor{colorbrewer4}{RGB}{253,174,97}
			\definecolor{colorbrewer5}{RGB}{254,224,144}
			\definecolor{colorbrewer6}{RGB}{224,243,248}
			\definecolor{colorbrewer7}{RGB}{171,217,233}
			\definecolor{colorbrewer8}{RGB}{116,173,209}
			\definecolor{colorbrewer9}{RGB}{69,117,180}
			\definecolor{colorbrewer10}{RGB}{49,54,149}
		},
		colorbrewer values/11/.code={
			\definecolor{colorbrewer1}{RGB}{165,0,38}
			\definecolor{colorbrewer2}{RGB}{215,48,39}
			\definecolor{colorbrewer3}{RGB}{244,109,67}
			\definecolor{colorbrewer4}{RGB}{253,174,97}
			\definecolor{colorbrewer5}{RGB}{254,224,144}
			\definecolor{colorbrewer6}{RGB}{255,255,191}
			\definecolor{colorbrewer7}{RGB}{224,243,248}
			\definecolor{colorbrewer8}{RGB}{171,217,233}
			\definecolor{colorbrewer9}{RGB}{116,173,209}
			\definecolor{colorbrewer10}{RGB}{69,117,180}
			\definecolor{colorbrewer11}{RGB}{49,54,149}
		}
	},
	colorbrewer scheme/RdYlGn/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{252,141,89}
			\definecolor{colorbrewer2}{RGB}{255,255,191}
			\definecolor{colorbrewer3}{RGB}{145,207,96}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{215,25,28}
			\definecolor{colorbrewer2}{RGB}{253,174,97}
			\definecolor{colorbrewer3}{RGB}{166,217,106}
			\definecolor{colorbrewer4}{RGB}{26,150,65}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{215,25,28}
			\definecolor{colorbrewer2}{RGB}{253,174,97}
			\definecolor{colorbrewer3}{RGB}{255,255,191}
			\definecolor{colorbrewer4}{RGB}{166,217,106}
			\definecolor{colorbrewer5}{RGB}{26,150,65}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{215,48,39}
			\definecolor{colorbrewer2}{RGB}{252,141,89}
			\definecolor{colorbrewer3}{RGB}{254,224,139}
			\definecolor{colorbrewer4}{RGB}{217,239,139}
			\definecolor{colorbrewer5}{RGB}{145,207,96}
			\definecolor{colorbrewer6}{RGB}{26,152,80}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{215,48,39}
			\definecolor{colorbrewer2}{RGB}{252,141,89}
			\definecolor{colorbrewer3}{RGB}{254,224,139}
			\definecolor{colorbrewer4}{RGB}{255,255,191}
			\definecolor{colorbrewer5}{RGB}{217,239,139}
			\definecolor{colorbrewer6}{RGB}{145,207,96}
			\definecolor{colorbrewer7}{RGB}{26,152,80}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{215,48,39}
			\definecolor{colorbrewer2}{RGB}{244,109,67}
			\definecolor{colorbrewer3}{RGB}{253,174,97}
			\definecolor{colorbrewer4}{RGB}{254,224,139}
			\definecolor{colorbrewer5}{RGB}{217,239,139}
			\definecolor{colorbrewer6}{RGB}{166,217,106}
			\definecolor{colorbrewer7}{RGB}{102,189,99}
			\definecolor{colorbrewer8}{RGB}{26,152,80}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{215,48,39}
			\definecolor{colorbrewer2}{RGB}{244,109,67}
			\definecolor{colorbrewer3}{RGB}{253,174,97}
			\definecolor{colorbrewer4}{RGB}{254,224,139}
			\definecolor{colorbrewer5}{RGB}{255,255,191}
			\definecolor{colorbrewer6}{RGB}{217,239,139}
			\definecolor{colorbrewer7}{RGB}{166,217,106}
			\definecolor{colorbrewer8}{RGB}{102,189,99}
			\definecolor{colorbrewer9}{RGB}{26,152,80}
		},
		colorbrewer values/10/.code={
			\definecolor{colorbrewer1}{RGB}{165,0,38}
			\definecolor{colorbrewer2}{RGB}{215,48,39}
			\definecolor{colorbrewer3}{RGB}{244,109,67}
			\definecolor{colorbrewer4}{RGB}{253,174,97}
			\definecolor{colorbrewer5}{RGB}{254,224,139}
			\definecolor{colorbrewer6}{RGB}{217,239,139}
			\definecolor{colorbrewer7}{RGB}{166,217,106}
			\definecolor{colorbrewer8}{RGB}{102,189,99}
			\definecolor{colorbrewer9}{RGB}{26,152,80}
			\definecolor{colorbrewer10}{RGB}{0,104,55}
		},
		colorbrewer values/11/.code={
			\definecolor{colorbrewer1}{RGB}{165,0,38}
			\definecolor{colorbrewer2}{RGB}{215,48,39}
			\definecolor{colorbrewer3}{RGB}{244,109,67}
			\definecolor{colorbrewer4}{RGB}{253,174,97}
			\definecolor{colorbrewer5}{RGB}{254,224,139}
			\definecolor{colorbrewer6}{RGB}{255,255,191}
			\definecolor{colorbrewer7}{RGB}{217,239,139}
			\definecolor{colorbrewer8}{RGB}{166,217,106}
			\definecolor{colorbrewer9}{RGB}{102,189,99}
			\definecolor{colorbrewer10}{RGB}{26,152,80}
			\definecolor{colorbrewer11}{RGB}{0,104,55}
		}
	},
	colorbrewer scheme/Set1/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{228,26,28}
			\definecolor{colorbrewer2}{RGB}{55,126,184}
			\definecolor{colorbrewer3}{RGB}{77,175,74}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{228,26,28}
			\definecolor{colorbrewer2}{RGB}{55,126,184}
			\definecolor{colorbrewer3}{RGB}{77,175,74}
			\definecolor{colorbrewer4}{RGB}{152,78,163}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{228,26,28}
			\definecolor{colorbrewer2}{RGB}{55,126,184}
			\definecolor{colorbrewer3}{RGB}{77,175,74}
			\definecolor{colorbrewer4}{RGB}{152,78,163}
			\definecolor{colorbrewer5}{RGB}{255,127,0}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{228,26,28}
			\definecolor{colorbrewer2}{RGB}{55,126,184}
			\definecolor{colorbrewer3}{RGB}{77,175,74}
			\definecolor{colorbrewer4}{RGB}{152,78,163}
			\definecolor{colorbrewer5}{RGB}{255,127,0}
			\definecolor{colorbrewer6}{RGB}{255,255,51}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{228,26,28}
			\definecolor{colorbrewer2}{RGB}{55,126,184}
			\definecolor{colorbrewer3}{RGB}{77,175,74}
			\definecolor{colorbrewer4}{RGB}{152,78,163}
			\definecolor{colorbrewer5}{RGB}{255,127,0}
			\definecolor{colorbrewer6}{RGB}{255,255,51}
			\definecolor{colorbrewer7}{RGB}{166,86,40}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{228,26,28}
			\definecolor{colorbrewer2}{RGB}{55,126,184}
			\definecolor{colorbrewer3}{RGB}{77,175,74}
			\definecolor{colorbrewer4}{RGB}{152,78,163}
			\definecolor{colorbrewer5}{RGB}{255,127,0}
			\definecolor{colorbrewer6}{RGB}{255,255,51}
			\definecolor{colorbrewer7}{RGB}{166,86,40}
			\definecolor{colorbrewer8}{RGB}{247,129,191}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{228,26,28}
			\definecolor{colorbrewer2}{RGB}{55,126,184}
			\definecolor{colorbrewer3}{RGB}{77,175,74}
			\definecolor{colorbrewer4}{RGB}{152,78,163}
			\definecolor{colorbrewer5}{RGB}{255,127,0}
			\definecolor{colorbrewer6}{RGB}{255,255,51}
			\definecolor{colorbrewer7}{RGB}{166,86,40}
			\definecolor{colorbrewer8}{RGB}{247,129,191}
			\definecolor{colorbrewer9}{RGB}{153,153,153}
		}
	},
	colorbrewer scheme/Set2/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{102,194,165}
			\definecolor{colorbrewer2}{RGB}{252,141,98}
			\definecolor{colorbrewer3}{RGB}{141,160,203}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{102,194,165}
			\definecolor{colorbrewer2}{RGB}{252,141,98}
			\definecolor{colorbrewer3}{RGB}{141,160,203}
			\definecolor{colorbrewer4}{RGB}{231,138,195}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{102,194,165}
			\definecolor{colorbrewer2}{RGB}{252,141,98}
			\definecolor{colorbrewer3}{RGB}{141,160,203}
			\definecolor{colorbrewer4}{RGB}{231,138,195}
			\definecolor{colorbrewer5}{RGB}{166,216,84}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{102,194,165}
			\definecolor{colorbrewer2}{RGB}{252,141,98}
			\definecolor{colorbrewer3}{RGB}{141,160,203}
			\definecolor{colorbrewer4}{RGB}{231,138,195}
			\definecolor{colorbrewer5}{RGB}{166,216,84}
			\definecolor{colorbrewer6}{RGB}{255,217,47}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{102,194,165}
			\definecolor{colorbrewer2}{RGB}{252,141,98}
			\definecolor{colorbrewer3}{RGB}{141,160,203}
			\definecolor{colorbrewer4}{RGB}{231,138,195}
			\definecolor{colorbrewer5}{RGB}{166,216,84}
			\definecolor{colorbrewer6}{RGB}{255,217,47}
			\definecolor{colorbrewer7}{RGB}{229,196,148}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{102,194,165}
			\definecolor{colorbrewer2}{RGB}{252,141,98}
			\definecolor{colorbrewer3}{RGB}{141,160,203}
			\definecolor{colorbrewer4}{RGB}{231,138,195}
			\definecolor{colorbrewer5}{RGB}{166,216,84}
			\definecolor{colorbrewer6}{RGB}{255,217,47}
			\definecolor{colorbrewer7}{RGB}{229,196,148}
			\definecolor{colorbrewer8}{RGB}{179,179,179}
		}
	},
	colorbrewer scheme/Set3/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{141,211,199}
			\definecolor{colorbrewer2}{RGB}{255,255,179}
			\definecolor{colorbrewer3}{RGB}{190,186,218}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{141,211,199}
			\definecolor{colorbrewer2}{RGB}{255,255,179}
			\definecolor{colorbrewer3}{RGB}{190,186,218}
			\definecolor{colorbrewer4}{RGB}{251,128,114}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{141,211,199}
			\definecolor{colorbrewer2}{RGB}{255,255,179}
			\definecolor{colorbrewer3}{RGB}{190,186,218}
			\definecolor{colorbrewer4}{RGB}{251,128,114}
			\definecolor{colorbrewer5}{RGB}{128,177,211}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{141,211,199}
			\definecolor{colorbrewer2}{RGB}{255,255,179}
			\definecolor{colorbrewer3}{RGB}{190,186,218}
			\definecolor{colorbrewer4}{RGB}{251,128,114}
			\definecolor{colorbrewer5}{RGB}{128,177,211}
			\definecolor{colorbrewer6}{RGB}{253,180,98}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{141,211,199}
			\definecolor{colorbrewer2}{RGB}{255,255,179}
			\definecolor{colorbrewer3}{RGB}{190,186,218}
			\definecolor{colorbrewer4}{RGB}{251,128,114}
			\definecolor{colorbrewer5}{RGB}{128,177,211}
			\definecolor{colorbrewer6}{RGB}{253,180,98}
			\definecolor{colorbrewer7}{RGB}{179,222,105}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{141,211,199}
			\definecolor{colorbrewer2}{RGB}{255,255,179}
			\definecolor{colorbrewer3}{RGB}{190,186,218}
			\definecolor{colorbrewer4}{RGB}{251,128,114}
			\definecolor{colorbrewer5}{RGB}{128,177,211}
			\definecolor{colorbrewer6}{RGB}{253,180,98}
			\definecolor{colorbrewer7}{RGB}{179,222,105}
			\definecolor{colorbrewer8}{RGB}{252,205,229}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{141,211,199}
			\definecolor{colorbrewer2}{RGB}{255,255,179}
			\definecolor{colorbrewer3}{RGB}{190,186,218}
			\definecolor{colorbrewer4}{RGB}{251,128,114}
			\definecolor{colorbrewer5}{RGB}{128,177,211}
			\definecolor{colorbrewer6}{RGB}{253,180,98}
			\definecolor{colorbrewer7}{RGB}{179,222,105}
			\definecolor{colorbrewer8}{RGB}{252,205,229}
			\definecolor{colorbrewer9}{RGB}{217,217,217}
		},
		colorbrewer values/10/.code={
			\definecolor{colorbrewer1}{RGB}{141,211,199}
			\definecolor{colorbrewer2}{RGB}{255,255,179}
			\definecolor{colorbrewer3}{RGB}{190,186,218}
			\definecolor{colorbrewer4}{RGB}{251,128,114}
			\definecolor{colorbrewer5}{RGB}{128,177,211}
			\definecolor{colorbrewer6}{RGB}{253,180,98}
			\definecolor{colorbrewer7}{RGB}{179,222,105}
			\definecolor{colorbrewer8}{RGB}{252,205,229}
			\definecolor{colorbrewer9}{RGB}{217,217,217}
			\definecolor{colorbrewer10}{RGB}{188,128,189}
		},
		colorbrewer values/11/.code={
			\definecolor{colorbrewer1}{RGB}{141,211,199}
			\definecolor{colorbrewer2}{RGB}{255,255,179}
			\definecolor{colorbrewer3}{RGB}{190,186,218}
			\definecolor{colorbrewer4}{RGB}{251,128,114}
			\definecolor{colorbrewer5}{RGB}{128,177,211}
			\definecolor{colorbrewer6}{RGB}{253,180,98}
			\definecolor{colorbrewer7}{RGB}{179,222,105}
			\definecolor{colorbrewer8}{RGB}{252,205,229}
			\definecolor{colorbrewer9}{RGB}{217,217,217}
			\definecolor{colorbrewer10}{RGB}{188,128,189}
			\definecolor{colorbrewer11}{RGB}{204,235,197}
		},
		colorbrewer values/12/.code={
			\definecolor{colorbrewer1}{RGB}{141,211,199}
			\definecolor{colorbrewer2}{RGB}{255,255,179}
			\definecolor{colorbrewer3}{RGB}{190,186,218}
			\definecolor{colorbrewer4}{RGB}{251,128,114}
			\definecolor{colorbrewer5}{RGB}{128,177,211}
			\definecolor{colorbrewer6}{RGB}{253,180,98}
			\definecolor{colorbrewer7}{RGB}{179,222,105}
			\definecolor{colorbrewer8}{RGB}{252,205,229}
			\definecolor{colorbrewer9}{RGB}{217,217,217}
			\definecolor{colorbrewer10}{RGB}{188,128,189}
			\definecolor{colorbrewer11}{RGB}{204,235,197}
			\definecolor{colorbrewer12}{RGB}{255,237,111}
		}
	},
	colorbrewer scheme/Spectral/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{252,141,89}
			\definecolor{colorbrewer2}{RGB}{255,255,191}
			\definecolor{colorbrewer3}{RGB}{153,213,148}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{215,25,28}
			\definecolor{colorbrewer2}{RGB}{253,174,97}
			\definecolor{colorbrewer3}{RGB}{171,221,164}
			\definecolor{colorbrewer4}{RGB}{43,131,186}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{215,25,28}
			\definecolor{colorbrewer2}{RGB}{253,174,97}
			\definecolor{colorbrewer3}{RGB}{255,255,191}
			\definecolor{colorbrewer4}{RGB}{171,221,164}
			\definecolor{colorbrewer5}{RGB}{43,131,186}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{213,62,79}
			\definecolor{colorbrewer2}{RGB}{252,141,89}
			\definecolor{colorbrewer3}{RGB}{254,224,139}
			\definecolor{colorbrewer4}{RGB}{230,245,152}
			\definecolor{colorbrewer5}{RGB}{153,213,148}
			\definecolor{colorbrewer6}{RGB}{50,136,189}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{213,62,79}
			\definecolor{colorbrewer2}{RGB}{252,141,89}
			\definecolor{colorbrewer3}{RGB}{254,224,139}
			\definecolor{colorbrewer4}{RGB}{255,255,191}
			\definecolor{colorbrewer5}{RGB}{230,245,152}
			\definecolor{colorbrewer6}{RGB}{153,213,148}
			\definecolor{colorbrewer7}{RGB}{50,136,189}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{213,62,79}
			\definecolor{colorbrewer2}{RGB}{244,109,67}
			\definecolor{colorbrewer3}{RGB}{253,174,97}
			\definecolor{colorbrewer4}{RGB}{254,224,139}
			\definecolor{colorbrewer5}{RGB}{230,245,152}
			\definecolor{colorbrewer6}{RGB}{171,221,164}
			\definecolor{colorbrewer7}{RGB}{102,194,165}
			\definecolor{colorbrewer8}{RGB}{50,136,189}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{213,62,79}
			\definecolor{colorbrewer2}{RGB}{244,109,67}
			\definecolor{colorbrewer3}{RGB}{253,174,97}
			\definecolor{colorbrewer4}{RGB}{254,224,139}
			\definecolor{colorbrewer5}{RGB}{255,255,191}
			\definecolor{colorbrewer6}{RGB}{230,245,152}
			\definecolor{colorbrewer7}{RGB}{171,221,164}
			\definecolor{colorbrewer8}{RGB}{102,194,165}
			\definecolor{colorbrewer9}{RGB}{50,136,189}
		},
		colorbrewer values/10/.code={
			\definecolor{colorbrewer1}{RGB}{158,1,66}
			\definecolor{colorbrewer2}{RGB}{213,62,79}
			\definecolor{colorbrewer3}{RGB}{244,109,67}
			\definecolor{colorbrewer4}{RGB}{253,174,97}
			\definecolor{colorbrewer5}{RGB}{254,224,139}
			\definecolor{colorbrewer6}{RGB}{230,245,152}
			\definecolor{colorbrewer7}{RGB}{171,221,164}
			\definecolor{colorbrewer8}{RGB}{102,194,165}
			\definecolor{colorbrewer9}{RGB}{50,136,189}
			\definecolor{colorbrewer10}{RGB}{94,79,162}
		},
		colorbrewer values/11/.code={
			\definecolor{colorbrewer1}{RGB}{158,1,66}
			\definecolor{colorbrewer2}{RGB}{213,62,79}
			\definecolor{colorbrewer3}{RGB}{244,109,67}
			\definecolor{colorbrewer4}{RGB}{253,174,97}
			\definecolor{colorbrewer5}{RGB}{254,224,139}
			\definecolor{colorbrewer6}{RGB}{255,255,191}
			\definecolor{colorbrewer7}{RGB}{230,245,152}
			\definecolor{colorbrewer8}{RGB}{171,221,164}
			\definecolor{colorbrewer9}{RGB}{102,194,165}
			\definecolor{colorbrewer10}{RGB}{50,136,189}
			\definecolor{colorbrewer11}{RGB}{94,79,162}
		}
	},
	colorbrewer scheme/YlGn/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{247,252,185}
			\definecolor{colorbrewer2}{RGB}{173,221,142}
			\definecolor{colorbrewer3}{RGB}{49,163,84}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,204}
			\definecolor{colorbrewer2}{RGB}{194,230,153}
			\definecolor{colorbrewer3}{RGB}{120,198,121}
			\definecolor{colorbrewer4}{RGB}{35,132,67}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,204}
			\definecolor{colorbrewer2}{RGB}{194,230,153}
			\definecolor{colorbrewer3}{RGB}{120,198,121}
			\definecolor{colorbrewer4}{RGB}{49,163,84}
			\definecolor{colorbrewer5}{RGB}{0,104,55}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,204}
			\definecolor{colorbrewer2}{RGB}{217,240,163}
			\definecolor{colorbrewer3}{RGB}{173,221,142}
			\definecolor{colorbrewer4}{RGB}{120,198,121}
			\definecolor{colorbrewer5}{RGB}{49,163,84}
			\definecolor{colorbrewer6}{RGB}{0,104,55}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,204}
			\definecolor{colorbrewer2}{RGB}{217,240,163}
			\definecolor{colorbrewer3}{RGB}{173,221,142}
			\definecolor{colorbrewer4}{RGB}{120,198,121}
			\definecolor{colorbrewer5}{RGB}{65,171,93}
			\definecolor{colorbrewer6}{RGB}{35,132,67}
			\definecolor{colorbrewer7}{RGB}{0,90,50}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,229}
			\definecolor{colorbrewer2}{RGB}{247,252,185}
			\definecolor{colorbrewer3}{RGB}{217,240,163}
			\definecolor{colorbrewer4}{RGB}{173,221,142}
			\definecolor{colorbrewer5}{RGB}{120,198,121}
			\definecolor{colorbrewer6}{RGB}{65,171,93}
			\definecolor{colorbrewer7}{RGB}{35,132,67}
			\definecolor{colorbrewer8}{RGB}{0,90,50}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,229}
			\definecolor{colorbrewer2}{RGB}{247,252,185}
			\definecolor{colorbrewer3}{RGB}{217,240,163}
			\definecolor{colorbrewer4}{RGB}{173,221,142}
			\definecolor{colorbrewer5}{RGB}{120,198,121}
			\definecolor{colorbrewer6}{RGB}{65,171,93}
			\definecolor{colorbrewer7}{RGB}{35,132,67}
			\definecolor{colorbrewer8}{RGB}{0,104,55}
			\definecolor{colorbrewer9}{RGB}{0,69,41}
		}
	},
	colorbrewer scheme/YlGnBu/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{237,248,177}
			\definecolor{colorbrewer2}{RGB}{127,205,187}
			\definecolor{colorbrewer3}{RGB}{44,127,184}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,204}
			\definecolor{colorbrewer2}{RGB}{161,218,180}
			\definecolor{colorbrewer3}{RGB}{65,182,196}
			\definecolor{colorbrewer4}{RGB}{34,94,168}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,204}
			\definecolor{colorbrewer2}{RGB}{161,218,180}
			\definecolor{colorbrewer3}{RGB}{65,182,196}
			\definecolor{colorbrewer4}{RGB}{44,127,184}
			\definecolor{colorbrewer5}{RGB}{37,52,148}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,204}
			\definecolor{colorbrewer2}{RGB}{199,233,180}
			\definecolor{colorbrewer3}{RGB}{127,205,187}
			\definecolor{colorbrewer4}{RGB}{65,182,196}
			\definecolor{colorbrewer5}{RGB}{44,127,184}
			\definecolor{colorbrewer6}{RGB}{37,52,148}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,204}
			\definecolor{colorbrewer2}{RGB}{199,233,180}
			\definecolor{colorbrewer3}{RGB}{127,205,187}
			\definecolor{colorbrewer4}{RGB}{65,182,196}
			\definecolor{colorbrewer5}{RGB}{29,145,192}
			\definecolor{colorbrewer6}{RGB}{34,94,168}
			\definecolor{colorbrewer7}{RGB}{12,44,132}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,217}
			\definecolor{colorbrewer2}{RGB}{237,248,177}
			\definecolor{colorbrewer3}{RGB}{199,233,180}
			\definecolor{colorbrewer4}{RGB}{127,205,187}
			\definecolor{colorbrewer5}{RGB}{65,182,196}
			\definecolor{colorbrewer6}{RGB}{29,145,192}
			\definecolor{colorbrewer7}{RGB}{34,94,168}
			\definecolor{colorbrewer8}{RGB}{12,44,132}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,217}
			\definecolor{colorbrewer2}{RGB}{237,248,177}
			\definecolor{colorbrewer3}{RGB}{199,233,180}
			\definecolor{colorbrewer4}{RGB}{127,205,187}
			\definecolor{colorbrewer5}{RGB}{65,182,196}
			\definecolor{colorbrewer6}{RGB}{29,145,192}
			\definecolor{colorbrewer7}{RGB}{34,94,168}
			\definecolor{colorbrewer8}{RGB}{37,52,148}
			\definecolor{colorbrewer9}{RGB}{8,29,88}
		}
	},
	colorbrewer scheme/YlOrBr/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{255,247,188}
			\definecolor{colorbrewer2}{RGB}{254,196,79}
			\definecolor{colorbrewer3}{RGB}{217,95,14}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,212}
			\definecolor{colorbrewer2}{RGB}{254,217,142}
			\definecolor{colorbrewer3}{RGB}{254,153,41}
			\definecolor{colorbrewer4}{RGB}{204,76,2}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,212}
			\definecolor{colorbrewer2}{RGB}{254,217,142}
			\definecolor{colorbrewer3}{RGB}{254,153,41}
			\definecolor{colorbrewer4}{RGB}{217,95,14}
			\definecolor{colorbrewer5}{RGB}{153,52,4}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,212}
			\definecolor{colorbrewer2}{RGB}{254,227,145}
			\definecolor{colorbrewer3}{RGB}{254,196,79}
			\definecolor{colorbrewer4}{RGB}{254,153,41}
			\definecolor{colorbrewer5}{RGB}{217,95,14}
			\definecolor{colorbrewer6}{RGB}{153,52,4}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,212}
			\definecolor{colorbrewer2}{RGB}{254,227,145}
			\definecolor{colorbrewer3}{RGB}{254,196,79}
			\definecolor{colorbrewer4}{RGB}{254,153,41}
			\definecolor{colorbrewer5}{RGB}{236,112,20}
			\definecolor{colorbrewer6}{RGB}{204,76,2}
			\definecolor{colorbrewer7}{RGB}{140,45,4}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,229}
			\definecolor{colorbrewer2}{RGB}{255,247,188}
			\definecolor{colorbrewer3}{RGB}{254,227,145}
			\definecolor{colorbrewer4}{RGB}{254,196,79}
			\definecolor{colorbrewer5}{RGB}{254,153,41}
			\definecolor{colorbrewer6}{RGB}{236,112,20}
			\definecolor{colorbrewer7}{RGB}{204,76,2}
			\definecolor{colorbrewer8}{RGB}{140,45,4}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,229}
			\definecolor{colorbrewer2}{RGB}{255,247,188}
			\definecolor{colorbrewer3}{RGB}{254,227,145}
			\definecolor{colorbrewer4}{RGB}{254,196,79}
			\definecolor{colorbrewer5}{RGB}{254,153,41}
			\definecolor{colorbrewer6}{RGB}{236,112,20}
			\definecolor{colorbrewer7}{RGB}{204,76,2}
			\definecolor{colorbrewer8}{RGB}{153,52,4}
			\definecolor{colorbrewer9}{RGB}{102,37,6}
		}
	},
	colorbrewer scheme/YlOrRd/.style={
		colorbrewer values/.is choice,	
		colorbrewer values/3/.code={
			\definecolor{colorbrewer1}{RGB}{255,237,160}
			\definecolor{colorbrewer2}{RGB}{254,178,76}
			\definecolor{colorbrewer3}{RGB}{240,59,32}
		},
		colorbrewer values=3,
		colorbrewer values/4/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,178}
			\definecolor{colorbrewer2}{RGB}{254,204,92}
			\definecolor{colorbrewer3}{RGB}{253,141,60}
			\definecolor{colorbrewer4}{RGB}{227,26,28}
		},
		colorbrewer values/5/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,178}
			\definecolor{colorbrewer2}{RGB}{254,204,92}
			\definecolor{colorbrewer3}{RGB}{253,141,60}
			\definecolor{colorbrewer4}{RGB}{240,59,32}
			\definecolor{colorbrewer5}{RGB}{189,0,38}
		},
		colorbrewer values/6/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,178}
			\definecolor{colorbrewer2}{RGB}{254,217,118}
			\definecolor{colorbrewer3}{RGB}{254,178,76}
			\definecolor{colorbrewer4}{RGB}{253,141,60}
			\definecolor{colorbrewer5}{RGB}{240,59,32}
			\definecolor{colorbrewer6}{RGB}{189,0,38}
		},
		colorbrewer values/7/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,178}
			\definecolor{colorbrewer2}{RGB}{254,217,118}
			\definecolor{colorbrewer3}{RGB}{254,178,76}
			\definecolor{colorbrewer4}{RGB}{253,141,60}
			\definecolor{colorbrewer5}{RGB}{252,78,42}
			\definecolor{colorbrewer6}{RGB}{227,26,28}
			\definecolor{colorbrewer7}{RGB}{177,0,38}
		},
		colorbrewer values/8/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,204}
			\definecolor{colorbrewer2}{RGB}{255,237,160}
			\definecolor{colorbrewer3}{RGB}{254,217,118}
			\definecolor{colorbrewer4}{RGB}{254,178,76}
			\definecolor{colorbrewer5}{RGB}{253,141,60}
			\definecolor{colorbrewer6}{RGB}{252,78,42}
			\definecolor{colorbrewer7}{RGB}{227,26,28}
			\definecolor{colorbrewer8}{RGB}{177,0,38}
		},
		colorbrewer values/9/.code={
			\definecolor{colorbrewer1}{RGB}{255,255,204}
			\definecolor{colorbrewer2}{RGB}{255,237,160}
			\definecolor{colorbrewer3}{RGB}{254,217,118}
			\definecolor{colorbrewer4}{RGB}{254,178,76}
			\definecolor{colorbrewer5}{RGB}{253,141,60}
			\definecolor{colorbrewer6}{RGB}{252,78,42}
			\definecolor{colorbrewer7}{RGB}{227,26,28}
			\definecolor{colorbrewer8}{RGB}{189,0,38}
			\definecolor{colorbrewer9}{RGB}{128,0,38}
		}
	}
}

==> kronecker.tex <==
If $ \bm{X} $ and $ \bm{Y} $ are $ m \times n $ and $ p \times q $ matrices,
then the Kronecker product  
$ \bm{X} \otimes \bm{Y} $
is the $ mn \times pq $ block matrix.
Assuming the $ ( i, j ) $ entry of $ \bm{X} $ and $ \bm{Y} $ are respectively
denoted by $ x_{i,j} $, $ y_{i,j} $,
the Kronecker product is achieved by 

{\footnotesize
\[
\bm{X} \otimes \bm{Y} 
%=
%\left(
%\begin{array}{c c c}
%x_{0,0} & \cdots & x_{0,n-1} \\
%\vdots & \ddots  & \vdots \\
%x_{m-1,0} & \cdots & x_{m-1,n-1} \\
%\end{array}
%\right)
%\otimes
%\left(
%\begin{array}{c c c}
%y_{0,0} & \cdots & y_{0,q-1} \\
%\vdots & \ddots  & \vdots \\
%y_{p-1,0} & \cdots & y_{p-1,q-1} \\
%\end{array}
%\right)
%\]
%\[
=
\left(
\begin{array}{c c c}
x_{0,0} \bm{Y} & \cdots & x_{0,q-1} \bm{Y} \\
\vdots & \ddots  & \vdots \\
x_{m-1,0} \bm{Y} & \cdots & x_{m-1,q-1} \bm{Y} \\
\end{array}
\right)
\]
%\[
%=
%\left(
%\begin{array}{c c c c c c c c}
%x_{0,0} y_{0,0} & \cdots & x_{0,0} y_{0,q-1}   & \cdots & \cdots & x_{0,n-1} y_{0,0} & \cdots & x_{0,n-1} y_{0,q-1} \\ 
%\vdots & \ddots  & \vdots     &   &   & \vdots & \ddots  & \vdots  \\
%x_{0,0} y_{p-1,0} & \cdots & x_{0,0} y_{p-1,q-1} & \cdots & \cdots & x_{0,n-1} y_{p-1,0} & \cdots & x_{0,n-1} y_{p-1,q-1}  \\
%\vdots &   &  \vdots  & \ddots &   & \vdots &   & \vdots  \\
%\vdots &   &  \vdots  &    & \ddots   & \vdots &   & \vdots  \\
%x_{m-1,0} y_{0,0} & \cdots & x_{m-1,0} y_{0,q-1}   & \cdots & \cdots & x_{m-1,n-1} y_{0,0} & \cdots & x_{m-1,n-1} y_{0,q-1} \\ 
%\vdots & \ddots  & \vdots     & \cdots & \cdots & \vdots & \ddots  & \vdots  \\
%x_{m-1,0} y_{p-1,0} & \cdots & x_{m-1,0} y_{p-1,q-1} & \cdots & \cdots & x_{m-1,n-1} y_{p-1,0} & \cdots & x_{m-1,n-1} y_{p-1,q-1}  \\
%\end{array}
%\right)
%\]
}

For each entry, 
$ (\bm{X} \otimes \bm{Y})_{p(r-1)+v,q(s-1)+w}=x_{rs} y_{vw} $.

%Letting 
%{\footnotesize%
%\[
%A = 
%\left( \begin{array}{c c c c}
%a_{0,0} & \cdots & a_{0,k-1} \\
%\vdots &  & \vdots \\
%a_{m-1,0} & \cdots & a_{m-1,k-1} \\
%\end{array}
%\right),
%\]
%\[
%B = 
%\left( \begin{array}{c c c c}
%b_{0,0} & \cdots & b_{0,n-1} \\
%\vdots &  & \vdots \\
%b_{k-1,0} & \cdots & b_{k-1,n-1} \\
%\end{array}
%\right), \mbox{~and~}
%\]
%\[
%C = 
%\left( \begin{array}{c c c c}
%c_{0,0} & \cdots & c_{0,n-1} \\
%\vdots &  & \vdots \\
%c_{m-1,0} & \cdots & c_{m-1,n-1} \\
%\end{array}
%\right)
%\]%
%}
%$ C := A B + C $ computes
%\[
%c_{i,j} := \sum_{p=0}^{k-1} a_{i,p} b_{p,j} +
%c_{i,j}.
%\]





==> limitations.tex <==

combine task parallelism with data parallelism for more than two levels.



==> pgfplot_template.tex <==
\begin{tikzpicture}[scale=.5]
%\begin{tikzpicture}
\begin{axis}[
%width=5cm,
%height=5cm,
title={$m=k=n$, 1 core},
xlabel={ $m = k = n$ },
ylabel={\emph{Effective} GFLOPS ($ 2 \cdot  m \cdot  n \cdot k / time $)},
  xmin=0,
  xmax=10000,
  ymin=20,
  ymax=34,
  xtick={1000,2000,3000,4000,5000,6000,7000,8000,9000,10000},
  ytick={5, 10, 15, 20, 25, 28.36, 30, 34},
  scaled x ticks=false,
  scaled x ticks=base 10:-3,
  %/pgf/number format/sci subscript,
  grid=major,
  %scaled y ticks = false
  %x tick label style={/pgf/number format/1000 sep = \thinspace},
  %/pgf/number format/fixed,
  %mark=square*,blue
  %axis background/.style={fill=blue!10},
  axis background/.style={fill=lightgray!20},
]

\addplot[
  %dotted,
  %dashed,
  red,
  %mark=*,
  %mark=x,
  %mark=triangle*,
  %only marks,
  %mark=diamond*,
  %mark=*,
  %mark=none,
  %mark=pentagon*,
  %mark=otimes,
  %mark=diamond*,
  %mark size=2.0pt,
  %mark options={scale=0.5,fill=white},
  %thick,
  %solid,
  line width=1pt,
] file {plotdata/strassen_1_abc.dat};

%\pgfplotsset{
%cycle list={%
%{red, mark=*}, {blue,mark=*},
%{red, mark=x}, {blue,mark=x},
%{red, mark=square*}, {blue,mark=square*},
%{red, mark=triangle*}, {blue,mark=triangle*},
%{red, mark=diamond*}, {blue,mark=diamond*},
%{red, mark=pentagon*}, {blue,mark=pentagon*}
%},
%legend style={
%at={(0.5,-0.2)},
%anchor=north,
%legend columns=2,
%cells={anchor=west},
%font=\footnotesize,
%rounded corners=2pt,
%},
%xlabel=$x$,ylabel=$f(x)$
%}
\addlegendentry{$a$}

\end{axis}
\end{tikzpicture}

%\addlegendentry{1-level \strassen{}}
%\addlengendentry{ $ \langle 2, 2, 2 \rangle $\\ }

%\legend{ 
%%{}$ \langle 2, 2, 2 \rangle $\\
%}

